Figures as Interfaces: Toward LLM-Native Artifacts for Scientific Discovery

Large language models (LLMs) are transforming scientific workflows, not only through their generative capabilities but also through their emerging ability to use tools, reason about data, and coordinate complex analytical tasks. Yet in most human-AI collaborations, the primary outputs, figures, are still treated as static visual summaries: once rendered, they are handled by both humans and multimodal LLMs as images to be re-interpreted from pixels or captions. The emergent capabilities of LLMs open an opportunity to fundamentally rethink this paradigm. In this paper, we introduce the concept of LLM-native figures: data-driven artifacts that are simultaneously human-legible and machine-addressable. Unlike traditional plots, each artifact embeds complete provenance: the data subset, analytical operations and code, and visualization specification used to generate it. As a result, an LLM can "see through" the figure--tracing selections back to their sources, generating code to extend analyses, and orchestrating new visualizations through natural-language instructions or direct manipulation. We implement this concept through a hybrid language-visual interface that integrates LLM agents with a bidirectional mapping between figures and underlying data. Using the science of science domain as a testbed, we demonstrate that LLM-native figures can accelerate discovery, improve reproducibility, and make reasoning transparent across agents and users. More broadly, this work establishes a general framework for embedding provenance, interactivity, and explainability into the artifacts of modern research, redefining the figure not as an end product, but as an interface for discovery. For more details, please refer to the demo video available at www.llm-native-figure.com.

==> sections/03-results.tex <==
\section{Results}
\label{section:results} 

\input{sections/03-1-framework}
\input{sections/03-2-evaluation}

==> sections/archive/00-Abstract/00-abstract_v1_20251015.tex <==
\title[Article Title]{Hybrid Human-AI Interfaces for Discovery: Combining Natural Language and Visualization for Interactive Data Exploration} 

% Data Art Conference at Boston, 2025-06
\abstract{
% The insights emerging from the large-scale data from the Science of Science (SciSci) field are profoundly reshaping and accelerating the global science and innovation landscape. 
% To fully utilize the potential of these insights, whether to accelerate scientific discovery or inform decisions by science policy-makers like funding agencies and university leaders, we must rethink how we explore and communicate such data. 
% Over the past decade, data-driven approaches have evolved from traditional data science methodologies to more intuitive visualization tools for decision-making and artworks for public communication. 
% Today, with the advent of generative AI, we see an opportunity to propose new design and interaction principles for data exploration and communication. 
% In this talk, I will introduce \systemname, a proof-of-concept platform that reimagines data exploration in SciSci through generative AI and interactive visualization techniques. 
% At its core is a new design paradigm that combines Language User Interfaces (LUI) with Graphical User Interfaces (GUI).  
% By integrating these technologies and human-AI collaboration workflow, \systemname points toward a new mode of engaging with data, one that is analytical, accessible, and expressive. 
% Looking ahead, 
% the underlying design paradigm utilizing generative AI and data visualization in \systemname also hold broader potential to support more artistic formats for communicating science, exploring its aesthetics and creative dimensions in what we call ``the art of science.''
}








%%==================================%%
%% Sample for unstructured abstract %%
%%==================================%%

% \abstract{The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. Authors are advised to check the author instructions for the journal they are submitting to for word limits and if structural elements like subheadings, citations, or equations are permitted.}

%%================================%%
%% Sample for structured abstract %%
%%================================%%

% \abstract{\textbf{Purpose:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Methods:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Results:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Conclusion:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.}

==> sections/archive/00-Abstract/00-abstract_v2_20251201.tex <==
\abstract{
Large language models (LLMs) are transforming scientific workflows, not only through their generative capabilities but also through their emerging ability to use tools, reason about data, and coordinate complex analytical tasks. 
Yet in most human–AI collaborations, the primary outputs—figures—remain static visual summaries: interpretable by humans, but opaque to machines. 
We introduce the concept of LLM-native figures—data-driven artifacts that are simultaneously human-legible and machine-addressable. 
Unlike traditional plots, each artifact embeds complete provenance: the data subset, code, and visualization specification used to generate it. 
As a result, an LLM can “see through” the figure—tracing selections back to their sources, generating code to extend analyses, and orchestrating new visualizations through natural dialogue or direct manipulation. 
We implement this concept through a hybrid language–visual interface that integrates LLM agents with a bidirectional mapping between figures and underlying data. Using the science-of-science domain as a testbed, we demonstrate that LLM-native figures accelerate discovery, improve reproducibility, and make reasoning transparent across agents and users. 
More broadly, this work establishes a general framework for embedding provenance, interactivity, and explainability into the artifacts of modern research—redefining the figure not as an end-product, but as an interface for discovery.
}

==> sections/archive/01-introduction/01-introduction_v1_20250521.tex <==
\section{Introduction}
\label{section:introduction}

% ======== 1. Motivation =========
Science has long served as an important driving force for human development, bringing in improved global health, driving innovation and economic growth, and informing policy decisions. 
To accelerate scientific advancement and inform science policy-making, the Science of Science (SciSci) field has emerged. 
It leverages large-scale datasets from the scientific ecosystem, including upstream funding data and downstream societal impacts, to distill data evidence and insights that uncover historical patterns of scientific progress and suggest future developments such as technological breakthroughs.
% To fully utilize the potential of these insights, whether to accelerate scientific discovery or inform decisions by science policy-makers like funding agencies and university leaders, we must rethink how we explore and communicate such data. 

% ======== 2. Challenges =========
While data-driven approaches have significantly advanced over the past decade across domains including computational social science and SciSci, they still face major challenges in supporting scientific discovery and decision-making. 
% (1) Envolving analysis questions
% old technique: not supported by traditional data science methods
% solution: multi-agent + LUI: 实时生成任意insights
First, new datasets and analysis scenarios are emerging, driven by the rapidly shifting global context, including technological advancements, political changes, and economic developments, making the traditional case-by-case data science approaches less effective and flexible. 
% (2) Deep-dive analysis
% old technique: LUI
% solution: GUI (visualization + interaction/coordination) -- bring in "artifact", allow intuitive data insight representation and accurate and deep data exploration
Second, navigating the large-scale scientific data to perform deep-dive analysis and extract and communicate actionable insights remains difficult, especially for users like decision-makers who often lack the time or expertise to engage in thorough data exploration. 
% (3) Reuse "artifact". 
Third, science consumers like decision-makers often engage in repetitive high-level tasks such as funding new projects by funding agencies and adjusting research strategies by universities leaders. 
These scenarios demand tools that not only present insights intuitively but also support efficient, fine-grained, and iterative data exploration. 
% Tools for intuitive insights presentation and efficient and fine-grained data exploration for routine decision-making scenarios are thus required. 


% ======== 3. Two New Techniques =========
% LUI
% (1) Interpreting user intention, using Q&A (conversational AI): understand user intent. It assists in narrowing down human fuzzy ideas into concrete data aspects, based on HAI conversation and data insights. 
% (2) Enabling flexible analysis workflow (tool use): flexibly assemble and generate any dashboard systems based on user intent. It will automatically understand users’ questions and call proper tools to solve the problem, enhanced by RAG techniques.
The recent development of large language models has opened new avenues for scientific discovery and decision-making in SciSci. 
A growing number of tools and platforms are developed across academia and industry to either fully automate the scientific discovery process using AI agent systems~\cite{shneiderman1983direct} or involve human in the analysis loop through chatbot-style interfaces~\cite{microsoftdiscovery, shao2025sciscigpt}. 
However, language user interfaces (LUIs) like chatbots often rely on linear exploration logic and purely textual presentations of insights. 
These limitations make it difficult for human researchers and decision-makers to engage in the kind of divergent, non-linear exploration that mirrors human reasoning such as mind mapping. 
As a result, it becomes challenging to deeply investigate insights or precisely control and iterate on the analysis workflow and results. 
% 
% GUI: vis
% (1) Visualization (static): intuitive data insight delivery.
% (2) Interaction and coordination: efficient data exploration for accurate and repetitive data analysis (decision-making) tasks.
In contrast, graphical user interfaces (GUIs), such as interactive visualization dashboards, offer distinct advantages. 
They enhance cognitive processing and insight generation by transforming abstract and complex data into visible, tangible representations~\cite{ware2019information}, and enable human to quickly identify trends, patterns, and anomalies in a way that purely textual interfaces cannot achieve. 
Moreover, their interactivity further allows for precise, continuous, and spatial manipulation of visual elements~\cite{shneiderman1983direct} and thus simplifies the data exploration process, offering clarity and efficiency in understanding the data. 


% ======== 4. Our Solution: SciSciCanvas =========
% In this paper, we explore the potential of new design and interaction principles for data exploration and communication to facilitate scientific discovery and decision-making in SciSci. 
In this paper, we introduce \systemname, a proof-of-concept platform that reimagines data exploration in SciSci. 
% through the integration of generative AI and interactive visualization techniques. 
% frontend
At its core is a new design paradigm that combines Language User Interfaces (LUI) with Graphical User Interfaces (GUI). 
The LUI, through the conversational AI, interprets user analysis intentions and translates them into specific analysis tasks and data dimensions. 
The GUI, through interactive visualization dashboards, presents insights intuitively and enables flexible, in-depth exploration via direct manipulation (e.g., brushing and filtering), thereby reducing ambiguity and enhancing analytical efficiency.  
% backend
Powered by an underlying multi-agent LLM engine with fine-grained action-level control, the system transforms user intent into data-driven \textbf{``artifacts''}-- interactive and coordinated visualization dashboards--through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to support iterative exploration. 
These artifacts support both deep dives into insights with graphics operations and are reusable across future exploration tasks with similar analytical needs. 
% SciSci database querying, analyzing the data with various data science approaches and SciSci domain knowledges, generating,  editing, and extending interactive and coordinated visualization dashboards that allow iteratively exploration.
% These artifacts could allow deep dive into data insights by iteratively and accurately refining the visual insights or extending to new visualization and coordinate, and is reusable in future data exploration with similar analysis needs. 
% 
By integrating LLM agents, visualization, and human-AI collaboration workflow, \systemname points toward a new mode of engaging with data--one that supports non-linear exploration and is intuitive, accessible, and expressive. 
Contribution list:
\begin{itemize}
    \item A proof-of-concept system, \systemname, that intergrates LUI and GUI interfaces and a multi-agent framework to allow intuitive data exploration and deep dive in Science and decision-making.  
    \item System evaluation. The system is evaluated through practical usage scenarios and quantitative studies.
    \item A human-AI collaboration framework for using LUI and GUI for future scientific discovery and decision-making (HAI4Science). 
\end{itemize} 


% The insights emerging from the Science of Science (SciSci) research are profoundly reshaping and accelerating the global science and innovation landscape. 
% Leveraging these insights to inform SciSci decisions by stakeholders such as funders, university leaders, and policymakers is critical. 
% For example, strategic investment by funding agencies can boost the production of high-impact research. 
% Universities need to identify faculty whose research is with transnational power, facilitating knowledge transfer and technology development. 
% Decisions made in these contexts have the power to directly influence the direction and impact of scientific progress, with the potential to further significantly enhance human quality of life.

% Given the complexity and significance of these questions, data-driven tools are increasingly favored by SciSci decision-makers to support real-world, dynamic decisionmaking. However, (1) these decision-making problems are often undefined with ambiguous data analysis needs. There is a lack of well-defined, data-driven approaches to solving these complex decision-making problems. Furthermore, (2) decision-makers are continually confronted with new datasets and evolving decision scenarios, driven by the rapidly changing global context, including technological advancements, political changes, and economic developments. Traditional expert-oriented and highly customized system design approaches are inadequate in these scenarios due to the lack of flexibility and efficiency in designing such analysis tools in real-time. On the other hand, (3) decision-makers often engage in repetitive high-level decision-making tasks such as selecting PIs to fund (by funding agencies) and finding recent papers to file patents (by universities). Tools for intuitive insights presentation and efficient and fine-grained data exploration for routine decision-making scenarios are thus required. Existing solutions, such as general-purpose tools like Web of Science (WOS) and Scopus, offer broad data querying capabilities but lack the specific insights and workflows tailored to SciSci decision-making. Meanwhile, more specialized tools (e.g., InnovationInsights and FundingtheFrontier) are narrowly tailored to particular problems, limiting their flexibility and general applicability across different decision contexts.

% Here, we outline the ways in which LUI + GUI—the synergistic combination of language user interface (LUI) and graphics user interface (GUI)—can be the most effective approach for SciSci decision-makers who mostly do not have a background in complex data analysis. We present SciPilotGPT, an all-in-one platform for understanding decision-maker’s analysis intentions, enabling intuitive data exploration, and generating data-driven decision-making workflows. Specifically, the LUI, through the conversational AI, facilitates the interpretation of users’ high-level and vague intentions and “transforms” them into specific analysis tasks and data aspects. The GUI, through interactive visualization dashboards, presents data insights intuitively and facilitates flexible, in-depth exploration through “direct manipulation” (e.g., brushing and filtering [1]), reducing ambiguity and enhancing decision-making efficiency.

% This new interaction method (Fig. 2) integrates an LLM module to understand user questions, fetch and present data insights, and formulate decision-making workflows; a visualization module to present data insights intuitively and facilitate free-form data exploration; and a database module which consolidates diverse data sources from the SciSci ecosystem (Fig. 1). The system is available online (xxx.com) and is designed for scalability, allowing for the integration of additional data sources and decision-making scenarios. This platform represents a significant advancement in making sophisticated data analysis accessible to a broader range of SciSci stakeholders. TODO: add more open-source details. Contribution list:

% A human-AI collaboration framework for using LUI and GUI in SciSci decision-making.

% A proof-of-concept demo showcasing the potential of our framework for SciSci decision-makers. 

% System evaluation. The system is evaluated through practical usage scenarios and quantitative studies.

==> sections/archive/01-introduction/01-introduction_v2.1_20250529.tex <==
\section{Introduction}
\label{section:introduction}

% - Overall: v1 framing太像SciSciGPT了。reframe成general technique出发，用SciSci作为一个test domain
% - Details
%     - Title里面`Discovery`这个词: 自己去想，重新写motivation;
%     - 不要讲Generative UI. 因为他scope很大，我们只是dashboard+vis
%     - 怎么motivate SciSci这个domain: 这个domain有rich dataset, 满足前面讲的所有特性。可以加一段justify SciSci重要性
%     - future work自己去想，重新写motivation
    
Recent advances in generative artificial intelligence (GenAI) have fundamentally reshaped how humans interact with data, extract insights, and inform critical decisions. 
Central to this progress are Large Language Models (LLMs), which have popularized conversational Language User Interfaces (LUIs) capable of translating natural language intent into complex analytical actions in real-time, providing unprecedented accessibility. 
These interfaces are transforming human-AI interactions not only in everyday queries but also in expert-oriented specialized tasks such as scientific discovery~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt} and high-stake decision-making~\cite{xx}, by synthesizing knowledge and data from diverse sources. 
% These interfaces not only change the human-AI conversation in daily life query, but also for expert-oriented scenarios like scientific discovery~\cite{penai2025deepresearch, google2025deepresearch, oshao2025sciscigpt} and high-stake decision-making~\cite{xx} by synthesizing data from diverse sources. % to empasize data-driven scenarios. 
However, as these systems proliferate, a crucial limitation has emerged: LUIs, while accessible, are often linear and opaque, and the natural language inputs they rely on are inherently ambiguous, making them poorly suited for the rich, non-linear, accurate, and iterative exploration that defines human sense-making and discovery. 
% However, as these systems proliferate, a crucial limitation has emerged: LUIs alone are often linear, opaque, ambiguous, and poorly suited for the kind of rich, non-linear, and iterative exploration that characterizes human sense-making and discovery. 



% GUI
% (1) visual representation
% (2) interactivity
Meanwhile, decades of research in human-computer interaction have shown that Graphical User Interfaces (GUIs), through visual representations and direct manipulations~\cite{shneiderman1983direct, ware2019information} such as widgets and dashboards, enable more precise and efficient data exploration and allow users to identify patterns, compare alternatives, and dive deep into insights in ways that text-based interfaces alone cannot. 
% enable users to efficiently and accurately explore patterns, compare alternatives, and surface insights in ways that text alone cannot. 
Yet traditional GUIs typically require substantial manual effort to accommodate ambiguous questions and design analysis workflows, resulting in rigid and pre-defined systems that lack adaptability and expressiveness in open-ended analytical scenarios with evolving datasets. 
% Meanwhile, more specialized tools (e.g., Innova tionInsights and FundingtheFrontier) are narrowly tailored to particular problems, limiting their flexibility and general applicability across different decision contexts.

To overcome these limitations, we propose a new design paradigm for human sense-making and data-driven discovery, which natively integrates the strengths of LUI and GUI, harnessing the flexible, expressive and real-time reasoning of conversational AI with the intuitive, powerful visual affordances of interactive data visualization. 
In this paradigm, users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not only as text, but as interactive data-driven \textbf{``artifacts''} that can be further manipulated, explored, reused, and iterated upon. 
% and return results not only as text, but as interactive visual and data-driven ``artifacts'' that can be further manipulated, explored, or iterated upon. 
This interaction loop empowers users to not only receive insights intuitively but also actively guide and control the analysis process by combining the best of both worlds: the creativity and context sensitivity of language, with the clarity and efficiency of visual exploration.

To demonstrate the power and generality of this approach, we present \systemname, a prototype system developed in the Science of Science (SciSci) domain---an essential field for understanding and accelerating scientific enterprise. 
We select SciSci as a testbed due to its representative challenges our paradigm aims to address: rich and evolving data from the scientific ecosystem; complex scientific discovery tasks such as tracing the evolution of knowledge; and high-stakes decision-making scenarios including identifying untapped innovation potential by university leaders and developing strategic funding allocations by funding agencies. 
% Science has long served as an important driving force for human development, bringing in improved global health, driving innovation and economic growth, and informing policy decisions. 
% To accelerate scientific advancement and inform science policy-making, the Science of Science (SciSci) field has emerged. 
% It leverages large-scale datasets from the scientific ecosystem, including upstream funding data and downstream societal impacts, to distill data evidence and insights that uncover historical patterns of scientific progress and suggest future developments such as technological breakthroughs.
% Its complex data and real-world policy-making scenarios, such as university leaders seeking to uncover untapped innovation potential and funding agencies developing strategic investments, make it ideal for developing and validating this new paradigm. 
% 
In \systemname, LLM-powered agents can query, analyze, and visualize complex scientific data, while users seamlessly switch between natural language and direct manipulation to explore hypotheses, generate insights, and support science policy decisions. 
The resulting visual \textbf{artifacts}---interactive, coordinated dashboards---enable non-linear, iterative exploration and are reusable in future exploration tasks with similar analytical goals.
% The provided visual \textbf{artifacts}---interactive and coordinated visualization dashboards---support non-linear iterative exploration and are reusable in future exploration tasks with similar analytical needs.
\wyf{(yifang: to add more tech details after finishing the \textit{Method} section: multi-agents with action-level control and optimization, ...)}
% – through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to 



% % backend
% Powered by an underlying multi-agent LLM engine with fine-grained action-level control, the system transforms user intent into data-driven \textbf{``artifacts''}-- interactive and coordinated visualization dashboards--through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to support iterative exploration. 
% These artifacts support both deep dives into insights with graphics operations and are reusable across future exploration tasks with similar analytical needs. 
% % 
% By integrating LLM agents, visualization, and human-AI collaboration workflow, \systemname points toward a new mode of engaging with data--one that supports non-linear exploration and is intuitive, accessible, and expressive. 

Our contributions are threefold:
\begin{itemize}
    \item \textbf{A proof-of-concept system.} We developed \systemname to demonstrate how integrating LUI and GUI interfaces with multi-agent LLMs enables flexible, intuitive, and deep data exploration for human sense-making and discovery in SciSci.  
    \item \textbf{Evaluation.} Through real-world usage scenarios and quantitative studies, we show that this hybrid approach improves efficiency, insight generation, and user satisfaction over LUI- or GUI-only approaches. 
    \item \textbf{A generalizable design paradigm.} More broadly, we distill our system design and empirical findings into a new paradigm, \wyf{\textbf{xxxxx}}, that extends beyond the SciSci domain, charting a path toward next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    \wyf{(generalizability levels: 
        [level 1]: SciSciCanvas (use SciSci as an example domain); 
        [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
        [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
        [level 4]: HAI for all scenarios (general public + expert-oriented systems)
    )}
    % \item \textbf{A generalizable design paradigm. We distill our design and findings into a design paradigm, \textbf{HAI4Science (?)}, that can be generalized beyond SciSci, charting a path for next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    % } 
    % A human-AI collaboration framework for using LUI and GUI for future scientific discovery and decision-making (HAI4Science). 
\end{itemize} 


Overall, through this work, we aim to catalyze a broader shift toward hybrid interfaces that elevate both human and AI capabilities, accelerating discovery and decision-making in science and beyond.



















==> sections/archive/01-introduction/01-introduction_v2.2_20251011.tex <==
\section{Introduction}
\label{section:introduction}
% Idea: LLM can generate everything, 我们的novelty是在于：在探索过程中，LLM生成了real-time insights，then drill down to explore more insights – iterative process to facilitate discovery. 
%     我们的contribution并不是LUI + GUI，而是这种LLM驱动的动态生成data insights的过程，辅助人类explore。

    
Recent advances in generative artificial intelligence (GenAI) have fundamentally reshaped how humans interact with data, extract insights, and inform critical decisions. 
At the forefront of this revolution are Large Language Models (LLMs), which have democratized access to sophisticated analytical capabilities through conversational AI interfaces. 
These Language User Interfaces (LUIs), powered by underlying LLMs, can translate natural language intent into complex analytical actions in real-time, providing unprecedented accessibility to data-driven discovery.
% Central to this progress are Large Language Models (LLMs), which have popularized conversational AI that utilizes LLM and Language User Interfaces (LUIs) capable of translating natural language intent into complex analytical actions in real-time, providing unprecedented accessibility. 
By lowering barriers to complex computation, LUIs have already begun to reshape domains ranging from everyday consumer choices to expert practices in scientific research~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt} and high-stakes decision-making~\cite{xx}. 
% by synthesizing domain-specific knowledge from diverse sources through techniques such as retrieval-augmented generation (RAG) and leveraging specialized analytical tools tailored to specific domains.
% Beyond everyday applications such as shopping and diet, these interfaces are also reshaping expert-oriented domains, including scientific research~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt} and high-stakes decision-making~\cite{xx}, by synthesizing domain-specific knowledge from diverse sources through techniques such as retrieval-augmented generation (RAG) and leveraging specialized analytical tools tailored to specific domains. 
% % These interfaces are transforming human-AI interactions not only in everyday queries but also in expert-oriented specialized tasks such as scientific discovery~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt} and high-stake decision-making~\cite{xx}, by synthesizing knowledge like RAG and database from diverse sources and utilizing external tools for tailored analysis for specific domains.

However, as these interfaces proliferate across critical applications, a fundamental limitation has emerged: while accessible, they operate through linear, opaque interactions that poorly align with humans' naturally non-linear and iterative exploration processes. 
Moreover, the inherent ambiguity of natural language inputs makes these systems inefficient and inaccurate for precisely targeting and specifying insights for deeper investigation, which is a critical requirement for rigorous scientific discovery and high-stakes decision-making. 
% 
% 
% for the rich, non-linear, accurate, and iterative exploration that defines scientific discovery and decision-making. 
% However, as these systems proliferate, a crucial limitation has emerged: LUIs alone are often linear, opaque, ambiguous, and poorly suited for the kind of rich, non-linear, and iterative exploration that characterizes human sense-making and discovery. 



% GUI
% (1) visual representation
% (2) interactivity
Meanwhile, decades of research in human-computer interaction have shown that Graphical User Interfaces (GUIs) excel at providing intuitive, efficient access to information through visual representations and direct manipulation~\cite{shneiderman1983direct, ware2019information}. 
% through visual representations and direct manipulations~\cite{shneiderman1983direct, ware2019information}, such as interactive widgets, provide intuitive and quick access to information.
In the context of data-driven discovery, data visualization and visual analytics serve as essential approaches for uncovering hidden insights through visual features that statistical approaches may overlook~\cite{anscombe1973graphs} and for supporting precise, efficient, and back-and-forth exploration~\cite{keim2008visual}.  
These approaches enable users to identify complex patterns, compare alternatives, and dive deep into insights in ways that are often inaccessible through text-based interfaces alone. 
% enable users to efficiently and accurately explore patterns, compare alternatives, and surface insights in ways that text alone cannot. 
Yet traditional GUIs for data analysis~\cite{wang2023innovationinsights, wang2025funding} typically require substantial manual effort to accommodate the ambiguous user tasks and analytical approaches~\cite{munzner2014visualization}. 
As a result, they tend toward rigid, pre-defined structures for specific user requirements that lack the adaptability and expressiveness essential for dynamic analytical scenarios with evolving datasets and user questions. 
% including established visual analytics interfaces~\cite{wang2023innovationinsights, wang2025funding}, 
% As a result, they tend to be rigid and pre-defined, lacking the adaptability and expressiveness needed for open-ended analytical scenarios with evolving datasets. 
% Meanwhile, more specialized tools (e.g., Innova tionInsights and FundingtheFrontier) are narrowly tailored to particular problems, limiting their flexibility and general applicability across different decision contexts. 

To overcome these limitations, we propose a new design paradigm for data-driven discovery and decision-making, which natively integrates the complementary strengths of both LUI and GUI. 
This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not only as text, but as interactive visualizations that can be further manipulated and extended. 
% reused, and iterated upon. 
% and return results not only as text, but as interactive visual and data-driven ``artifacts'' that can be further manipulated, explored, or iterated upon. 
Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of novel insights delivered through both textual explanations and visual exploration tools. 
Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration.

To demonstrate the broad applicability of this approach, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.
% SciSci serves as a representative testbed with challenges our paradigm is designed to address: 
% rich and evolving datasets from the global scientific ecosystem that includes research papers, patents, policies, etc, and the complex citation relations among different entities; 
% complex discovery tasks such as tracing the evolution of knowledge and identifying emerging research frontiers; 
% and high-stakes decision-making scenarios (\eg, identifying untapped innovation potential by university leaders and developing strategic funding allocations by funding agencies). 
% 
In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, and visualize the results. 
These outputs are embodied as ``data-driven artifacts''--interactive, editable, extendable, and reusable dashboards that support non-linear, iterative exploration across related analytical tasks. 
% producing \textbf{data-driven ``artifacts''}---interactive, editable, and extendable dashboards that support non-linear, iterative exploration and can be reused across tasks with similar analytical goals. 
% \wyf{(Sounds repeating the prev paragraph?)} 
% These artifacts support two core operations that embody an iterative data exploration process: (1) \textbf{editing} existing visualizations to refine or reorient the analysis focus, and (2) \textbf{extending} from specific data points within visualizations to generate new, coordinated dashboards that allow users to progressively deepen their understanding through dynamic interaction. 
Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

More broadly, we synthesize our system design and empirical findings into a new conceptual model, \wyf{\textbf{xxx} (Fig.~\ref{fig:model})}, that generalizes beyond the SciSci domain and this hybrid interface. 
This model charts a path toward next-generation human–AI collaboration systems that overcome the limitations of language- or visualization-only paradigms, enabling expert-oriented scientific discovery and decision-making across disciplines. 
% charting a path toward next-generation human-AI collaboration systems that transcend the constraints of either interface alone for future \wyf{expert-oriented (?)} scientific discovery and decision-making across disciplines.   

Overall, through this work, we aim to catalyze a broader shift toward hybrid interfaces that elevate both human and AI capabilities, accelerating discovery and decision-making in science and beyond.



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/model.jpg}
    \caption{The conceptual model (draft): iterative exploration for data-driven discovery.}
    \label{fig:model}
\end{figure}













% The provided visual \textbf{artifacts}---interactive and coordinated visualization dashboards---support non-linear iterative exploration and are reusable in future exploration tasks with similar analytical needs.
% \wyf{(yifang: to add more tech details after finishing the \textit{Method} section: multi-agents with action-level control and optimization, ...)}
% – through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to 



% % backend
% Powered by an underlying multi-agent LLM engine with fine-grained action-level control, the system transforms user intent into data-driven \textbf{``artifacts''}-- interactive and coordinated visualization dashboards--through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to support iterative exploration. 
% These artifacts support both deep dives into insights with graphics operations and are reusable across future exploration tasks with similar analytical needs. 
% % 
% By integrating LLM agents, visualization, and human-AI collaboration workflow, \systemname points toward a new mode of engaging with data--one that supports non-linear exploration and is intuitive, accessible, and expressive. 

% Our contributions are threefold:
% \begin{itemize}
    % \item \textbf{A proof-of-concept system.} We developed \systemname to demonstrate how integrating LUI and GUI interfaces with multi-agent LLMs enables flexible, intuitive, and deep data exploration for human sense-making and discovery in SciSci.  
    % \item \textbf{Evaluation.} Through real-world usage scenarios and quantitative studies, we show that this hybrid approach improves efficiency, insight generation, and user satisfaction over LUI- or GUI-only approaches. 
    % \item \textbf{A generalizable design paradigm.} More broadly, we distill our system design and empirical findings into a new paradigm, \wyf{\textbf{xxxxx}}, that extends beyond the SciSci domain, charting a path toward next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    % \wyf{(generalizability levels: 
    %     [level 1]: SciSciCanvas (use SciSci as an example domain); 
    %     [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
    %     [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
    %     [level 4]: HAI for all scenarios (general public + expert-oriented systems)
    % )}
    % \item \textbf{A generalizable design paradigm. We distill our design and findings into a design paradigm, \textbf{HAI4Science (?)}, that can be generalized beyond SciSci, charting a path for next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    % } 
    % A human-AI collaboration framework for using LUI and GUI for future scientific discovery and decision-making (HAI4Science). 
% \end{itemize} 





















==> sections/archive/01-introduction/01-introduction_v2.3_20251016.tex <==
\section{Introduction}
\label{section:introduction}
% Idea: LLM can generate everything, 我们的novelty是在于：在探索过程中，LLM生成了real-time insights，then drill down to explore more insights – iterative process to facilitate discovery. 
%     我们的contribution并不是LUI + GUI，而是这种LLM驱动的动态生成data insights的过程，辅助人类explore。
Recent advances in generative artificial intelligence (GenAI) have fundamentally reshaped how humans interact with data, extract insights, and inform critical decisions. 
At the forefront of this revolution are Large Language Models (LLMs), which have democratized access to sophisticated analytical capabilities through conversational AI interfaces. 
These Language User Interfaces (LUIs), powered by underlying LLMs, can translate natural language intent into complex analytical actions in real-time, providing unprecedented accessibility to data-driven discovery.
By lowering barriers to complex computation and analysis, LUIs have already begun to reshape domains ranging from everyday consumer choices to expert practices in scientific research~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt} and high-stakes decision-making~\cite{tu2025towards, harvey-ai}. 

However, as these interfaces proliferate across diverse applications, a fundamental limitation has emerged: while accessible, they operate through linear, opaque interactions that poorly align with humans' naturally non-linear and iterative exploration processes~\cite{bates1989design, white2009exploratory}. 
Moreover, the inherent ambiguity of natural language inputs makes these tools inefficient and inaccurate for precisely targeting and specifying insights for deeper investigation, which is a critical requirement for rigorous data-driven scientific discovery and high-stakes decision-making. 
% 
% 
% for the rich, non-linear, accurate, and iterative exploration that defines scientific discovery and decision-making. 
% However, as these systems proliferate, a crucial limitation has emerged: LUIs alone are often linear, opaque, ambiguous, and poorly suited for the kind of rich, non-linear, and iterative exploration that characterizes human sense-making and discovery. 



% GUI
% (1) visual representation
% (2) interactivity
Meanwhile, decades of research in human-computer interaction have shown that Graphical User Interfaces (GUIs) excel at providing intuitive, efficient access to information through visual representations and direct manipulation~\cite{shneiderman1983direct, ware2019information}. 
In the context of data-driven discovery, data visualization and visual analytics serve as essential approaches for uncovering hidden insights through visual features that statistical approaches may overlook~\cite{anscombe1973graphs} and for supporting precise, efficient, and back-and-forth exploration~\cite{keim2008visual}.  
These approaches enable users to identify complex patterns, compare alternatives, and dive deep into insights in ways that are often inaccessible through text-based interfaces alone. 
Yet traditional GUIs for data analysis~\cite{wang2023innovationinsights, wang2025funding} typically require substantial manual effort to accommodate the ambiguous user tasks and analytical approaches~\cite{munzner2014visualization}. 
As a result, they tend toward rigid, pre-defined structures for specific user requirements that lack the adaptability and expressiveness essential for dynamic analytical scenarios with evolving datasets and user questions. 

To overcome these limitations, \wyf{we propose a conceptual model (Fig.~\ref{fig:model}) that includes a new design paradigm} for data-driven discovery and decision-making, which natively integrates the complementary strengths of both LUI and GUI and is powered by LLM.  
This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

\wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
Humans are good at pattern recognition and intuitive understanding through visual images; 
GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% This dual representation allows humans and AI to ``see through'' the visual abstraction by linking user-interested data regions back to the source data for deeper analysis and iterative reasoning. 
% Such a capability transforms figures from passive outputs into active interfaces for discovery, establishing a foundation for a new generation of AI-assisted data analysis systems in which every visualization becomes both a window for humans and a reasoning substrate for machines/AI.
}

Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% These outputs are embodied as ``data-driven artifacts''--interactive, editable, extendable, and reusable dashboards that support non-linear, iterative exploration across related analytical tasks. 
Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

\wyf{
Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
}

\wyf{
Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
}


% \wyf{[yifang]: or maybe we should move this part before this demo system? So that the logic would be: motivation -> conceptual model -> demo domain and system. 
% We believe that our conceptual model, illustrative system design, and empirical findings can be extended and generalized beyond the SciSci domain as a foundation for all future applications that include data exploration. 
% }
% This model charts a path toward next-generation human–AI collaboration systems that overcome the limitations of language- or visualization-only paradigms, enabling expert-oriented scientific discovery and decision-making across disciplines. 

% Overall, through this work, we aim to catalyze a broader shift toward hybrid interfaces that elevate both human and AI capabilities, accelerating discovery and decision-making in science and beyond.



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/model.jpg}
    \caption{The conceptual model (draft): iterative exploration for data-driven discovery.}
    \label{fig:model}
\end{figure}













% The provided visual \textbf{artifacts}---interactive and coordinated visualization dashboards---support non-linear iterative exploration and are reusable in future exploration tasks with similar analytical needs.
% \wyf{(yifang: to add more tech details after finishing the \textit{Method} section: multi-agents with action-level control and optimization, ...)}
% – through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to 



% % backend
% Powered by an underlying multi-agent LLM engine with fine-grained action-level control, the system transforms user intent into data-driven \textbf{``artifacts''}-- interactive and coordinated visualization dashboards--through a suite of core capabilities including querying SciSci databases, performing data analysis informed by domain knowledge, and generating, editing, and extending dashboards to support iterative exploration. 
% These artifacts support both deep dives into insights with graphics operations and are reusable across future exploration tasks with similar analytical needs. 
% % 
% By integrating LLM agents, visualization, and human-AI collaboration workflow, \systemname points toward a new mode of engaging with data--one that supports non-linear exploration and is intuitive, accessible, and expressive. 

% Our contributions are threefold:
% \begin{itemize}
    % \item \textbf{A proof-of-concept system.} We developed \systemname to demonstrate how integrating LUI and GUI interfaces with multi-agent LLMs enables flexible, intuitive, and deep data exploration for human sense-making and discovery in SciSci.  
    % \item \textbf{Evaluation.} Through real-world usage scenarios and quantitative studies, we show that this hybrid approach improves efficiency, insight generation, and user satisfaction over LUI- or GUI-only approaches. 
    % \item \textbf{A generalizable design paradigm.} More broadly, we distill our system design and empirical findings into a new paradigm, \wyf{\textbf{xxxxx}}, that extends beyond the SciSci domain, charting a path toward next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    % \wyf{(generalizability levels: 
    %     [level 1]: SciSciCanvas (use SciSci as an example domain); 
    %     [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
    %     [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
    %     [level 4]: HAI for all scenarios (general public + expert-oriented systems)
    % )}
    % \item \textbf{A generalizable design paradigm. We distill our design and findings into a design paradigm, \textbf{HAI4Science (?)}, that can be generalized beyond SciSci, charting a path for next-generation human-AI systems that move beyond the constraints of either interface alone for future scientific discovery and decision-making. 
    % } 
    % A human-AI collaboration framework for using LUI and GUI for future scientific discovery and decision-making (HAI4Science). 
% \end{itemize} 

==> sections/archive/01-introduction/01-introduction_v3_20260206.tex <==
\section{Introduction}
\label{section:introduction}

% start with background -- figure, rather than LLM/chatbot's limication
Figures play a central role in scientific discovery~\cite{anscombe1973graphs}. 
They summarize complex data, reveal patterns, and communicate results in a visual form that is both concise and interpretable~\cite{anscombe1973graphs}. 
% By leveraging human visual perception, figures enable intuitive understanding and exploratory reasoning that go beyond what text or summary statistics alone can provide~\cite{anscombe1973graphs}.
% leveraging human visual perception to enable intuitive understanding and exploratory reasoning beyond what text or summary statistics alone can provide~\cite{anscombe1973graphs}.
A figure is often the endpoint of analysis and the centerpiece of scientific reasoning that transforms data into insight. 
Yet for all their importance, figures remain designed primarily for human interpretation. 
They capture relationships between variables but conceal the underlying data, code, and transformations that produced them.

% new opportunity brought by LLM
The emergence of large language models (LLMs) offers an opportunity to rethink this paradigm. 
Beyond text generation, LLMs increasingly serve as computational agents capable of reasoning, coding, and executing analytic workflows~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt, tu2025towards, harvey-ai}.  
When LLM agents generates a figure, it possesses complete knowledge of the artifact's provenance~\cite{lasser2020creating, konkol2020publishing, ziemann2023five, curvenote, e-life, pasquier2017practical, rupprecht2020improving}, including its dataset, analytical process, and visualization. 
From the model's perspective, a figure is not a static image but a structured object whose components can be queried, revised, and extended. 
This capability implies that, in principle, figures can be more interpretable to LLMs than to humans, providing a foundation for new modes of scientific reasoning and interaction.

% what we did - 1: conceptual framework
This paper introduces a framework for constructing LLM-native figures: data-driven artifacts that are simultaneously human-legible and machine-interpretable. 
Each artifact encapsulates not only the visualization but also its full provenance, including user interactions, data subset, and code. 
The framework establishes a bidirectional mapping between the figure and its underlying analytical components, allowing LLMs to translate natural-language prompts into structured analytical actions and to interpret visual selections or edits as executable operations.

% what we did - 2: proof-of-concept system
To instantiate this framework, we develop \systemname, a proof-of-concept system for the science-of-science domain that implements LLM-native figures and data-driven artifacts. 
Users can interact with figures and data insights using hybrid inputs (natural language and direct manipulations~\cite{shneiderman1983direct, ware2019information, keim2008visual, munzner2014visualization}). 
% \wyf{[To discuss: whether to say for the scisci domain? because we also use \systemname to implement the climate case. The only difference is the use of different domain dataset and domain knowledge (such as paper literature)].} 
The system interprets user intent, analyzes data, and records every analytic step, including user instructions, code execution, visualization generation and coordination, and user interaction, in an artifact store that preserves version history and enables full reproducibility. 
\systemname also serves as the basis for the case study and computational evaluation presented in Section~\ref{subsection:case-study} and~\ref{subsection:computational-evaluation}.

Together, these contributions establish a foundation for LLM-native scientific artifacts that bridge human and machine reasoning. 
By transforming figures from static endpoints into interactive, provenance-aware interfaces, this work advances a general method for collaborative discovery in the era of large language models.


% 一个新的点在于LLM怎么让原先的dashboard交互变得不一样？促进scientific discovery etc.
% Idea: LLM can generate everything, 我们的novelty是在于：在探索过程中，LLM生成了real-time insights，then drill down to explore more insights – iterative process to facilitate discovery. 
% 我们的contribution并不是LUI + GUI，而是这种LLM驱动的动态生成data insights的过程，辅助人类explore。

% related work: 
% humans' naturally non-linear and iterative exploration processes~\cite{bates1989design, white2009exploratory}

% In the context of data-driven discovery, data visualization and visual analytics serve as essential approaches for uncovering hidden insights through visual features that statistical approaches may overlook~\cite{anscombe1973graphs} and for supporting precise, efficient, and back-and-forth exploration~\cite{keim2008visual}.  
% These approaches enable users to identify complex patterns, compare alternatives, and dive deep into insights in ways that are often inaccessible through text-based interfaces alone. 
% Yet traditional GUIs for data analysis~\cite{wang2023innovationinsights, wang2025funding} typically require substantial manual effort to accommodate the ambiguous user tasks and analytical approaches~\cite{munzner2014visualization}. 


% % our method
% To overcome these limitations, \wyf{we propose a conceptual model (Fig.~\ref{fig:model}) that includes a new design paradigm} for data-driven discovery and decision-making, which natively integrates the complementary strengths of both LUI and GUI and is powered by LLM.  
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }



==> sections/archive/02-related-work/02-related-work-20260315.tex <==
\section{Related Work}
\label{section:related-work}
% Done: /Users/yifangwang/Library/CloudStorage/Dropbox/theory-paper
% TODO: 
% 1. /Users/yifangwang/Library/CloudStorage/Dropbox/nu/1-scisci-projects/3-holistic-vis-system-4-scisci/2-related-work
% /Users/yifangwang/Library/CloudStorage/Dropbox/theory-paper/9-scisci

Our framework builds on recent advances in AI-powered scientific discovery, interactive visual data exploration, and human-LLM interaction, which together provide a critical foundation for accelerating human understanding in data-rich domains. 
% , and generative user interfaces. 

\textbf{LLMs and AI agents for scientific discovery.} 
Recent breakthroughs in LLMs and AI agents have opened unprecedented opportunities for automating and augmenting scientific discovery across disciplines~\cite{zheng2025automation, zhang2024comprehensivesurvey, wang2023scientific}. 
These developments span diverse domains, including drug discovery in biology~\cite{zhang2025scientific, ghafarollahi2025sciagents} and chemistry~\cite{zheng2025large}, algorithmic innovation in computer science~\cite{lu2024ai}, large-scale behavioral studies in social science~\cite{manning2024automated}, and general statistics and data science~\cite{maojun2025survey, inala2024data, sun2024survey, hong2024data, guo2024ds, shao2025sciscigpt, wang2019human}, among others.
% 1. backend: AI agents
These systems typically build LLM-driven engines to automate full or partial research pipelines~\cite{lu2024ai}, from hypothesis generation, experimental design, code execution~\cite{guo2024ds}, and data-insight extraction~\cite{hong2024data, huang2025biomni, sphinx2026, observable2026canvas}, to figure generation~\cite{zhu2026paperbanana, plottie2026} and manuscript preparation. 
Many incorporate advanced LLM capabilities, including planning and reasoning, external tool integration~\cite{gao2025democratizing}, and retrieval-augmented generation (RAG). 
% 2. frontend: IDE, command-line based, to recent conversational AI -- reduce coding demand for users. 
These tools range from fully autonomous command-line tools and packages~\cite{lu2024ai, hong2024data, guo2024ds} 
% to integrated development environments (IDEs) requiring programming expertise~\cite{xx}, 
to more recent conversational interfaces that keep humans in the discovery loop through natural language interaction~\cite{openai2025deepresearch, google2025deepresearch, microsoftdiscovery, shao2025sciscigpt}. 
% 
% limitations: 

Despite their power, most of these systems constrain the discovery process to linear, end-to-end workflows or simple conversational exchanges. This approach contrasts sharply with the inherently iterative, non-linear nature of human scientific reasoning.
Their reliance on text-based outputs, occasionally complemented by static figures or tables, establishes a "one-shot" interaction paradigm that limits dynamic exploration and iterative reasoning. 
% 
Furthermore, these linear workflows make it difficult to trace analytical provenance, as they lack a well-structured record of the exploration process. 
Although new forms of computationally reproducible research (\eg, Curvenote~\cite{curvenote} and eLife's computationally reproducible article~\cite{e-life}) and studies~\cite{lasser2020creating, konkol2020publishing, ziemann2023five} have been proposed to increase transparency and reproducibility in open science by using digital-coding notebooks and interactive articles to link paper text to its underlying figures, code, and data, these systems focus on the final stage of research rather than supporting the iterative data exploration that precedes it.
% These end-to-end insight generation or linear human-AI exploration logic are contradict to humans' naturally non-linear exploration logic which requires back and forth. 
% Moreover, the pure text return or even with static figures and data tables also make the exploration 'one-shot'  in a single turn -- 不符合discovery back and forth的特性. 
% "The user interface is crucial for attracting users at first glance. Current research on user interface design can be broadly categorized into four types: Integrated Development Environment-based (IDE-based), Independent System, Command line-based (Commandbased), and Operation System-based (OS-based)." --Section 3.3: A Survey on Large Language Model-based Agents for Statistics and Data Science


\textbf{Visual data exploration.} 
Data visualization has long been recognized as a powerful tool of scientific discovery, enabling humans to uncover hidden patterns, generate insights that traditional statistical methods might miss, and present and communicate findings efficiently~\cite{anscombe1973graphs}. 
Through direct manipulations~\cite{shneiderman1983direct}, interactive visualizations such as dashboards provide intuitive access to complex information across multiple data dimensions, supporting the comprehensive exploration essential for discovery. 
% Data visualization such as interactive dashboards have been regarded as a powerful tool to deliver data insights and enable data exploration intuitively and comprehensively across different visualization components (that shows different data dimensions) through direct manipulations~\cite{shneiderman1983direct}. 
% 1. VA
However, traditional visual analytics systems~\cite{keim2008visual}, while powerful, are rigid and tailored to specific analysis tasks. Moreover, they require substantial manual effort and extensive collaboration with domain experts throughout their development, from initial task analysis and data modeling to visual design and system integration~\cite{munzner2014visualization, wang2023innovationinsights, wang2025funding}. 
% New tools have also been developed to allow users configuring dashboards step by step using low-level data attributes and queries~\cite{observable-canvases}. 
% New tools have also be developed to allow users configure dashboards with low-level data attributes step-by-step~\cite{observable-canvases}. 
% Conventional visual analytics systems have been developed to assist human in exploring and navigating complex data and inform decisions in a customized way that tailored at a specific group of target users and domain experts. 
% This process requires huge manual efforts and iteration with domain experts from task analysis, data transformation and modeling, to visual design, and system integration~\cite{munzner2014visualization, wang2023innovationinsights}. 

% 2. AI4VIS
Recent advances in AI and LLMs have begun to address these limitations through automated chart generation~\cite{tableauagent, tian2024chartgpt, wang2023llm4vis, dibia2023lida}, single-visualization manipulation and refinement~\cite{wang2023data, wang2025data}, multi-view dashboard creation with automated task decomposition~\cite{zhao2024lightva, zhao2024leva, lange2025yac}, and proactive AI-assisted insight exploration~\cite{zhao2025proactiveva}.
% The development of AI and LLM have bought new techniques to allow generating visual data insights in a more flexible way, including automatic visualization generation~\cite{tableauagent, tian2024chartgpt, wang2023llm4vis, dibia2023lida} and visualization manipulation and authoring~\cite{wang2023data, wang2025data} of a single chart, and multi-view generation with task decomposition~\cite{zhao2024lightva, zhao2024leva}. 
% 
% limitations
Yet these tools remain fundamentally limited: they either support only single-round chart generation, require advanced analysis and programming skills for chart manipulation, or generate complete visual analytics systems based solely on users' initial analysis goals. 
As a result, these approaches are not able to accommodate the dynamic, open-ended nature of scientific exploration, where questions and analytical directions evolve continuously as new insights emerge. 
% However, these tools either only support single round visualization generation, require high coding skills to manipulate charts, or generate a visual analytics systems at once based on user's initial analysis goals -- which means user's task是一开始定义好的不允许修改的，are limited to support discovery and decision-making which are always with a iterative and open data exploration space. 
% \wyf{[yifang: add one more paper: ProvenanceWidgets: https://provenancewidgets.github.io/]}

% 3. human-LLM interaction
% 1. design paradigm for human-LLM interaction
% 2. Generative UI for general tasks (beyond data analysis)
\textbf{Human-LLM interaction.} 
The rise of LLMs and generative AI has highlighted the need for a new way of thinking about user interface design in the human-computer interaction community, inspiring both new interaction modes~\cite{gao2024taxonomy, shen2025prompting, he2025plan} and innovative interface designs~\cite{luera2024survey, chen2025generative}. 
Among these, generative and malleable user interfaces have gained significant attention in both industry (\eg, ChatGPT Canvas~\cite{chatgpt-canvas} and Claude Artifact~\cite{claude-artifact}) and academia~\cite{chen2025generative, cao2025generative, suh2023sensecape}. 
These interfaces enable users to iteratively generate and refine digital artifacts, such as code, documents, and dashboards, through conversational interaction with LLMs, supporting a wide range of activities from everyday tasks~\cite{cao2025generative, suh2023sensecape} to creative ideation~\cite{you2025designmanager} and data analysis~\cite{bigquery-canvases}. 
% 
While these systems move beyond traditional chat-based interfaces by supporting iterative artifact refinement, most are designed for assembling interfaces rather than data-driven discovery. 
Tasks such as scientific exploration demand complex analytical workflows, iterative deep dives, and fine-grained control over data insights to support scientific rigor, reproducibility, and transparency. 
Existing systems either overlook these requirements or rely on users to interact directly with low-level code and data schemas~\cite{bigquery-canvases}. 
% Although these works go beyond the conversational chat interfaces which generate an artifact for iterative refinement, they either do not target at data-driven discovery which requires complex data analysis procedure and back-and-forth and deep-dive for data exploration which requires fine grained zoom in of data insights, or still require facing low-level code and data schema to do low-level editing~\cite{bigquery-canvases}. 
% 3. canvas-based tool
% Google data canvas: https://www.youtube.com/watch?v=r_nDZSrWaYk
% https://observablehq.com/platform/canvases and chrome-extension://efaidnbmnnnibpcajpcglclefindmkaj/https://static.observablehq.com/resources/ObservableCanvasesDatasheet_0425.pdf 



% Our solution: toward hybrid human-AI discovery interfaces
\medskip
\wyf{Better to summarize the gap, because the following sentences are repeating 3.1 P1.} 
Our conceptual framework and prototype system are powered by an underlying multi-agent LLM framework that enables real-time, dynamic data exploration through both natural language queries (Language User Interface, LUI) and interactive dashboards (Graphical User Interface, GUI). 
Users can progressively explore emerging questions and insights based on existing visual discoveries, which is an iterative process that naturally mirrors how scientists conduct discovery across diverse analytical domains. 


==> sections/archive/03-1-framework/03-1-framework_v1_20251030.tex <==
\section{Conceptual Framework}
\label{section:conceptual-framework} 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/framework.jpg}
    \caption{The conceptual framework for iterative exploration for data-driven scientific discovery.}
    \label{fig:framework}
\end{figure}


\subsection{Overview}
\label{subsection:framework-overview}
The proposed framework redefines a scientific figure as a composite computational artifact that is both human-legible and machine-interpretable. 
We refer to such artifacts as \textbf{LLM-native figures}. Each artifact encapsulates the full analytical provenance underlying its visualization--linking the rendered image, the visualization specification, the data subset, and the computational process that produced it. 
This representation enables two-way translation: 
language models can generate and manipulate figures through natural-language instructions, 
and user interactions with the figure can be automatically interpreted as structured analytical operations \wyf{for further deep dive}.

The framework consists of three primary components \wyf{(Fig. 1)}:
(1) a \textbf{representation schema} that defines the structure of LLM-native figures;
(2) a \textbf{bidirectional mapping engine} that connects visual elements to their underlying data and analytic transformations; and
(3) an \wyf{\textbf{artifact store}} that captures complete provenance across iterative analytical steps.
Together, these components transform figures from static outputs into dynamic interfaces for transparent, reproducible, and collaborative computation \wyf{in data-driven scientific discovery}. 


\subsection{Representation of LLM-Native Figures}
\label{subsection:framework-representation}
Each LLM-native figure $F$ is represented as a tuple: 

\begin{equation}
F = \{V, S, D, C, M\}
\end{equation}

where $V$ denotes the rendered visualization (\eg, an SVG or raster image), 
$S$ is the declarative visualization specification, such as a Vega-Lite schema~\cite{satyanarayan2016vega}, that encodes visual mappings between \wyf{data attributes and visual channels (\eg, width, size, and color)}, 
$D$ represents the underlying data used or captured in the visualization, including \wyf{data subsets and corresponding schema, and user selection and filters}, 
% metadata on source, schema, and selection filters, 
$C$ records the executable analytical code (\eg, Python or SQL) that generated $D$ and $V$, 
and $M$ captures metadata \wyf{of the exploration history}, including timestamps, version identifiers, natural-language summaries, and links to related artifacts.

This structured representation ensures that every visual element in $V$ is traceable to the corresponding data entries in $D$ and the computational steps in $C$. 
Conversely, any modification to $S$, $D$, or $C$ automatically updates $V$ and records the change in $M$. 
The tuple thus forms a closed and reproducible description of the analytical state at the moment the figure is produced.


\subsection{Bidirectional Mapping}
\label{subsection:framework-bidirectional-mapping}
Central to the framework is a bidirectional mapping between visual and analytical representations. 
The mapping enables two classes of operations:

\begin{itemize}
    \item \textbf{Language-to-visual operations.} Natural-language instructions are parsed by the LLM into structured analytical actions, such as data filtering, transformation, and visual encoding, that modify $S$, $D$, or $C$, resulting in an updated $V$ \wyf{(Fig.~\ref{fig:framework}, path: \textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3})}. 
    \item \textbf{Visual-to-analytical operations.} User interactions with the visualization (\eg, clicking a data point, selecting a region, or modifying an axis) are translated into structured analytical commands that reference the affected data subset and trigger corresponding updates to the analytical pipeline \wyf{(Fig.~\ref{fig:framework}, path: \textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c})}.
\end{itemize} 


Formally, these mappings are implemented through \wyf{a semantic layer} that maintains correspondences between visual marks in $V$ and their provenance within $D$ and $C$. 
This layer allows the LLM to reason over the structure of the visualization, \wyf{identify which analytical operations produced each element, and generate consistent updates}. 

The bidirectional mapping extends beyond static translation: it supports compositional reasoning, where a sequence of natural-language and visual interactions are merged into a coherent analytical plan. 
This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


\subsection{Artifact Store and Provenance}
\label{subsection:framework-artifact-store}

\wyf{Todo: think about moving artifact definition from Method to here.}

All analytical operations are recorded in an artifact store, a version-controlled ledger that tracks the evolution of each figure and its underlying analyses. 
Each entry in the store consists of: 

\begin{itemize}
    \item \textbf{Action record}: the users' natural-language prompt or visual action, its parsed structured representation, and the execution context; 
    \item \textbf{Execution result}: the updated analytical code $C_t$, \wyf{data subset $D_t$}, and visualization specification $S_t$;
    \item \textbf{Derived artifact}: the resulting figure $F_t$ and metadata $M_t$;
    \item \textbf{Parent linkage}: references to preceding artifacts to maintain the complete analytical lineage.
\end{itemize}

This structure forms a directed acyclic graph of artifacts, where each node represents a reproducible state and each edge an analytical transformation. 
The graph allows any prior state to be reconstructed or branched, ensuring traceability and supporting collaborative editing among multiple users or agents.

The artifact store serves two key functions. 
First, it enforces \textit{reproducibility}: every output is linked to an executable record of how it was produced. 
Second, it enables reasoning \textit{transparency}: by exposing the intermediate steps of analysis, both humans and models can audit and explain results at any level of detail. 


\subsection{Integration with Large Language Models}
\label{subsection:framework-llm}
Large language models interact with the framework through an action–observation loop. 
The model receives user instructions and contextual information from the artifact store, generates candidate analytical actions, reasoning over complex data, and validates them through code execution.
Execution outputs--including errors, visualization updates, and text summaries--are fed back to the model for refinement.

To constrain the model's behavior and ensure reliability, LLMs could choose analytical actions from an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
% To constrain the model's behavior and ensure reliability, the system employs an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
The LLM operates within this space, translating natural-language input into valid action sequences that are interpretable, executable, and reversible through provenance records.
\wyf{Domain-specific customizations (\eg, tailored AI agents and tool designs~\cite{gao2025democratizing}) could be integrated into this framework to enhance these capabilities to specialized domain contexts.}

This integration turns the LLM into an orchestrator of analytical operations rather than a black-box generator, aligning model reasoning with the explicit structure of the computational pipeline.


\subsection{Summary}
\label{subsection:framework-summary}
The framework establishes a general method for constructing and reasoning with machine-interpretable scientific artifacts. 
By embedding analytical provenance within each figure, maintaining bidirectional mappings between visualization and data, and recording every analytical step in an artifact store, the approach enables transparent, reproducible, and mixed-initiative data exploration. 
\wyf{These properties form the foundation for evaluating the system's performance and generality in the next section.}








% % %%%%%%%%%%%%%%%%% prev introduction part %%%%%%%%%%%%%%%%%
% % our method
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }







% \wyf{(generalizability levels: 
%         [level 1]: SciSciCanvas (use SciSci as an example domain); 
%         [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
%         [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
%         [level 4]: HAI for all scenarios (general public + expert-oriented systems)
%     )}


% 宋阳秋老师2025.05刚发的一个survey: https://github.com/HKUST-KnowComp/Awesome-LLM-Scientific-Discovery 


% Tiantian:
% 4. In different scenarios, how AI and human can collaborate — can we think of a framework that can incoorperate SciSciGPT and SciSciCanvas? — in both interaction design, and underlying HAI4Science workflow?


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-1.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-2.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



% Framework for Integrating SciSciGPT and SciSciCanvas
% A unified HAI4Science workflow could blend both systems:
% Interaction Design
% Language-to-Visualization Bridging: Users pose questions via SciSciGPT (LUI), which generates interactive visual artifacts in SciSciCanvas (GUI).
% Bidirectional Control: Modify a chart (GUI) to auto-update the LLM’s context (e.g., "Focus on papers from 2020–2025"), enabling mixed-initiative exploration.

% Underlying Workflow
% Multi-Agent Collaboration: SciSciGPT parses intent and delegates tasks (e.g., trend analysis) to domain-specific AI agents, while SciSciCanvas renders results as manipulable visualizations.
% Iterative Refinement: Users toggle between refining hypotheses (LUI) and adjusting visual parameters (GUI), creating a closed-loop discovery process.







% 7. Automation
% Definition: Use of computational techniques to conduct repetitive analytical tasks, freeing researchers for higher-level conceptual work.

% Support: Jordan & Mitchell (2015); Kitano (2016).

% - Shift of human roles: transfer from executor to idea generator.
% - Scientific discovery workflow: step by step, AI take over low-level roles.
% - During this shifting, think about transparency, rigous of discovery process

==> sections/archive/03-1-framework/03-1-framework_v2_20251114.tex <==
\section{Conceptual Framework}
\label{section:conceptual-framework} 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/framework.jpg}
    \caption{The conceptual framework for iterative exploration for data-driven scientific discovery.
    % 
    \textbf{Left}: Five-layer structure of the framework, including user inputs, AI outputs (LLM-native figures and data-driven artifacts) and the underlying LLM engine and databases. 
    % 
    \textbf{Top-Right}: structure of an LLM-native figure at timestamp $t$, which supports bidirectional mapping between visual ($V$) and analytical ($C$ and $D$) representations, along with associated metadata $M$. 
    % 
    \textbf{Bottom-Right}: Definition of a data-driven artifact. 
    Starting from a focal figure, analyses can be iteratively refined or extended, supporting non-linear human exploration logic. Two example interaction modes are illustrated:
    (1) \textit{Manipulating} existing figures to refine or reorient the analysis focus, and
    (2) \textit{Drilling down} from user-interested data points within the focal figure to generate new, coordinated figures that enable progressive, in-depth exploration through filtering and brushing. 
    \wyf{TODO: add one more component: paper text + figure (one A4 page (Case 1: policy paper)), and scientific discovery properties (transparency, reproducibility)--conceptually draw several curves to demonstrate tracing procedure, along with code, data, vis, human non-linear logic, etc.}
    }
    \label{fig:framework}
\end{figure}


\subsection{Overview}
\label{subsection:framework-overview}
The proposed framework redefines a scientific figure as a composite computational artifact that is both human-legible and machine-interpretable. 
We refer to such artifacts as \textbf{LLM-native figures}. 
Each artifact encapsulates the full analytical provenance underlying its visualization, linking the rendered image, the visualization specification, the generated data insight, the data subset, and the computational process that produced it. 
This representation enables two-way translation: 
language models can generate through natural-language instructions (Fig.~\ref{fig:framework}-\textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3}), 
and user graphical interactions \wyf{and natural-language instructions} with the figure can be automatically interpreted as structured analytical operations for deep dive (Fig.~\ref{fig:framework}-\textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c}).

The framework consists of three primary components \wyf{(Fig.~\ref{??})}:
(1) a \textbf{representation schema} that defines the structure of LLM-native figures (Sec.~\ref{subsection:framework-llm-native-figure});
(2) a \textbf{bidirectional mapping engine} that connects visual elements to their underlying data and analytic transformations (Sec.~\ref{subsection:framework-bidirectional-mapping}); and
(3) a \textbf{data-driven artifact} that captures complete provenance across iterative analytical steps (Sec.~\ref{subsection:framework-data-driven-artifact}).
Together, these components transform figures from static outputs into dynamic interfaces for transparent and reproducible computation. 


\subsection{Representation of LLM-Native Figures}
\label{subsection:framework-llm-native-figure}
Each LLM-native figure at timestamp $t$ is represented as a tuple: 
\wyf{[Yifang: think about whether to add QA pair here. I feel we may not add here. But try to mention QA (especially user input: LUI and GUI) in somewhere.]}
\begin{equation}
F_t = \{I, V, C, D, M\}
\end{equation}
where 
\wyf{$I$ represents user inputs including natural-language instructions and graphical interactions on the visualization (\eg, selection and filtering) [yifang: this is also a special point of LLM-native Figure: be bound with Q\&A. But rethink about implementation: current \textit{dashboard} table does not have this attribute, instead, it is stored at table \textit{message_attachments}. And these user input may come from the prev figure, not this generated figure. TODO: figure out if this could be mapped to Method section.]}, 
$V$ denotes the rendered visualization, which could be represented by multiple modalities, including the raster image, the declarative visualization specification (\eg, Vega-Lite schema~\cite{satyanarayan2016vega}) that encodes visual mappings between data attributes and visual channels (\eg, size and color) and supports interactive behaviors, 
\wyf{and the textual summary of the visualization’s key insights.} 
% where $V$ denotes the rendered visualization (\eg, an SVG or raster image), 
% $S$ is the declarative visualization specification, such as a Vega-Lite schema~\cite{satyanarayan2016vega}, that encodes visual mappings between \wyf{data attributes and visual channels (\eg, width, size, and color)}, 
$C$ records \wyf{the analytical actions (Sec.~\ref{subsection:method-action-space})} and corresponding executable code (\eg, SQL and Python) that generated $D$ and $V$, 
$D$ represents the underlying data used in the visualization (\eg, data subsets and associated data schema, and aggregated results used for rendering),
% metadata on source, schema, and selection filters, 
and $M$ represents the metadata associated with this figure within the user's exploration history, including the timestamp $t$, version identifier, text summary of user behaviors, and links to corresponding data-driven artifacts.

This structured representation ensures that every visual element in $V$ is traceable to the corresponding computational steps in $C$ and data entries in $D$. 
Conversely, any modification to $D$ or $C$ automatically updates $V$ and records the change in $M$. 
The tuple thus forms a closed and reproducible description of the analytical state at the moment the figure is produced.


\subsection{Bidirectional Mapping}
\label{subsection:framework-bidirectional-mapping}
Central to the framework is a bidirectional mapping between visual and analytical representations of a figure. 
The mapping enables two classes of operations:

\begin{itemize}
    \item \textbf{Analytical-to-visual operations.} User natural-language instructions are parsed by the LLM into structured analytical actions, such as data filtering, transformation, modeling, and visualization, that modify $C$ or $D$, resulting in an updated $V$ \wyf{(Fig.~\ref{fig:framework}, path: \textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3})}. 
    \item \textbf{Visual-to-analytical operations.} User interactions on $V$ (\eg, clicking a data point, selecting a region, or modifying an axis) together with natural-language instructions are are interpreted by the LLM and translated into structured analytical commands that reference the affected data subset $D$ and trigger corresponding updates to the analytical pipeline ($C$ and $D$) to refine existing insights or enable deeper insight exploration~\wyf{(Fig.~\ref{fig:framework}, path: \textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c})}.
\end{itemize} 

Formally, these mappings are implemented through \wyf{a semantic layer} that maintains correspondences between visual representation in $V$ and their provenance within $C$ and $D$. 
This layer allows the LLM to reason over the structure of the visualization, identify which analytical operations produced each visual element, and generate consistent updates. 

The bidirectional mapping extends beyond static translation: it supports compositional reasoning, where a sequence of natural-language and graphical interactions are merged into a coherent analytical plan. 
This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


\subsection{Artifact and Provenance}
\label{subsection:framework-data-driven-artifact}
All LLM-Native Figures together with their visual and analytical operations \wyf{(actions)} are recorded in a \textbf{data-driven artifact} (Fig.~\ref{fig:data-driven-artifact}), a reusable, composable unit of exploration comprising one or more coordinated figures that encode the human's iterative analytical logic.
% a version-controlled ledger that records one or more figures and their exploration history, capturing both intra-figure revisions and inter-figure coordination that links a figure to its derived successors.
% a version-controlled ledger that tracks the evolution of each figure and its underlying analyses, as well as its coordinated other figures. 
Each artifact records not only the resulting figures but also the sequence of thought: the \textit{manipulations}---edit existing figures to refine or reorient the analysis focus, \textit{drill-downs}---analyses that generate new, coordinated figures from user-selected data points, and the transitions that produced them. 
Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, revisited, and shared across similar analysis tasks. 

% 维度1: artiface和figure的关系
Each artifact $A$ at timestamp $t$ consists of: 
\begin{itemize}
    \item \textbf{User input}: the users' natural-language instruction or graphical interaction and its parsed structured representation (Fig.~\ref{fig:framework}-\textit{User Input}); 
    \item \textbf{Analytical execution result}: 
    the analytical operation invoked by the user input, including the updated analytical code $C$ and corresponding \wyf{data subset $D$} that define the computation underpinning the figure (Fig.~\ref{fig:framework}-\textit{LLM-Native Figure: Analytical Representation});
    \item \textbf{Derived figure}: the derived or updated figure $F_t$ and its associated metadata $M$ (Fig.~\ref{fig:framework}-\textit{LLM-Native Figure: Visual Representation}); 
    \item \textbf{Coordination linkage}: the updated coordination graph that records how the figures within the artifact are connected to one another by different brushing and filtering schema. 
    % \item \textbf{Execution result}: the updated analytical code $C_t$, \wyf{data subset $D_t$}, and visualization specification $S_t$;
    % \item \textbf{Derived artifact}: the resulting figure $F_t$ and metadata $M_t$;
    % \item \textbf{Parent linkage}: references to preceding artifacts to maintain the complete analytical lineage.
\end{itemize}

% 维度2: artiface自身的版本控制
Additionally, an artifact $A$ is maintained as a version-controlled ledger ($A_{t_1}$, $A_{t_2}$, ... $A_{t_n}$), which forms a directed acyclic graph of artifact versions, where each node represents a reproducible state and each edge an analytical transformation. 
The graph allows any prior state to be reconstructed or branched, ensuring traceability and supporting collaborative editing among multiple users or AI agents.

The design of data-driven artifact serves two key functions. 
First, it enforces \textit{reproducibility}: every output is linked to an executable record of how it was produced. 
Second, it enables reasoning \textit{transparency}: by exposing the intermediate steps of analysis \wyf{(such as action-level reasoning -- to write at Method seciton)}, both humans and models can audit and explain results at any level of detail. 

\wyf{[yifang: To revise the last paragraph above: reconsider whether \textit{user_input} should be included in the artifact or the dashboard. It feels somewhat inappropriate from an implementation perspective, though it fits better conceptually within the framework description.]}


\subsection{Integration with Large Language Models}
\label{subsection:framework-llm}
Large language models interact with the framework through an plan-action–observation loop. 
The model receives user instructions and interactions, along with contextual information from the artifact and conversational history, to generate candidate analytical actions, reasoning over complex data, and validates them through code execution.
Execution outputs, including visualization and textual insights, generated data, and potential errors, are then fed back to the model to inform the next step of action selection. 

To constrain the model's behavior and ensure reliability, LLMs could choose analytical actions from an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization) (Sec.~\ref{subsection:method-action-space}). 
% To constrain the model's behavior and ensure reliability, the system employs an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
The LLM operates within this space, translating natural-language input into valid action sequences that are interpretable, executable, and reversible through provenance records.
Domain-specific customizations (\eg, tailored AI agents and tool designs~\cite{gao2025democratizing}) could be integrated into this framework to enhance these capabilities to specialized domain contexts.

This integration turns the LLM into an orchestrator of analytical operations rather than a black-box generator, aligning model reasoning with the explicit structure of the computational pipeline.


\subsection{Summary}
\label{subsection:framework-summary}
The framework establishes a general method for constructing and reasoning with machine-interpretable scientific artifacts. 
By embedding analytical provenance within each figure, maintaining bidirectional mappings between visualization and data, and recording every analytical step in an artifact store, the approach enables transparent, reproducible, and mixed-initiative data exploration. 
\wyf{These properties form the foundation for evaluating the system's performance and generality in the next section.}








% % %%%%%%%%%%%%%%%%% prev introduction part %%%%%%%%%%%%%%%%%
% % our method
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }







% \wyf{(generalizability levels: 
%         [level 1]: SciSciCanvas (use SciSci as an example domain); 
%         [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
%         [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
%         [level 4]: HAI for all scenarios (general public + expert-oriented systems)
%     )}


% 宋阳秋老师2025.05刚发的一个survey: https://github.com/HKUST-KnowComp/Awesome-LLM-Scientific-Discovery 


% Tiantian:
% 4. In different scenarios, how AI and human can collaborate — can we think of a framework that can incoorperate SciSciGPT and SciSciCanvas? — in both interaction design, and underlying HAI4Science workflow?


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-1.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-2.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



% Framework for Integrating SciSciGPT and SciSciCanvas
% A unified HAI4Science workflow could blend both systems:
% Interaction Design
% Language-to-Visualization Bridging: Users pose questions via SciSciGPT (LUI), which generates interactive visual artifacts in SciSciCanvas (GUI).
% Bidirectional Control: Modify a chart (GUI) to auto-update the LLM’s context (e.g., "Focus on papers from 2020–2025"), enabling mixed-initiative exploration.

% Underlying Workflow
% Multi-Agent Collaboration: SciSciGPT parses intent and delegates tasks (e.g., trend analysis) to domain-specific AI agents, while SciSciCanvas renders results as manipulable visualizations.
% Iterative Refinement: Users toggle between refining hypotheses (LUI) and adjusting visual parameters (GUI), creating a closed-loop discovery process.







% 7. Automation
% Definition: Use of computational techniques to conduct repetitive analytical tasks, freeing researchers for higher-level conceptual work.

% Support: Jordan & Mitchell (2015); Kitano (2016).

% - Shift of human roles: transfer from executor to idea generator.
% - Scientific discovery workflow: step by step, AI take over low-level roles.
% - During this shifting, think about transparency, rigous of discovery process

==> sections/archive/03-1-framework/03-1-framework_v3_20251201.tex <==
\subsection{Conceptual Framework}
\label{subsection:conceptual-framework} 
\newlyadded{We propose our conceptual framework about LLM-native figures with core components, including the representation of a figure, the bi-directional mapping between visual and analytical operations, the data-driven artifact, and how the backbone of the figure--LLM engine--support scientific provenance.} 


\subsubsection{Overview}
\label{subsubsection:framework-overview}
% \wyf{[TODO]: make the term: artifact consistent.}
The proposed framework redefines a scientific figure as a composite computational object that is both human-legible and machine-interpretable. 
We refer to such figures as \textbf{LLM-native figures}. 
Each LLM-native figure encapsulates the full analytical provenance underlying its visualization, linking the rendered image, the visualization specification, the generated data insight, the data subset, and the computational process that produced it.

% example scenario: climate
\newlyadded{
To illustrate the core ideas behind the framework, we use a simple scientific task involving structured observational data. 
Consider a researcher analyzing environmental sensor data collected over multiple years, including monthly temperature, \wyf{humidity, and air-quality [yifang: need to add more tables in DB]} measurements. 
The researcher issues the natural-language instruction:
\textit{``Plot the temporal trend of the temperature by month in the state of Florida in the last year (2024).''}
% “Plot the average daily temperature by month for the last five years.”
The system responds with a line plot showing 12 monthly temperatures for Florida (Fig.~\ref{fig:bidirectional-mapping}-A1). 
The researcher then brush to filter the months of June–August in the visualization to examine and compare summer temperatures with other states (Fig.~\ref{fig:bidirectional-mapping}-A2). 
The system interprets this interaction, identifies the corresponding data subset, and refines the analysis by generating a second figure that compares the average summer temperatures during those months across different states (Fig.~\ref{fig:bidirectional-mapping}-A5).
% The researcher then brush to filter the months of June–August in the visualization to examine summer patterns in greater detail. 
% The system interprets this interaction, identifies the corresponding data subset, and refines the analysis by generating a second figure that compares the month-to-month variability during those months across the five-year period.
}

% key feature of LLM-native figure
\newlyadded{
This simple example illustrates the two key capabilities of the framework:
\textbf{(1) Analytical operations → Visualization}. 
Natural-language instructions are translated into structured analytical steps that filter, aggregate, and visualize data (Fig.~\ref{fig:framework}-\textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3}). 
\textbf{(2) Visualization → Analytical operations}. % → Updated analysis
Interactions on the figure, such as selecting a range, clicking on a mark, or modifying an axis, and together with natural-language instructions, are treated as inputs that trigger corresponding analytical operations for follow-up analysis (Fig.~\ref{fig:framework}-\textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c}). 
In both cases, the system records how each figure is produced: the data subset extracted, the transformations applied, and the visualization specification generated. 
Together, these components form a machine-interpretable \textbf{LLM-native figure} that can be reused, recomposed, or extended in subsequent steps, and thus transform scientific figures from static outputs into dynamic interfaces for transparent and reproducible computation. 
}

\newlyadded{
The remainder of this section generalizes the ideas from this simple example and formalizes the framework's representation (Sec.~\ref{subsubsection:framework-llm-native-figure}), bidirectional mapping (Sec.~\ref{subsubsection:framework-bidirectional-mapping}), and provenance model based on data-driven artifact (Sec.~\ref{subsubsection:framework-data-driven-artifact}).
}
% The framework consists of three primary components (Fig.~\ref{fig:framework}):
% (1) a \textbf{representation schema} that defines the structure of LLM-native figures (Sec.~\ref{subsection:framework-llm-native-figure});
% (2) a \textbf{bidirectional mapping engine} that connects visual elements to their underlying data and analytic transformations (Sec.~\ref{subsection:framework-bidirectional-mapping}); and
% (3) a \textbf{data-driven artifact} that captures complete provenance across iterative analytical steps (Sec.~\ref{subsection:framework-data-driven-artifact}).
% Together, these components transform figures from static outputs into dynamic interfaces for transparent and reproducible computation. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/extended-chart.jpg}
    \caption{ 
    \newlyadded{Dynamic generation, coordination, and preservation of LLM-native figures. 
    (A) Drill-down figure generation. 
    % The process of generating a new figure for drill-down. 
    Starting from an existing figure that displays the 12-month temperature trend in Florida (A1), the user brushes a temporal interval and specify a follow-up analytical intent in natural language (A2).
    The framework applies the \textbf{Visualization-to-Analytical operations} mapping to translate these mixed-modality inputs into precise database queries (A3),  enabling the system to retrieve exactly the subset of data implied by the user's visual and linguistic cues.  
    It then applies the \textbf{Analytical operations-to-Visualization} mapping to generate a new interactive figure that supports deeper exploration (A5). 
    % First, the framework uses the \textbf{Visualization-to-Analysis} mapping (A1-A3) to transfer the user interactions (\ie, brushing a time period) and natural language intent (A2) to data points (A3). 
    % It then uses the \textbf{Analytics-to-Visualization} mapping to generate the new interactive figure (A5). 
    (B) Real-time coordination between linked figures. 
    When users adjust the focus in one figure (\eg, brushing a different temporal window, B1), the linked figure updates automatically (B3). 
    To enable fast, stable coordination, the system pre-computes and stores the coordination relation and executable code template at the moment the new figure is created (A4), allowing subsequent interactions to directly retrieve and update the relevant code (B2) to query database.
    % Users can brush to filter another time period (B1), and the data in the other figure will be updated automatically (B3). 
    % Specifically, to make the coordination more efficient, during the implementation, we first generate and store the coordination link and code template when first generating the new figure (A4), so that in the following up analysis, the system could directly loop up the coordination link and code and update the code accordingly based on the new filtering criteria (B2). 
    (C) Persistent, revisitable artifacts. 
    The linked figures, together with their underlying code, data, and coordination rules, are all stored in the data-driven artifact that captures the user's exploration trajectory and supports future revisits, refinements, and extensions. 
    }
    }
    \label{fig:bidirectional-mapping}
\end{figure}




\subsubsection{Representation of LLM-Native Figures}
\label{subsubsection:framework-llm-native-figure}

\newlyadded{Building on the example above, each figure (Fig.~\ref{fig:framework}-A) produced by the system at timestamp $t$ is represented as a structured format:}
% Each LLM-native figure at timestamp $t$ is represented as a tuple: 

\begin{equation}
F_t = \{V_t, C_t, D_t, M_t\}
% F_t = \{I, V, C, D, M\}
\end{equation}

where 
% $I$ represents user's intent and inputs including natural-language instructions and graphical interactions on the visualization such as selection and brushing (Fig.~\ref{fig:bidirectional-mapping}-A2, Fig.~\ref{fig:framework}-User Input). 
$V_t$ denotes the rendered visualization (Fig.~\ref{fig:framework}-A1), represented by multiple modalities including the raster image (\eg, PNG), the declarative visualization specification (\eg, Vega-Lite JSON schema~\cite{satyanarayan2016vega}) that encodes visual mappings that transform data attributes into visual channels (\eg, position, size, and color) and supports interactive behaviors, 
and the textual summary of the visualization’s key insights.
\newlyadded{Each visual mark in the visualization ($V_t$) (\eg, a point, bar, or line segment) has a unique identifier that maps to corresponding rows or groups in the dataset ($D_t$, Fig.~\ref{fig:framework}-A3). 
Together, these modalities make the figure not only human-readable but computationally navigable.} 
% where $V$ denotes the rendered visualization (\eg, an SVG or raster image), 
% $S$ is the declarative visualization specification, such as a Vega-Lite schema~\cite{satyanarayan2016vega}, that encodes visual mappings between \wyf{data attributes and visual channels (\eg, width, size, and color)}, 
$C_t$ records the analytical actions (Sec.~\ref{subsection:method-action-space}) and corresponding executable code (\eg, SQL and Python) that generated $D_t$ and $V_t$ (Fig.~\ref{fig:framework}-A2).
$D_t$ represents the underlying data used in the visualization, such as data subsets and associated data schema, and aggregated results used for rendering (Fig.~\ref{fig:framework}-A3),
% metadata on source, schema, and selection filters, 
and $M_t$ represents the metadata associated with this figure within the user's exploration history, such as the timestamp $t$, version identifier, type and description of user operations, and links to corresponding data-driven artifacts (Fig.~\ref{fig:framework}-A4).

This structured representation ensures that every visual element in $V_t$ is traceable to the corresponding computational steps in $C_t$ and data entries in $D_t$. 
Conversely, any modification to $D_t$ or $C_t$ automatically updates $V_t$ and records the change in $M_t$. 
The tuple thus forms a closed and reproducible description of the analytical state at the moment the figure is produced.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/framework.jpg}
    \caption{The conceptual framework for iterative exploration for data-driven scientific discovery.
    % 
    \textbf{Left}: Five-layer structure of the framework, including user inputs, AI outputs (LLM-native figures and data-driven artifacts) and the underlying LLM engine and databases. 
    % 
    \textbf{Top-Right}: structure of an LLM-native figure at timestamp $t$, which supports bidirectional mapping between visual ($V$) and analytical ($C$ and $D$) representations, along with associated metadata $M$. 
    % 
    \textbf{Bottom-Right}: Definition of a data-driven artifact. 
    Starting from a focal figure, analyses can be iteratively refined or extended, supporting non-linear human exploration logic. Two example interaction modes are illustrated:
    (1) \textit{Manipulating} existing figures to refine or reorient the analysis focus, and
    (2) \textit{Drilling down} from user-interested data points within the focal figure to generate new, coordinated figures that enable progressive, in-depth exploration through filtering and brushing. 
    }
    \label{fig:framework}
\end{figure}



\subsubsection{Bidirectional Mapping Between Visualization and Analysis}
\label{subsubsection:framework-bidirectional-mapping}
Central to the framework is a bidirectional mapping between visual and analytical representations of a figure. 
The mapping enables two classes of operations:

\begin{itemize}
    \item \textbf{Analytical operations-to-Visualization.} 
    % \item \textbf{Language-to-Analytical-to-Visualization.} 
    \newlyadded{The user instruction (\ie, \textit{``Plot the temporal trend of the temperature by month in the state of Florida in the last year (2024)''}) is parsed by the LLM into a sequence of analytical actions (Sec.~\ref{subsection:method-action-space}), including selecting relevant tables and columns (\eg, the \textit{temperature}, \textit{year}, and \textit{state} fields), filter rows (\eg, by \textit{state} and \textit{year} fields), and assigning the chart type, visual encoding, chart interactions, and textual insights.} 
    These actions will generate code $C$ and compute data $D$, resulting in a new or updated visualization $V$ to render the figure (Fig.~\ref{fig:bidirectional-mapping}-A1, Fig.~\ref{fig:framework}-path: \textsquarenumber{1} → \textsquarenumber{2} → \textsquarenumber{3}).
    % User natural-language instructions are parsed by the LLM into structured analytical actions, such as data filtering, transformation, modeling, and visualization, that modify $C$ or $D$, resulting in an updated $V$ \wyf{(Fig.~\ref{fig:framework}, path: \textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3})}. 
    \item \textbf{Visualization-to-Analytical operations.} 
    \newlyadded{
    When the user brushes the figure with the time range June-August in the generated temporal line chart and ask a follow-up question about the summer period (Fig.~\ref{fig:bidirectional-mapping}-A2), 
    % to compare the average temperature of each state in the selected summer period, 
    the system identifies the corresponding visual brushed area, retrieves the relevant data in $D$ (\ie, filtering the data to those months), and combines the filtered subset of data with the user instruction to construct a new sequence of analytical actions before generating an updated figure (Fig.~\ref{fig:framework}-path: \textsquarecharacter{a} → \textsquarecharacter{b} → \textsquarecharacter{c}).
    }
    % User interactions on $V$ (\eg, clicking a data point, selecting a region, or modifying an axis) together with natural-language instructions are are interpreted by the LLM and translated into structured analytical commands that reference the affected data subset $D$ and trigger corresponding updates to the analytical pipeline ($C$ and $D$) to refine existing insights or enable deeper insight exploration~\wyf{(Fig.~\ref{fig:framework}, path: \textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c})}.
\end{itemize} 

\newlyadded{Formally, the framework maintains a mapping relationship:
\begin{equation}
% R_t = \{\,(\mathrm{visual\_mark},\ \mathrm{data\_rows},\ \mathrm{code})\,\}
R_t = \{\,(\mathrm{visual\_mark},\ \mathrm{data\_rows},\ \mathrm{analytical\_operation})\,\}
% 花括号 { } 表示集合（set），圆括号 ( ) 表示元组（tuple）
\end{equation}
associating each visual element and GUI interaction with the data and computation codes that produced it. 
This mapping enables consistent, verifiable round-trips between visual states and analytical states, allowing figures to serve as reliable interactive interfaces for scientific reasoning.
}
% Formally, these mappings are implemented through \wyf{a semantic layer} that maintains correspondences between visual representation in $V$ and their provenance within $C$ and $D$. 
% This layer allows the LLM to generate 
% reason over the structure of the visualization, identify which analytical operations produced each visual element, and generate consistent updates. 
% The bidirectional mapping extends beyond static translation: it supports compositional reasoning, where a sequence of natural-language and graphical interactions are merged into a coherent analytical plan. 
This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


\subsubsection{Artifact and Provenance}
\label{subsubsection:framework-data-driven-artifact}
\newlyadded{
Every analytical step, whether triggered by language or by visual interaction, passes through a single execution pipeline. The framework understands the user intent ($I_t$), generates and executes code ($C_t$) in a controlled environment, updates the data subset ($D_t$), and generates a new visualization ($V_{t+1}$).
}
All figures together with their analysis codes, underlying data, and coordination rules are recorded in a \textbf{data-driven artifact} (Fig.~\ref{fig:framework}-B and Fig.~\ref{fig:bidirectional-mapping}-C), a reusable, composable unit of exploration comprising one or more coordinated figures that encode the human's iterative analytical logic.
% a version-controlled ledger that records one or more figures and their exploration history, capturing both intra-figure revisions and inter-figure coordination that links a figure to its derived successors.
% a version-controlled ledger that tracks the evolution of each figure and its underlying analyses, as well as its coordinated other figures. 
Each artifact records not only the resulting figures but also the sequence of thought: \textit{manipulation}---iterates existing figures to refine or reorient the analysis focus, and \textit{drill-down} or \textit{bottom-up}---analyses that generate new, coordinated figures from user-selected data points, and the transitions that produced them. 
Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, revisited, and shared across similar analysis tasks. 

% 维度1: artiface和figure的关系
Each artifact $A$ at timestamp $t$ consists of: 
\begin{itemize}
    \item \textbf{User input ($I_t$)}: the users' natural-language instruction or graphical interaction and its parsed structured representation (Fig.~\ref{fig:framework}-\textit{User Input}); 
    \item \textbf{Derived figures ($F_t$)}: one or more figures generated during the exploration of a research problem. Each figure includes the analytical execution result (code $C_t$ and data $D_t$), the resulting visualization $V_t$, and associated meta information $M_t$ (Fig.~\ref{fig:framework}-A). 
    % \item \textbf{Analytical execution result ($C_t$, $D_t$)}: 
    % the analytical operation invoked by the user input, including the updated analytical code $C_t$ and corresponding data $D_t$ that define the computation underpinning the figure (Fig.~\ref{fig:framework}-A2, A3);
    % \item \textbf{Derived visualization ($V_t$, $M_t$)}: the derived or updated visualization $V_t$ and its associated metadata $M_t$ (Fig.~\ref{fig:framework}-A1, A4); 
    \item \textbf{Coordination linkage and schema}: the updated coordination graph and code that records how the figures within the same artifact are connected to one another by different brushing and filtering schema (Fig.~\ref{fig:bidirectional-mapping}-A4, B2). 
    % \item \textbf{Execution result}: the updated analytical code $C_t$, \wyf{data subset $D_t$}, and visualization specification $S_t$;
    % \item \textbf{Derived artifact}: the resulting figure $F_t$ and metadata $M_t$;
    % \item \textbf{Parent linkage}: references to preceding artifacts to maintain the complete analytical lineage.
\end{itemize}

% 维度2: artiface自身的版本控制
Additionally, an artifact $A$ is maintained as a version-controlled ledger ($A_{t_1}$, $A_{t_2}$, ... $A_{t_n}$), which forms a directed acyclic graph of artifact versions, where each node represents a reproducible state and each edge an analytical transformation. 
The graph allows any prior state to be reconstructed or branched, ensuring traceability and supporting collaborative editing among multiple users or AI agents.

The design of data-driven artifact serves two key functions. 
First, it enforces \textit{reproducibility}: every output is linked to an executable record of how it was produced. 
Second, it enables reasoning \textit{transparency}: by exposing the intermediate steps of analysis \wyf{(such as action-level reasoning -- to write at Method seciton)}, both humans and models can audit and explain results at any level of detail. 

% \wyf{[yifang: To revise the last paragraph above: reconsider whether \textit{user_input} should be included in the artifact or the dashboard. It feels somewhat inappropriate from an implementation perspective, though it fits better conceptually within the framework description.]}


\subsubsection{Integration with Large Language Models}
\label{subsubsection:framework-llm}
Large language models interact with the framework through an plan-action–observation loop (Sec.~\ref{section:methods}). 
The model receives user instructions and interactions, along with contextual information from the artifact and conversational history, to generate candidate analytical actions, reasoning over complex data, and validates them through code execution.
Execution outputs, including visualization and textual insights, generated data, and potential errors, are then fed back to the model to inform the next step of action selection. 

To constrain the model's behavior and ensure reliability, LLMs could choose analytical actions from an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization) (Sec.~\ref{subsection:method-action-space}). 
% To constrain the model's behavior and ensure reliability, the system employs an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
The LLM operates within this space, translating natural-language input into valid action sequences that are interpretable, executable, and reversible through provenance records.
Domain-specific customizations (\eg, tailored AI agents and tool designs~\cite{gao2025democratizing}) could be integrated into this framework to enhance these capabilities to specialized domain contexts.

This integration turns the LLM into an orchestrator of analytical operations rather than a black-box generator, aligning model reasoning with the explicit structure of the computational pipeline.


\subsubsection{Summary}
\label{subsubsection:framework-summary}
The framework establishes a general method for constructing and reasoning with machine-interpretable scientific artifacts. 
By embedding analytical provenance within each figure, maintaining bidirectional mappings between visualization and data, and recording every analytical step in an artifact store, the approach enables transparent, reproducible, and mixed-initiative data exploration. 
\wyf{These properties form the foundation for evaluating the system's performance and generality in the next section.}








% % %%%%%%%%%%%%%%%%% prev introduction part %%%%%%%%%%%%%%%%%
% % our method
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }







% \wyf{(generalizability levels: 
%         [level 1]: SciSciCanvas (use SciSci as an example domain); 
%         [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
%         [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
%         [level 4]: HAI for all scenarios (general public + expert-oriented systems)
%     )}


% 宋阳秋老师2025.05刚发的一个survey: https://github.com/HKUST-KnowComp/Awesome-LLM-Scientific-Discovery 


% Tiantian:
% 4. In different scenarios, how AI and human can collaborate — can we think of a framework that can incoorperate SciSciGPT and SciSciCanvas? — in both interaction design, and underlying HAI4Science workflow?


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-1.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-2.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



% Framework for Integrating SciSciGPT and SciSciCanvas
% A unified HAI4Science workflow could blend both systems:
% Interaction Design
% Language-to-Visualization Bridging: Users pose questions via SciSciGPT (LUI), which generates interactive visual artifacts in SciSciCanvas (GUI).
% Bidirectional Control: Modify a chart (GUI) to auto-update the LLM’s context (e.g., "Focus on papers from 2020–2025"), enabling mixed-initiative exploration.

% Underlying Workflow
% Multi-Agent Collaboration: SciSciGPT parses intent and delegates tasks (e.g., trend analysis) to domain-specific AI agents, while SciSciCanvas renders results as manipulable visualizations.
% Iterative Refinement: Users toggle between refining hypotheses (LUI) and adjusting visual parameters (GUI), creating a closed-loop discovery process.







% 7. Automation
% Definition: Use of computational techniques to conduct repetitive analytical tasks, freeing researchers for higher-level conceptual work.

% Support: Jordan & Mitchell (2015); Kitano (2016).

% - Shift of human roles: transfer from executor to idea generator.
% - Scientific discovery workflow: step by step, AI take over low-level roles.
% - During this shifting, think about transparency, rigous of discovery process

==> sections/archive/03-1-framework/03-1-framework_v4_20251223.tex <==
\subsection{Conceptual Framework}
% \subsection{\newlyadded{Conceptual Framework: LLM-native Figures and Data-Driven Artifacts}}
\label{subsection:conceptual-framework} 
We propose our conceptual framework about LLM-native figures with core components, including the representation of a figure, the bi-directional mapping between visual and analytical operations, the data-driven artifact, and how the backbone of the figure (\ie, the LLM engine) support scientific provenance.


\subsubsection{Overview}
\label{subsubsection:framework-overview}
The proposed framework redefines a scientific figure as a composite computational object that is both human-legible and machine-interpretable. 
We refer to such figures as \textit{LLM-native figures}. 
Each LLM-native figure encapsulates the full analytical provenance underlying its visualization, linking the rendered image, the visualization specification, the generated data insight, the data subset, and the computational process that produced it.

% example scenario: climate
To illustrate the core ideas behind the framework, we use a simple scientific task \newlyadded{in climate science} that involves structured observational data. 
\newlyadded{Understanding regional climate variability, especially seasonal temperature dynamics, is central to research on extreme heat, climate change attribution, and ecological and public-health risk assessment~\cite{jia2024seasonal, bhattarai2025understanding}.} 
Consider a researcher analyzing environmental sensor data collected over multiple years, including monthly temperature, \wyf{humidity, and air-quality [yifang: to add more tables in DB]} measurements collected across U.S. states. 
The researcher begins with the natural-language instruction:
\textit{``Plot the temporal trend of the temperature by month in the state of Florida in the last year (2024).''}
% “Plot the average daily temperature by month for the last five years.”
% generation
The system interprets the analytical intent using the database schema and description, invoking a sequence of data filtering, analysis, and visualization actions and responds with a line plot showing 12 monthly temperatures for Florida (Fig.~\ref{fig:bidirectional-mapping}-A1). 
% \systemname then compiles these components into a Vega-Lite specification for display as an interactive figure (Fig.~\ref{fig:bidirectional-mapping}-A1), while simultaneously rendering and storing a static image of the visualization in the database to support reproducibility, provenance tracking, and future reuse within the data-driven artifact.
% % data insights
\newlyadded{The visualization reveals a gradual warming through spring, consistent with subtropical seasonal cycles, 
followed by nearly four months of sustained summer heat characteristic of persistent U.S. Southeast heatwaves~\cite{raghavendra2019floridian, jia2024seasonal}.
% followed by sustained high temperatures spanning nearly four months, a pattern widely discussed in studies of persistent summer heatwaves in the U.S. Southeast~\cite{raghavendra2019floridian, jia2024seasonal}. 
A sharper cooling onset in early autumn further distinguishes Florida’s seasonal asymmetry.}

% drill-down and generation.
\newlyadded{
Motivated by these patterns, the researcher seeks to contextualize Florida's summer temperatures relative to other states. 
After brushing the time interval from June to August on the line chart, the researcher issues a follow-up instruction:
\textit{``Show me the average temperature of each U.S. state during the selected time range, and rank them from hottest to coolest.''} 
The system combines GUI interactions and natural-language input (Fig.~\ref{fig:bidirectional-mapping}-A2, Sec.~\ref{subsubsection:framework-data-driven-artifact}-\textit{bottom-up}) to trigger a new action sequence. 
It re-queries the database with the updated time range, computes state-level mean temperatures, and sorts the results (Fig.~\ref{fig:bidirectional-mapping}-A3). 
The system then generates a second figure (a bar chart) summarizing summer temperature rankings across states (Fig.~\ref{fig:bidirectional-mapping}-A5), showing that Texas and Florida emerge as the two hottest states, consistent with climatological assessments of regional heat extremes. 
}

% coordination
\newlyadded{
The researcher then examines seasonal shifts in the rankings. 
Brushing the winter months (November–December) on the line chart (Fig.~\ref{fig:bidirectional-mapping}-B1) immediately updates the coordinated bar chart (Fig.~\ref{fig:bidirectional-mapping}-B3).
In winter, the spatial pattern changes differently: Hawaii becomes the warmest region due to its tropical climate, while continental states cluster at much lower temperatures.
% The winter comparison highlights a markedly different spatial pattern \wyf{([yifang]: consider adding a geo map)}: Hawaii becomes the warmest region, reflecting its tropical climate regime, in contrast to the continental states whose temperatures converge at substantially lower values. 
This seasonal contrast illustrates how regional climate heterogeneity emerges across temporal scales, which is an important consideration in climate impact modeling and adaptation planning. 
}

% key feature of LLM-native figure
This simple example illustrates the two key capabilities of the framework:
\textbf{(1) Analytical operations → Visualization}. 
Natural-language instructions are translated into structured analytical steps that filter, aggregate, and visualize data (Fig.~\ref{fig:framework}-\textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3}). 
\textbf{(2) Visualization → Analytical operations}. % → Updated analysis
Interactions on the figure, such as selecting a range, clicking on a mark, or modifying an axis, and together with natural-language instructions, are treated as inputs that trigger corresponding analytical operations for follow-up analysis (Fig.~\ref{fig:framework}-\textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c}). 
In both cases, the system records how each figure is produced: the data subset extracted, the transformations applied, and the visualization generated. 
Together, these components form a machine-interpretable \textbf{LLM-native figure} that can be reused, recomposed, or extended in subsequent steps, and thus transform scientific figures from static outputs into dynamic interfaces for transparent and reproducible computation. 

The remainder of this section generalizes the ideas from this simple example and formalizes the framework's representation (Sec.~\ref{subsubsection:framework-llm-native-figure}), bidirectional mapping (Sec.~\ref{subsubsection:framework-bidirectional-mapping}), and provenance model based on data-driven artifact (Sec.~\ref{subsubsection:framework-data-driven-artifact}).
% The framework consists of three primary components (Fig.~\ref{fig:framework}):
% (1) a \textbf{representation schema} that defines the structure of LLM-native figures (Sec.~\ref{subsection:framework-llm-native-figure});
% (2) a \textbf{bidirectional mapping engine} that connects visual elements to their underlying data and analytic transformations (Sec.~\ref{subsection:framework-bidirectional-mapping}); and
% (3) a \textbf{data-driven artifact} that captures complete provenance across iterative analytical steps (Sec.~\ref{subsection:framework-data-driven-artifact}).
% Together, these components transform figures from static outputs into dynamic interfaces for transparent and reproducible computation. 




\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/extended-chart.jpg}
    \vspace{1pt}
    \caption{ 
    Dynamic generation, coordination, and preservation of LLM-native figures. 
    (A) Drill-down figure generation. 
    % The process of generating a new figure for drill-down. 
    Starting from an existing figure that displays the 12-month temperature trend in Florida (A1), the user brushes a temporal interval and specify a follow-up analytical intent in natural language (A2).
    The framework applies the \textbf{Visualization → Analytical operations} mapping to translate these mixed-modality inputs into precise database queries (A3),  enabling the system to retrieve exactly the subset of data implied by the user's visual and linguistic cues.  
    It then applies the \textbf{Analytical operations → Visualization} mapping to generate a new interactive figure that supports deeper exploration (A5). 
    % First, the framework uses the \textbf{Visualization-to-Analysis} mapping (A1-A3) to transfer the user interactions (\ie, brushing a time period) and natural language intent (A2) to data points (A3). 
    % It then uses the \textbf{Analytics-to-Visualization} mapping to generate the new interactive figure (A5). 
    (B) Real-time coordination between linked figures. 
    When users adjust the focus in one figure (\eg, brushing a different temporal window, B1), the linked figure updates automatically (B3). 
    To enable fast, stable coordination, the system pre-computes and stores the coordination relation and executable code template at the moment the new figure is created (A4), allowing subsequent interactions to directly retrieve and update the relevant code (B2) to query database.
    % Users can brush to filter another time period (B1), and the data in the other figure will be updated automatically (B3). 
    % Specifically, to make the coordination more efficient, during the implementation, we first generate and store the coordination link and code template when first generating the new figure (A4), so that in the following up analysis, the system could directly loop up the coordination link and code and update the code accordingly based on the new filtering criteria (B2). 
    (C) Persistent, revisitable artifacts. 
    The linked figures, together with their underlying code, data, and coordination rules, are all stored in the data-driven artifact that captures the user's exploration trajectory and supports future revisits, refinements, and extensions. 
    }
    \label{fig:bidirectional-mapping}
\end{figure}



\subsubsection{Representation of LLM-Native Figures}
\label{subsubsection:framework-llm-native-figure}
Building on the example above, each figure (Fig.~\ref{fig:framework}-A) produced by the system at timestamp $t$ is represented as a structured format:
% Each LLM-native figure at timestamp $t$ is represented as a tuple: 

\begin{equation}
F_t = \{V_t, C_t, D_t, M_t\}
% F_t = \{I, V, C, D, M\}
\end{equation}

where 
% $I$ represents user's intent and inputs including natural-language instructions and graphical interactions on the visualization such as selection and brushing (Fig.~\ref{fig:bidirectional-mapping}-A2, Fig.~\ref{fig:framework}-User Input). 
$V_t$ denotes the rendered visualization (Fig.~\ref{fig:framework}-A1), represented by multiple modalities: (1) the rendered raster image (\eg, PNG), (2) a textual summary of key insights, and (3) the declarative visualization specification (\eg, Vega-Lite JSON schema~\cite{satyanarayan2016vega}) that encodes visual mappings that transform data attributes into visual channels (\eg, position, size, and color) and supports interactive behaviors.
Each visual mark in the visualization ($V_t$) (\eg, a point, bar, or line segment) has a unique identifier that maps to corresponding rows or groups in the dataset ($D_t$, Fig.~\ref{fig:framework}-A3). 
Together, these modalities make the figure not only human-readable but computationally navigable.
% where $V$ denotes the rendered visualization (\eg, an SVG or raster image), 
% $S$ is the declarative visualization specification, such as a Vega-Lite schema~\cite{satyanarayan2016vega}, that encodes visual mappings between \wyf{data attributes and visual channels (\eg, width, size, and color)}, 
$C_t$ records the analytical actions (Sec.~\ref{subsection:method-action-space}) and corresponding executable code (\eg, SQL and Python) that generated $D_t$ and $V_t$ (Fig.~\ref{fig:framework}-A2).
$D_t$ represents the underlying data used in the visualization, such as data subsets and associated data schema, and aggregated results used for rendering (Fig.~\ref{fig:framework}-A3),
% metadata on source, schema, and selection filters, 
and $M_t$ represents the metadata associated with this figure within the user's exploration history, such as the timestamp $t$, version identifier, type and description of user operations, and links to corresponding data-driven artifacts (Fig.~\ref{fig:framework}-A4).

This structured representation ensures that every visual element in $V_t$ is traceable to the corresponding computational steps in $C_t$ and data entries in $D_t$. 
Conversely, any modification to $D_t$ or $C_t$ automatically updates $V_t$ and records the change in $M_t$. 
The tuple thus forms a closed and reproducible description of the analytical state at the moment the figure is produced.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/framework.jpg}
    \vspace{1pt}
    \caption{The conceptual framework for iterative exploration for data-driven scientific discovery.
    % 
    \textbf{Left}: Five-layer structure of the framework, including user inputs, AI outputs (LLM-native figures and data-driven artifacts) and the underlying LLM engine and databases. 
    % 
    \textbf{Top-Right}: structure of an LLM-native figure at timestamp $t$, which supports bidirectional mapping between visual ($V$) and analytical ($C$ and $D$) representations, along with associated metadata $M$. 
    % 
    \textbf{Bottom-Right}: Definition of a data-driven artifact. 
    Starting from a focal figure, analyses can be iteratively refined or extended, supporting non-linear human exploration logic. Two example interaction modes are illustrated:
    (1) \textit{Manipulating} existing figures to refine or reorient the analysis focus, and
    (2) \textit{Drilling down} from user-interested data points within the focal figure to generate new, coordinated figures that enable progressive, in-depth exploration through filtering and brushing. 
    \wyf{[Yifang TODO]: update data table in A3: match climate case; move icon B1 and B2 to left-buttom.}
    }
    \label{fig:framework}
\end{figure}



\subsubsection{Bidirectional Mapping Between Visualization and Analysis}
\label{subsubsection:framework-bidirectional-mapping}
\newlyadded{
To support reliable round-trips between visual and analytical representations of a figure, our framework maintains a formal bidirectional mapping $R_t$ at time $t$ that links visual marks and GUI interactions in $V_t$ to the underlying analytical operations $C_t$ and data rows $D_t$ that produced them:
\begin{equation}
R_t = \{\,(\mathrm{visual\_mark}, \ \mathrm{data\_rows},\ \mathrm{analytical\_operation})\,\}
\end{equation}
This mapping forms the basis of two complementary transformations: 
% The mapping enables two classes of operations:
}

\begin{itemize}
    \item \textbf{Analytical operations → Visualization.} 
    % \item \textbf{Language-to-Analytical-to-Visualization.} 
    The user instruction (\eg, \textit{``Plot the temporal trend of the temperature by month in the state of Florida in the last year (2024)''}) is parsed by the LLM into a sequence of analytical actions ($\mathrm{analytical\_operation}$, Sec.~\ref{subsection:method-action-space}), including selecting relevant tables and columns (\eg, the \textit{temperature}, \textit{year}, and \textit{state} fields), filter rows (\eg, by \textit{state} and \textit{year} fields), and assigning the chart type, visual encoding, chart interactions, and textual insights.
    These actions will generate code $C$ and compute data $D$ ($\mathrm{data\_rows}$), resulting in a new or updated visualization $V$ with a set of visual marks ($\mathrm{visual\_mark}$) to render the figure (Fig.~\ref{fig:bidirectional-mapping}-A1, Fig.~\ref{fig:framework}-path: \textsquarenumber{1} → \textsquarenumber{2} → \textsquarenumber{3}).
    % User natural-language instructions are parsed by the LLM into structured analytical actions, such as data filtering, transformation, modeling, and visualization, that modify $C$ or $D$, resulting in an updated $V$ \wyf{(Fig.~\ref{fig:framework}, path: \textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3})}. 
    
    \item \textbf{Visualization → Analytical operations.} 
    When the user brushes the figure with the time range June-August in the generated temporal line chart $V_t$ and ask a follow-up question about the summer period (Fig.~\ref{fig:bidirectional-mapping}-A2), 
    % to compare the average temperature of each state in the selected summer period, 
    via $R_t$, the system identifies the corresponding visual brushed area, retrieves the relevant data in $D$ (\ie, filtering the data to those months to obtain $\mathrm{data\_rows}$), and combines the filtered subset of data with the user instruction to construct a new sequence of analytical actions ($\mathrm{analytical\_operation}$) before generating a second figure (Fig.~\ref{fig:bidirectional-mapping}-A3 and A4, Fig.~\ref{fig:framework}-path: \textsquarecharacter{a} → \textsquarecharacter{b} → \textsquarecharacter{c}).
    % User interactions on $V$ (\eg, clicking a data point, selecting a region, or modifying an axis) together with natural-language instructions are are interpreted by the LLM and translated into structured analytical commands that reference the affected data subset $D$ and trigger corresponding updates to the analytical pipeline ($C$ and $D$) to refine existing insights or enable deeper insight exploration~\wyf{(Fig.~\ref{fig:framework}, path: \textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c})}.
\end{itemize} 

This mapping enables consistent, verifiable transitions between visual and analytical states, allowing figures to serve as reliable interactive interfaces for scientific reasoning.
This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


% Formally, the framework maintains a mapping relationship:
% \begin{equation}
% % R_t = \{\,(\mathrm{visual\_mark},\ \mathrm{data\_rows},\ \mathrm{code})\,\}
% R_t = \{\,(\mathrm{visual\_mark}, \ \mathrm{data\_rows},\ \mathrm{analytical\_operation})\,\}
% % 花括号 { } 表示集合（set），圆括号 ( ) 表示元组（tuple）
% \end{equation}
% associating each visual element and GUI interaction with the data and computation codes that produced it. 
% \newlyadded{In the climate example, brushing June–August corresponds to a set of $\mathrm{visual\_mark}$ in $V_t$; 
% via $R_t$, this selection is first accurately mapped to the filtering range (by the Vega-Lite specification), then to a set of $\mathrm{analytical\_operation}$ and code $C_t$ that can link to specific $\mathrm{data\_rows}$ in $D_t$ (by LLM).}
% This mapping enables consistent, verifiable round-trips between visual states and analytical states, allowing figures to serve as reliable interactive interfaces for scientific reasoning.
% % Formally, these mappings are implemented through \wyf{a semantic layer} that maintains correspondences between visual representation in $V$ and their provenance within $C$ and $D$. 
% % This layer allows the LLM to generate 
% % reason over the structure of the visualization, identify which analytical operations produced each visual element, and generate consistent updates. 
% % The bidirectional mapping extends beyond static translation: it supports compositional reasoning, where a sequence of natural-language and graphical interactions are merged into a coherent analytical plan. 
% This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


\subsubsection{Artifact and Provenance}
\label{subsubsection:framework-data-driven-artifact}
Every analytical step, whether triggered by language or by visual interaction, passes through a single execution pipeline. The framework understands the user intent ($I_t$), generates and executes code ($C_t$) in a controlled environment, updates the data subset ($D_t$), and generates a new visualization ($V_{t+1}$).
All figures together with their analysis codes, underlying data, and coordination rules are recorded in a \textbf{data-driven artifact} (Fig.~\ref{fig:bidirectional-mapping}-C, Fig.~\ref{fig:framework}-B), a reusable, composable unit of exploration comprising one or more coordinated figures that encode the human's iterative analytical logic.
\newlyadded{Where a figure captures a single analytical question, an artifact captures the trajectory of states across one or multiple figures and the coordination relationships that link them.}
% a version-controlled ledger that records one or more figures and their exploration history, capturing both intra-figure revisions and inter-figure coordination that links a figure to its derived successors.
% a version-controlled ledger that tracks the evolution of each figure and its underlying analyses, as well as its coordinated other figures. 
Each artifact records not only the resulting figures but also the sequence of thought: \textit{manipulation}---iterates an existing figure within a fixed artifact node to refine or reorient the analysis focus by updating $C_t$, $V_t$, and $D_t$ (optionally), and \textit{drill-down} or \textit{bottom-up}---generates new, coordinated figures from user-selected data points, thereby extending the artifact and analysis logic. 
Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, revisited, and shared across similar analysis tasks. 

% 维度1: artiface和figure的关系
Each artifact $A$ at timestamp $t$ consists of: 
\begin{itemize}
    \item \textbf{User input ($I_t$)}: the users' natural-language instruction or graphical interaction and its parsed structured representation (Fig.~\ref{fig:framework}-\textit{User Input}); 
    \item \textbf{Derived figures ($F_t$)}: one or more figures (Sec.~\ref{subsubsection:framework-llm-native-figure}) generated during the exploration of a research problem. Each figure includes the analytical execution result (code $C_t$ and data $D_t$), the resulting visualization $V_t$, and associated meta information $M_t$ (Fig.~\ref{fig:framework}-A). 
    % \item \textbf{Analytical execution result ($C_t$, $D_t$)}: 
    % the analytical operation invoked by the user input, including the updated analytical code $C_t$ and corresponding data $D_t$ that define the computation underpinning the figure (Fig.~\ref{fig:framework}-A2, A3);
    % \item \textbf{Derived visualization ($V_t$, $M_t$)}: the derived or updated visualization $V_t$ and its associated metadata $M_t$ (Fig.~\ref{fig:framework}-A1, A4); 
    \item \textbf{Coordination linkage and schema}: the updated coordination graph and code that records how the figures within the same artifact are connected to one another by different brushing and filtering schema (Fig.~\ref{fig:bidirectional-mapping}-A4, B2). 
    \newlyadded{Once the user filters another data region of interest, the data and visualization on the linked figures will be automatically updated to show the selected set of data (Fig.~\ref{fig:bidirectional-mapping}-B1-B3).} 
    % \item \textbf{Execution result}: the updated analytical code $C_t$, \wyf{data subset $D_t$}, and visualization specification $S_t$;
    % \item \textbf{Derived artifact}: the resulting figure $F_t$ and metadata $M_t$;
    % \item \textbf{Parent linkage}: references to preceding artifacts to maintain the complete analytical lineage.
\end{itemize}

% 维度2: artiface自身的版本控制
Additionally, an artifact $A$ is maintained as a version-controlled ledger ($A_{t_1}$, $A_{t_2}$, ... $A_{t_n}$), which forms a directed acyclic graph of artifact versions, where each node represents a reproducible state and each edge an analytical transformation. 
The graph allows any prior state to be reconstructed or branched, ensuring traceability and supporting collaborative editing among multiple users or AI agents.

The design of data-driven artifact serves two key functions. 
First, it enforces \textit{reproducibility}: every output is linked to an executable record of how it was produced. 
Second, it enables reasoning \textit{transparency}: by exposing the intermediate steps of analysis \wyf{(such as action-level reasoning -- to write at Method seciton)}, both humans and models can audit and explain results at any level of detail. 

% \wyf{[yifang: To revise the last paragraph above: reconsider whether \textit{user_input} should be included in the artifact or the dashboard. It feels somewhat inappropriate from an implementation perspective, though it fits better conceptually within the framework description.]}


\subsubsection{Integration with Large Language Models}
\label{subsubsection:framework-llm}
Large language models interact with the framework through an plan-action–observation loop (Sec.~\ref{section:methods}). 
The model receives user instructions and interactions, along with contextual information from the artifact and conversational history, to generate candidate analytical actions, reasoning over complex data, and validates them through code execution.
Execution outputs, including visualization and textual insights, generated data, and potential errors, are then fed back to the model to inform the next step of action selection. 

To constrain the model's behavior and ensure reliability, LLMs chooses actions from a constrained \textit{action space} (Sec.~\ref{subsection:method-action-space}) that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
% To constrain the model's behavior and ensure reliability, the system employs an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
The LLM operates within this space, translating natural-language input into valid action sequences that are interpretable, executable, and reversible through provenance records.
Domain-specific customizations (\eg, tailored AI agents and tool designs~\cite{gao2025democratizing}) could be integrated into this framework to enhance these capabilities to specialized domain contexts.

This integration turns the LLM into an orchestrator of analytical operations rather than a black-box generator, aligning model reasoning with the explicit structure of the computational pipeline.


\subsubsection{Summary}
\label{subsubsection:framework-summary}
The framework establishes a general method for constructing and reasoning with machine-interpretable scientific artifacts. 
By embedding analytical provenance within each figure, maintaining bidirectional mappings between visualization and data, and recording every analytical step in an artifact store, the approach enables transparent, reproducible, and mixed-initiative data exploration. 
\wyf{These properties form the foundation for evaluating the system's performance and generality in the next section.}








% % %%%%%%%%%%%%%%%%% prev introduction part %%%%%%%%%%%%%%%%%
% % our method
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }







% \wyf{(generalizability levels: 
%         [level 1]: SciSciCanvas (use SciSci as an example domain); 
%         [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
%         [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
%         [level 4]: HAI for all scenarios (general public + expert-oriented systems)
%     )}


% 宋阳秋老师2025.05刚发的一个survey: https://github.com/HKUST-KnowComp/Awesome-LLM-Scientific-Discovery 


% Tiantian:
% 4. In different scenarios, how AI and human can collaborate — can we think of a framework that can incoorperate SciSciGPT and SciSciCanvas? — in both interaction design, and underlying HAI4Science workflow?


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-1.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-2.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



% Framework for Integrating SciSciGPT and SciSciCanvas
% A unified HAI4Science workflow could blend both systems:
% Interaction Design
% Language-to-Visualization Bridging: Users pose questions via SciSciGPT (LUI), which generates interactive visual artifacts in SciSciCanvas (GUI).
% Bidirectional Control: Modify a chart (GUI) to auto-update the LLM’s context (e.g., "Focus on papers from 2020–2025"), enabling mixed-initiative exploration.

% Underlying Workflow
% Multi-Agent Collaboration: SciSciGPT parses intent and delegates tasks (e.g., trend analysis) to domain-specific AI agents, while SciSciCanvas renders results as manipulable visualizations.
% Iterative Refinement: Users toggle between refining hypotheses (LUI) and adjusting visual parameters (GUI), creating a closed-loop discovery process.







% 7. Automation
% Definition: Use of computational techniques to conduct repetitive analytical tasks, freeing researchers for higher-level conceptual work.

% Support: Jordan & Mitchell (2015); Kitano (2016).

% - Shift of human roles: transfer from executor to idea generator.
% - Scientific discovery workflow: step by step, AI take over low-level roles.
% - During this shifting, think about transparency, rigous of discovery process

==> sections/archive/03-1-framework/03-1-framework_v5_20260206.tex <==
\subsection{Conceptual Framework}
\label{subsection:conceptual-framework} 
We propose our conceptual framework about LLM-native figures with core components, including the representation of a figure, the bi-directional mapping between visual and analytical operations, the data-driven artifact, and how the backbone of the figure (\ie, the LLM engine) support scientific provenance.

\textbf{Overview.}
The proposed framework redefines a scientific figure as a composite computational object that is both human-legible and machine-interpretable. 
We refer to such figures as \textit{LLM-native figures}. 
Each LLM-native figure encapsulates the full analytical provenance underlying its visualization, linking the rendered image, the visualization specification, the generated data insight, the data subset, and the computational process that produced it.
To make the framework concrete, let us begin with a simple, hypothetical example. 
Imagine a climate researcher studying historical monthly temperature records across U.S. states. 
She issues a natural-language query such as:
\textit{``Plot the average monthly temperature in Florida over the past ten years (2014 to 2024).''}
% 1. generate ego chart
The system responds with a line chart in which the horizontal axis denotes calendar months and vertical axis represents the average temperature of each month in Florida (Fig.~\ref{fig:bidirectional-mapping}a). 
At this point, the figure looks entirely familiar, resembling a standard plot that scientists from many disciplines might produce for their analyses. 
% 2. generate extended chart
The interaction becomes more interesting when the researcher begins to use the figure itself as an interface. 
She then asks how Florida's summer compares with other states, brushing over the summer months on the Florida chart and requests: 
\textit{``Show me the average temperature of each U.S. state in the past 10 years (2014-2024), and rank them from hottest to coolest.''}
The system interprets this selection interaction as a request (Fig.~\ref{fig:bidirectional-mapping}b, Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (\textit{bottom-up})) to focus on the subset of rows corresponding to June–August, aggregates those data across all states (Fig.~\ref{fig:bidirectional-mapping}c), and generates a new bar chart ranking states by their average summer temperature (Fig.~\ref{fig:bidirectional-mapping}e). 
% 3. cross-chart coordination
If she repeats the same gesture over winter months (Fig.~\ref{fig:bidirectional-mapping}f), the bar chart updates to show a different ordering (Fig.~\ref{fig:bidirectional-mapping}h), making it straightforward to contrast seasonal patterns without writing new queries or code. 
Because both charts are linked through a shared underlying representation, subsequent operations, such as filtering to coastal states, splitting by decade, or changing to a different aggregation, can be issued either in language or via further interactions on the figures.
% summary
This illustrative scenario captures the two key capabilities we seek: natural-language instructions that drive analytical operations and generate visualizations, and visual interactions that are mapped back to the underlying data and analytical pipeline. 
In the next subsection, we formalize how LLM-native figures represent these states and how the framework maintains the bidirectional mapping between visualization and analysis.
% drill-down and generation.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/extended-chart.jpg}
    \vspace{1pt}
    \caption{ 
    \bodyfigurelabel{fig:Figure1}
    Dynamic generation, coordination, and preservation of LLM-native figures. 
    Example for drilling down figure generation: 
    % The process of generating a new figure for drill-down. 
    starting from an existing figure that displays the 12-month temperature trend in Florida (\textbf{a}), the user brushes a temporal interval and specify a follow-up analytical intent in natural language (\textbf{b}).
    The framework applies the \textbf{Visualization → Analytical operations} mapping to translate these mixed-modality inputs into precise database queries (\textbf{c}),  enabling the system to retrieve exactly the subset of data implied by the user's visual and linguistic cues.  
    It then applies the \textbf{Analytical operations → Visualization} mapping to generate a new interactive figure that supports deeper exploration (\textbf{e}). 
    % First, the framework uses the \textbf{Visualization-to-Analysis} mapping (A1-A3) to transfer the user interactions (\ie, brushing a time period) and natural language intent (A2) to data points (A3). 
    % It then uses the \textbf{Analytics-to-Visualization} mapping to generate the new interactive figure (A5). 
    Example for real-time coordination between linked figures: 
    when users adjust the focus in one figure (\eg, brushing a different temporal window, \textbf{f}), the linked figure updates automatically (\textbf{h}). 
    To enable fast, stable coordination, the system pre-computes and stores the coordination relation and executable code template at the moment the new figure is created (\textbf{d}), allowing subsequent interactions to directly retrieve and update the relevant code (\textbf{g}) to query database.
    % Users can brush to filter another time period (B1), and the data in the other figure will be updated automatically (B3). 
    % Specifically, to make the coordination more efficient, during the implementation, we first generate and store the coordination link and code template when first generating the new figure (A4), so that in the following up analysis, the system could directly loop up the coordination link and code and update the code accordingly based on the new filtering criteria (B2). 
    \textbf{i}, Persistent, revisitable artifacts. 
    The linked figures, together with their underlying code, data, and coordination rules, are all stored in the data-driven artifact that captures the user's exploration trajectory and supports future revisits, refinements, and extensions. 
    }
    \label{fig:bidirectional-mapping}
\end{figure}


\textbf{Representation of LLM-Native Figures.}
Building on the example above, each figure (Fig.~\ref{fig:framework}f) produced by the system at timestamp $t$ is represented as a structured format:
% Each LLM-native figure at timestamp $t$ is represented as a tuple: 

\begin{equation}
F_t = \{V_t, C_t, D_t, M_t\}
% F_t = \{I, V, C, D, M\}
\end{equation}

where 
% $I$ represents user's intent and inputs including natural-language instructions and graphical interactions on the visualization such as selection and brushing (Fig.~\ref{fig:bidirectional-mapping}b, Fig.~\ref{fig:framework}-User Input). 
$V_t$ denotes the rendered visualization (Fig.~\ref{fig:framework}f-V), represented by multiple modalities: (1) the rendered raster image (\eg, PNG), (2) a textual summary of key insights, and (3) the declarative visualization specification (\eg, Vega-Lite JSON schema~\cite{satyanarayan2016vega}) that encodes visual mappings that transform data attributes into visual channels (\eg, position, size, and color) and supports interactive behaviors.
Each visual mark in the visualization ($V_t$) (\eg, a point, bar, or line segment) has a unique identifier that maps to corresponding rows or groups in the dataset ($D_t$, Fig.~\ref{fig:framework}f-D). 
Together, these modalities make the figure not only human-readable but computationally navigable.
% where $V$ denotes the rendered visualization (\eg, an SVG or raster image), 
% $S$ is the declarative visualization specification, such as a Vega-Lite schema~\cite{satyanarayan2016vega}, that encodes visual mappings between \wyf{data attributes and visual channels (\eg, width, size, and color)}, 
$C_t$ records the analytical actions (Sec.~\ref{subsection:method-llm}) and corresponding executable code (\eg, SQL and Python) that generated $D_t$ and $V_t$ (Fig.~\ref{fig:framework}f-C).
$D_t$ represents the underlying data used in the visualization, such as data subsets and associated data schema, and aggregated results used for rendering (Fig.~\ref{fig:framework}f-D),
% metadata on source, schema, and selection filters, 
and $M_t$ represents the metadata associated with this figure within the user's exploration history, such as the timestamp $t$, version identifier, type and description of user operations, and links to corresponding data-driven artifacts (Fig.~\ref{fig:framework}f-M).
% summary
This structured representation ensures that every visual element in $V_t$ is traceable to the corresponding computational steps in $C_t$ and data entries in $D_t$. 
Conversely, any modification to $D_t$ or $C_t$ automatically updates $V_t$ and records the change in $M_t$. 
The tuple thus forms a closed and reproducible description of the analytical state at the moment the figure is produced.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/framework.jpg}
    \vspace{1pt}
    \caption{
    \bodyfigurelabel{fig:Figure2}
    The conceptual framework for iterative exploration for data-driven scientific discovery.
    % 
    \textbf{a}-\textbf{e}, Five-layer structure of the framework, including user inputs, AI outputs (LLM-native figures and data-driven artifacts) and the underlying LLM engine and databases. 
    % 
    \textbf{f}, Structure of an LLM-native figure at timestamp $t$, which supports bidirectional mapping between visual ($V$) and analytical ($C$ and $D$) representations, along with associated metadata $M$. 
    % 
    \textbf{g}, Definition of a data-driven artifact. 
    Starting from a focal figure, analyses can be iteratively refined or extended, supporting non-linear human exploration logic. Two example interaction modes are illustrated:
    (1) \textit{Manipulating} existing figures to refine or reorient the analysis focus, and
    (2) \textit{Drilling down} from user-interested data points within the focal figure to generate new, coordinated figures that enable progressive, in-depth exploration through filtering and brushing. 
    \wyf{[Yifang TODO]: update data table in A3: match climate case; move icon B1 and B2 to left-buttom.}
    }
    \label{fig:framework}
\end{figure}


\textbf{Bidirectional Mapping.}
To support reliable round-trips between visual and analytical representations of a figure, our framework maintains a formal bidirectional mapping $R_t$ at time $t$ that links visual marks and GUI interactions in $V_t$ to the underlying analytical operations $C_t$ and data rows $D_t$ that produced them:
\begin{equation}
R_t = \{\,(\mathrm{visual\_mark}, \ \mathrm{data\_rows},\ \mathrm{analytical\_operation})\,\}
\end{equation}
This mapping forms the basis of two complementary transformations: 

\begin{itemize}
    \item \textbf{Analytical operations → Visualization.} 
    % \item \textbf{Language-to-Analytical-to-Visualization.} 
    The user instruction (\eg, \textit{``Plot the average monthly temperature in Florida over the past ten years (2014 to 2024)''}) is parsed by the LLM into a sequence of analytical actions ($\mathrm{analytical\_operation}$, Sec.~\ref{subsection:method-llm}), including selecting relevant tables and columns (\eg, the \textit{temperature}, \textit{year}, and \textit{state} fields), filter rows (\eg, by \textit{state} and \textit{year} fields), and assigning the chart type, visual encoding, chart interactions, and textual insights.
    These actions will generate code $C$ and compute data $D$ ($\mathrm{data\_rows}$), resulting in a new or updated visualization $V$ with a set of visual marks ($\mathrm{visual\_mark}$) to render the figure (Fig.~\ref{fig:bidirectional-mapping}a, Fig.~\ref{fig:framework}-path: \textsquarenumber{1} → \textsquarenumber{2} → \textsquarenumber{3}).
    % User natural-language instructions are parsed by the LLM into structured analytical actions, such as data filtering, transformation, modeling, and visualization, that modify $C$ or $D$, resulting in an updated $V$ \wyf{(Fig.~\ref{fig:framework}, path: \textsquarenumber{1} to \textsquarenumber{2} to \textsquarenumber{3})}. 
    
    \item \textbf{Visualization → Analytical operations.} 
    When the user brushes the figure with the time range June-August in the generated temporal line chart $V_t$ and ask a follow-up question about the summer period (Fig.~\ref{fig:bidirectional-mapping}b), 
    % to compare the average temperature of each state in the selected summer period, 
    via $R_t$, the system identifies the corresponding visual brushed area, retrieves the relevant data in $D$ (\ie, filtering the data to those months to obtain $\mathrm{data\_rows}$), and combines the filtered subset of data with the user instruction to construct a new sequence of analytical actions ($\mathrm{analytical\_operation}$) before generating a second figure (Fig.~\ref{fig:bidirectional-mapping}c and A4, Fig.~\ref{fig:framework}-path: \textsquarecharacter{a} → \textsquarecharacter{b} → \textsquarecharacter{c}).
    % User interactions on $V$ (\eg, clicking a data point, selecting a region, or modifying an axis) together with natural-language instructions are are interpreted by the LLM and translated into structured analytical commands that reference the affected data subset $D$ and trigger corresponding updates to the analytical pipeline ($C$ and $D$) to refine existing insights or enable deeper insight exploration~\wyf{(Fig.~\ref{fig:framework}, path: \textsquarecharacter{a} to \textsquarecharacter{b} to \textsquarecharacter{c})}.
\end{itemize} 

This mapping enables consistent, verifiable transitions between visual and analytical states, allowing figures to serve as reliable interactive interfaces for scientific reasoning.
This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


% Formally, the framework maintains a mapping relationship:
% \begin{equation}
% % R_t = \{\,(\mathrm{visual\_mark},\ \mathrm{data\_rows},\ \mathrm{code})\,\}
% R_t = \{\,(\mathrm{visual\_mark}, \ \mathrm{data\_rows},\ \mathrm{analytical\_operation})\,\}
% % 花括号 { } 表示集合（set），圆括号 ( ) 表示元组（tuple）
% \end{equation}
% associating each visual element and GUI interaction with the data and computation codes that produced it. 
% \newlyadded{In the climate example, brushing June–August corresponds to a set of $\mathrm{visual\_mark}$ in $V_t$; 
% via $R_t$, this selection is first accurately mapped to the filtering range (by the Vega-Lite specification), then to a set of $\mathrm{analytical\_operation}$ and code $C_t$ that can link to specific $\mathrm{data\_rows}$ in $D_t$ (by LLM).}
% This mapping enables consistent, verifiable round-trips between visual states and analytical states, allowing figures to serve as reliable interactive interfaces for scientific reasoning.
% % Formally, these mappings are implemented through \wyf{a semantic layer} that maintains correspondences between visual representation in $V$ and their provenance within $C$ and $D$. 
% % This layer allows the LLM to generate 
% % reason over the structure of the visualization, identify which analytical operations produced each visual element, and generate consistent updates. 
% % The bidirectional mapping extends beyond static translation: it supports compositional reasoning, where a sequence of natural-language and graphical interactions are merged into a coherent analytical plan. 
% This capability enables mixed-initiative workflows in which humans and LLMs alternate between specifying intentions in language and refining results through direct manipulation.


% \subsubsection{Artifact and Provenance}
% \label{subsubsection:framework-data-driven-artifact}
\textbf{Artifact and Provenance.}
Every analytical step, whether triggered by language or by visual interaction, passes through a single execution pipeline. The framework understands the user intent ($I_t$), generates and executes code ($C_t$) in a controlled environment, updates the data subset ($D_t$), and generates a new visualization ($V_{t+1}$).
All figures together with their analysis codes, underlying data, and coordination rules are recorded in a \textbf{data-driven artifact} (Fig.~\ref{fig:bidirectional-mapping}i, Fig.~\ref{fig:framework}g), a reusable, composable unit of exploration comprising one or more coordinated figures that encode the human's iterative analytical logic.
Where a figure captures a single analytical question, an artifact captures the trajectory of states across one or multiple figures and the coordination relationships that link them.
% a version-controlled ledger that records one or more figures and their exploration history, capturing both intra-figure revisions and inter-figure coordination that links a figure to its derived successors.
% a version-controlled ledger that tracks the evolution of each figure and its underlying analyses, as well as its coordinated other figures. 
Each artifact records not only the resulting figures but also the sequence of thought: \textit{manipulation}---iterates an existing figure within a fixed artifact node to refine or reorient the analysis focus by updating $C_t$, $V_t$, and $D_t$ (optionally), and \textit{drill-down} or \textit{bottom-up}---generates new, coordinated figures from user-selected data points, thereby extending the artifact and analysis logic. 
Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, revisited, and shared across similar analysis tasks. 
% 
% 维度1: artiface和figure的关系
Each artifact $A_t$ at timestamp $t$ consists of: 
\begin{itemize}
    \item \textbf{User input ($I_t$)}: the users' natural-language instruction or graphical interaction and its parsed structured representation (Fig.~\ref{fig:framework}-\textit{User Input}); 
    \item \textbf{Derived figures ($F_t$)}: one or more figures generated during the exploration of a research problem. Each figure includes the analytical execution result (code $C_t$ and data $D_t$), the resulting visualization $V_t$, and associated meta information $M_t$ (Fig.~\ref{fig:framework}f). 
    % \item \textbf{Analytical execution result ($C_t$, $D_t$)}: 
    % the analytical operation invoked by the user input, including the updated analytical code $C_t$ and corresponding data $D_t$ that define the computation underpinning the figure (Fig.~\ref{fig:framework}-A2, A3);
    % \item \textbf{Derived visualization ($V_t$, $M_t$)}: the derived or updated visualization $V_t$ and its associated metadata $M_t$ (Fig.~\ref{fig:framework}-A1, A4); 
    \item \textbf{Coordination linkage and schema}: the updated coordination graph and code that records how the figures within the same artifact are connected to one another by different brushing and filtering schema (Fig.~\ref{fig:bidirectional-mapping}d, B2). 
    Once the user filters another data region of interest, the data and visualization on the linked figures will be automatically updated to show the selected set of data (Fig.~\ref{fig:bidirectional-mapping}f-B3). 
    % \item \textbf{Execution result}: the updated analytical code $C_t$, \wyf{data subset $D_t$}, and visualization specification $S_t$;
    % \item \textbf{Derived artifact}: the resulting figure $F_t$ and metadata $M_t$;
    % \item \textbf{Parent linkage}: references to preceding artifacts to maintain the complete analytical lineage.
\end{itemize}

% 维度2: artiface自身的版本控制
Additionally, an artifact $A$ is maintained as a version-controlled ledger ($A_{t_1}$, $A_{t_2}$, ... $A_{t_n}$), which forms a directed acyclic graph of artifact versions, where each node represents a reproducible state and each edge an analytical transformation. 
The graph allows any prior state to be reconstructed or branched, ensuring traceability and supporting collaborative editing among multiple users or AI agents.
% summary
The design of data-driven artifact serves two key functions. 
First, it enforces \textit{reproducibility}: every output is linked to an executable record of how it was produced. 
Second, it enables reasoning \textit{transparency}: by exposing the intermediate steps of analysis(such as action-level reasoning and results), both humans and models can audit and explain results at any level of detail. 

% \wyf{[yifang: To revise the last paragraph above: reconsider whether \textit{user_input} should be included in the artifact or the dashboard. It feels somewhat inappropriate from an implementation perspective, though it fits better conceptually within the framework description.]}


% \subsubsection{Integration with Large Language Models}
% \label{subsubsection:framework-llm}
\textbf{Integration with Large Language Models.} 
Large language models interact with the framework through an plan-action–observation loop (Sec.~\ref{section:methods}). 
The model receives user instructions and interactions, along with contextual information from the artifact and conversational history, to generate candidate analytical actions, reasoning over complex data, and validates them through code execution.
Execution outputs, including visualization and textual insights, generated data, and potential errors, are then fed back to the model to inform the next step of action selection. 
% 
To constrain the model's behavior and ensure reliability, LLMs chooses actions from a constrained \textit{action space} (Sec.~\ref{subsection:method-llm}) that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
% To constrain the model's behavior and ensure reliability, the system employs an \textbf{action space} that defines permissible operations (\eg, filtering, transformation, modeling, and visualization). 
The LLM operates within this space, translating natural-language input into valid action sequences that are interpretable, executable, and reversible through provenance records.
Domain-specific customizations (\eg, tailored AI agents and tool designs~\cite{gao2025democratizing}) could be integrated into this framework to enhance these capabilities to specialized domain contexts.
% 
This integration turns the LLM into an orchestrator of analytical operations rather than a black-box generator, aligning model reasoning with the explicit structure of the computational pipeline.


% \subsubsection{Summary}
% \label{subsubsection:framework-summary}
% \vspace{8pt}
The framework establishes a general method for constructing and reasoning with machine-interpretable scientific artifacts. 
By embedding analytical provenance within each figure, maintaining bidirectional mappings between visualization and data, and recording every analytical step in an artifact store, the approach enables transparent, reproducible, and mixed-initiative data exploration. 
These properties form the foundation for evaluating the system's performance and generality in the next section.








% % %%%%%%%%%%%%%%%%% prev introduction part %%%%%%%%%%%%%%%%%
% % our method
% This paradigm combines the flexible, expressive, and real-time reasoning capabilities of conversational AI with the intuitive and powerful visual affordances and precise manipulation capabilities of interactive data visualization. 
% Users can fluidly articulate their questions and hypotheses in natural language, while AI agents dynamically interpret these requests, plan and execute relevant analyses, and deliver results not merely as text, but as \textbf{\textit{data-driven ``artifacts''}} -- a series of interactive visualizations that can be further manipulated, extended, iterated upon, and reused. 

% \wyf{Critically, each visualization generated by the AI is not only perceived by humans as a static image~\cite {shao2025sciscigpt}, 
% but also serves as a computationally traceable compression of all underlying data points perceived by GenAI. 
% This dual representation transforms data insights into both a perceptual object for humans and a reasoning substrate for machines. 
% Humans are good at pattern recognition and intuitive understanding through visual images; 
% GenAI, conversely, excels at understanding, tracing, reconstructing, and reasoning over the complete data context behind those images. 
% By uniting these complementary modes of perception, the model allows humans and AI to ``see through'' the visual abstraction of data insights by linking user-selected data regions of interest back to their source data for deeper analysis and iterative reasoning. 
% This capability redefines figures from passive outputs into active interfaces for discovery, establishing a conceptual foundation for the next generation of AI-assisted data analysis systems in which every visualization becomes simultaneously a window for human insight and a medium for machine intelligence.
% }

% Through this iterative interaction loop, new exploratory questions and analytical directions naturally emerge, leading to the generation of new insights delivered through both textual explanations and visual exploration tools. 
% Ultimately, this paradigm empowers users not only to receive insights intuitively but also to actively guide and control the analysis process by combining the creativity and context sensitivity of language with the clarity and efficiency of visual exploration. 

% To demonstrate the broad applicability of this paradigm, we present \systemname, a proof-of-concept system developed for the Science of Science (SciSci) domain--an essential field for understanding and accelerating scientific enterprise and technological innovation. 
% SciSci provides a representative testbed with challenges well matched to our paradigm: rich and emerging datasets spanning grants, research papers, patents, policies, etc., with complex citation linkages; 
% evolving and complex analysis tasks such as tracing the evolution of knowledge and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies.

% In \systemname, LLM-powered AI agents serve as the ``driver'' of the system, leveraging sophisticated reasoning and planning capabilities with fine-grained action-level control to interpret user requests, query large-scale databases, transform and analyze data, visualize the results, and enable a non-linear data exploration process using data-driven artifacts. 
% Through this \textbf{hybrid interface} combining \underline{LUI} and \underline{GUI}, and orchestrated by underlying \underline{LLM agents}, users can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes.

% Through real-world usage scenarios and \wyf{quantitative evaluations}, we demonstrate that this hybrid human-AI interface significantly improves efficiency, insight generation, and user satisfaction compared to LUI-only or GUI-only alternatives, while maintaining the rigor essential for discovery and decision-making. 

% \wyf{
% Together, our conceptual model, system design, and empirical findings outline a blueprint for the next generation of data-driven systems. 
% Beyond the SciSci domain, the conceptual model offers a generalizable foundation for human–AI collaboration frameworks that seamlessly integrate natural language interfaces and graphics user interfaces, enabling more transparent, creative, and rigorous scientific discovery and decision-making across disciplines and applications.
% }

% \wyf{
% Ultimately, through this work, we aim to catalyze a broader transformation in how humans and AI reason together, moving from isolated interfaces and workflows toward hybrid systems that amplify both human intuition and machine intelligence, accelerating the pace of discovery and innovation in science and beyond.
% }







% \wyf{(generalizability levels: 
%         [level 1]: SciSciCanvas (use SciSci as an example domain); 
%         [level 2]: go beyond \textbf{SciSci} --- hybrid user interfaces (LUI + GUI) for discovery and human sense-making; 
%         [level 3]: go beyond \textbf{LUI + GUI} --- human-AI collaboration for expert-oriented systems (e.g., for scientific discovery and decision-making) --- \textbf{HAI4Science}; 
%         [level 4]: HAI for all scenarios (general public + expert-oriented systems)
%     )}


% 宋阳秋老师2025.05刚发的一个survey: https://github.com/HKUST-KnowComp/Awesome-LLM-Scientific-Discovery 


% Tiantian:
% 4. In different scenarios, how AI and human can collaborate — can we think of a framework that can incoorperate SciSciGPT and SciSciCanvas? — in both interaction design, and underlying HAI4Science workflow?


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-1.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/discussion-2.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}



% Framework for Integrating SciSciGPT and SciSciCanvas
% A unified HAI4Science workflow could blend both systems:
% Interaction Design
% Language-to-Visualization Bridging: Users pose questions via SciSciGPT (LUI), which generates interactive visual artifacts in SciSciCanvas (GUI).
% Bidirectional Control: Modify a chart (GUI) to auto-update the LLM’s context (e.g., "Focus on papers from 2020–2025"), enabling mixed-initiative exploration.

% Underlying Workflow
% Multi-Agent Collaboration: SciSciGPT parses intent and delegates tasks (e.g., trend analysis) to domain-specific AI agents, while SciSciCanvas renders results as manipulable visualizations.
% Iterative Refinement: Users toggle between refining hypotheses (LUI) and adjusting visual parameters (GUI), creating a closed-loop discovery process.







% 7. Automation
% Definition: Use of computational techniques to conduct repetitive analytical tasks, freeing researchers for higher-level conceptual work.

% Support: Jordan & Mitchell (2015); Kitano (2016).

% - Shift of human roles: transfer from executor to idea generator.
% - Scientific discovery workflow: step by step, AI take over low-level roles.
% - During this shifting, think about transparency, rigous of discovery process

==> sections/archive/03-2-evaluation/03-2-evaluation_v3_20251201.tex <==
% \section{Results}
% \label{section:evaluation} 
% We evaluate the usefulness of our conceptual framework and demo system using two case studies and an expert interview. 

\subsection{Case Study} 
\label{subsection:case-study} 
We evaluate the usefulness of our conceptual framework and demo system using two case studies using two example scientific domains. 

\subsubsection{\newlyadded{Case Study 1: Climate Study}} 
\label{subsection:case-1-climate} 
\newlyadded{
We first revisit the motivating example introduced in Section~\ref{subsection:conceptual-framework} and expand it into a comprehensive analytical scenario situated in the climate sciences. 
Understanding regional climate variability, especially seasonal temperature dynamics, is central to research on extreme heat, climate change attribution, and ecological and public-health risk assessment~\cite{jia2024seasonal, bhattarai2025understanding}. 
Here we illustrate how \systemname supports such analyses by enabling iterative, mixed-modality exploration of multi-year environmental sensor records.
Assume a climate scientist studying long-term surface observations, including monthly temperature, \wyf{humidity, and air-quality} indices collected across U.S. states. 
The researcher begins with the natural-language instruction: 
% We first revisit the example scenario used in Section~\ref{subsection:conceptual-framework} in the climate domain, by providing a more comprehensive exploration logic. 
% Assume a researcher analyzing environmental sensor data collected over multiple years, including monthly temperature, humidity, and air-quality measurements. The researcher issues the natural-language instruction: 
\textit{``Plot the temporal trend of the temperature by month in the state of Florida in the last year (2024).''}
}

% generation
\newlyadded{
\systemname first interprets the analytical intent using the database schema and description, invoking a sequence of data-filtering actions (\eg, \actionname{select_table} and \actionname{filter_rows}) to identify the relevant tables, extract the appropriate fields, and constrain the data by state and year. 
This process produces a temporally indexed dataframe capable of answering the query.
Next, visualization-related actions (\eg, \actionname{add_chart_type}, \actionname{add_encoding}, and \actionname{add_params}) select a suitable chart type (\ie, a monthly line chart), determine the visual encoding and interactions, generate textual summaries of salient data patterns. 
\systemname then compiles these components into a Vega-Lite specification for display as an interactive figure (Fig.~\ref{fig:bidirectional-mapping}-A1), while simultaneously rendering and storing a static image of the visualization in the database to support reproducibility, provenance tracking, and future reuse within the data-driven artifact.
% \systemname first interprets user's analysis intent with the database schema and description, and called a list of filtering actions to select tables and columns that are relevant to the problem. and further filter the data by constraints (\ie, specific state and year). 
% This generates the temporally dataframe that is able to answer user's query. 
% Next, the system calls a list of visualization-related actions to select proper chart types, visualization encodings and interactions, and generate textual insights, to finally generate Vega-Lite specification code to return as the result figure. 
% data insights
The visualization reveals a gradual warming through spring, consistent with subtropical seasonal cycles, followed by sustained high temperatures spanning nearly four months, a pattern widely discussed in studies of persistent summer heatwaves in the U.S. Southeast~\cite{raghavendra2019floridian, jia2024seasonal}. 
A sharper cooling onset in early autumn further distinguishes Florida’s seasonal asymmetry.
% The researcher noticed a relatively slow 回暖 trend from windter to summer and a quicker 降温 trend at fall. 
% And the summer duration is long across nearly four months. 
}

% drill-down and generation.
\newlyadded{
Motivated by these patterns, the researcher seeks to contextualize Florida's summer temperatures relative to other states. 
After brushing the interval from June to August on the line chart, the researcher issues a follow-up instruction:
\textit{``Show me the average temperature of each U.S. state during the selected time range, and rank them from hottest to coolest.''} 
\systemname integrates both GUI interactions and natural-language input (Fig.~\ref{fig:bidirectional-mapping}-A2), and executes a new action sequence: re-querying the database with the updated temporal scope, applying aggregation operations to compute state-level mean temperatures, and sorting the results (Fig.~\ref{fig:bidirectional-mapping}-A3).
The system then generates a bar chart summarizing the national temperature ranking for the summer months (Fig.~\ref{fig:bidirectional-mapping}-A5), showing that Texas and Florida emerge as the two hottest states, consistent with climatological assessments of regional heat extremes. 
% Curious about the national tempreture difference in summer across different states, the researcher brush the time period between June and August, and asked a follow-up question: 
% \textit{``Show me the average temperature of each U.S. state during the selected time range, and rank them from hottest to coolest.''} 
% \systemname takes both the GUI interaction and language instructions (Fig.~\ref{fig:bidirectional-mapping}-A2) and excute a sequence of actions to query the database again with an additional temporal scope. 
% Additional data transformation actions are also involved to group by the data by states to calculate the average temporeture and sort the results accordingly. 
% The suystem then generate a new bar chart to show the tempreture ranking in summer of all states in US (Fig.~\ref{fig:bidirectional-mapping}-A5). 
% Texas and Florida are the top 2 hottest states in the summer. 
}

% coordination
\newlyadded{
The researcher next asks how these rankings shift across seasons. 
By brushing the winter months (November to December) on the original line chart (Fig.~\ref{fig:bidirectional-mapping}-B1), the coordinated bar chart updates immediately (Fig.~\ref{fig:bidirectional-mapping}-B3). 
The winter comparison highlights a markedly different spatial pattern: Hawaii becomes the warmest region, reflecting its tropical climate regime, in contrast to the continental states whose temperatures converge at substantially lower values. 
This seasonal contrast illustrates how regional climate heterogeneity emerges across temporal scales, which is an important consideration in climate impact modeling and adaptation planning. 
% The researcher is also interested in compare the average temporetures in other seasons, so the researcher brush the line chart again to filter the winter between Nov and Dec and the bar chart update the data imediately (Fig.~\ref{fig:bidirectional-mapping}-B3). 
% It turns out that Hawaii becomes the hottest state, meaning a different xxx compared with the summer. 
}

\subsubsection{Case Study 2: Innovation Landscape at Universities} 
\label{subsection:case-2-ii} 
% \wyf{[Yifang] Goal of the case: three functions of the system: 
% 1. modify chart (change x and y axises), 
% 2. basic statistical analysis, 
% 3. extend chart, but also modify chart.
% }

% \wyf{[Yifang]: double check the tongnee of the writing: maybe its a usage scenario, not a case -- using we vs. he/she. Check other NC paper.}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/case-2-ii.jpg}
    \caption{Case study 2: Innovation Landscape at Universities.
    }
    \label{fig:case-1}
\end{figure}

Studying the innovation landscape of research has become a central challenge in both the Science of Science (SciSci) community where researchers aim to map the dual frontiers of science and technology~\cite{ahmadpoor2017dual, liang2022systematic, yin2022public} and among university leaders and science policy-makers seeking to accelerate technology transfer and amplify research impact~\cite{wang2023innovationinsights, wang2025funding}. 
Yet uncovering such latent potential remains analytically demanding: the relevant signals are distributed across heterogeneous data sources, and the exploratory questions evolve rapidly as new insights emerge. 
To illustrate how \systemname supports this dynamic analytical process, we conducted a case study using innovation-related data from a top U.S. research university. 

% step 1: generation
A SciSci researcher starts to explore the innovation landscape from the individual inventor level: 
\textit{``Show me the distribution of inventors based on their number of invention disclosures (as y axis) and number of their papers cited by patents (as x axis)''}
% \textit{``Show me the distribution of all inventors at this university in terms of their current patent activity and their hidden research potential relevant to technological use.''} 
% \systemname initiates the analysis through the \planner agent, which constructs an initial action plan: including data filtering, analysis, and visualization. 
Through the plan–action–execution loop, the system generates a sequence of atomic actions (\eg, \actionname{select_table}, \actionname{project_column}, and \actionname{add_chart_type}, Fig.~\ref{fig:case-1}-A), automatically executes the associated code, and synthesizes the results.
Finally, an interactive scatterplot is returned showing the inventor distribution of this university (Fig.~\ref{fig:case-1}-A), with x axis encodes papers cited by patents (a proxy for technological potential) and the y axis encodes invention disclosures (a proxy for present-day innovation activity). 
Hover interactions expose precise values for each inventor, enabling accurate inspection of outliers and potential inventors \wyf{(Fig.~\ref{xx})}.

% 
% step 2: modify chart
% 1. adjust scale (log scale)
The researcher notices that most inventors cluster tightly in the lower-left region due to the heavy-tailed nature of both measures. This compression obscures meaningful structure and hinders the identification of high-potential individuals. 
Thus, the researcher selects the figure and requested: 
\textit{``Update the chart to turn the x and y values into log scale. Using the formula: x = log(x + 1) to avoid zero.''} 
% \textit{``Help me adjust the values of the x and y axes to log scale to make the distribution clearer.''} 
Here, the system shifts from generation to manipulation. 
The system takes the existing visualization and underlying data as inputs, infers the user’s intent, and triggers a new chain of actions to transform the data (\eg, \actionname{derive_column}) and update the visual encoding (\eg, \actionname{modify_encoding}), and regenerates the scatterplot with a log transformations applied to both axes, providing a clearer, more discriminative view of the inventor distribution    (Fig.~\ref{fig:case-1}-B).
% \wyf{(add a figure to show chart and action list)}. 
% This step exemplifies one strength of the hybrid interface: users do not need to regenerate the plot from scratch nor understand the underlying visualization grammar. 
% Instead, they simply articulate their analytic need, and the system performs fine-grained, context-aware modifications through a transparent sequence of actions. 
% 2. regression line
% 我就是不确定，我们基于log的数值，做regression，make sense不 -- yifan: 可以的！

% step 3: gender difference / other meta information (department) 
Beyond the overall distribution, the researcher quickly notices a small group of individuals with higher number of invention disclosures (Fig.~\ref{fig:case-1}-C, left). 
% the researcher quickly notices a visually distinctive cluster of faculty located along the lower boundary of the scatterplot: individuals with no recorded invention disclosures, yet whose research papers have been cited by external patent assignees---a group of faculty with untapped innovation potential! 
% This pattern raises a natural follow-up question: who are the researchers contributing scientific knowledge that is being used technologically, despite not participating directly in invention disclosure activities? 
To examine this group, the researcher brushes the corresponding region through direct manipulation on the scatterplot and poses two follow-up queries: 
\textit{``show me the gender distribution''} and \textit{``show me the department information''}. 
% 
The system uses both the natural-language request and the GUI-based selection as joint input signals, triggering a new sequence of atomic actions. 
It then generates a bar chart summarizing the gender distribution and a pie chart showing the departmental composition of the selected group \wyf{(Fig.~\ref{fig:case-1}-C, D, E)}, enabling quick assessment of demographic patterns among these faculty. 
% 
By comparing the gender distributions of different subgroups, the researcher observes a clear disparity between faculty with higher numbers of invention disclosures (Fig.~\ref{fig:case-1}-C) and those with few or none (Fig.~\ref{fig:case-1}-D): 
male faculty members appear more likely to have disclosed inventions than their female counterparts (from two bar charts). 
% 
Additionally, when examining departmental composition (from two pie charts), faculty with frequent invention disclosures are disproportionately concentrated in fields such as biomedical engineering, chemistry, and materials science, reflecting the uneven distribution of patenting activity across research areas within the university. 

% \wyf{The returned result shows that most of the faculty with untapped potential are males, ... 
% Compare faculty in terms of: 
% gender, department, and tenure-status.
% [Yifang]: (1) to discuss what insight to deliver. Untapped potential seems not a good direction -- more like decision-making; shall we here study data insights?
% (2) to use the coordination function: change to filter another region for comparison.
% } 

% "Numerous factors can contribute to this gender gap, such as unequal access to education and mentorship, funding disparities, prevailing norms and stereotypes and structural barriers in patenting and commercialization processes. A better understanding of these challenges would help to broaden the pool of innovators.

% Similarly, we see a large difference between tenure-track and tenured faculty members: tenured researchers patent their work at a higher rate. But one doesn’t magically become more innovative the moment tenure is granted. The causes of this gap are probably distinct from those of the gender one, and might include promotion incentives and what counts towards tenure. But both discrepancies point to untapped opportunities for innovation."

% step 4: 
% 4.1 tracable with code (SQL, Python), data, and vis code
% 4.2 save artifact for future exploration (there are other universities' data comming in). 

To ensure analytical rigor, the researcher downloads the underlying data, generated code, and visualization outputs from each figure to verify the procedure and results. 
The entire chat session, including the data-driven artifact, is also saved for future analysis, enabling replication and facilitating cross-institutional comparisons as additional university datasets become available. 
% Taking notes about the data insights and findings, the researcher downloads the relevant data, code, and visualization image from each figure to double check the procedure. 
% He also save the conversation along with this artifact for future analysis -- as there are more data from other universities coming in -- a great chance to check the robustness of the insights across different research institutions. 

This case demonstrates how researchers can use LLM-native figures to iteratively explore data, both by refining existing visualizations and by generating new, contextually linked ones.



\subsubsection{Case Study 3: Science Use in Public Policy} 
\label{subsection:case-3-science-policy} 
Zander's paper. 
% Note: currently, raw data are only six tables: `/home/yifangwang/visual-gpt/visual-gpt-backend/data/case-study-1-20250606`. 
% TODO: Consider adding a complete list of all tables in SciSciNet and Overton? Or Not? 



\subsection{Computational Evaluation}
\label{subsection:computational-evaluation} 
\newlyadded{The objective of this evaluation is to validate the core technical properties of LLM-native figures, 
\wyf{that the user intent can be interpreted correctly and return relevant data, code, and visualization (generative power)}, 
that interactions on a visualization can be reliably mapped back to the underlying analytical state (mapping fidelity), 
that each figure contains sufficient provenance for exact reconstruction (round-trip reproducibility), 
and that the framework supports multi-step scientific analysis in realistic domains (case study demonstration). 
These properties correspond directly to the framework's contributions and collectively establish the feasibility of figures as machine-interpretable scientific artifacts.}

\newlyadded{We intentionally focus on \wyf{artifact-level and system-level} validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface design.}

\wyf{[Yifang: Check this AI paper to generate reasonable test set: https://arxiv.org/html/2510.10397v1.]}


\subsubsection{Mapping Fidelity}
\label{subsubsection:evaluation-accurary}
\newlyadded{We first assess whether visual interactions, such as clicking or brushing on a figure, can be accurately mapped to the correct underlying data rows and analytic operations. 
This evaluation directly tests the framework's core claim that figures can function as reliable computational interfaces.} 

\newlyadded{
\textbf{Test Design.} 
Using datasets in the case study, We generate a suite of visualizations for which ground-truth correspondences between visual marks and data rows are known. 
These include: 
bar charts (single/grouped),
line charts (single/multi-series),
scatter plots with color encodings, 
pie charts, 
faceted visualizations. 
For each chart, we programmatically generate a set of interactions, including 
single-mark clicks and 1D and 2D brushes. 
% combined selections across marks or facets. 
For each interaction, \systemname retrieves the data subset implied by the selected marks via the mapping table $R_t$. 
We then compare this retrieved subset D and relevant actions and codes against the ground-truth \wyf{(check manually)}, and obtained the precision metric (in total and breakdown by chart type).
}

\newlyadded{
\textbf{Results.}
% High F1 scores across chart types would demonstrate that LLM-native figures provide a robust visual-to-analytical bridge.
xxxxx.
}


\subsubsection{Round-Trip Reproducibility}
\label{subsubsection:evaluation-reproducibility}
\newlyadded{To evaluate whether an LLM-native figure artifact provides complete provenance, enabling precise re-execution of the analytical workflow and deterministic reconstruction of the figure.}

\newlyadded{
\textbf{Test Design.} 
We sample a large set of figures $F_t={V_t,D_t,C_t,M_t}$ produced during system use. 
For each figure, we use $C_t$ and underlying database to recompute the data ($D_g$) and generate visualization ($V_g$). 
Then we compare the stored and reconstructed figures at two levels:
(1) Specification-level equality (JSON structural comparison) 
and (2) Visual similarity (visual-mark-level equivalence: same mark IDs, encodings, and positions, etc.). 
We calculate the percentages of figures that are with the exact spec equality and the visually identical reconstructions respectively. 
} 

\newlyadded{
\textbf{Results.} 
% High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
xxxxx.
}


\subsubsection{Discussion}
\newlyadded{
Failure analysis (e.g., reproducibility-missing provenance, mismatched encodings, rendering differences). 
}



% \subsection{User Study} 
% \textbf{Participants}: SciSci researchers from different "research age". 

% \textbf{Task}: three case studies, same setting of data. 

% \textbf{Benchmark}: Python/Jupyter Notebook, SciSciGPT. 

% \textbf{Evaluation dimensions}: 
% (1) Efficiency: time and accuracy. -- same analysis tasks in the case study. 
% (2) Expressiveness: number of insights generated. -- do not limit analysis tasks, only limit the high-level research question. To test: the number of insights generated; the diversity of insights generated. 

% \subsection{Expert Interview} 
% (1) Use \textit{Five-point Likert Scale} to allow users score different dimensions of the system: usability, etc. 

% (2) Qualitative evaluation: summarize their feedback in terms of hybrid user interface, LLM agent engine, and suggestions (especially for data-driven scientific discovery and LLM-native figures to be presented in their research paper -- open science related questions). 


==> sections/archive/03-2-evaluation/03-2-evaluation_v4_20260206.tex <==
\subsection{Case Study} 
\label{subsection:case-study} 
Having illustrated the mechanics of our domain-independent conceptual framework through a didactic climate example (Sec.~\ref{subsection:conceptual-framework}), we now demonstrate its utility in a domain where the demands on analytical reasoning are substantially greater. 
The Science of Science (SciSci) field~\cite{fortunato2018science, wang2021science} provides an ideal testbed: its research landscape is rich with heterogeneous, rapidly evolving datasets and requires analytical workflows that are inherently iterative, exploratory, and decision-driven.
% 
% \textbf{Innovation Landscape at Universities.}
Within this context, studying the innovation landscape of research has become a central challenge in both the SciSci community where researchers aim to map the dual frontiers of science and technology~\cite{ahmadpoor2017dual, liang2022systematic, yin2022public} and among university leaders and science policy-makers seeking to accelerate technology transfer and amplify research impact~\cite{wang2023innovationinsights, wang2025funding}. 
Yet uncovering such untapped potential remains analytically demanding: the relevant signals are distributed across heterogeneous data sources, and the exploratory questions evolve rapidly as new insights emerge. 
To illustrate how \systemname supports this dynamic analytical process, we conducted a case study using innovation-related data from a top U.S. research university. 

% step 1: generation
A SciSci researcher first uses \systemname to explore the innovation landscape from the individual inventor level: 
\textit{``Show me the distribution of inventors based on their number of invention disclosures (as y axis) and number of their papers cited by patents (as x axis)''}
% \textit{``Show me the distribution of all inventors at this university in terms of their current patent activity and their hidden research potential relevant to technological use.''} 
% \systemname initiates the analysis through the \planner agent, which constructs an initial action plan: including data filtering, analysis, and visualization. 
Through the plan–action–execution loop, the system generates a sequence of atomic actions (\eg, \actionname{select_table} and \actionname{add_chart_type}, executes the associated code, and returns an interactive scatterplot showing the inventor distribution of this university (Fig.~\ref{fig:case-1}a), with y axis encodes invention disclosures (a proxy for present-day innovation activity) and x axis encodes papers cited by patents (a proxy for technological potential). 

% 
% step 2: modify chart
% 1. adjust scale (log scale)
The researcher notices that most inventors cluster tightly in the lower-left region due to the heavy-tailed nature of both measures. 
This compression obscures meaningful structure and hinders the identification of high-potential individuals. 
Thus, the researcher selects the figure and requested: 
\textit{``Update the chart to turn the x and y values into log scale. Using the formula: x = log(x + 1) to avoid zero.''} 
% \textit{``Help me adjust the values of the x and y axes to log scale to make the distribution clearer.''} 
Here, the system shifts from generation to manipulation (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (\textit{manipulation})). 
The system takes the existing visualization and underlying data as inputs, infers the user's intent, and triggers a new chain of actions to transform the data (\eg, \actionname{derive_column}) and update the visual encoding (\eg, \actionname{update_encoding}), and regenerates the scatterplot with a log transformations applied to both axes, providing a clearer, more discriminative view of the inventor distribution (Fig.~\ref{fig:case-1}b, c).
The overall distribution exhibits a positive relationship between the two metrics, suggesting that patent-cited publications may serve as a useful indicator of a researcher's inventive activity.
Hover interactions expose precise values for each inventor, enabling accurate inspection of outliers and potential inventors (Fig.~\ref{fig:case-1}b).
% \wyf{(add a figure to show chart and action list)}. 
% This step exemplifies one strength of the hybrid interface: users do not need to regenerate the plot from scratch nor understand the underlying visualization grammar. 
% Instead, they simply articulate their analytic need, and the system performs fine-grained, context-aware modifications through a transparent sequence of actions. 
% 2. regression line
% 我就是不确定，我们基于log的数值，做regression，make sense不 -- yifan: 可以的！

% step 3: extend chart: gender difference / other meta information (department) 
Beyond the overall distribution, the researcher quickly notices a small group of individuals with higher number of invention disclosures (Fig.~\ref{fig:case-1}d). 
% the researcher quickly notices a visually distinctive cluster of faculty located along the lower boundary of the scatterplot: individuals with no recorded invention disclosures, yet whose research papers have been cited by external patent assignees---a group of faculty with untapped innovation potential! 
% This pattern raises a natural follow-up question: who are the researchers contributing scientific knowledge that is being used technologically, despite not participating directly in invention disclosure activities? 
To examine this group, the researcher brushes the corresponding region through direct manipulation on the scatterplot and poses two follow-up queries: 
\textit{``show me the gender distribution using a bar chart''} and \textit{``show me the department information using a pie chart''} (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (\textit{drill-down})). 
% 
The system uses both the natural-language request and the GUI-based selection as joint input signals, triggering a new sequence of atomic actions. 
It then generates a bar chart summarizing the gender distribution and a pie chart showing the departmental composition of the selected group (Fig.~\ref{fig:case-1}d), enabling quick assessment of demographic patterns among these faculty. 
% 
By comparing the gender distributions of different subgroups, the researcher observes a clear disparity between faculty with higher numbers of invention disclosures (Fig.~\ref{fig:case-1}d) and those with few or none (Fig.~\ref{fig:case-1}e): 
male faculty members appear more likely to have disclosed inventions than their female counterparts (from two bar charts, Fig.~\ref{fig:case-1}d, e). 
When examining departmental composition (from two pie charts, Fig.~\ref{fig:case-1}d, e), faculty with frequent invention disclosures are disproportionately concentrated in fields such as biomedical engineering, chemistry, and materials science, reflecting the uneven distribution of patenting activity across research areas within the university. 

A contrasting pattern emerges when the distribution is examined along the x-axis, which captures the potential predictor (the number of publications cited by patents) of commercialization activities (Fig.~\ref{fig:case-1}f). 
Unlike the y-axis comparison, where faculty with high numbers of disclosed inventions are all male, researchers with high x-axis values comprise both male and female faculty. 
Notably, in the bottom-right region of the scatterplot (Fig.~\ref{fig:case-1}f), where researchers have no disclosed inventions yet their publications are heavily cited by patents, the proportion of female faculty is substantial. 
This subgroup represents researchers with significant untapped innovation potential: their research has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
% This subgroup represents researchers with significant but unrealized innovation potential: their research has demonstrable technological relevance, yet has not been translated into their own patent disclosures, in other words, faculty with untapped innovation potential. 
% \wyf{To discuss: Should we add a concluding sentence that highlights the downstream decision-making step (e.g., the SciSci researcher quickly shares the insight with the TTO, and together they identify faculty with untapped potential for follow-up engagement)?}
% 
Taken together, these patterns suggest a gendered asymmetry between realized and unrealized innovation, where male researchers are more likely to have already converted research into inventions, while many female researchers exhibit comparable innovation potential that remains untapped.

% \wyf{The returned result shows that most of the faculty with untapped potential are males, ... 
% Compare faculty in terms of: 
% gender, department, and tenure-status.
% [Yifang]: (1) to discuss what insight to deliver. Untapped potential seems not a good direction -- more like decision-making; shall we here study data insights?
% (2) to use the coordination function: change to filter another region for comparison.
% } 

% "Numerous factors can contribute to this gender gap, such as unequal access to education and mentorship, funding disparities, prevailing norms and stereotypes and structural barriers in patenting and commercialization processes. A better understanding of these challenges would help to broaden the pool of innovators.

% Similarly, we see a large difference between tenure-track and tenured faculty members: tenured researchers patent their work at a higher rate. But one doesn’t magically become more innovative the moment tenure is granted. The causes of this gap are probably distinct from those of the gender one, and might include promotion incentives and what counts towards tenure. But both discrepancies point to untapped opportunities for innovation."

% step 4: 
% 4.1 tracable with code (SQL, Python), data, and vis code
% 4.2 save artifact for future exploration (there are other universities' data comming in). 

To ensure analytical rigor, the researcher downloads the underlying data, generated code, and visualization outputs from each figure to verify the procedure and results. 
The entire chat session, including the data-driven artifact, is also saved for future analysis, enabling replication and facilitating cross-institutional comparisons as additional university datasets become available. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/case-ii.jpg}
    \vspace{1pt}
    \caption{
    \bodyfigurelabel{fig:Figure3}
    Case study: innovation landscape at universities.
    }
    \label{fig:case-1}
\end{figure}


% % Dashun (2025-12-23): 
% % You have nice material there, but it’s partly TODO, and it opens up new interpretive risks. I’d just skip this. 
% % Keep only SciSci innovation as main case; remove policy results (not moving it to Supplement; this way we can save it for rebuttal).

% \textbf{\newlyadded{Science Use in Public Policy.}} 
% % \wyf{Dashun (2025-12-01): 
% % optionally fold the policy example into 1–2 paragraphs at the end, or move it to Supplement.
% % Either move it to Supplement as a “second SciSci vignette” or weave a 1–2 paragraph policy example into the SciSci case study section if you want to hint at breadth. 
% % }
% \newlyadded{
% Scientific evidence is widely regarded as a cornerstone of modern public policy, shaping legislative responses to complex societal challenges such as climate change, public health, and food security~\cite{furnas2025partisan, furnas2025partisanfunding}.
% At the same time, prior research has shown that the uptake, framing, and interpretation of scientific evidence can be systematically shaped by political context, particularly under conditions of sustained partisan polarization~\cite{mccarty2016polarized}.
% This raises a fundamental question at the intersection of science and governance: beyond differences in rhetoric or funding priorities, do policy-makers from different political parties also draw on systematically different bodies of scientific knowledge?
% }

% \newlyadded{
% To explore this question, the SciSci researcher begins by examining what kinds of science are cited in policy, before turning to how those patterns may diverge across parties.
% As an initial overview, the researcher selects policy documents from the U.S. House Energy and Commerce Committee, a central venue for legislation on health, energy, and agriculture, and asks:
% \textit{``Show me the distribution of all these policies’ cited papers based on paper title similarity.''}
% \systemname first filters the policy corpus by source and extracts the associated cited papers.
% To show the latent topical structure without imposing predefined categories, the system applies two analysis actions (\ie, \actionname{text_embedding} followed by \actionname{dimension_reduction}) and generates a scatterplot in which each point represents a cited paper positioned by semantic similarity (Fig.~\ref{fig:case-2-science-policy}).
% \wyf{TODO: color the plot by party affiliation using policy data from Zander’s dataset.}
% Having identified visually separable clusters, the researcher then seeks to ground these abstract regions in concrete scientific content.
% Using direct manipulation, the researcher circles distinct regions of the scatterplot and issue a follow-up request:
% \textit{``Give me a table showing the list of all these selected papers with attributes including paper title and DOI.''}
% In response, the system maps the visual selection back to the underlying database, filters the corresponding records, and returns a raw data table for inspection.
% Through this drill-down, the researcher finds two topical clusters (Fig.~\ref{fig:case-2-science-policy}): one centered on \textit{Nutrition and Agricultural Impacts}, and another focused on \textit{Infectious Disease Prevention and Response}.
% These clusters reflect substantively different dimensions of policy-relevant science, highlighting how health, food systems, and disease control co-exist within the committee's evidence base.
% \wyf{TODO: add discussions of different topic distribution of papers by two parties).}
% }

% \newlyadded{
% Together, this exploration suggests that science use in public policy is not monolithic but organized around distinct thematic regimes that can be explored through interactive, data-driven analysis.
% More importantly, the ability to align these topical structures with political attributes opens the door to systematically examining whether partisan divides extend beyond \textit{how} science is discussed to \textit{which science is mobilized} in the first place, which is an insight with direct implications for evidence-based governance and science–policy communication.
% }
% % Science has long been regarded as essential to policy-making, serving as one of the primary sources of evidence that informs decisions to tackle societal challenges such as climate change and public health~\cite{furnas2025partisan, furnas2025partisanfunding}. 
% % Yet, as the rising political polarization still exists~\cite{mccarty2016polarized}, the SciSci researcher is curisous about whether science use by policy-makers are also different in different parties. 
% % Thus, the researcher first select a policy source type from House Energy and Commerce Committee and take a look at the cited paper's topics as an overview: 
% % ``Show me the distribution of all these policies' (from House Energy and Commerce Committee) cited papers based on paper title similarity.'' 
% % \systemname firsts extract a list of paper by the filtering criteria and calls two analysis actions (\ie, \actionname{text_embedding} and \actionname{dimension_reduction}) as the similarity measures and finally generates a scatterplot of all the cited papers (Fig.~\ref{fig:case-2-science-policy}). 
% % \wyf{TODO: color the plot using the party label (to process the data from Zander's paper).}
% % Curious about the paper topics, the researcher circles different regions and asked ``Give me a table showing the list of all these selected papers with attributes including paper title and doi.''. 
% % The system respond by filtering the data and return the raw data tables. 
% % Two regions of topics are shown (Fig.~\ref{fig:case-2-science-policy}), one focusing on Nutrition and Agricultural Impacts and another focusing on Infectious Disease Prevention and Response. 
% % \wyf{TODO: add discussion of different topic distribution of papers by two parties).}
% % }

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/case2-science-policy.jpg}
%     \vspace{1pt}
%     \caption{\newlyadded{Case study: science use in policy-making. Left: a small cluster of papers on Nutrition and Agricultural Impacts; Right: a cluster of papers focused on Infectious Disease Prevention and Response.}}
%     \label{fig:case-2-science-policy}
% \end{figure}


% \vspace{pt}
The case study demonstrates how researchers can use LLM-native figures to iteratively explore data, both by refining existing visualizations and by generating new, contextually linked ones in an example scientific domain. 
Unlike conventional tools where users must manually recreate views, repeat transformations, or rely on static figures with no provenance, our approach preserves each analytical step as a versioned, navigable artifact. 
This enables researchers not only to trace and validate how insights were produced, but also to extend or revisit any point in the exploration trajectory, supporting a form of mixed-initiative, provenance-rich analysis that existing systems do not provide.




\subsection{Computational Evaluation}
\label{subsection:computational-evaluation} 
The objective of this evaluation is to validate the core technical properties of LLM-native figures, that the user intent can be interpreted correctly and return relevant data, code, and visualization, and interactions on a visualization can be reliably mapped back to the underlying analytical state (mapping fidelity, Sec.~\ref{subsection:conceptual-framework}-Bidirectional Mapping), 
that each figure contains sufficient provenance for exact reconstruction (round-trip reproducibility, Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), 
and that the framework supports multi-step scientific analysis in realistic domains (case study, Sec.~\ref{subsection:case-study}). 
These properties correspond directly to the framework's contributions and collectively establish the feasibility of figures as machine-interpretable scientific artifacts.
% 
We intentionally focus on artifact-level and system-level validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface design.
% \wyf{[Yifang: Check this AI paper to generate reasonable test set: https://arxiv.org/abs/2510.10397.]}
% \wyf{How to generate these test cases: (1) manually (current method). Or, (2) given the dataset and table description, we ask LLM to generate a list of questions for each type of (figure_type, interaction_type, tier_type).}


% \subsubsection{Mapping Fidelity}
% \label{subsubsection:evaluation-accurary}
\textbf{Mapping fidelity.} 
We evaluate the mapping fidelity of the bidirectional mapping mechanism (Sec.~\ref{subsection:conceptual-framework}): 
(1) whether user questions can be accurately transformed into visual data insights, and
(2) whether visual interactions, such as clicking or brushing on a figure, can be accurately mapped back to the intended subsets of underlying data and the appropriate analytic operations. 
This evaluation directly tests the framework's core claim that figures can function as reliable computational interfaces.

Test Design.  
We adopt a structured, coverage-oriented evaluation strategy that treats mapping fidelity as a functional correctness problem over a well-defined interaction space. 
Using the datasets from our case studies, we construct a test suite consisting of paired queries, where each test case includes: 
(1) an initial user question that requires generating a figure and (2) a follow-up question that depends on a specific visual interaction with that figure to generate a new visualization or update the existing figure. 
This design mirrors realistic usage patterns in which users alternate between language-based queries and direct manipulation.
% 
To ensure systematic coverage and reduce evaluator bias, we use an LLM to generate 309 valid test cases, each with 3 sub-tasks (Supplementary Notes 3.1). 
Test cases are diversified along three dimensions: 
(1) figure type (\eg, bar, line, pie, scatter plots, and tables),
(2) interaction type (\eg, single-mark selection, one-dimensional interval brushing, and two-dimensional brushing), 
and (3) analytical complexity, with \textit{tier-1} cases representing canonical scenarios involving a single table and minimal transformation, and \textit{tier-2} cases reflecting realistic workflows that require joins across multiple tables, aggregations, or modeling operations.
% and (4) reference solution logic, which specifies the expected data subset, transformation steps, and analytical outcome for each case.
% Representative examples of the test cases are provided in the Supplementary Information (Supplementary Note~\ref{subsection:si-computational-evaluation}). 
% 
We evaluate mapping fidelity along both directions of the language–visualization loop using three metrics across all test cases.
\textit{Execution Success Rate} is the proportion of test cases in which the system successfully completes the end-to-end execution and returns a usable visualization artifact (i.e., no execution failure and a chart is generated).
\textit{Conditional Accuracy} (conditional on success) is the proportion of cases in which the generated analytical process and results are semantically and logically correct with respect to the user's intended analysis.
\textit{End-to-end Accuracy} is the proportion of cases in which the figures are both successfully generated and analytically correct. 
% in which the system successfully completes execution (\ie, success) and the resulting analytical process and outputs are semantically and logically correct with respect to the user’s intended analysis (\ie, accurate). 
% which captures the proportion of cases that are both successfully generated and analytically correct.

Results.
% 1. analysis -> vis
We first assess the mapping from analytical operations to visualization using the initial question in each test case. 
Given a user instruction, \systemname generates a sequence of actions to retrieve and analyze data and produce an interactive figure. 
We evaluate the correctness of the generated code (SQL, Python, and Vega-Lite), the retrieved data subset $D$, and the resulting figures through manual inspection by two authors and cross-validated with the generated LLM-based solution.
\systemname achieves an overall \textit{Execution Success Rate} of \wyf{$96.7\%$} and \textit{End-to-end Accuracy} of \wyf{$92.7\%$} (Fig.~\ref{fig:computational-evaluation}-Initial Question). 
Most inaccurate cases stem from SQL generation, such as failures to perform fuzzy matching for user-specified concepts (\eg, querying “Computer Science” verbatim when the database stores ``computer science'') and misidentification of the analytical entity (\eg, returning counts of researchers instead of papers). 
% the accuracy of generating incorrect Vega-Lite is low, only one case mis-encode the y axis attribute. 
% Specifically, the accuracy of correctly generating data filtering and transformation queries (SQL), together with optional analytical code (Python), is \wyf{xx}. 
% Conditional on correct data retrieval, the accuracy of generating valid visualization specifications is \wyf{xx}. 
% Figure~\ref{??} further breaks down performance by visualization type, showing consistently high success rates across chart categories.
% \wyf{Add one sentence to discuss chart type variations.}
% 
% 
% 2. vis -> analysis (two methods: follow-up question-answering, coordination)
% \wyf{We only need to calc the accuracy of SQL step in 2nd figure generation, no need to calc vis generation step.}
Second, we assess the mapping from visualization back to analytical operations using two approaches: follow-up question-answering and inter-figure coordination. 
% 2.1 follow-up question-answering
In the task of follow-up question-answering, for each figure–interaction pair, \systemname maps selected visual marks to a data query via the relation $R_t$ and generates the corresponding analytical actions. 
We examine the results of the generated SQL query $C$ and the retrieved data subset $D$. 
% 
When users select visual marks or regions on the figure, the system correctly infers the corresponding data filtering and transformation logic with \wyf{$78.8\%$} \textit{End-to-End Accuracy} (Fig.~\ref{fig:computational-evaluation}-Follow-up Question, SQL generation). 
% failure analysis
% Among the cases with inaccurate SQL generation, 
We observe that inaccuracy arises when translating GUI interactions (\eg, brushing or clicking) into SQL filtering logic.  
For instance, a continuous x-axis brush $[a, b]$ may be incorrectly mapped to a discrete ``IN'' predicate rather than a ``BETWEEN'' range condition. 
% For example, given the GUI selection of x-axis range $[a, b]$, the model may misinterpret this continuous selection as a discrete set, generating an IN condition over boundary values rather than a BETWEEN range predicate for an axis-aligned brush.
This problem highlights the need for more explicit guidance, such as structured prompts or interaction-aware constraints, to ensure that GUI-derived filtering semantics are faithfully translated into SQL predicates in future LLM system designs. 
% 2.2 coordination update
Fot inter-figure coordination, when users select or brush an updated region of interest, the system updates the coordinated figure by modifying the underlying SQL query to retrieve the corresponding data. 
The resulting \textit{End-to-End Accuracy} reaches \wyf{$92.0\%$} (Fig.~\ref{fig:computational-evaluation}–Coordination).
Most inaccurate cases arise from errors in SQL regeneration, typically due to the introduction of unnecessary filtering conditions or incorrect substitution of the original query predicates. 
% The majority of inaccurate cases are typically due to introducing unnecessary filtering conditions or incorrectly substituting the original query predicates. 

% 3. round-trip reproducibility
\textbf{Round-trip reproducibility.}
Because all actions, code, and parameters used to generate a figure are explicitly recorded, each LLM-native figure artifact preserves complete analytical provenance. 
This design, by nature, enables deterministic reconstruction of the original figure by re-executing its stored codes against the underlying data. 
% as all the actions and codes of generating a figure have been recorded, our LLM-native figure artifact by nature preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Notes 3.3).
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% Deviations occur only in cases involving inherent non-determinism, such as stochastic analytical procedures that involves random xxx (e.g., dimensionality reduction or random sampling without fixed seeds). 
% % including LLM-generated textual summaries and 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% This evaluation tests whether LLM-native figures function as reproducible computational objects rather than ephemeral presentation outputs.
% \textbf{Results.} 
% High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% \wyf{
% Across the \wyf{180} generated figures, round-trip reproducibility is achieved for nearly all figures. 
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% }.


\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/mapping_fidelity.pdf}
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure4}
        Result of computational evaluation.
    }
    \label{fig:computational-evaluation}
\end{figure}


% \subsubsection{Round-Trip Reproducibility}
% \label{subsubsection:evaluation-reproducibility}
% \wyf{Note: test case: lack of LLM-based Python code.}
% We evaluate whether an LLM-native figure artifact preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
% This evaluation tests whether LLM-native figures function as reproducible computational objects rather than ephemeral presentation outputs.
% % To evaluate whether an LLM-native figure artifact provides complete provenance, enabling precise re-execution of the analytical workflow and deterministic reconstruction of the figure.

% \textbf{Test Design.} 
% We use the same set of 200 test cases described above and store all figures $F_t={V_t, D_t, C_t, M_t}$ generated succesfully during their execution. 
% For each figure, we re-execute the stored code $C_t$ against the original database to regenerate the data subset $D_g$ and the corresponding visualization $V_g$. 
% We then compare the original and reconstructed figures at two levels: (1) specification-level equivalence, assessed via structural comparison of the visualization specifications (JSON); 
% and (2) visual-level equivalence, assessed by matching visual marks, encodings, and positional attributes. 
% We report the proportion of figures that are exactly reproducible at the specification level and those that are visually identical despite potential non-semantic specification differences.

% \textbf{Results.} 
% % High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% \wyf{
% Across the \wyf{180} generated figures, round-trip reproducibility is achieved for nearly all figures. 
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% }.


% \subsubsection{Discussion}
% \newlyadded{
% Failure analysis (e.g., reproducibility-missing provenance, mismatched encodings, rendering differences). 
% Fill in with a short failure-mode paragraph: e.g., missing spec fields, nondeterministic defaults, or database changes. This will earn reviewer trust.
% \wyf{Erzhuo's suggestion: we also report failure cases with persentage and some examples.}
% }



% \subsection{User Study} 
% \textbf{Participants}: SciSci researchers from different "research age". 

% \textbf{Task}: three case studies, same setting of data. 

% \textbf{Benchmark}: Python/Jupyter Notebook, SciSciGPT. 

% \textbf{Evaluation dimensions}: 
% (1) Efficiency: time and accuracy. -- same analysis tasks in the case study. 
% (2) Expressiveness: number of insights generated. -- do not limit analysis tasks, only limit the high-level research question. To test: the number of insights generated; the diversity of insights generated. 

% \subsection{Expert Interview} 
% (1) Use \textit{Five-point Likert Scale} to allow users score different dimensions of the system: usability, etc. 

% (2) Qualitative evaluation: summarize their feedback in terms of hybrid user interface, LLM agent engine, and suggestions (especially for data-driven scientific discovery and LLM-native figures to be presented in their research paper -- open science related questions). 


==> sections/archive/03-2-evaluation/03-2-evaluation_v5_20260322_gender.tex <==
\subsection{Case Study} 
\label{subsection:case-study} 

The climate example in Sec.~\ref{subsection:conceptual-framework} provides a simple illustration of the mechanics of our domain-independent conceptual framework. \wyf{Here we demonstrate its utility through \systemname, an instantiation of the proposed framework developed for the science of science (SciSci) domain. SciSci provides an ideal testbed because it combines massive, heterogeneous datasets spanning grants, publications, and patents with complex research problems, such as tracing knowledge evolution, and high-stakes decision-making scenarios, such as strategic funding allocation.} 
% an ideal testbed because relevant signals are distributed across heterogeneous linked datasets and exploratory questions evolve rapidly as new insights emerge
% The SciSci field~\cite{fortunato2018science, wang2021science} provides an ideal testbed: 
% large-scale heterogeneous data, spanning grants, publications, and patents with complex citation networks;
% complicated research problems, such as tracing knowledge evolution and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as strategic funding allocation and university innovation assessment.

% Innovation Landscape at Universities.
Understanding the innovation landscape of research has become a central challenge in the SciSci community, where researchers aim to map the dual frontiers of science and technology~\cite{ahmadpoor2017dual, liang2022systematic, yin2022public}, and among university leaders and science policymakers seeking to accelerate technology transfer and amplify research impact~\cite{wang2023innovationinsights, wang2025funding}. 
Yet uncovering such untapped potential remains challenging: Relevant signals are distributed across heterogeneous data sources, and exploratory questions evolve rapidly as new insights emerge. 
\wyf{In this case, we use \systemname to explore innovation-related data from a leading U.S. research university.}
% To illustrate how \systemname supports this dynamic analytical process, we conduct a case study using innovation-related data from a leading U.S. research university. 

% step 1: generation
A SciSci researcher first asks \systemname to explore the innovation landscape at the individual inventor level: 
\textit{``Show me the distribution of inventors based on their number of invention disclosures (as y axis) and number of papers cited by patents (as x axis).''}
% \textit{``Show me the distribution of all inventors at this university in terms of their current patent activity and their hidden research potential relevant to technological use.''} 
Through the plan–action–execution loop, the system generates a sequence of atomic actions (\eg, \actionname{select_table} and \actionname{add_chart_type}), executes the associated code, and returns an interactive scatterplot showing the inventor distribution at this university (Fig.~\ref{fig:Figure3}a), with the y-axis encoding invention disclosures (a proxy for present-day innovation activity) and the x-axis encoding papers cited by patents (a proxy for technological potential). 


% step 2: modify chart
% 1. adjust scale (to log scale)
The researcher notices that most inventors cluster tightly in the lower-left region due to the heavy-tailed nature of both measures. 
This compression obscures meaningful structure and hinders the identification of high-potential individuals. 
Thus, the researcher selects the figure and requests: 
\textit{``Update the chart to turn the x and y values into log scale. Use the formula: x = log(x + 1) to avoid zero.''} 
% \textit{``Help me adjust the values of the x and y axes to log scale to make the distribution clearer.''} 
Here, the system shifts from generation to manipulation (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance). 
The system takes the existing visualization and underlying data as inputs, infers the user's intent, triggers a new chain of actions to transform the data (\eg, \actionname{derive_column}) and update the visual encoding (\eg, \actionname{update_encoding}), and regenerates the scatterplot with log transformations applied to both axes, providing a clearer, more discriminative view of the inventor distribution (Fig.~\ref{fig:Figure3}b, c).
The overall distribution indicates a positive relationship between the two metrics, suggesting that patent-cited publications may serve as a useful indicator of a researcher's innovation activity.
Hover interactions expose precise values for each inventor, enabling accurate inspection of potential inventors and outliers (Fig.~\ref{fig:Figure3}b).
% \wyf{(add a figure to show chart and action list)}. 
% This step exemplifies one strength of the hybrid interface: users do not need to regenerate the plot from scratch nor understand the underlying visualization grammar. 
% Instead, they simply articulate their analytic need, and the system performs fine-grained, context-aware modifications through a transparent sequence of actions. 
% 2. regression line
% based on log results, add regression: yifan: make sense!

% step 3: extend chart: gender difference / other meta information (department) 
Within the overall distribution, the researcher quickly notices a small group of individuals with particularly high numbers of invention disclosures (Fig.~\ref{fig:Figure3}d). 
% the researcher quickly notices a visually distinctive cluster of faculty located along the lower boundary of the scatterplot: individuals with no recorded invention disclosures, yet whose research papers have been cited by external patent assignees---a group of faculty with untapped innovation potential! 
% This pattern raises a natural follow-up question: who are the researchers contributing scientific knowledge that is being used technologically, despite not participating directly in invention disclosure activities? 
To examine this group, the researcher brushes the corresponding region through direct manipulation on the scatterplot and poses two follow-up queries to drill down: 
\textit{``show me the gender distribution using a bar chart''} and \textit{``show me the department information using a pie chart''} (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance). 
% "Show me the tenure status distribution using a bar chart."
% "Among these researchers, show the distribution of tenure status for female researchers using a bar chart."
% "Among these researchers, show the distribution of tenure status for male researchers using a bar chart."
% 
The system uses both the natural-language request and the GUI-based selection as joint input signals, triggering a new sequence of atomic actions. 
It then generates a bar chart summarizing the gender distribution and a pie chart showing the departmental composition of the selected group (Fig.~\ref{fig:Figure3}d), enabling quick assessment of demographic patterns among these faculty. 
By comparing the gender distributions of different subgroups, the researcher observes a clear disparity between faculty with higher numbers of invention disclosures (Fig.~\ref{fig:Figure3}d) and those with few or none (Fig.~\ref{fig:Figure3}e): 
male faculty members appear more likely to have disclosed inventions than their female counterparts (Fig.~\ref{fig:Figure3}d, e, two bar charts), and faculty with frequent invention disclosures are disproportionately concentrated in fields such as biomedical engineering, chemistry, and materials science, reflecting the uneven distribution of patenting activity across research areas within the university (Fig.~\ref{fig:Figure3}d, e, two pie charts). 

A contrasting pattern emerges when the distribution is examined along the x-axis, which captures the number of publications cited by patents, a potential predictor of commercialization activities (Fig.~\ref{fig:Figure3}f). 
Unlike the y-axis comparison, where faculty with high numbers of disclosed inventions are all male, researchers with high x-axis values comprise both male and female faculty. 
Notably, in the bottom-right region of the scatterplot (Fig.~\ref{fig:Figure3}f), where researchers have no disclosed inventions yet their publications are heavily cited by patents, the proportion of female faculty is substantial. 
This subgroup represents researchers with significant untapped innovation potential: their research has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
% This subgroup represents researchers with significant but unrealized innovation potential: their research has demonstrable technological relevance, yet has not been translated into their own patent disclosures, in other words, faculty with untapped innovation potential. 
% 
Taken together, these patterns suggest a gendered asymmetry between realized and unrealized innovation, where male researchers are more likely to have already converted research into inventions, while many female researchers exhibit comparable innovation potential that remains untapped.
% "Numerous factors can contribute to this gender gap, such as unequal access to education and mentorship, funding disparities, prevailing norms and stereotypes and structural barriers in patenting and commercialization processes. A better understanding of these challenges would help to broaden the pool of innovators. 
% Similarly, we see a large difference between tenure-track and tenured faculty members: tenured researchers patent their work at a higher rate. But one doesn’t magically become more innovative the moment tenure is granted. The causes of this gap are probably distinct from those of the gender one, and might include promotion incentives and what counts towards tenure. But both discrepancies point to untapped opportunities for innovation."

% step 4: 
% 4.1 tracable with code (SQL, Python), data, and vis code
% 4.2 save artifact for future exploration (there are other universities' data comming in). 
To ensure analytical rigor, the researcher downloads the underlying data, generated code, and visualization outputs from each figure to verify the procedure and results. 
The entire chat session, including the data-driven artifact, is also saved for future analysis, enabling replication and facilitating cross-institutional comparisons as additional university datasets become available. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260209/case-ii.jpg}
    \vspace{1pt}
    \caption{
    \bodyfigurelabel{fig:Figure3}
    \textbf{Case study: university innovation landscape.}
    \textbf{(a)} The figure generated for the first user query. 
    \textbf{(b)} The updated figure after adjusting the x- and y-axes to log scales. 
    \textbf{(c)} Screenshots of the streaming output when generating and updating a figure.
    \textbf{(d-f)} Comparison of different groups of researchers after filtering and coordinating across multiple figures. 
    }
    % \label{fig:case-1}
\end{figure}

This case study demonstrates that LLM-native figures support iterative, provenance-rich exploration. 
Unlike conventional tools that require manual reconstruction or produce static outputs, our approach records each analytical step as a versioned, navigable artifact, enabling mixed-initiative analysis that existing systems do not provide.
% This case study demonstrates that LLM-native figures support iterative, provenance-rich exploration, enabling researchers to refine existing visualizations, generate contextually linked follow-up views, and revisit any point in the analytical trajectory. 
% Unlike conventional tools that require manual reconstruction of views or produce static figures with no provenance, our approach records each analytical step as a versioned, navigable artifact, supporting a form of mixed-initiative analysis that existing systems do not provide.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below: remove science-policy case for this round
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Dashun (2025-12-23): 
% % You have nice material there, but it’s partly TODO, and it opens up new interpretive risks. I’d just skip this. 
% % Keep only SciSci innovation as main case; remove policy results (not moving it to Supplement; this way we can save it for rebuttal).

% \textbf{\newlyadded{Science Use in Public Policy.}} 
% % \wyf{Dashun (2025-12-01): 
% % optionally fold the policy example into 1–2 paragraphs at the end, or move it to Supplement.
% % Either move it to Supplement as a “second SciSci vignette” or weave a 1–2 paragraph policy example into the SciSci case study section if you want to hint at breadth. 
% % }
% \newlyadded{
% Scientific evidence is widely regarded as a cornerstone of modern public policy, shaping legislative responses to complex societal challenges such as climate change, public health, and food security~\cite{furnas2025partisan, furnas2025partisanfunding}.
% At the same time, prior research has shown that the uptake, framing, and interpretation of scientific evidence can be systematically shaped by political context, particularly under conditions of sustained partisan polarization~\cite{mccarty2016polarized}.
% This raises a fundamental question at the intersection of science and governance: beyond differences in rhetoric or funding priorities, do policy-makers from different political parties also draw on systematically different bodies of scientific knowledge?
% }

% \newlyadded{
% To explore this question, the SciSci researcher begins by examining what kinds of science are cited in policy, before turning to how those patterns may diverge across parties.
% As an initial overview, the researcher selects policy documents from the U.S. House Energy and Commerce Committee, a central venue for legislation on health, energy, and agriculture, and asks:
% \textit{``Show me the distribution of all these policies’ cited papers based on paper title similarity.''}
% \systemname first filters the policy corpus by source and extracts the associated cited papers.
% To show the latent topical structure without imposing predefined categories, the system applies two analysis actions (\ie, \actionname{text_embedding} followed by \actionname{dimension_reduction}) and generates a scatterplot in which each point represents a cited paper positioned by semantic similarity (Fig.~\ref{fig:case-2-science-policy}).
% \wyf{TODO: color the plot by party affiliation using policy data from Zander’s dataset.}
% Having identified visually separable clusters, the researcher then seeks to ground these abstract regions in concrete scientific content.
% Using direct manipulation, the researcher circles distinct regions of the scatterplot and issue a follow-up request:
% \textit{``Give me a table showing the list of all these selected papers with attributes including paper title and DOI.''}
% In response, the system maps the visual selection back to the underlying database, filters the corresponding records, and returns a raw data table for inspection.
% Through this drill-down, the researcher finds two topical clusters (Fig.~\ref{fig:case-2-science-policy}): one centered on \textit{Nutrition and Agricultural Impacts}, and another focused on \textit{Infectious Disease Prevention and Response}.
% These clusters reflect substantively different dimensions of policy-relevant science, highlighting how health, food systems, and disease control co-exist within the committee's evidence base.
% \wyf{TODO: add discussions of different topic distribution of papers by two parties).}
% }

% \newlyadded{
% Together, this exploration suggests that science use in public policy is not monolithic but organized around distinct thematic regimes that can be explored through interactive, data-driven analysis.
% More importantly, the ability to align these topical structures with political attributes opens the door to systematically examining whether partisan divides extend beyond \textit{how} science is discussed to \textit{which science is mobilized} in the first place, which is an insight with direct implications for evidence-based governance and science–policy communication.
% }
% % Science has long been regarded as essential to policy-making, serving as one of the primary sources of evidence that informs decisions to tackle societal challenges such as climate change and public health~\cite{furnas2025partisan, furnas2025partisanfunding}. 
% % Yet, as the rising political polarization still exists~\cite{mccarty2016polarized}, the SciSci researcher is curisous about whether science use by policy-makers are also different in different parties. 
% % Thus, the researcher first select a policy source type from House Energy and Commerce Committee and take a look at the cited paper's topics as an overview: 
% % ``Show me the distribution of all these policies' (from House Energy and Commerce Committee) cited papers based on paper title similarity.'' 
% % \systemname firsts extract a list of paper by the filtering criteria and calls two analysis actions (\ie, \actionname{text_embedding} and \actionname{dimension_reduction}) as the similarity measures and finally generates a scatterplot of all the cited papers (Fig.~\ref{fig:case-2-science-policy}). 
% % \wyf{TODO: color the plot using the party label (to process the data from Zander's paper).}
% % Curious about the paper topics, the researcher circles different regions and asked ``Give me a table showing the list of all these selected papers with attributes including paper title and doi.''. 
% % The system respond by filtering the data and return the raw data tables. 
% % Two regions of topics are shown (Fig.~\ref{fig:case-2-science-policy}), one focusing on Nutrition and Agricultural Impacts and another focusing on Infectious Disease Prevention and Response. 
% % \wyf{TODO: add discussion of different topic distribution of papers by two parties).}
% % }

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/case2-science-policy.jpg}
%     \vspace{1pt}
%     \caption{\newlyadded{Case study: science use in policy-making. Left: a small cluster of papers on Nutrition and Agricultural Impacts; Right: a cluster of papers focused on Infectious Disease Prevention and Response.}}
%     \label{fig:case-2-science-policy}
% \end{figure}




\subsection{Computational Evaluation}
\label{subsection:computational-evaluation} 
To further assess the feasibility of LLM-native figures, we evaluate the fidelity of the bidirectional mapping mechanism (Sec.~\ref{subsection:conceptual-framework}), the core design for figures to function as reliable computational interfaces.
Specifically, we test whether: 
(1) user questions can be accurately transformed into visual data insights (\ie, Analytical operations → Visualization), and
(2) visual interactions, such as clicking or brushing on a figure, can be accurately mapped back to the intended subsets of underlying data and the appropriate analytical operations (\ie, Visualization → Analytical operations). 
%we evaluate whether \systemname reliably maps between user intent, analytical operations, and visual interaction, the core requirement for figures to function as machine-interpretable scientific artifacts. Specifically, we test whether 
%validate three core technical properties of \systemname. Specifically, we test whether (1) 
%the system can interpret user intent correctly and return relevant data, code, and visualization, while reliably mapping interactions on a visualization back to the underlying analytical state (Sec.~\ref{subsection:conceptual-framework}-Bidirectional Mapping), 
%(2) each figure contains sufficient provenance for exact reconstruction of the analysis (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), 
%and (3) the framework supports multi-step scientific analysis in realistic domains (Sec.~\ref{subsection:case-study}). 
%Together, these properties correspond directly to the framework's contributions and demonstrate that figures as function as machine-interpretable scientific artifacts.
We focus on this functional validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface implementation.
% We intentionally focus on artifact-level and system-level validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface design.

% \wyf{
% Low-level differences arise only when the original analysis involves non-deterministic operations, such as stochastic analytical operations.
% \textbf{Round-trip reproducibility.}
% In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
% Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% }

%\textbf{Mapping fidelity.} 
\textbf{Test Design}.  
We adopt a structured, coverage-oriented evaluation strategy that treats mapping fidelity as a functional correctness problem over a well-defined interaction space. 
Using the datasets from our case study, we construct a test suite of paired queries. Each test case includes an initial user question that requires the generation of a figure, and a follow-up question that depends on a specific visual interaction with that figure to produce a new or updated visualization. 
This design mirrors realistic usage patterns in which users alternate between language-based queries and direct manipulation.

To ensure systematic coverage and reduce evaluator bias, we use an LLM to generate  \wyf{308} valid test cases, each with three sub-tasks (Supplementary Notes 3.1). 
Test cases are diversified along three dimensions: 
(1) figure type (\eg, bar, line, pie, scatter plots, and tables),
(2) interaction type (\eg, single-mark selection, one-dimensional interval brushing, and two-dimensional brushing), 
and (3) analytical complexity, with tier 1 cases representing simple scenarios involving a single table and minimal transformation, and tier 2 cases reflecting realistic workflows that require joins across multiple tables, aggregations, or modeling operations.
% and (4) reference solution logic, which specifies the expected data subset, transformation steps, and analytical outcome for each case.
% Representative examples of the test cases are provided in the Supplementary Information (Supplementary Note~\ref{subsection:si-computational-evaluation}). 
% 
We evaluate mapping fidelity along both directions of the language–visualization loop using three metrics across all test cases.
\textit{Execution Success Rate} is the proportion of test cases in which the system successfully completes the end-to-end execution and returns a usable visualization artifact (i.e., no execution failure and a chart is generated).
\textit{Conditional Accuracy} (conditional on success) is the proportion of cases in which the generated analytical process and results are semantically and logically correct with respect to the user's intended analysis.
\textit{End-to-End Accuracy} is the proportion of cases in which the figures are both successfully generated and analytically correct. 

\textbf{Results.}
% 1. analysis -> vis
We first assess the mapping from analytical operations to visualization using the initial question in each test case. 
Given a user instruction, \systemname generates a sequence of actions to retrieve and analyze data and produce an interactive figure. 
We evaluate the correctness of the generated code (SQL, Python, and Vega-Lite), the retrieved data subset $D$, and the resulting figures through manual inspection by two authors and cross-validation with the generated LLM-based solution.
\systemname achieves an overall \textit{Execution Success Rate} of \wyf{$96.7\%$} and \textit{End-to-End Accuracy} of \wyf{$92.7\%$} (Fig.~\ref{fig:Figure4}-Initial Question). 
Most inaccurate cases stem from SQL generation errors, such as failures to perform fuzzy matching for user-specified concepts (\eg, querying “Computer Science” verbatim when the database stores ``computer science'') and misidentification of the analytical entity (\eg, returning counts of researchers instead of papers). 
% the accuracy of generating incorrect Vega-Lite is low, only one case mis-encode the y axis attribute. 
% Specifically, the accuracy of correctly generating data filtering and transformation queries (SQL), together with optional analytical code (Python), is \wyf{xx}. 
% Conditional on correct data retrieval, the accuracy of generating valid visualization specifications is \wyf{xx}. 
% Figure~\ref{??} further breaks down performance by visualization type, showing consistently high success rates across chart categories.
% \wyf{Add one sentence to discuss chart type variations.}
% 
% 
% 2. vis -> analysis (two methods: follow-up question-answering, coordination)
% Note: We only need to calc the accuracy of SQL step in 2nd figure generation, no need to calc vis generation step.

Second, we assess the mapping from visualization back to analytical operations using two approaches: follow-up question-answering and inter-figure coordination. 
% 2.1 follow-up question-answering
In the follow-up question-answering task, for each figure–interaction pair, \systemname maps selected visual marks to a data query via the relation $R_t$ and generates the corresponding analytical actions. 
We examine the results of the generated SQL query $C$ and the retrieved data subset $D$. 
% 
When users select visual marks or regions on the figure, the system correctly infers the corresponding data filtering and transformation logic with \wyf{$79.8\%$} \textit{End-to-End Accuracy} (Fig.~\ref{fig:Figure4}-Follow-up Question, SQL generation). 
% failure analysis
% Among the cases with inaccurate SQL generation, 
We observe that occasional inaccuracies arise when translating GUI interactions (\eg, brushing or clicking) into SQL filtering logic.  
For instance, a continuous x-axis brush with a range of $[a, b]$ may be incorrectly mapped to a discrete ``IN'' predicate rather than a ``BETWEEN'' range condition. 
This problem highlights the need for more explicit guidance, such as structured prompts or interaction-aware constraints, to ensure that GUI-derived filtering semantics are faithfully translated into SQL predicates in future LLM system designs. 
% 2.2 coordination update
For inter-figure coordination, when users select or brush an updated region of interest, the system updates the coordinated figure by modifying the underlying SQL query to retrieve the corresponding data. 
The resulting \textit{End-to-End Accuracy} is \wyf{$91.0\%$} (Fig.~\ref{fig:Figure4}–Coordination).
% Most inaccurate cases arise from errors in updating SQL filtering logic in response to new user interactions (\ie, brushing a new region on a figure), typically due to the introduction of unnecessary filtering conditions or incorrect substitution of the original query predicates. 
% The majority of inaccurate cases are typically due to introducing unnecessary filtering conditions or incorrectly substituting the original query predicates. 

% 3. round-trip reproducibility
%\textbf{Round-trip reproducibility.}
%Because all actions, code, and parameters used to generate a figure are explicitly recorded, each LLM-native figure artifact preserves complete analytical provenance. 
%This design, by nature, enables deterministic reconstruction of the original figure by re-executing its stored codes against the underlying data. 
% as all the actions and codes of generating a figure have been recorded, our LLM-native figure artifact by nature preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
%In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
%Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
%In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% including LLM-generated textual summaries and 
% High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mapping_fidelity.pdf}
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure4}
       \textbf{Computational evaluation results.}
    }
    % \label{fig:computational-evaluation}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below: old version (Round-Trip Reproducibility & User Study), temporally abandoned
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Round-Trip Reproducibility}
% \label{subsubsection:evaluation-reproducibility}
% \wyf{Note: test case: lack of LLM-based Python code.}
% We evaluate whether an LLM-native figure artifact preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
% This evaluation tests whether LLM-native figures function as reproducible computational objects rather than ephemeral presentation outputs.
% % To evaluate whether an LLM-native figure artifact provides complete provenance, enabling precise re-execution of the analytical workflow and deterministic reconstruction of the figure.

% \textbf{Test Design.} 
% We use the same set of 200 test cases described above and store all figures $F_t={V_t, D_t, C_t, M_t}$ generated succesfully during their execution. 
% For each figure, we re-execute the stored code $C_t$ against the original database to regenerate the data subset $D_g$ and the corresponding visualization $V_g$. 
% We then compare the original and reconstructed figures at two levels: (1) specification-level equivalence, assessed via structural comparison of the visualization specifications (JSON); 
% and (2) visual-level equivalence, assessed by matching visual marks, encodings, and positional attributes. 
% We report the proportion of figures that are exactly reproducible at the specification level and those that are visually identical despite potential non-semantic specification differences.

% \textbf{Results.} 
% % High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% \wyf{
% Across the \wyf{180} generated figures, round-trip reproducibility is achieved for nearly all figures. 
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% }.


% \subsubsection{Discussion}
% \newlyadded{
% Failure analysis (e.g., reproducibility-missing provenance, mismatched encodings, rendering differences). 
% Fill in with a short failure-mode paragraph: e.g., missing spec fields, nondeterministic defaults, or database changes. This will earn reviewer trust.
% \wyf{Erzhuo's suggestion: we also report failure cases with persentage and some examples.}
% }



% \subsection{User Study} 
% \textbf{Participants}: SciSci researchers from different "research age". 

% \textbf{Task}: three case studies, same setting of data. 

% \textbf{Benchmark}: Python/Jupyter Notebook, SciSciGPT. 

% \textbf{Evaluation dimensions}: 
% (1) Efficiency: time and accuracy. -- same analysis tasks in the case study. 
% (2) Expressiveness: number of insights generated. -- do not limit analysis tasks, only limit the high-level research question. To test: the number of insights generated; the diversity of insights generated. 

% \subsection{Expert Interview} 
% (1) Use \textit{Five-point Likert Scale} to allow users score different dimensions of the system: usability, etc. 

% (2) Qualitative evaluation: summarize their feedback in terms of hybrid user interface, LLM agent engine, and suggestions (especially for data-driven scientific discovery and LLM-native figures to be presented in their research paper -- open science related questions). 

==> sections/archive/03-2-evaluation/03-2-evaluation_v6_20260907.tex <==
\subsection{Case Study} 
\label{subsection:case-study} 

The climate example in Sec.~\ref{subsection:conceptual-framework} provides a simple illustration of the mechanics of our domain-independent conceptual framework. 
Here we demonstrate its utility through \systemname, an instantiation of the proposed framework developed for the science of science (SciSci) domain (Supplementary Note 2.2). 
SciSci provides an ideal testbed because it combines massive, heterogeneous datasets spanning grants, publications, and patents with complex research problems, such as tracing knowledge evolution, and high-stakes decision-making scenarios, such as strategic funding allocation.
Here, we present four case studies in SciSci, with a fifth in \todiscuss{Supplementary Note x.x}.
% an ideal testbed because relevant signals are distributed across heterogeneous linked datasets and exploratory questions evolve rapidly as new insights emerge
% The SciSci field~\cite{fortunato2018science, wang2021science} provides an ideal testbed: 
% large-scale heterogeneous data, spanning grants, publications, and patents with complex citation networks;
% complicated research problems, such as tracing knowledge evolution and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as strategic funding allocation and university innovation assessment.


\subsubsection{Innovation Landscape at Universities}
Understanding the innovation landscape of research has become a central challenge in the SciSci community, where researchers aim to map the dual frontiers of science and technology~\cite{ahmadpoor2017dual, liang2022systematic, yin2022public}, and among university leaders and science policymakers seeking to accelerate technology transfer and amplify research impact~\cite{wang2023innovationinsights, wang2025funding}. 
Yet uncovering untapped innovation potential remains challenging: Relevant signals are distributed across heterogeneous data sources, and exploratory questions evolve rapidly as new insights emerge. 
In this case, we use \systemname to explore innovation-related data from a leading U.S. research university.
% To illustrate how \systemname supports this dynamic analytical process, we conduct a case study using innovation-related data from a leading U.S. research university. 

% step 1: generation
A SciSci researcher first asks \systemname to explore the innovation landscape at the individual inventor level: 
\textit{``Show me the distribution of inventors based on their number of invention disclosures (as y axis) and number of papers cited by patents (as x axis).''} 
% \textit{``Show me the distribution of all inventors at this university in terms of their current patent activity and their hidden research potential relevant to technological use.''} 
Through the plan–action–execution loop, the system generates a sequence of atomic actions (\eg, \actionname{select_table} and \actionname{add_chart_type}), executes the associated code, and returns an interactive scatterplot showing the inventor distribution at this university (Fig.~\ref{fig:Figure3}a), with the y-axis encoding invention disclosures (a proxy for present-day innovation activity) and the x-axis encoding papers cited by patents (a proxy for technological potential). 


% step 2: modify chart
% 1. adjust scale (to log scale)
The researcher notices that most inventors cluster tightly in the lower-left region due to the heavy-tailed nature of both measures. 
This compression obscures meaningful structure and hinders the identification of high-potential individuals. 
Thus, the researcher selects the figure and requests: 
\textit{``Update the chart to use log scales on both axes. Customize the calculation to apply log(value + 1) so zero values are handled.''}
% \textit{``Update the chart to plot log-transformed x and y values, computed as log(value + 1) so that zero values are handled.''}
% \textit{``Update the chart to turn the x and y values into log scale. Use the formula: x = log(x + 1) to avoid zero.''} 
% \textit{``Help me adjust the values of the x and y axes to log scale to make the distribution clearer.''} 
Here, the system shifts from generation to manipulation (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance). 
The system takes the existing visualization and underlying data as inputs, infers the user's intent, triggers a new chain of actions to transform the data (\eg, \actionname{derive_column}) and update the visual encoding (\eg, \actionname{update_encoding}), and regenerates the scatterplot with log transformations applied to both axes, providing a clearer, more discriminative view of the inventor distribution (Fig.~\ref{fig:Figure3}b, c).
The overall distribution indicates a positive relationship between the two metrics, suggesting that patent-cited publications may serve as a useful indicator of a researcher's innovation activity.
Hover interactions expose precise values for each inventor, enabling accurate inspection of potential inventors and outliers (Fig.~\ref{fig:Figure3}b).
% 2. regression line
% based on log results, add regression: yifan: make sense!

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-1-innovationinsights-20260831.jpg}  % figures/20260409/case-ii.jpg
    \vspace{1pt}
    \caption{
    \bodyfigurelabel{fig:Figure3}
    \textbf{Case study: university innovation landscape.}
    \textbf{(a)} The figure generated for the first user query. 
    \textbf{(b)} The updated figure after adjusting the x- and y-axes to log scales. 
    \textbf{(c)} Screenshots of the streaming output when generating and updating a figure.
    \textbf{(d-e)} Comparison of different groups of researchers after filtering and coordinating across multiple figures. 
    \textbf{(f)} Screenshot of the data-driven artifact. 
    }
    % \label{fig:case-1}
\end{figure}


% step 3: extend chart: gender difference / other meta information (department) 
\wyf{
Within the overall distribution, the researcher quickly notices a small group of individuals with particularly high numbers of invention disclosures (Fig.~\ref{fig:Figure3}d, left scatter plot). 
% note: should refer to the brushed region at the bottom.
To examine this group, the researcher brushes the corresponding region through direct manipulation on the scatterplot and poses a follow-up query to drill down: 
\textit{``show me the department distribution using a bar chart.''}
The system uses both the natural-language request and the GUI-based selection as joint inputs, triggering a new sequence of atomic actions. 
It then generates a bar chart summarizing the departmental composition of the selected group (Fig.~\ref{fig:Figure3}d, left bar chart), enabling quick assessment of demographic patterns among these highly active inventors.
% insights
% 1. department
By brushing different regions on the scatterplot and comparing the department composition of this group against those with few or no invention disclosures (Fig.~\ref{fig:Figure3}d, right scatter plot), the researcher observes that faculty with frequent invention disclosures are disproportionately concentrated in fields such as chemistry and materials science, reflecting the uneven distribution of patenting activity across research areas within the university (Fig.~\ref{fig:Figure3}d, two bar charts).
}

\wyf{
The researcher also notices an interesting group in the bottom region of the scatter plot (Fig.~\ref{fig:Figure3}e, scatter plot): these faculty have no disclosed inventions, yet their publications are cited by patents. 
% the x-axis captures the number of publications cited by patents, a potential predictor of commercialization activities 
This subgroup represents researchers with significant untapped innovation potential: their work has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
Curious about the relationship between this untapped potential and their tenure status~\cite{tripodi2025tenure}, the researcher brushes these researchers and asks analogous queries for senior and junior faculty, \eg, \textit{``show the distribution of all senior faculty (tenure "Attained"), comparing those within this selected region of researchers against those who are not, using a pie chart.''} 
% \textit{``show the distribution of senior faculty (tenure "Attained") out of all senior faculty in the dataset by counting the number of faculty using a pie chart.''} 
% and \textit{``show the distribution of all junior faculty (Tenure Eligible), comparing those within this selected region of researchers against those who are not, using a pie chart.''}
% insights
Interestingly, nearly half of junior faculty fall within the selected region, compared to only about one-third of senior faculty (Fig.~\ref{fig:Figure3}e, two pie charts). 
% This indicates junior faculty are more likely than senior faculty to appear in the group of researchers whose work is cited by patents despite not engaging in invention activities.
% The researcher is very excited to find these new insights. 
This asymmetry points to a novel discovery.
Junior faculty, whose career advancement depends primarily on publications and grants, have strong incentives to prioritize academic output over other impacts such as direct engagement with patenting, yet their research is nonetheless absorbed by the technology sector, as evidenced by patent citations. 
Senior faculty, by contrast, are more likely to have established the industry collaborations and institutional networks that facilitate direct participation in invention disclosure and technology transfer.
The observed divergence suggests that a substantial reservoir of commercially relevant knowledge produced by junior faculty remains unrealized by the formal technology transfer pipeline, highlighting a structural gap between academic incentive systems and innovation outcomes that merits systematic investigation.
% Junior faculty, whose career advancement depends primarily on publications and grants~\cite{sanberg2014changing}, have strong academic incentives to prioritize academic output over other impacts such as direct engagement with the patenting process, though their research nonetheless generates knowledge that is absorbed downstream by the technology sector, as evidenced by patent citations to their publications. 
% Senior faculty, by contrast, are more likely to have established industry collaborations, laboratory infrastructure, and institutional networks that facilitate direct participation in invention disclosure and technology transfer. 
}
% This asymmetry suggests a difference in roles along the science–technology pipeline: the academic incentives for junior faculty focus more on research publications, whereas senior faculty are more likely to participate directly in invention processes through patenting activities.
% This explorative exploration help the researcher find new initial insights about the relationship between tenure status and innovation potentials and worth for a deeper dive for systematic analysis. 


% It then generates a bar chart summarizing the gender distribution and a pie chart showing the departmental composition of the selected group (Fig.~\ref{fig:Figure3}d), enabling quick assessment of demographic patterns among these faculty. 
% By comparing the gender distributions of different subgroups, the researcher observes a clear disparity between faculty with higher numbers of invention disclosures (Fig.~\ref{fig:Figure3}d) and those with few or none (Fig.~\ref{fig:Figure3}e): 
% male faculty members appear more likely to have disclosed inventions than their female counterparts (Fig.~\ref{fig:Figure3}d, e, two bar charts), and faculty with frequent invention disclosures are disproportionately concentrated in fields such as biomedical engineering, chemistry, and materials science, reflecting the uneven distribution of patenting activity across research areas within the university (Fig.~\ref{fig:Figure3}d, e, two pie charts). 

% A contrasting pattern emerges when the distribution is examined along the x-axis, which captures the number of publications cited by patents, a potential predictor of commercialization activities (Fig.~\ref{fig:Figure3}f). 
% Unlike the y-axis comparison, where faculty with high numbers of disclosed inventions are all male, researchers with high x-axis values comprise both male and female faculty. 
% Notably, in the bottom-right region of the scatterplot (Fig.~\ref{fig:Figure3}f), where researchers have no disclosed inventions yet their publications are heavily cited by patents, the proportion of female faculty is substantial. 
% This subgroup represents researchers with significant untapped innovation potential: their research has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
% Taken together, these patterns suggest a gendered asymmetry between realized and unrealized innovation, where male researchers are more likely to have already converted research into inventions, while many female researchers exhibit comparable innovation potential that remains untapped.


% step 4: 
% 4.1 tracable with code (SQL, Python), data, and vis code
% 4.2 save artifact for future exploration (there are other universities' data comming in). 
To ensure analytical rigor, the researcher downloads the underlying data, generated code, and visualization outputs from each figure to verify the procedure and results. 
The entire chat session, including the data-driven artifact (Fig.~\ref{fig:Figure3}f), is also saved for future analysis, enabling replication and facilitating cross-institutional comparisons as additional university datasets become available. 

This case study illustrates how LLM-native figures support iterative, provenance-rich exploration. 
Unlike conventional tools that require manual reconstruction or produce static outputs, our approach records each analytical step as a versioned, navigable artifact, enabling mixed-initiative analysis that existing systems do not provide.
% This case study demonstrates that LLM-native figures support iterative, provenance-rich exploration, enabling researchers to refine existing visualizations, generate contextually linked follow-up views, and revisit any point in the analytical trajectory. 
% Unlike conventional tools that require manual reconstruction of views or produce static figures with no provenance, our approach records each analytical step as a versioned, navigable artifact, supporting a form of mixed-initiative analysis that existing systems do not provide.



\subsubsection{\newlyadded{Use of Science in Public Policy}}

\newlyadded{
Scientific evidence is widely regarded as a cornerstone of public policy, shaping legislative responses to complex societal challenges such as climate change and public health~\cite{furnas2025partisan, furnas2025partisanfunding}.
Prior research has shown that the uptake, framing, and interpretation of scientific evidence can be systematically shaped by the political context, particularly under conditions of sustained partisan polarization~\cite{mccarty2016polarized}.
This raises a fundamental question at the intersection of science and governance: do policymakers from different political parties draw on systematically different bodies of scientific knowledge?
}

% 1. overview scatterplot
\newlyadded{
To explore this question, the SciSci researcher uses Nexus to select the science policy dataset \todiscuss{(Supplementary Note x.x)} and uses the data to determine the kinds of science that are used in policy. 
% before turning to how those patterns may diverge across parties.
To see an initial overview, the researcher selects policy documents from the U.S. House Energy and Commerce Committee, a central venue for legislation on health and energy, and instructs:
\textit{``Show a scatterplot of all the papers cited by the House Energy \& Commerce Committee policies (committee short name is "hsif00"), where each point is one unique paper title and doi and is positioned by its title text embedding.''} 
% \textit{``Show me the distribution of all these policies’ cited papers based on paper title similarity.''}
\systemname first filters the policy corpus by source committee and extracts the cited papers, along with their titles.
% To show the latent topical structure without imposing predefined categories, 
Next, the system applies two complex analysis actions (\actionname{text_embedding} followed by \actionname{dimension_reduction}) and generates a scatterplot in which each point represents a cited paper positioned by semantic similarity.
The figure shows clear topic clusters based on the paper's visual distribution (Fig.~\ref{fig:Figure4}a). 
}

% 2. update scatterplot: highlight by color. 
\newlyadded{Interested in the differences between paper topics cited by Democrats and Republicans, the researcher asks: 
\textit{``Assign a dark blue color to a paper point if at least one House Energy \& Commerce Committee policy (committee short name is "hsif00") citing that paper was written under Democratic party control; otherwise, color it light grey. Reuse the existing scatterplot layout, and keep each paper's coordinates and the axis limits unchanged.''}
The system then takes the generated figure and the underlying data as input to query the original database, adding each paper-policy citation pair with a new attribute about party control. It updates the data in the figure as well as the visual encoding, and it returns an updated scatterplot with papers that are cited by policies that were written under Democratic control highlighted in blue (Fig.~\ref{fig:Figure4}b). 
}

% 3. extend chart generation and coordination
\newlyadded{
% 1. generation
Having identified visually distinct clusters, the researcher then seeks to understand the scientific content represented by each region. The researcher circles a cluster on the scatterplot and issues a follow-up request to summarize the paper topics: \textit{``Looking at the selected region, generate a topic label based on titles of papers cited by policies written under Democratic party control.''} The researcher also asks the system to list five of these papers to confirm the accuracy of the topic label: \textit{``Looking at the selected region and  papers cited by policies written under Democratic party control, provide a raw data table with each paper's title and doi. Return the first five paper records.''} 
The system queries the database for the papers in the circled region, retrieves their titles, and calls the LLM to determine the region's topic. It then returns a sample of the papers' metadata so that the researcher can cross-validate the inferred label.
% 2. coordination
The researcher then brushes several other visual clusters and records the representative topics: \textit{e-cigarette health effects, marketing, and regulation} (Fig.~\ref{fig:Figure4}c) and \textit{alcohol-impaired driving prevention and traffic safety} (Fig.~\ref{fig:Figure4}e). 
}

% 4. fork analysis
\newlyadded{
The researcher next turns to papers produced under  Republican control. Selecting the existing Democratic artifact, the researcher requests:
\textit{``Repeat the same analysis and artifact for the other party---this time using policies and papers associated with Republican control.''}
% \textit{``Apply the same analysis and artifact to another party's associated policies and papers: Republican control, party_control = 'R'''.}
The analysis  is nearly identical, with minor adjustments to the data query and visualization representation. 
The system forks the same artifact, including its underlying code, data, and figure, and then determines the analysis and visualization information to be updated: it queries the other party's papers, updates the visualization with the new set of papers, and changes the color to a party-appropriate shade using the LLM's world knowledge. It also updates the figure title and description. 
The forked artifact for the Republican case then appears in the session. 
Following the same procedure, the researcher identifies representative topics such as \textit{high school sports injuries and safety} (Fig.~\ref{fig:Figure4}d). 
}
% \todiscuss{TODO: add discussions of different topic distribution of papers by two parties).}

\todiscuss{
This case suggests that Democrats and Republicans draw on distinct bodies of
scientific research in policy-making. The pattern emerged through the complementary interaction modes in \systemname: direct graphical selection captured visually emergent topic clusters that natural language cannot describe precisely, and artifact forking replicated the entire pipeline for the other party from a single instruction.
Partisan divides may thus extend beyond \textit{how} science is discussed to \textit{which} science informs policy in the first place, with direct implications for evidence-based governance.
}
% Having identified visually separable clusters, the researcher then seeks to ground these abstract regions in concrete scientific content.
% Using direct manipulation, the researcher circles distinct regions of the scatterplot and issue a follow-up request:
% \textit{``Give me a table showing the list of all these selected papers with attributes including paper title and DOI.''}
% In response, the system maps the visual selection back to the underlying database, filters the corresponding records, and returns a raw data table for inspection.
% Through this drill-down, the researcher finds two topical clusters (Fig.~\ref{fig:case-2-science-policy}): one centered on \textit{Nutrition and Agricultural Impacts}, and another focused on \textit{Infectious Disease Prevention and Response}.
% These clusters reflect substantively different dimensions of policy-relevant science, highlighting how health, food systems, and disease control co-exist within the committee's evidence base.
% \wyf{TODO: add discussions of different topic distribution of papers by two parties).}
% }

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-2-science-policy-20260831.jpg}
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure4}
        \newlyadded{\textbf{Case study: science use in public policy.} 
            \textbf{(a)} The scatterplot generated for the initial query, showing all papers cited by policy documents.
            \textbf{(b)} An in-place manipulation of the same figure highlighting papers cited by Democratic-associated policy documents.
            \textbf{(c)} An extension of the artifact: the user brushes a region of interest, and the system generates a coordinated figure summarizing the topic label of the selected paper cluster.
            \textbf{(d)} The artifact forked from Democratic- to Republican-associated papers, re-executing the identical analytical chain on a new data scope and revealing markedly different paper topic distributions across the two parties.
            \textbf{(e)} Coordination in action: changing the graphical selection region propagates to the linked topic summary, while the underlying data table remains accessible for cross-validating the generated labels.
        }
    }
    % \label{fig:case-2-science-policy}
\end{figure}



\subsubsection{\newlyadded{The Impact of Science Funding}}
% note: no coordination reflected
\newlyadded{
Understanding the impact of science funding is critical to ensuring that research investments align with societal needs~\cite{bush2021science, yin2022public, wang2025funding}, a question of immense interest to funding agencies, national policymakers, and university leaders who allocate scarce resources across a complex research landscape. 
While emerging datasets now link grants to downstream outcomes well beyond publications, including patents, clinical trials, policy documents, and news coverage~\cite{yin2022public, wang2025funding, furnas2025partisan}, assessing this broad impact remains challenging: the evidence is scattered across heterogeneous databases, and portfolio-level questions about where funding goes naturally cascade into questions about who receives it and what impact it generates. 
In this case, we use \systemname and a science funding dataset \todiscuss{(Supplementary Note x.x)} to examine the funding portfolio of the National Institute on Aging (NIA), tracing an analytical chain from allocation to representation to impact.
}

\newlyadded{
A SciSci researcher begins by asking \systemname for a portfolio overview: 
\textit{``For grants awarded by the National Institute on Aging, show the total funding amount by Level 0 research field, sorted from highest to lowest.''} 
% Through the plan–action–execution loop, 
The system searches for the funder, filters grants to those awarded by the NIA, joins each grant to its field classification, and aggregates funding by field, returning a ranked bar chart that spans multiple top-level research fields (Fig.~\ref{fig:Figure5}a, c). 
The portfolio is dominated by the four top-funded grant fields: \textit{biological sciences}, \textit{health sciences}, \textit{biomedical and clinical sciences}, and \textit{psychology}.
}

\newlyadded{Struck by this concentration, the researcher turns from the funding to the recipients, asking who leads the research these grants support. 
The researcher brushes the bars for the three top-funded fields using direct manipulation (Fig.~\ref{fig:Figure5}a) and poses a follow-up query: 
\textit{``Compare the gender shares of principal investigators within these selected fields using a grouped bar chart, and include an additional ``Overall" group showing the gender share across all fields.''} 
Taking the brushed region and the natural-language request as joint inputs, the system maps the selected bars back to their field conditions and inherits the NIA scope from the parent figure, so that every downstream comparison remains within the same portfolio. It then computes the share of distinct principal investigators (PIs) by gender within each field and constructs the requested ``Overall" baseline across all NIA grants.
% , a comparison group absent from the visual selection itself. 
The resulting grouped bar chart (Fig.~\ref{fig:Figure5}b) reveals a consistent imbalance: male PIs outnumber female PIs in every top-funded field, with the disparity in \textit{biological sciences} and \textit{biomedical and clinical sciences} exceeding the overall gap.
}

\newlyadded{Representation, however, is only part of the story. The researcher next asks if grants led by female PIs differ in impact.  
The researcher selects the single bar representing \textit{biomedical and clinical sciences} and issues a computationally precise request: 
\textit{``For this selected field, use a radar chart to compare male and female PIs' average grant-level impact. Use the precomputed impact metrics (number of publications, patents, clinical trials, and citations from policy documents, news, patents, and clinical trials). Average each metric over PI-grant records within each gender, then normalize each dimension by the maximum across the two genders.''} 
The system translates this specification into the corresponding aggregation pipeline: 
it averages the seven precomputed impact measures over PI–grant records within each gender, applies the normalization, and renders an overlaid radar chart (Fig.~\ref{fig:Figure5}d). 
% The two impact profiles are comparable in overall shape but differ in composition. 
% Average publication counts are nearly identical, and grants led by male PIs score higher on patent-oriented dimensions (patents produced and citations from patents) and on clinical trials conducted, whereas grants led by female PIs attract more citations from clinical trials, policy documents (17.0 vs. 12.6 per PI–grant record), and news media. 
Female PIs are underrepresented in this heavily funded field, yet their grants perform at least as well on many of the impact measures examined here: average publication output is nearly identical, and grants led by female PIs record higher average citations from policy documents, news media, and clinical trials---a pattern the researcher had not anticipated and that prior analyses had not surfaced.
% echoing patterns surfaced by dedicated funding-impact analyses~\cite{wang2025funding}.
}


\todiscuss{
Though descriptive, this asymmetry between representation and realized impact bears directly on evidence-based funding allocation and merits systematic investigation--for example, controlling for career stage, funding scale, and team composition.
Notably, conventional gender-gap analyses, which center on publications, citations, and funding amounts~\cite{lariviere2013bibliometrics,huang2020historical,oliveira2019comparison}, would not surface this pattern. It becomes visible only when grants are connected to their downstream societal uses through newly available data linkages~\cite{yin2022public, wang2025funding}. \systemname distilled these complex raw tables \todiscuss{(Supplementary Note x.x)} into a concrete visual finding within a handful of intuitive and efficient interactions.
% This case study illustrates how our tool compresses a multi-stage funding-impact analysis---one that traditionally requires purpose-built visual analytics systems~\cite{wang2025funding} or ad hoc scripting---into a chain of three linked figures driven by natural language and direct manipulation. 
% 
% Each interaction progressively narrows the analytical scope, from an agency's portfolio, to the demographic composition of its top-funded fields, to gender-specific impact profiles within a single field, while provenance guarantees that every comparison remains anchored to the same underlying funding portfolio.
}

% \textbf{Draft figure caption. }Figure X: Case study: the impact of science funding. (a) The ranked bar chart was generated for the initial query, showing total NIA funding across 22 Level 0 research fields. (b) After the user brushes the three top-funded fields, the grouped bar chart compares gender shares of distinct PIs within each selected field, alongside an Overall baseline computed across all fields. (c) After the user selects the bar for Biomedical and Clinical Sciences, the radar chart compares male and female PIs' average grant-level impact across seven normalized dimensions (publications, patents, clinical trials, and citations from policy documents, news, patents, and clinical trials).


\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-3-and-4-funding-impact-and-disruption-20260831.jpg}  
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure5}
        \newlyadded{
            \textbf{Case studies.}
            \textbf{(a-d) The impact of science funding.} 
            Starting from the distribution of grant funding across research fields \textbf{(a, c)}, the researcher compares the gender composition of principal investigators (PIs) within the brushed fields \textbf{(b)}, then zooms into a single field to contrast the multi-dimensional impact of male- and female-led grants in a radar chart \textbf{(d)}.
            Color encodings are designed to be semantically aligned across all figures within the same data-driven artifact.
            \textbf{(e-i) Disruptive science across fields and nations.}
            Beginning from a replication of a known macro-level pattern~\cite{park2023papers} \textbf{(e, f)}, new insights emerge as the analysis is drilled down to the relative ranking of disruption scores across countries \textbf{(g-i)}.
        }
    }
    % \label{fig:case-1}
\end{figure}






\subsubsection{\newlyadded{Disruptive Science across Fields and Nations}}
% \subsubsection{\newlyadded{Science Impact Across Fields and Nations}}

\newlyadded{
Whether science is losing its capacity to disrupt has been a central concern for the SciSci community, fueling debates about slowing scientific progress despite the exponential growth of the literature~\cite{jones2009burden, park2023papers, wu2019large}. 
In this case, we use \systemname and the SciSciNet~\cite{lin2023sciscinet} dataset in a reproduce-then-extend exploration: it first replicates established macro-level findings, then carries the same analytical chain into largely unexamined dimensions, where new insights emerge.
% In this case, we first use \systemname to reproduce existing macro-level patterns and then to interrogate the heterogeneity beneath them.
}  

\newlyadded{A SciSci researcher starts the exploration with an aggregate view: 
\textit{``Show the average disruption score of papers by publication year from 1950 to 2015.''} 
The system aggregates paper-level disruption scores by publication year and returns a line chart (Fig.~\ref{fig:Figure5}e), which shows that the average disruption declines persistently across the entire period. 
% The system aggregates paper-level disruption scores by publication year and returns a line chart (Fig. Ya) that reproduces the canonical finding: average disruption declines persistently across the entire period~\cite{park2023papers}. 
The researcher then drills down into the analysis: 
\textit{``Split this line into multiple lines to compare the top five research fields (Level 0) with the most papers.''} 
The system shifts from figure generation to manipulation: it identifies the five fields with the largest paper volumes, augments the existing aggregation with a field grouping, and updates the visual encoding in the figure, transforming the single trend into five field-level trajectories (Fig.~\ref{fig:Figure5}f). 
All five fields decline in concert, though not uniformly: physics and chemistry, initially the most disruptive, fall steepest, while computer science declines most gently, moving from last to near the top.
% The updated figure shows that the decline is pervasive—every major field trends downward—but far from uniform: physics and chemistry, the most disruptive fields at mid-century with average scores more than double that of computer science, fall steeply, whereas computer science starts lowest yet declines most gently, ending the period among the most disruptive fields on a per-paper basis.
}

\newlyadded{The field-level heterogeneity, like the aggregate decline, replicates patterns documented in prior work~\cite{park2023papers}. 
Nations, by contrast, are an axis this literature leaves largely unexamined. 
Thus, the researcher moves from replication to new analysis, selecting the line representing \textit{Medicine} and posing a computationally precise follow-up: 
% This heterogeneity raises a sharper question: 
% within a field, is the geography of disruptive research stable? 
% The researcher selects the line representing computer science and poses a computationally precise follow-up: 
\textit{``For the selected field, from 2000 to 2015, compare countries by average disruption score, counting each paper once per country (deduplicate multiple authors from the same country). Then among the 20 countries with the most papers in the selected field over this period, rank the countries within each year by average disruption score (rank 1 means the highest; ranks range from 1 to 20 within the 20-country pool). Show the annual rank trajectories of only the five countries with the most papers, as a multi-line chart.''}
% 
The system executes the corresponding multi-step analysis (\eg, restricting the pool to the twenty largest producers, computing within-year ranks, and displaying the five highest-volume countries) and returns a rank-trajectory chart (Fig.~\ref{fig:Figure5}g). 
% (\eg, deduplicating authorship so that each paper counts once per country, restricting the pool to the twenty largest producers, computing within-year ranks, and displaying the five highest-volume countries) 
The result shows that national standings in this field evolve only gradually: the five largest paper producers remain in the upper half of the twenty-country pool throughout, with the United States and China drifting slowly upward and the United Kingdom and Japan slowly downward---movements that unfold over the past decade.
% decade-long movements with no abrupt reordering of the hierarchy
% coordination 
Selecting other field lines and re-issuing the same request re-executes the identical pipeline with only the field condition changed, and \textit{Computer Science} tells a
strikingly different story (Fig.~\ref{fig:Figure5}h, i): 
China, near the bottom of the twenty-country pool in the early-to-mid 2000s, vaults into the top ranks around 2008–2011 and remains there through 2015, while several incumbent leaders drift downward.
}

% conclusion
\todiscuss{
These trajectories suggest that beneath the universal decline in average disruptiveness lies an actively shifting national landscape, and that its dynamics are field-specific.
% : abrupt ascents, as in China's rise in computer science during a period of rapid national expansion of computing research, coexist with gradual, sustained climbs, as in the United States in biology and chemistry. 
% Because the ranking conditions on the largest producers and counts each paper once per country, these shifts reflect changes in the average disruptiveness of national research output rather than sheer publication volume—precisely the kind of compositional dynamics that aggregate indicators conceal [Park et al. 2023].
% As in the previous cases, every derived statistic remains auditable: expanding each figure's reasoning process exposes the deduplication, pooling, and ranking steps as executable operations, and the full chain—from the reproduced global trend to the national rank trajectories—is preserved as a data-driven artifact that can be re-executed for any field, period, or country pool. 
This case study thus illustrates a reproduce-then-extend mode of exploration that LLM-native figures make natural: a published macro-level pattern is first re-established as a verifiable starting point and then progressively decomposed, by field and then by nation, through figure extension and user interactions. 
As concerns about slowing disruptive science mount, the capacity to monitor not only whether disruption is declining but also where and for whom it is rising or eroding speaks directly to science policy debates on research portfolios and national competitiveness.
}

% \textbf{Draft figure caption.} Figure Y: Case study: disruptive science across fields and nations. (a) The line chart generated for the initial query, showing the average disruption score of papers by publication year (1950–2015) and reproducing the aggregate decline reported in prior work. (b) The same figure after an in-place edit that splits the trend by the five research fields with the most papers, revealing pervasive but heterogeneous declines. (c) After the user selects the computer-science line, the follow-up figure ranks the twenty largest producing countries by average per-paper disruption within each year (2000–2015; rank 1 = highest, y-axis inverted) and displays the five highest-volume countries, revealing China's abrupt ascent into the top ranks around 2008–2011.







\subsection{Computational Evaluation}
\label{subsection:computational-evaluation} 
To further assess the feasibility of LLM-native figures, we evaluate the fidelity of the bidirectional mapping mechanism (Sec.~\ref{subsection:conceptual-framework}), the core design for figures to function as reliable computational interfaces.
Specifically, we test whether: 
(1) user questions can be accurately transformed into visual data insights (\ie, Analytical operations → Visualization), and
(2) visual interactions, such as clicking or brushing on a figure, can be accurately mapped back to the intended subsets of underlying data and the appropriate analytical operations (\ie, Visualization → Analytical operations). 
%we evaluate whether \systemname reliably maps between user intent, analytical operations, and visual interaction, the core requirement for figures to function as machine-interpretable scientific artifacts. Specifically, we test whether 
%validate three core technical properties of \systemname. Specifically, we test whether (1) 
%the system can interpret user intent correctly and return relevant data, code, and visualization, while reliably mapping interactions on a visualization back to the underlying analytical state (Sec.~\ref{subsection:conceptual-framework}-Bidirectional Mapping), 
%(2) each figure contains sufficient provenance for exact reconstruction of the analysis (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), 
%and (3) the framework supports multi-step scientific analysis in realistic domains (Sec.~\ref{subsection:case-study}). 
%Together, these properties correspond directly to the framework's contributions and demonstrate that figures as function as machine-interpretable scientific artifacts.
We focus on this functional validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface implementation.
% We intentionally focus on artifact-level and system-level validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface design.

% \wyf{
% Low-level differences arise only when the original analysis involves non-deterministic operations, such as stochastic analytical operations.
% \textbf{Round-trip reproducibility.}
% In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
% Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% }

%\textbf{Mapping fidelity.} 
\textbf{Test Design}.  
We adopt a structured, coverage-oriented evaluation strategy that treats mapping fidelity as a functional correctness problem over a well-defined interaction space. 
Using the datasets from our case study, we construct a test suite of paired queries. Each test case includes an initial user question that requires the generation of a figure, and a follow-up question that depends on a specific visual interaction with that figure to produce a new or updated visualization. 
This design mirrors realistic usage patterns in which users alternate between language-based queries and direct manipulation.

To ensure systematic coverage and reduce evaluator bias, we use an LLM to generate  \wyf{308} valid test cases, each with three sub-tasks (Supplementary Note 3.1). 
Test cases are diversified along three dimensions: 
(1) figure type (\eg, bar, line, pie, scatter plots, and tables),
(2) interaction type (\eg, single-mark selection, one-dimensional interval brushing, and two-dimensional brushing), 
and (3) analytical complexity, with tier 1 cases representing simple scenarios involving a single table and minimal transformation, and tier 2 cases reflecting realistic workflows that require joins across multiple tables, aggregations, or modeling operations.
% and (4) reference solution logic, which specifies the expected data subset, transformation steps, and analytical outcome for each case.
% Representative examples of the test cases are provided in the Supplementary Information (Supplementary Note~\ref{subsection:si-computational-evaluation}). 
% 
We evaluate mapping fidelity along both directions of the language–visualization loop using three metrics across all test cases.
\textit{Execution Success Rate} is the proportion of test cases in which the system successfully completes the end-to-end execution and returns a usable visualization artifact (i.e., no execution failure and a chart is generated).
\textit{Conditional Accuracy} (conditional on success) is the proportion of cases in which the generated analytical process and results are semantically and logically correct with respect to the user's intended analysis.
\textit{End-to-End Accuracy} is the proportion of cases in which the figures are both successfully generated and analytically correct. 

\textbf{Results.}
% 1. analysis -> vis
We first assess the mapping from analytical operations to visualization using the initial question in each test case. 
Given a user instruction, \systemname generates a sequence of actions to retrieve and analyze data and produce an interactive figure. 
We evaluate the correctness of the generated code (SQL, Python, and Vega-Lite), the retrieved data subset $D$, and the resulting figures through manual inspection by two authors and cross-validation with the generated LLM-based solution (Supplementary Note 3.2).
\systemname achieves an overall \textit{Execution Success Rate} of \wyf{$96.7\%$} and \textit{End-to-End Accuracy} of \wyf{$92.7\%$} (Fig.~\ref{fig:Figure6}-Initial Question). 
Most inaccurate cases stem from SQL generation errors, such as failures to perform fuzzy matching for user-specified concepts (\eg, querying “Computer Science” verbatim when the database stores ``computer science'') and misidentification of the analytical entity (\eg, returning counts of researchers instead of papers). 
% the accuracy of generating incorrect Vega-Lite is low, only one case mis-encode the y axis attribute. 
% Specifically, the accuracy of correctly generating data filtering and transformation queries (SQL), together with optional analytical code (Python), is \wyf{xx}. 
% Conditional on correct data retrieval, the accuracy of generating valid visualization specifications is \wyf{xx}. 
% Figure~\ref{??} further breaks down performance by visualization type, showing consistently high success rates across chart categories.
% \wyf{Add one sentence to discuss chart type variations.}
% 
% 
% 2. vis -> analysis (two methods: follow-up question-answering, coordination)
% Note: We only need to calc the accuracy of SQL step in 2nd figure generation, no need to calc vis generation step.

Second, we assess the mapping from visualization back to analytical operations using two approaches: follow-up question-answering and inter-figure coordination. 
% 2.1 follow-up question-answering
In the follow-up question-answering task, for each figure–interaction pair, \systemname maps selected visual marks to a data query via the relation $R_t$ and generates the corresponding analytical actions. 
We examine the results of the generated SQL query $C$ and the retrieved data subset $D$. 
% 
When users select visual marks or regions on the figure, the system correctly infers the corresponding data filtering and transformation logic with \wyf{$79.8\%$} \textit{End-to-End Accuracy} (Fig.~\ref{fig:Figure6}-Follow-up Question, SQL generation). 
% failure analysis
% Among the cases with inaccurate SQL generation, 
We observe that occasional inaccuracies arise when translating GUI interactions (\eg, brushing or clicking) into SQL filtering logic.  
For instance, a continuous x-axis brush with a range of $[a, b]$ may be incorrectly mapped to a discrete ``IN'' predicate rather than a ``BETWEEN'' range condition. 
This problem highlights the need for more explicit guidance, such as structured prompts or interaction-aware constraints, to ensure that GUI-derived filtering semantics are faithfully translated into SQL predicates in future LLM system designs. 
% 2.2 coordination update
For inter-figure coordination, when users select or brush an updated region of interest, the system updates the coordinated figure by modifying the underlying SQL query to retrieve the corresponding data. 
The resulting \textit{End-to-End Accuracy} is \wyf{$91.0\%$} (Fig.~\ref{fig:Figure6}–Coordination).
% Most inaccurate cases arise from errors in updating SQL filtering logic in response to new user interactions (\ie, brushing a new region on a figure), typically due to the introduction of unnecessary filtering conditions or incorrect substitution of the original query predicates. 
% The majority of inaccurate cases are typically due to introducing unnecessary filtering conditions or incorrectly substituting the original query predicates. 

% 3. round-trip reproducibility
%\textbf{Round-trip reproducibility.}
%Because all actions, code, and parameters used to generate a figure are explicitly recorded, each LLM-native figure artifact preserves complete analytical provenance. 
%This design, by nature, enables deterministic reconstruction of the original figure by re-executing its stored codes against the underlying data. 
% as all the actions and codes of generating a figure have been recorded, our LLM-native figure artifact by nature preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
%In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
%Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
%In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% including LLM-generated textual summaries and 
% High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mapping_fidelity.pdf}
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure6}
       \textbf{Computational evaluation results.}
    }
    % \label{fig:computational-evaluation}
\end{figure}




\subsection{\newlyadded{User Study}}
\label{subsection:user-study} 

\newlyadded{To assess the usefulness and potential benefits of LLM-native figures and data-driven artifacts for researchers, we conducted a within-subject user study with SciSci researchers using \systemname, our instantiation of the design. 
The study complements the computational evaluation in Sec.~\ref{subsection:computational-evaluation}, which established the fidelity of the bidirectional mapping, with evidence on how researchers actually perform exploratory analysis with the system. 
We compared \systemname against a baseline that mirrors participants' everyday workflow on two exploratory data analysis tasks adapted from the case studies introduced before, \todiscuss{measuring task success, completion time, workload, usability, and perceived value}, and we collected qualitative feedback on how the design changes the role of figures in the scientific discovery process. 
}


\subsubsection{\newlyadded{Participants and Study Procedure}}
\label{subsection:participants-and-study-procedure} 

\newlyadded{\textbf{Participants.} 
We invited 12 SciSci researchers (P1–P12; 5 female, 7 males; aged 24--45, $M = 31.3$) through professional networks. 
Participants spanned career stages: 2 predoctoral researchers, 3 PhD students (third year or later), 5 postdoctoral researchers, and 2 research assistant professors, with 3-10 years of experience in quantitative data analysis. 
All participants routinely analyze large-scale SciSci data and reported prior experience with LLM-based coding assistants (\eg, Claude Code~\cite{claudecode} and Codex~\cite{codex}) for code generation and for creating and editing visualizations. 
None of the participants was involved in the development of \systemname or had used it before the study. 
% Detailed demographic information is provided in \todiscuss{Supplementary Table xx}.
}

\newlyadded{\textbf{Baseline.}
The baseline system is a computational server with settings identical to those of \systemname (the same server, coding environment, and database access). 
Researchers were free to use their conventional tools (e.g., VS Code and Jupyter notebooks) and programming languages (e.g., Python and R) to mimic their daily data analysis workflow, and could use LLM assistance through Claude Code~\cite{claudecode}. 
We asked participants to use the Claude Sonnet 4.5 model in the baseline, the same model that powers \systemname, so that differences between the two conditions reflect our design rather than the capability of the underlying model.
}

\newlyadded{\textbf{Study Procedure.} 
Each study session was conducted remotely via Zoom with screen sharing and lasted about two hours. 
Participants first completed the consent form and the demographics questionnaire. 
We then introduced the project background and provided a 15-minute tutorial on \systemname using the Climate Change example from Sec.~\ref{subsection:conceptual-framework}.
Researchers could ask questions throughout to confirm their understanding. 
We also helped them set up the baseline environment and gave them time to configure it to match their usual data analysis workflow.
% 
% 
Next, researchers were asked to reproduce two data exploration tasks adapted from the case studies in Sec.~\ref{subsection:case-study}. 
Each task was decomposed into multiple steps that were delivered one at a time~\cite{xx, xx}: an initial question that generates a figure, two follow-up questions conditioned on a subset of the previous figure, and a coordination step that re-applies the analysis to a different selection. 
For each task, we provided natural-language data analysis requirements, reference chart types, and the data schema and descriptions of the underlying database. 
Each participant completed the two tasks, one using \systemname and the other using the baseline. 
To fully counterbalance the assignment of tasks to conditions and the order of conditions, we generated all four combinations (e.g., Task 1 with \systemname followed by Task 2 with the baseline, or the reverse) and assigned three participants to each.
% so that each condition was used with each task by six participants and used first by six participants. 
In each task, participants worked through the steps at their own pace and were encouraged to think aloud. 
After each task, participants completed two questionnaires assessing workload and usability of the tool they had just used. 
Upon completion of the two tasks, participants freely explored the datasets in \systemname for 10 minutes, then completed a questionnaire on the usefulness and user experience of its core features, and we further conducted a semi-structured interview to gather their experiences and feedback, including comparisons with their conventional workflow and the practical impact of the tool. 
(see \todiscuss{Supplementary Note xx} for the materials used in the user study). 
% 
With participants' permission, we recorded the video and audio of each session, together with their interactions with the tools (all prompts, GUI interactions, and generated artifacts in \systemname; notebooks, code files, and exported Claude Code session logs in the baseline). 
Each participant received compensation of US\$20 for their time. 
The study was approved by the Institutional Review Board of Northwestern University. 
}



\subsubsection{\newlyadded{Results}}

% 1. 任务成功率 + 完成时间（+ 交互次数）   [需要从录像/日志编码，数据尚未收集]
\textbf{Task performance.} 
1. completion time
2. accuracy
We review the analysis results from \systemname and the baseline. 
% placeholder for now.



% 2. SUS & NASA-TLX 
\newlyadded{\textbf{Usability.}
% 1. Overall statistical results
We assess the tool's usability using the System Usability Scale (SUS)~\cite{brooke1996sus}. 
Researchers rated \systemname as substantially more usable than the baseline ($M = 89.4$, $SD = 10.7$ for \systemname and $M = 64.8$, $SD = 20.1$ for the baseline).
% (SUS: $M = 89.4$, $SD = 10.7$ vs. $M = 64.8$, $SD = 20.1$; mean difference $24.6$, $95\% CI$ $[13.5, 35.0]$; Wilcoxon signed-rank $W = 3$, $p = 0.002$, $r = 0.92$). 
\systemname falls in the "excellent" range, whereas the baseline falls between "OK" and "good"~\cite{bangor2008empirical}. 
Eleven of the twelve participants gave \systemname the higher score, and eleven rated it above the conventional benchmark of 68~\cite{sauro2011practical}, compared with five for the baseline.
}
% % 2. Different dimensions
% Item-level comparisons (Supplementary Fig. S1) show that the difference is driven by integration and consistency of functions (Q5, Q6), cumbersomeness (Q8), and ease of use and learning (Q3, Q7, Q10), whereas willingness to use the tool frequently (Q1) and confidence (Q9) were high in both conditions, consistent with participants' extensive prior experience with LLM coding agents.
% % 3. Interview results to explain the results
% xxxx
% DirectGPT: "On the System Usability Scale, and for the specifc given tasks, DirectGPT was rated 92 (typically considered “Excelent” [4]) whereas ChatGPT received a 53 (typically considered “OK”). This corresponds to a mean diference of 39 (95% CI: [27.3, 47.34], p<0.001)."


\newlyadded{\textbf{Perceived workload.}
\systemname also reduced perceived workload.
We use NASA Task Load Index (NASA-TLX)~\cite{hart1988development} to estimate the users' perceived cognitive load \todiscuss{(Fig.~\ref{xx})}. 
% overall
Participants exhibited a significantly higher task workload in the baseline condition based on the average score of the six NASA-TLX items ($M = 3.21$, $SD = 1.26$) compared to the system condition ($M = 1.89$, $SD = 0.81$; Wilcoxon signed-rank, $p = 0.009$).
% individual breakdown
For the individual items (illustrated in Fig.~\ref{xx}), \systemname was rated significantly lower than the baseline in regard to mental demand ($p = .047$), physical demand ($p = .023$), and frustration ($p = .039$; all p-values Holm-corrected across the six subscales), while the differences in temporal demand, performance, and effort did not reach significance. 
These results suggest that \systemname substantially lowers the cognitive and physical burden of conducting the analysis tasks and makes the overall process less frustrating.
}


% 3. 9 项 5 点 Likert
\newlyadded{\textbf{Perceived value of \systemname's design components.} 
We also analyzed user ratings of the usefulness of nine design components of \systemname on a 5-point scale (1 = not at all, 5 = very much), including conceptual level design, hybrid interface, multi-agent engine, and data management \todiscuss{(Fig.~\ref{xx})}. 
% 1. Overall statistical results
All nine design components are rated positively (Fig. Xc; $M > 4$ for every component). 
% 2. individual results
% 2-1. positive results
Bi-directional mapping and data-driven artifacts were rated most useful which are also the core design components of our work. 
\todiscuss{``add a user quote.'' (Px)}
The two data-management components, the SciSci domain database and the chat-history database, were both rated highly, \todiscuss{``add a user quote.'' (Px)}.
% 2-2. negative results and discussions
Within the multi-agent engine, the workflow itself was rated highly ($M = 4.50$, $SD = 0.90$) but showed the one researcher only rating of 2: \todiscuss{``add a user quote.'' (Px)}
% across all items, which coincided with interview comments about the latency of multi-step executions. 
Action-level reasoning received the lowest, though still positive, rating ($M = 4.25$, $SD = 0.75$): \todiscuss{researchers found the streamed action sequence more structured than a raw chain of thought (P2), but several asked for a summary of key reasoning steps at a level between the executed code and the rendered figure (P1, P3), a point we return to in the Discussion}. 
}


% 4. Results from semi-structured interview.
\textbf{Qualitative findings and suggestions.}
\todiscuss{
Respond to editor: Finally, the difference between the proposed tool and other existing tools -- such as Tableau, Power BI, and so on -- is not entirely clear.
}
In addition to the quantitative results on efficiency and workload, semi-structured interviews and think-aloud observations across the twelve sessions revealed three broader ways in which \systemname shaped scientific discovery. 

% --- Pros ----
% 0. Nexus faster / smoother / fewer prompts -- cross-validate above results
% \textit{(1) Efficiency, usefulness, and workload.}
% Participants attributed the usability and workload differences in the questionnaires to two concrete sources. 
% The first is the number of exchanges needed to get a usable result: 
% P07 found \systemname "a lot less redundant … less prone to errors, as we saw," having said of the baseline "this is why I don't use Claude, it takes too long"; P02 called the action-by-action output "more modular … clearer, more intuitive" than Claude's text; 
% P10 rated \systemname "not complex at all" with effort "very low" while calling his usual double-checking across "two or three" agent sessions "actually still pretty hard to use"; 
% and P08 concluded that, apart from the ability to run on his own data, "your system is more intuitive and easier to use." 
% % 
% The second source is where baseline time went. 
% Setting up the notebook environment cost between 13 and 30 minutes for three participants (P01, P07, P12) and caused login or permission problems for others (P03, P05), and, more importantly, verification dominated the analysis itself: P11 spent 26 minutes on the first baseline question "because I couldn't trust … did it use the right variable," P01 caught Claude Code double-counting grants that it had not de-duplicated, and P03 reported iterating "several dozen times" per figure in his daily practice because the agent "makes a bunch of mistakes." 
% The coding agent also over-produced or substituted its own choices (four plot variants for one request, P06; "it's doing much more than I ask it," P04; defaulting to top-cited rather than the first records, P09). Rough timings from the recordings, to be replaced by the coded completion times, show baseline tasks taking 17–60 minutes (median ≈ 31) against 17–31 minutes for \systemname (median ≈ 21), even though interview questions were interleaved into the \systemname tasks. Two caveats matter for interpreting these numbers. The fastest baseline runs were fast because participants did not verify: P02 pasted each instruction straight into Claude Code and finished in 17 minutes, later acknowledging "I really did not check … mine might well have problems," and P06 described his own role in the baseline as "an invisible yes-clicking machine." Conversely, \systemname was not free of cost: chart generation latency was the most common complaint (P01, P02, P09, P12; P02 rated the action-level stream "effective — 5; efficient — no"), a running analysis could not be interrupted or corrected mid-way as the Claude Code extension allows (P01, P05, P09), and interaction bugs forced restarts for P04 and P10, while P12's first chart was the only incorrect generation observed across the twelve sessions. Finally, participants noted that \systemname shifts rather than removes mental effort: P10 rated mental demand as still "fairly high, because the thinking is still very important — what science-policy question you want to investigate."

% 1. GUI selection and interactive figures
% T1' Baseline 里 region-selection 的困难（做 Science Policy baseline 的 6 人）
\textit{(1) Figures as the interface for the iterative discovery.}
% 1. interactive vis + LUI and GUI: make exploration more effecient and accurate
A consistent finding was that direct manipulation of interactive figures transformed analytical operations that were awkward, inefficient, or impossible in the baseline into lightweight visual interactions. 
All six researchers who completed the Science Policy task with the baseline had to improvise a way to tell the AI assistant which cluster of the embedding scatterplot they meant, for example, typing coordinate ranges read off the axes or uploaded annotated screenshots.
These workarounds often required repeated prompting, manual code modification, or approximate specification of the intended data subset.
By contrast, researchers using \systemname could directly select the relevant visual marks and use that graphical selection as input to subsequent analyses, reducing both interaction overhead and ambiguity in specifying analytical intent. 
Participants particularly valued the ability to derive new coordinated analyses from an existing figure and selection, replacing analytical steps that otherwise required manually modifying and rerunning code.
% ''That is very cool! It's very quick … I love this," P11), and replaced work that participants had to redo by hand in the baseline (P04: "just repeating … run the code again; this could have been automatized"). 
% P04, who develops visualization tools himself, noted that "creating derivative plots from another plot" is a capability "I can't see in any tool that I use currently." 
% 2. bring in new data exploration approaches beyond traditional data analysis methods -- 强调这种新的figure模态和human-agent交互形式给researcher带去了崭新的discovery method的变化，从而带去opportunity to bring in more effecient discovery process. 
Beyond efficiency, the interaction changed what participants usually do during the scientific discovery: a participant zooming into a cluster she said she "had never done" in her traditional workflow, participants drilling into subgroups and noticing gender differences they had not looked for, and participants proposing to extend published findings by adding variables or subgroups. 
% P05 observed that without the task she "would not have thought of doing this … I don't think I've ever zoomed in on one part in such an interactive way," a point we return to under scientific discovery.
% two typed coordinate ranges read off the axes (P05: "there's no way to highlight … I did my best, hope those are OK"; P06, after four failed attempts with screenshots: "in the end I had no other option, I directly told it the x and y range"), 
% three uploaded annotated screenshots and found the model's selection "approximately from X to Y, not very precise" (P09; also P07: "I don't think it's accurate … it's surprising"), 
% and one (P04) had Claude write an interactive matplotlib brush, remarking mid-way, "Oh my god, this would be much, much faster with your assistance." 
% P08 mentioned, with a coding agent, \textit{``you are constrained by having to describe things in natural language...on a figure, some directions, positions, you need to explain them in words; there is no direct manipulation.''} 
% (P09 rated graphical input above language input because "it compresses a lot of the pipeline and requirements into it"; P10: physical demand was "definitely less than with Claude, because a lot can be done directly through manipulation"), and as enabling a drill-down from an overview to a subset "without going back to the data" (P09), including heterogeneity analyses on a brushed subset (P12). The coordination operation, which re-applies a derived analysis to a new selection, drew the strongest affective reactions ("Amazing … so fast … wow," P08; "That is very cool! It's very quick … I love this," P11), and P04, who develops visualization tools himself, noted that "creating derivative plots from another plot" is a capability "I can't see in any tool that I use currently." 

% 2. Data-driven artifact and Canvas as externalized reasoning / mind map;
\textit{(2) The data-driven artifact as an externalized reasoning trace and mind-space.} 
Researchers repeatedly contrasted the data-driven artifact design with the linear nature of a computational notebook or chat, and described the difference in terms of cognitive load in addition to convenience. 
The second source of usefulness is that the canvas changed what participants could keep track of: an exploration that in a notebook or chat is, in P07's words, "squeezed down into just a line of analyses," became a structure they could see, branch and return to. 
Several volunteered the metaphor of a mind map or "mind-space" which can easily trace your entire exploration process and much better than a general AI agent, where sometimes you don't know what you did today and during the whole project.
P05 called it a "mind-space" problem, since a notebook "is not easy for the human brain to track," whereas the canvas matches "the most natural way a person remembers different analyses, and you can quickly extend one branch and not another").
while the canvas "would reduce cognitive load a lot," because a research project "is a network of these blocks, where this gets hidden because it's somehow in your brain." (P7)
a map that visualizes my thought process (P11).
P11 described losing insights and the reasons behind abandoned ideas between advisor meetings — "we have to come up with a new idea again" — and asked for exactly "a map that visualizes my thought process." 
% (P12: "the whole framework has the feel of a mind map … you can easily trace your entire exploration process; much better than a general agent, where sometimes you don't know what you did today"; P05 called it a "mind-space" problem, since a notebook "is not easy for the human brain to track" whereas the canvas matches "the most natural way a person remembers different analyses, and you can quickly extend one branch and not another"). 
% P07 put the contrast most sharply: with a coding agent "that entire network of analyses is squeezed down into just a line of analyses; you lose all the information," while the canvas "would reduce cognitive load a lot," because a research project "is a network of these blocks, where this gets hidden because it's somehow in your brain." 
% P08 valued seeing "the results of multi-step reasoning at the same time," which he currently approximates by asking Claude to run every possible analysis at once and picking afterwards, 
% and P11 gave an extended account of losing insights and the reasons behind abandoned ideas between advisor meetings, concluding that she wanted "a map that visualizes my thought process." 
Two further mechanisms were singled out: version rollback that does not contaminate the conversation and anchoring intermediate versions so that an error can be traced to the step that introduced it . 
% (P06: "when I want to go back to an earlier version, at least it won't be polluted"; he hit exactly this problem in the baseline when Claude Code reused a stale selection from its chat memory)
% (P05)
% Participants who did not experience the canvas as new still saw value in it: P04, who "forces" non-linear exploration through sequential tools, expected the main benefit for researchers who "don't know that they can do this nonlinear kind of exploration easily." 


% 2' Resume / portability across sessions; Sharing / publication as interactive artifact; Team / collaboration value
% 强调idea exploration history这件事很重要
% 长久以来，人们往往只看到论文的结果是好的，并且看到论文里描述的美好的故事。但是论文背后真正的想法以及思考的起点和轨迹，却无法得知。
% 更重要的是，这没有办法让AI完美替代研究员：）
% 于是，Stanford 研究人员不止蒸馏论文，还要来蒸馏论文背后的idea了。
% 所以，请帮助我们重构您论文的灵感来源（以便于我们kindly替代您吧
%LLMs show promise as tools for scientific discovery, from generating hypotheses to planning experiments and writing up results. But these systems are usually given their scientific context upfront. They are not tested on a fundamental step that we all had to face: identifying which prior work is worth building on.

% A final paper cannot fully capture the intellectual path behind a discovery: why certain prior work mattered, how different ideas came together, and which connections changed the direction of the research. Across the community, expert researchers collectively hold this missing layer of the scientific record.

% We are a research team at Stanford IRIS (Sohyeon Kim, Yoonho Lee), asking researchers to turn this firsthand knowledge into an author-validated dataset. We will publicly release it both as a benchmark for evaluating scientific-retrieval systems and as a training signal for future models that can navigate the scientific literature and identify which prior work is worth building on.

% Ultimately, we aim to answer: Given only an early-stage research question, can an LLM search a large scientific corpus and retrieve the prior work that offers genuine scientific inspiration, rather than papers that are merely topically related?

% 参与者还特别指出了两个进一步降低认知和追踪成本的机制。其一是版本回滚：研究人员可以返回早期版本，而不会使当前对话上下文受到旧状态的干扰或“污染”（P06）。其二是对中间版本进行锚定，使分析错误可以追溯到具体是哪一步引入的，从而增强整个探索过程的可追踪性。
% 即使部分参与者并不认为这种非线性探索方式本身是全新的，他们仍然看到了这种显式结构化的价值。例如，P04 表示，他目前会通过一系列顺序工具“强行”实现非线性探索，因此预计这种设计对于那些尚不知道如何方便地进行非线性探索的研究人员尤其有帮助。
% 进一步而言，这种对探索历史的保留还涉及跨会话恢复、共享以及作为交互式研究 artifact 进行发布的潜力。长期以来，科学论文主要呈现最终结果以及经过整理后的连贯叙事，却很少保留真正促成发现的思想轨迹：哪些已有工作最初带来了启发，不同想法如何逐渐连接起来，哪些分支被放弃，以及哪些意外联系最终改变了研究方向。最终论文因此无法完整记录发现背后的知识形成过程，而这些信息往往只存在于研究人员自己的记忆中。
% 这一缺失的“思想层”对于未来的 AI 科学发现系统同样重要。当前的大语言模型已经展现出生成假设、规划实验和撰写研究结果的潜力，但这类系统通常预先获得已经整理好的科学背景，而较少被要求完成一个研究人员必须面对的基础任务：从庞大的已有文献和可能路径中判断，哪些工作真正值得继续构建其上。换言之，除了蒸馏论文最终呈现的知识，未来的科学 AI 还可能需要学习论文背后未被正式记录的灵感来源、探索路径和研究判断。


% 3. Verification via download / provenance used in session; T3 Replication package / SI / open science
\textit{(3) Provenance, reproducibility and sharing.} 
Because every figure carried its data, SQL and code, verification became part of the task rather than a separate effort: 
% P11 downloaded the underlying records twice to check the topic labels the system produced for two clusters ("Let me check … ACA, e-cigarettes … yeah, this looks correct"), P10 did the same and found a label that was too specific ("it's just cigarettes, not specifically electronic"), and P01 read the exported action file while waiting for a result. 
This contrasts with the baseline, where provenance existed only if participants asked for it — 
% P08 had Claude Code emit a standalone HTML page with no saved code, and P03, when asked to check a result, observed that "there must be code in the back end, but I didn't ask it to output it." 
Participants projected three uses beyond the session. 
First, replication and open science: 
P06 asked whether the artifact could generate the replication package he finds "quite a hassle" to assemble, P03 wanted a one-click export to a runnable notebook "convenient to upload as SI," and P12 and P02 noted that downloadable code makes results "easier to replicate" and serves "open science." 
Second, portability: P06 wanted to move an artifact into a fresh session when a long chat's "memory messes things up," because "if I only paste an image over, it wouldn't know what it is," and P04, P10 and P11 valued reopening an artifact later ("that's super useful … unique," P04). 
Third, for science communication: P05 imagined a paper shipping "a traditional version plus a logic diagram of the visualization" so that "when the audience questions a sub-group, I click into it … it's defensible"; P08 argued that publishing the figure itself as an interactive artifact matters more than full replication because "people just look at the figures"; and P09 expected such artifacts to raise readers' trust "in your exploration process." 
At the same time, participants were clear that raw code is necessary but not sufficient for trust: P03 asked for "a summary — which steps I did and what each step did," because "a person can't check line by line"; P10 wanted a per-step data panel; P08 said he would never read the action log ("it is very long") and verifies with cross-check analyses instead; and P05 considered figure–code–data linkage only a more intuitive version of what a notebook already provides.




% --- Challenges ---
% 4. Verification burden as main baseline cost
% 5. Engineering suggestions: Own data / connect local data; Want human-readable step summary / intermediate data; Want less process detail (progress bar); Speed
% 6. Nexus for early exploration, not final figures


\textit{(4) Suggestions.} 
The most substantive is trust in intermediate data processing. Participants who work with many-to-many linkages (grants with several PIs and fields) worried that decisions such as de-duplication, unit of analysis, or dropping records with missing fields would be made silently: 
% note: 我们需要把这些问题frame成：有些情况下数据处理并没有标准的答案，A和B都可以，就看researcher怎么在后期解读 -- 可能两种方法都需要尝试。
% P01 "did not know how it handles it by default … especially drop-duplicate, this is very key," and P10, who had just noticed Claude Code's SQL excluding grants with missing age, feared that a polished chart would end verification altogether — "if it directly gives me a result, I won't double check, I'll just pass it" — and that "if you have ten processing stages and it makes a decision at each, the result may be slightly biased." 
The remedy they asked for is not more raw output but a human-readable summary at a level between the action stream and the code ("which steps I did and what each step did … the simpler the better," P03; "a simple overview of how it did it," P01), together with per-step intermediate data (P10), editable actions (P10), and the ability to interrupt and correct a running analysis as the Claude Code extension allows (P01, P05). 
Notably, other participants wanted less rather than more: P04 would replace the action stream with a progress bar, and P08 said he never reads such logs and verifies through cross-check analyses instead, which suggests progressive disclosure rather than a single level of detail. 
% 总结：这也反映了不同researcher对HAI合作生成的数据结果的validation的不同要求。需要后期系统中进行个性化配置。
% 
The second, and most frequent, request was to analyze one's own or local data (P01, P03, P04, P06, P08, P10): P08 identified this as Claude Code's one remaining advantage, and P03 said that with local-data connection and web access the system would be "more useful than Claude."
% 
The third concerned flexibility: widgets rather than natural language for cosmetic edits such as colours (P09), style transfer from a reference figure (P06), parallel analyses and multiple root charts (P05, P08), notes and rationale attached to nodes (P08, P11), notebook or full-package export (P03, P04), per-chart interaction guides or an onboarding tour (P04, P08), and AI-proposed next questions when a mark is clicked (P09, P06). Latency was mentioned by four participants, and we logged nine distinct interface bugs (Supplementary Note X), none of which affected task correctness except one wrong initial chart for P12.


Researchers also mentioned limits of the current selection vocabulary: they wanted a brush to persist so that successive questions condition on exactly the same marks (P03), several selections and their results kept side by side (P01, P03, P12), statistically defined rather than hand-picked outliers (P06), and a natural-language fallback when a chart's built-in interactions do not cover a need (P08); two participants initially confused click and brush, and the selection tooltip was flaky (P02, P04, P09, P10).

% action reasoning
P08 valued seeing "the results of multi-step reasoning at the same time," which he currently approximates by asking Claude to run every possible analysis at once and picking afterwards,

% artifact
The main limitation, raised independently by P05 and P08, is that the canvas currently supports only parent–child (drill-down) links: exploration that "expands the territory" into a parallel question rather than a subset, several root charts, merging two charts, and text notes or intermediate query results as first-class nodes were all requested, as were deleting nodes (P12) and recording each brush or coordination state as a revisitable version (P01, P05, P10, P12).


% Result Analysis
% Story: 
% 1.	一个pathway: 我们的study可以首先验证使用基于llm native figure这个concept的nexus提高了成功率、减少了时间 （SUS/TLX问卷），
% 2.	另一个pathway: 而这种变化的核心是llm native figure对于figure作用的重新定位和拓展（exploratory study问卷）。
% 这样的故事应该就比较清晰了

% 最后结果整理应该是这几部分：
% 1. usability (SUS): 俩tool比较
% 2. workload (TLX): 俩tool比较
% 3. 正确率和时间：俩tool比较
% 正确率评估方法: LLM-as-judge, human-as-judge (yifang)
% 正确率: GUI selection ask follow up question的时候，可能传统方法正确率低。
% 4. Nexus-specific questions: 关于核心feature的usefulness and user experience -- 打分
% 5. Nexus-specific questions：关于核心feature的usefulness and user experience -- 开放式问答和解释。也会涉及跟他们传统tool的定性比较，从文字获得一些反馈
% 6. 因为这个concept本身其实让figure这件事的地位发生了变化. 之前知识final present result的工具， 但现在可以变成explore的工具，同时兼具scientific provenance的作用（方便后面做复现啥的）
% Tiantian: 我觉得这是个很好的角度。如果我们的study能reveal这种变化对research的影响，那就太厉害了. 是不是还是可以通过monitor他们在图片上做action的行为来得到这个结果 -- 那可以做一些in-lab behaviour analysis 观察他们咋用的


% e.	editor 点名了 Tableau/Power BI，你要一句话回应为什么 baseline 是 notebook+LLM 而非 Tableau——现成证据就在你们自己的 SciSciGPT 论文里：专家访谈显示 SciSci 研究者的日常工具是 Jupyter/RStudio + ChatGPT/Claude。所以 notebook+LLM 才是该领域真实的 status quo。Tableau/Power BI 的问题另用两招覆盖：(a) Related Work 加一张能力对照表（provenance、bidirectional mapping、cross-figure coordination、artifact 维度）；(b) Study 2 招 1–2 名日常使用 Tableau/Power BI 的参与者，访谈提纲里加"与你日常工具相比"的问题——LightVA 拿到的那句 "Previously, using PowerBI required a lot of time and operations, but now it only takes a sentence" 就是这类问题产出的、可直接引用的证据。



% User study和Case Study结束以后：
% 1.	把server上所有文件copy下来，dropbox备份一份，硬盘备份一份。
% 2.	Then停止这个VM





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below: old version (Round-Trip Reproducibility & User Study), temporally abandoned
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Round-Trip Reproducibility}
% \label{subsubsection:evaluation-reproducibility}
% \wyf{Note: test case: lack of LLM-based Python code.}
% We evaluate whether an LLM-native figure artifact preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
% This evaluation tests whether LLM-native figures function as reproducible computational objects rather than ephemeral presentation outputs.
% % To evaluate whether an LLM-native figure artifact provides complete provenance, enabling precise re-execution of the analytical workflow and deterministic reconstruction of the figure.

% \textbf{Test Design.} 
% We use the same set of 200 test cases described above and store all figures $F_t={V_t, D_t, C_t, M_t}$ generated succesfully during their execution. 
% For each figure, we re-execute the stored code $C_t$ against the original database to regenerate the data subset $D_g$ and the corresponding visualization $V_g$. 
% We then compare the original and reconstructed figures at two levels: (1) specification-level equivalence, assessed via structural comparison of the visualization specifications (JSON); 
% and (2) visual-level equivalence, assessed by matching visual marks, encodings, and positional attributes. 
% We report the proportion of figures that are exactly reproducible at the specification level and those that are visually identical despite potential non-semantic specification differences.

% \textbf{Results.} 
% % High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% \wyf{
% Across the \wyf{180} generated figures, round-trip reproducibility is achieved for nearly all figures. 
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% }.


% \subsubsection{Discussion}
% \newlyadded{
% Failure analysis (e.g., reproducibility-missing provenance, mismatched encodings, rendering differences). 
% Fill in with a short failure-mode paragraph: e.g., missing spec fields, nondeterministic defaults, or database changes. This will earn reviewer trust.
% \wyf{Erzhuo's suggestion: we also report failure cases with persentage and some examples.}
% }



% \subsection{User Study} 
% \textbf{Participants}: SciSci researchers from different "research age". 

% \textbf{Task}: three case studies, same setting of data. 

% \textbf{Benchmark}: Python/Jupyter Notebook, SciSciGPT. 

% \textbf{Evaluation dimensions}: 
% (1) Efficiency: time and accuracy. -- same analysis tasks in the case study. 
% (2) Expressiveness: number of insights generated. -- do not limit analysis tasks, only limit the high-level research question. To test: the number of insights generated; the diversity of insights generated. 

% \subsection{Expert Interview} 
% (1) Use \textit{Five-point Likert Scale} to allow users score different dimensions of the system: usability, etc. 

% (2) Qualitative evaluation: summarize their feedback in terms of hybrid user interface, LLM agent engine, and suggestions (especially for data-driven scientific discovery and LLM-native figures to be presented in their research paper -- open science related questions). 

==> sections/archive/03-2-evaluation/03-2-evaluation_v7_20260918.tex <==
\subsection{Case Studies} 
\label{subsection:case-study} 

The climate example in Sec.~\ref{subsection:conceptual-framework} provides a simple illustration of the mechanics of our domain-independent conceptual framework. 
Here we demonstrate the utility of the proposed framework through \systemname, an instantiation tailored to the science of science (SciSci) domain (Supplementary Note 2.2). 
SciSci provides an ideal testbed because it combines massive, heterogeneous datasets spanning grants, publications, and patents;
complex research problems, such as tracing knowledge evolution; and high-stakes decision-making scenarios, such as strategic funding allocation.
We present four case studies in which \systemname is used to explore SciSci challenges.
% We present four case studies in which \systemname is used to explore SciSci challenges, with a fifth in \todiscuss{Supplementary Note x.x}.
% an ideal testbed because relevant signals are distributed across heterogeneous linked datasets and exploratory questions evolve rapidly as new insights emerge
% The SciSci field~\cite{fortunato2018science, wang2021science} provides an ideal testbed: 
% large-scale heterogeneous data, spanning grants, publications, and patents with complex citation networks;
% complicated research problems, such as tracing knowledge evolution and identifying emerging frontiers; 
% and high-stakes decision-making scenarios, such as strategic funding allocation and university innovation assessment.


\subsubsection{Case Study 1: Innovation Landscape at Universities}
In this case, we use \systemname and its integrated innovation-related dataset from a leading U.S. research university \todiscuss{(Supplementary Note x.x)}. 
Understanding the research innovation landscape has become a central research issue in SciSci, where researchers aim to map the dual frontiers of science and technology~\cite{ahmadpoor2017dual, liang2022systematic, yin2022public}, and a concern for university leaders and science policymakers seeking to accelerate technology transfer and amplify research impact~\cite{wang2023innovationinsights, wang2025funding}. 
Yet uncovering untapped innovation potential remains challenging: relevant signals are distributed across heterogeneous data sources, and exploratory questions evolve rapidly as new insights emerge. 
% To illustrate how \systemname supports this dynamic analytical process, we conduct a case study using innovation-related data from a leading U.S. research university. 

% step 1: generation
Imagine a researcher seeking to explore the innovation landscape at the level of individual inventors. 
The researcher might first ask \systemname:
% Imagine a researcher first ask \systemname to explore the innovation landscape at the individual inventor level: 
\textit{``Show me the distribution of inventors based on their number of invention disclosures (as y axis) and number of papers cited by patents (as x axis).''} 
% \textit{``Show me the distribution of all inventors at this university in terms of their current patent activity and their hidden research potential relevant to technological use.''} 
Through the plan–action–execution loop, the system generates a sequence of atomic actions (\eg, \actionname{select_table} and \actionname{add_chart_type}), executes the associated code, and returns an interactive scatterplot showing the inventor distribution at this university (Fig.~\ref{fig:Figure3}a), with the y-axis encoding invention disclosures (a proxy for present-day innovation activity) and the x-axis encoding papers cited by patents (a proxy for technological potential). 


% step 2: modify chart
% 1. adjust scale (to log scale)
The figure shows that most inventors cluster tightly in the lower-left region due to the heavy-tailed nature of both measures. 
This compression obscures meaningful structure and hinders the identification of high-potential individuals. 
The researcher might then select the figure and request:
% Thus, the researcher would select the figure and requests: 
\textit{``Update the chart to use log scales on both axes. Customize the calculation to apply log(value + 1) so zero values are handled.''}
% \textit{``Update the chart to plot log-transformed x and y values, computed as log(value + 1) so that zero values are handled.''}
% \textit{``Update the chart to turn the x and y values into log scale. Use the formula: x = log(x + 1) to avoid zero.''} 
% \textit{``Help me adjust the values of the x and y axes to log scale to make the distribution clearer.''} 
Here, the system shifts from generation to manipulation (Sec.~\ref{subsection:conceptual-framework}-Data-Driven Artifact and Provenance). 
The system takes the existing visualization and underlying data as inputs, infers the user's intent, triggers a new chain of actions to transform the data (\eg, \actionname{derive_column}) and update the visual encoding (\eg, \actionname{update_encoding}), and regenerates the scatterplot with log transformations applied to both axes, providing a clearer, more discriminative view of the inventor distribution (Fig.~\ref{fig:Figure3}b, c).
The overall distribution indicates a positive relationship between the two metrics, suggesting that patent-cited publications may serve as a useful indicator of a researcher's innovation activity.
Hover interactions expose precise values for each inventor, enabling accurate inspection of potential inventors and outliers (Fig.~\ref{fig:Figure3}b).
% 2. regression line
% based on log results, add regression: yifan: make sense!

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-1-innovationinsights-20260831.jpg}  % figures/20260409/case-ii.jpg
    \vspace{1pt}
    \caption{
    \bodyfigurelabel{fig:Figure3}
    \textbf{Case study: University innovation landscape.}
    \textbf{(a)} The figure generated for the first user query. 
    \textbf{(b)} The updated figure after adjusting the x- and y-axes to log scales. 
    \textbf{(c)} Screenshots of the streaming output when generating and updating a figure.
    \textbf{(d-e)} Comparison of different groups of researchers after filtering and coordinating across multiple figures. 
    \textbf{(f)} Screenshot of the data-driven artifact. 
    }
    % \label{fig:case-1}
\end{figure}


% step 3: extend chart: gender difference / other meta information (department) 
\wyf{
The overall distribution reveals a small group of individuals with particularly high numbers of invention disclosures (Fig.~\ref{fig:Figure3}d, left scatter plot). 
% note: should refer to the brushed region at the bottom.
To examine this group, the researcher might brush the corresponding region through direct manipulation on the scatterplot and pose a follow-up query to drill down: 
\textit{``show me the department distribution using a bar chart.''}
The system uses both the natural-language request and the GUI-based selection as joint inputs, triggering a new sequence of atomic actions. 
It then generates a bar chart summarizing the departmental composition of the selected group (Fig.~\ref{fig:Figure3}d, left bar chart), enabling quick assessment of departmental patterns among these highly active inventors.
% insights
% 1. department
By brushing different regions on the scatterplot and comparing the department composition of this group against those with few or no invention disclosures (Fig.~\ref{fig:Figure3}d, right scatterplot), the researcher would observe that faculty with frequent invention disclosures are disproportionately concentrated in fields such as chemistry and materials science, reflecting the uneven distribution of patenting activity across research areas within the university (Fig.~\ref{fig:Figure3}d, two bar charts).
}

\wyf{
The researcher might also notice an interesting group in the bottom region of the scatterplot (Fig.~\ref{fig:Figure3}e, scatterplot): these faculty have no disclosed inventions, yet their publications are cited by patents. 
% the x-axis captures the number of publications cited by patents, a potential predictor of commercialization activities 
This subgroup represents researchers with significant untapped innovation potential: their work has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
To examine the relationship between this untapped potential and their tenure status~\cite{tripodi2025tenure}, the researcher could brush the corresponding points and ask analogous queries for senior and junior faculty, 
\eg, \textit{``show the distribution of all senior faculty (tenure `Attained'), comparing those within this selected region of researchers against those who are not, using a pie chart.''} 
% \textit{``show the distribution of senior faculty (tenure "Attained") out of all senior faculty in the dataset by counting the number of faculty using a pie chart.''} 
% and \textit{``show the distribution of all junior faculty (Tenure Eligible), comparing those within this selected region of researchers against those who are not, using a pie chart.''}
% insights
Interestingly, nearly half of junior faculty fall within the selected region, compared to only about one-third of senior faculty (Fig.~\ref{fig:Figure3}e, two pie charts). 
% This indicates junior faculty are more likely than senior faculty to appear in the group of researchers whose work is cited by patents despite not engaging in invention activities.
% The researcher is very excited to find these new insights. 
This asymmetry points to a novel discovery.
Junior faculty, whose career advancement depends primarily on publications and grants, have strong incentives to prioritize academic output over other impacts such as direct engagement with patenting, yet their research is nonetheless absorbed by the technology sector, as evidenced by patent citations. 
Senior faculty, by contrast, are more likely to have established the industry collaborations and institutional networks that facilitate direct participation in invention disclosure and technology transfer.
The observed divergence suggests that a substantial reservoir of commercially relevant knowledge produced by junior faculty remains unrealized by the formal technology transfer pipeline, highlighting a structural gap between academic incentive systems and innovation outcomes that merits systematic investigation.
% Junior faculty, whose career advancement depends primarily on publications and grants~\cite{sanberg2014changing}, have strong academic incentives to prioritize academic output over other impacts such as direct engagement with the patenting process, though their research nonetheless generates knowledge that is absorbed downstream by the technology sector, as evidenced by patent citations to their publications. 
% Senior faculty, by contrast, are more likely to have established industry collaborations, laboratory infrastructure, and institutional networks that facilitate direct participation in invention disclosure and technology transfer. 
}
% This asymmetry suggests a difference in roles along the science–technology pipeline: the academic incentives for junior faculty focus more on research publications, whereas senior faculty are more likely to participate directly in invention processes through patenting activities.
% This explorative exploration help the researcher find new initial insights about the relationship between tenure status and innovation potentials and worth for a deeper dive for systematic analysis. 


% It then generates a bar chart summarizing the gender distribution and a pie chart showing the departmental composition of the selected group (Fig.~\ref{fig:Figure3}d), enabling quick assessment of demographic patterns among these faculty. 
% By comparing the gender distributions of different subgroups, the researcher observes a clear disparity between faculty with higher numbers of invention disclosures (Fig.~\ref{fig:Figure3}d) and those with few or none (Fig.~\ref{fig:Figure3}e): 
% male faculty members appear more likely to have disclosed inventions than their female counterparts (Fig.~\ref{fig:Figure3}d, e, two bar charts), and faculty with frequent invention disclosures are disproportionately concentrated in fields such as biomedical engineering, chemistry, and materials science, reflecting the uneven distribution of patenting activity across research areas within the university (Fig.~\ref{fig:Figure3}d, e, two pie charts). 

% A contrasting pattern emerges when the distribution is examined along the x-axis, which captures the number of publications cited by patents, a potential predictor of commercialization activities (Fig.~\ref{fig:Figure3}f). 
% Unlike the y-axis comparison, where faculty with high numbers of disclosed inventions are all male, researchers with high x-axis values comprise both male and female faculty. 
% Notably, in the bottom-right region of the scatterplot (Fig.~\ref{fig:Figure3}f), where researchers have no disclosed inventions yet their publications are heavily cited by patents, the proportion of female faculty is substantial. 
% This subgroup represents researchers with significant untapped innovation potential: their research has demonstrable technological relevance yet has not been translated into their own patent disclosures. 
% Taken together, these patterns suggest a gendered asymmetry between realized and unrealized innovation, where male researchers are more likely to have already converted research into inventions, while many female researchers exhibit comparable innovation potential that remains untapped.


% step 4: 
% 4.1 tracable with code (SQL, Python), data, and vis code
% 4.2 save artifact for future exploration (there are other universities' data comming in). 
To ensure analytical rigor, the researcher could download the underlying data, generated code, and visualization outputs from each figure to verify the procedure and results. 
The entire chat session, including the data-driven artifact (Fig.~\ref{fig:Figure3}f), is also saved for future analysis, enabling replication and facilitating cross-institutional comparisons as additional university datasets become available. 

This case study illustrates how LLM-native figures support descriptive analysis and provenance-rich exploration. 
Unlike conventional tools that require manual reconstruction or produce static outputs, our approach records each analytical step as a versioned, navigable artifact, enabling mixed-initiative analysis that existing systems do not provide.
% This case study demonstrates that LLM-native figures support iterative, provenance-rich exploration, enabling researchers to refine existing visualizations, generate contextually linked follow-up views, and revisit any point in the analytical trajectory. 
% Unlike conventional tools that require manual reconstruction of views or produce static figures with no provenance, our approach records each analytical step as a versioned, navigable artifact, supporting a form of mixed-initiative analysis that existing systems do not provide.



\subsubsection{\newlyadded{Case Study 2: Use of Science in Public Policy}}
\label{subsubsection:case2-science-policy}
\newlyadded{
The second case study explores the relationship between science and politics by tracing the scientific knowledge that informs policymaking.
Scientific evidence is widely regarded as a cornerstone of public policy, shaping legislative responses to complex societal challenges such as climate change and public health~\cite{furnas2025partisan, furnas2025partisanfunding}.
Prior research has shown that the uptake, framing, and interpretation of scientific evidence can be systematically shaped by the political context, particularly under conditions of sustained partisan polarization~\cite{mccarty2016polarized}.
This raises a fundamental question at the intersection of science and governance that can be examined with \systemname: do policymakers from different political parties draw on systematically different bodies of scientific knowledge?
}

% 1. overview scatterplot
\newlyadded{
To explore this question, a SciSci researcher could use \systemname and its integrated science policy dataset \todiscuss{(Supplementary Note x.x)} to determine the kinds of science that are used in policy. 
% before turning to how those patterns may diverge across parties.
As a tractable yet substantively rich starting point, the researcher might focus on documents from the U.S. House Committee on Energy and Commerce. 
The committee offers an analytically useful case because its science-intensive portfolio spans health, environmental regulation, and energy, generating citations to a heterogeneous range of scientific topics~\cite{furnas2025partisan}. 
The researcher could begin by asking: 
% To see an initial overview for policy documents from a specific committee, for example, U.S. House Energy and Commerce Committee (a central venue for legislation on health and energy)~\cite{furnas2025partisan}, the researcher could ask:
% To see an initial overview, the researcher specifies policy documents from the U.S. House Energy and Commerce Committee, a central venue for legislation on health and energy, and asks:
\textit{``Show a scatterplot of all the papers cited by House Energy \& Commerce Committee policies (committee short name is ``hsif00"), where each point is one unique paper title and doi and positioned by its title text embedding.''} 
% \textit{``Show me the distribution of all these policies’ cited papers based on paper title similarity.''}
\systemname first filters the policy corpus by source committee and extracts the cited papers along with their titles.
% To show the latent topical structure without imposing predefined categories, 
Next, the system applies two complex analysis actions (\actionname{text_embedding} followed by \actionname{dimension_reduction}) and generates a scatterplot in which each point represents a cited paper positioned by semantic similarity.
The figure shows clear topic clusters based on the visual distribution of the papers (Fig.~\ref{fig:Figure4}a). 
}

% 2. update scatterplot: highlight by color. 
\newlyadded{
To examine the differences between paper topics cited by Democrats and Republicans, the researcher could issue another query: 
\textit{``Assign a dark blue color to a paper point if at least one House Energy \& Commerce Committee policy (committee short name is ``hsif00") citing that paper is under Democratic party control; otherwise, color it light grey. Reuse the existing scatterplot layout, and keep each paper's coordinates and the axis limits unchanged.''}
The system then takes the generated figure and the underlying data as input to query the original database, adding each paper-policy citation pair with a new attribute about party control. 
It updates the data in the figure as well as the visual encoding, and it returns an updated scatterplot with papers that are cited by policies written under Democratic control highlighted in blue (Fig.~\ref{fig:Figure4}b). 
tion}

% 3. extend chart generation and coordination
\newlyadded{
% 1. generation
Having identified visually distinct clusters, the researcher might also seek to understand the scientific content represented by each region. The researcher could then circle a cluster on the scatterplot and issue a follow-up request to summarize the paper topics: 
\textit{``Looking at the selected region and for papers cited by policies under Democratic party control, generate a topic label based on paper titles.''} 
The system queries the database for the papers in the circled region, retrieves their titles, and calls the LLM to determine the region's topic. 
The researcher might also ask the system to list five of these papers to confirm the accuracy of the topic label: \textit{``Looking at the selected region and for papers cited by policies under Democratic party control, provide a raw data table with each paper's title and doi. Return the first five paper records.''} 
It then returns a sample of the papers' metadata so that the researcher can cross-validate the inferred label.
% 2. coordination
The researcher might then brush several other visual clusters and record the representative topics: \textit{e-cigarette health effects, marketing, and regulation} (Fig.~\ref{fig:Figure4}c) and \textit{alcohol-impaired driving prevention and traffic safety} (Fig.~\ref{fig:Figure4}e). 
}

% 4. fork analysis
\newlyadded{
To examine papers cited in policy documents produced while the committee was under Republican control, the researcher might select the existing artifact for the Democratic-control analysis and request:
% The researcher is then interested in papers cited by policies that are under Republican control. Selecting the existing Democratic artifact, the researcher requests:
\textit{``Repeat the same analysis and artifact for the other party---this time using policies and papers associated with Republican control.''}
% \textit{``Apply the same analysis and artifact to another party's associated policies and papers: Republican control, party_control = 'R'''.}
The analysis is nearly identical, with minor adjustments to the data query and visualization representation. 
The system forks the artifact, including its underlying code, data, and figure, and then determines the analysis and visualization information to be updated: it queries papers cited by policies produced while the committee was under Republican majority control, updates the visualization with the new set of papers, and changes the color to a shade of red associated with the Republican party, drawing on the LLM's general world knowledge. It also updates the figure title and description. 
The forked artifact for the Republican case then appears in the session. 
Following the same procedure, other representative topics would be identified, such as \textit{high school sports injuries and safety} (Fig.~\ref{fig:Figure4}d). 
}
% \todiscuss{TODO: add discussions of different topic distribution of papers by two parties).}

\todiscuss{
This exploration suggests that Democrats and Republicans draw on distinct bodies of scientific research in policymaking, with direct implications for evidence-based governance. 
The pattern emerges through the two complementary interaction modes in \systemname: direct graphical selection captured visually emergent topic clusters that natural language cannot describe precisely, and artifact forking replicated the entire pipeline for another party with a single instruction, replacing the manual, time-consuming, error-prone reconstruction required by conventional workflows.
}
% Having identified visually separable clusters, the researcher then seeks to ground these abstract regions in concrete scientific content.
% Using direct manipulation, the researcher circles distinct regions of the scatterplot and issue a follow-up request:
% \textit{``Give me a table showing the list of all these selected papers with attributes including paper title and DOI.''}
% In response, the system maps the visual selection back to the underlying database, filters the corresponding records, and returns a raw data table for inspection.
% Through this drill-down, the researcher finds two topical clusters (Fig.~\ref{fig:case-2-science-policy}): one centered on \textit{Nutrition and Agricultural Impacts}, and another focused on \textit{Infectious Disease Prevention and Response}.
% These clusters reflect substantively different dimensions of policy-relevant science, highlighting how health, food systems, and disease control co-exist within the committee's evidence base.
% \wyf{TODO: add discussions of different topic distribution of papers by two parties).}
% }

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-2-science-policy-20260916.jpg}
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure4}
        \newlyadded{\textbf{Case study: Use of science in public policy.} 
            \textbf{(a)} The scatterplot generated for the initial query, showing all papers cited by policy documents.
            \textbf{(b)} An in-place manipulation of the same figure highlighting papers cited by policy documents produced when the committee was under Democratic control.
            \textbf{(c)} An extension of the artifact: the user brushes a region of interest, and the system generates a coordinated figure summarizing the topic label of the selected paper cluster.
            \textbf{(d)} The artifact forked from Democratic- to Republican-associated papers, re-executing the same analytical chain on a new data scope and revealing markedly different paper topic distributions across the two parties.
            \textbf{(e)} Coordination in action: changing the graphical selection region propagates to the linked topic summary, while the underlying data table remains accessible for cross-validating the generated labels.
        }
    }
    % \label{fig:case-2-science-policy}
\end{figure}



\subsubsection{\newlyadded{Case Study 3: The Impact of Science Funding}}
\label{subsubsection:case3-funding-impact}
% note: no coordination reflected
\newlyadded{
In the third case, we use \systemname and an integrated science funding dataset \todiscuss{(Supplementary Note x.x)} to examine the funding portfolio of the National Institute on Aging (NIA), a major institute of the U.S. National Institutes of Health (NIH), tracing an analytical chain from funding allocation to representation to impact. 
% As funders allocate scarce resources across a complex research landscape, evaluating the impact of their investments beyond publications is critical to aligning science funding with societal needs~\cite{wang2025funding}.
Understanding the impact of science funding is critical to ensuring that research investments align with societal needs~\cite{bush2021science, yin2022public, wang2025funding}, a question of immense interest to funding agencies, national policymakers, and university leaders who allocate scarce resources across a complex research landscape. 
While emerging datasets now link grants to downstream outcomes well beyond publications, including patents, clinical trials, policy documents, and news coverage~\cite{yin2022public, wang2025funding, furnas2025partisan}, assessing this broad impact remains challenging: the evidence is scattered across heterogeneous databases, and portfolio-level questions about where funding goes naturally cascade into questions about who receives it and what impact it generates.
}

\newlyadded{
Here, a SciSci researcher could begin by asking \systemname for a portfolio overview: 
\textit{``For grants awarded by the National Institute on Aging, show the total funding amount by Level 0 research field, sorted from highest to lowest.''} 
% Through the plan–action–execution loop, 
The system searches for the funder, filters grants to those awarded by the NIA, joins each grant to its field classification, and aggregates funding by field, returning a ranked bar chart that spans multiple top-level research fields (Fig.~\ref{fig:Figure5}a, c). 
The portfolio is dominated by the four top-funded grant fields: \textit{biological sciences}, \textit{health sciences}, \textit{biomedical and clinical sciences}, and \textit{psychology}.
}

\newlyadded{Noticing this concentration, the researcher might turn from the funding to the recipients, asking who leads the research these grants support. 
To investigate, the researcher could brush the bars for the three top-funded fields using direct manipulation (Fig.~\ref{fig:Figure5}a) and pose a follow-up query: 
\textit{``Compare the gender shares of principal investigators within these selected fields using a grouped bar chart, and include an additional ``Overall" group showing the gender share across all fields.''} 
Taking the brushed region and the natural-language request as joint inputs, the system maps the selected bars back to their field conditions and inherits the NIA scope from the parent figure, so that every downstream comparison remains within the same portfolio. It then computes the share of distinct principal investigators (PIs) by gender within each field and constructs the requested ``Overall" baseline across all NIA grants.
% , a comparison group absent from the visual selection itself. 
The resulting grouped bar chart (Fig.~\ref{fig:Figure5}b) reveals a consistent imbalance: male PIs outnumber female PIs in every top-funded field, with the disparity in \textit{biological sciences} and \textit{biomedical and clinical sciences} exceeding the overall gap.
}

\newlyadded{
Given this finding regarding representation, the researcher might shift their focus to the question of research impact, asking whether the impact of grants led by female PIs differs from that of grants led by male PIs. 
To investigate this question, the researcher might select the single bar representing \textit{biomedical and clinical sciences} and issue a computationally precise request:
% Representation, however, is only part of the story. 
% The researcher next asks if grants led by female PIs differ in the resulting impact.  
% The researcher selects the single bar representing \textit{biomedical and clinical sciences} and issues a computationally precise request: 
\textit{``For this selected field, use a radar chart to compare male and female PIs' average grant-level impact. Use the precomputed impact metrics (number of publications, patents, clinical trials, and citations from policy documents, news, patents, and clinical trials). Average each metric over PI-grant records within each gender, then normalize each dimension by the maximum across the two genders.''} 
The system translates this specification into the corresponding aggregation pipeline: 
it averages the seven precomputed impact measures over PI–grant records within each gender, applies the normalization, and renders an overlaid radar chart (Fig.~\ref{fig:Figure5}d). 
% The two impact profiles are comparable in overall shape but differ in composition. 
% Average publication counts are nearly identical, and grants led by male PIs score higher on patent-oriented dimensions (patents produced and citations from patents) and on clinical trials conducted, whereas grants led by female PIs attract more citations from clinical trials, policy documents (17.0 vs. 12.6 per PI–grant record), and news media. 
While female PIs are underrepresented in this heavily funded field, the chart shows that their grants perform at least as well on many of the impact measures examined here: average publication output is nearly identical, and grants led by female PIs record higher average citations from policy documents, news media, and clinical trials---a pattern that prior analyses had not surfaced.
% echoing patterns surfaced by dedicated funding-impact analyses~\cite{wang2025funding}.
}


\todiscuss{
Though descriptive, this asymmetry between representation and realized impact bears directly on evidence-based funding allocation and merits systematic investigation---for example, controlling for career stage, funding scale, and team composition.
Notably, conventional gender-gap analyses, which center on publications, citations, and funding amounts~\cite{lariviere2013bibliometrics,huang2020historical,oliveira2019comparison}, would not surface this pattern. It becomes visible only when grants are connected to their downstream societal uses through newly available data linkages~\cite{yin2022public, wang2025funding}. \systemname helps the researcher to extract a concrete visual finding  from these complex raw tables in a short sequence of intuitive and efficient interactions.
% This case study illustrates how our tool compresses a multi-stage funding-impact analysis---one that traditionally requires purpose-built visual analytics systems~\cite{wang2025funding} or ad hoc scripting---into a chain of three linked figures driven by natural language and direct manipulation. 
% 
% Each interaction progressively narrows the analytical scope, from an agency's portfolio, to the demographic composition of its top-funded fields, to gender-specific impact profiles within a single field, while provenance guarantees that every comparison remains anchored to the same underlying funding portfolio.
}

% \textbf{Draft figure caption. }Figure X: Case study: the impact of science funding. (a) The ranked bar chart was generated for the initial query, showing total NIA funding across 22 Level 0 research fields. (b) After the user brushes the three top-funded fields, the grouped bar chart compares gender shares of distinct PIs within each selected field, alongside an Overall baseline computed across all fields. (c) After the user selects the bar for Biomedical and Clinical Sciences, the radar chart compares male and female PIs' average grant-level impact across seven normalized dimensions (publications, patents, clinical trials, and citations from policy documents, news, patents, and clinical trials).


\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260831-five-new-cases/case-3-and-4-funding-impact-and-disruption-20260916.jpg}  
    \vspace{1pt}
    \caption{
        \bodyfigurelabel{fig:Figure5}
        \newlyadded{
            \textbf{Case studies:}
            \textbf{(a-d) Impact of science funding.} 
            Starting from the distribution of grant funding across research fields \textbf{(a, c)}, the researcher could compare the gender composition of principal investigators (PIs) within the brushed fields \textbf{(b)}, then zoom into a single field to contrast the multidimensional impacts of male- and female-led grants in a radar chart \textbf{(d)}.
            Color encodings are designed to be semantically aligned across all figures within the same data-driven artifact.
            \textbf{(e-i) Disruptive science across fields and nations.}
            Beginning from a replication of a known macro-level pattern~\cite{park2023papers} \textbf{(e, f)}, new insights emerge as the analysis is drilled down to the relative ranking of disruption scores across countries \textbf{(g-i)}.
        }
    }
    % \label{fig:case-1}
\end{figure}






\subsubsection{\newlyadded{Case Study 4: Disruptive Science Across Fields and Nations}}
% \subsubsection{\newlyadded{Science Impact Across Fields and Nations}}

\newlyadded{
The final case study explores whether science is losing its capacity to disrupt, which has become a central concern in the SciSci community, fueling debates over whether scientific progress is slowing despite the exponential growth in the scientific literature~\cite{jones2009burden, park2023papers, wu2019large}. 
To examine this question, a SciSci researcher could use \systemname and the integrated SciSciNet dataset~\cite{lin2023sciscinet} in a reproduce-then-extend exploration, first replicating established macro-level findings and then carrying the same analytical chain into largely unexamined dimensions.
% In this case, we first use \systemname to reproduce existing macro-level patterns and then to interrogate the heterogeneity beneath them.
}  

\newlyadded{The SciSci researcher might begin this exploration with an aggregate view: \textit{``Show the average disruption score of papers by publication year from 1950 to 2015.''} 
The system aggregates paper-level disruption scores by publication year and returns a line chart (Fig.~\ref{fig:Figure5}e), which shows that the average disruption declines persistently across the entire period. 
% The system aggregates paper-level disruption scores by publication year and returns a line chart (Fig. Ya) that reproduces the canonical finding: average disruption declines persistently across the entire period~\cite{park2023papers}. 
The researcher could then drill down into the analysis: 
\textit{``Split this line into multiple lines to compare the top five research fields (Level 0) with the most papers.''} 
The system shifts from figure generation to manipulation: it identifies the five fields with the most papers, augments the existing aggregation with a field grouping, and updates the visual encoding in the figure, transforming the single trend into five field-level trajectories (Fig.~\ref{fig:Figure5}f). 
All five fields decline, though at different rates: physics and chemistry, initially the most disruptive, fall most sharply, while computer science declines more gradually, rising in relative rank from last to near the top.
% The updated figure shows that the decline is pervasive—every major field trends downward—but far from uniform: physics and chemistry, the most disruptive fields at mid-century with average scores more than double that of computer science, fall steeply, whereas computer science starts lowest yet declines most gently, ending the period among the most disruptive fields on a per-paper basis.
}

\newlyadded{This field-level heterogeneity and the aggregate decline replicate patterns documented in prior work~\cite{park2023papers}. Whether these trends extend uniformly across nations, however, remains largely unexamined in this literature. 
The researcher might therefore move from replication to new analysis by selecting the line for \textit{medicine} and posing a computationally precise follow-up request: 
% This heterogeneity raises a sharper question: 
% within a field, is the geography of disruptive research stable? 
% The researcher selects the line representing computer science and poses a computationally precise follow-up: 
\textit{``For the selected field, from 2000 to 2015, compare countries by average disruption score, counting each paper once per country (deduplicate multiple authors from the same country). Then among the 20 countries with the most papers in the selected field over this period, rank the countries within each year by average disruption score (rank 1 means the highest; ranks range from 1 to 20 within the 20-country pool). Show the annual rank trajectories of only the five countries with the most papers, as a multi-line chart.''}
% 
The system executes the corresponding multi-step analysis: it restricts the sample to the twenty largest producers, computes within-year ranks, plots trajectories for the five highest-volume countries, and returns a rank-trajectory chart (Fig.~\ref{fig:Figure5}g). 
% (\eg, deduplicating authorship so that each paper counts once per country, restricting the pool to the twenty largest producers, computing within-year ranks, and displaying the five highest-volume countries) 
The resulting chart shows that national standings in this field evolve only gradually. The five largest paper producers remain in the upper half of the twenty-country pool throughout the period, with the United States and China trending slowly upward and the United Kingdom and Japan trending slowly downward over this period.
% decade-long movements with no abrupt reordering of the hierarchy
% coordination 
Selecting another field and repeating the request re-executes the same pipeline with only the field condition changed. For \textit{computer science}, however, the result is strikingly different (Fig.~\ref{fig:Figure5}h, i): 
China rises from near the bottom of the twenty-country pool in the early to mid-2000s to the top ranks between 2008 and 2011, remaining there through 2015 while several incumbent leaders gradually decline.
}

% conclusion
\todiscuss{
These trajectories suggest that beneath the universal decline in average disruptiveness lies an actively shifting national landscape, and that its dynamics are field-specific.
% : abrupt ascents, as in China's rise in computer science during a period of rapid national expansion of computing research, coexist with gradual, sustained climbs, as in the United States in biology and chemistry. 
% Because the ranking conditions on the largest producers and counts each paper once per country, these shifts reflect changes in the average disruptiveness of national research output rather than sheer publication volume—precisely the kind of compositional dynamics that aggregate indicators conceal [Park et al. 2023].
% As in the previous cases, every derived statistic remains auditable: expanding each figure's reasoning process exposes the deduplication, pooling, and ranking steps as executable operations, and the full chain—from the reproduced global trend to the national rank trajectories—is preserved as a data-driven artifact that can be re-executed for any field, period, or country pool. 
As concerns about the declining disruptiveness of science mount, the ability to track not only whether disruption is falling but also where and for whom it is rising or eroding can directly inform science policy debates about research portfolios and national competitiveness.
This case study thus illustrates a reproduce-then-extend mode of exploration that LLM-native figures make natural: a published macro-level pattern is first re-established as a verifiable starting point and then progressively decomposed, by field and then by nation, through figure extension and user interactions. 
}

% \textbf{Draft figure caption.} Figure Y: Case study: disruptive science across fields and nations. (a) The line chart generated for the initial query, showing the average disruption score of papers by publication year (1950–2015) and reproducing the aggregate decline reported in prior work. (b) The same figure after an in-place edit that splits the trend by the five research fields with the most papers, revealing pervasive but heterogeneous declines. (c) After the user selects the computer-science line, the follow-up figure ranks the twenty largest producing countries by average per-paper disruption within each year (2000–2015; rank 1 = highest, y-axis inverted) and displays the five highest-volume countries, revealing China's abrupt ascent into the top ranks around 2008–2011.







\subsection{Computational Evaluation}
\label{subsection:computational-evaluation} 
To further assess the feasibility of LLM-native figures, we use \systemname to evaluate the fidelity of the bidirectional mapping mechanism (Sec.~\ref{subsection:conceptual-framework}), the core design for figures to function as reliable computational interfaces.
Specifically, we test whether: 
(1) user questions can be accurately transformed into visual data insights (\ie, Analytical operations → Visualization), and
(2) visual interactions, such as clicking or brushing on a figure, can be accurately mapped back to the intended subsets of underlying data and the appropriate analytical operations (\ie, Visualization → Analytical operations). 
% We focus on this functional validation rather than human-subject user studies, as the primary contribution of this work is a computational representation and reasoning framework rather than an interface implementation.

% \wyf{
% Low-level differences arise only when the original analysis involves non-deterministic operations, such as stochastic analytical operations.
% \textbf{Round-trip reproducibility.}
% In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
% Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% }

%\textbf{Mapping fidelity.} 
\textbf{Test Design}.  
We adopt a structured, coverage-oriented evaluation strategy that treats mapping fidelity as a functional correctness problem over a well-defined interaction space. 
Using the datasets from our Case Study 1, we construct a test suite of paired queries. Each test case includes an initial user question that requires the generation of a figure, and a follow-up question that depends on a specific visual interaction with that figure to produce a new or updated visualization. 
This design mirrors realistic usage patterns in which users alternate between language-based queries and direct manipulation.

To ensure systematic coverage and reduce evaluator bias, we use an LLM to generate  \wyf{308} valid test cases, each with three sub-tasks (Supplementary Note 3.1). 
Test cases are diversified along three dimensions: 
(1) figure type (\eg, bar charts, line charts, pie charts, scatter plots, and tables),
(2) interaction type (\eg, single-mark selection, one-dimensional interval brushing, and two-dimensional brushing), 
and (3) analytical complexity, with tier 1 cases representing simple scenarios involving a single table and minimal transformation, and tier 2 cases reflecting realistic workflows that require joins across multiple tables, aggregations, or modeling operations.
% and (4) reference solution logic, which specifies the expected data subset, transformation steps, and analytical outcome for each case.
% Representative examples of the test cases are provided in the Supplementary Information (Supplementary Note~\ref{subsection:si-computational-evaluation}). 
% 
We evaluate mapping fidelity along both directions of the language–visualization loop using three metrics across all test cases.
\textit{Execution Success Rate} is the proportion of test cases in which the system successfully completes the end-to-end execution and returns a usable visualization artifact (i.e., no execution failure and a chart is generated).
\textit{Conditional Accuracy} (conditional on success) is the proportion of cases in which the generated analytical process and results are semantically and logically correct with respect to the user's intended analysis.
\textit{End-to-End Accuracy} is the proportion of cases in which the figures are both successfully generated and analytically correct. 

\textbf{Results.}
% 1. analysis -> vis
We first assess the mapping from analytical operations to visualization using the initial question in each test case. 
Given a user instruction, \systemname generates a sequence of actions to retrieve and analyze data and produce an interactive figure. 
We evaluate the correctness of the generated code (SQL, Python, and Vega-Lite), the retrieved data subset $D$, and the resulting figures through manual inspection by two authors and cross-validation with the generated LLM-based solution (Supplementary Note 3.2).
\systemname achieves an overall \textit{Execution Success Rate} of \wyf{$96.7\%$} and \textit{End-to-End Accuracy} of \wyf{$92.7\%$} (Fig.~\ref{fig:Figure6}-Initial Question). 
Most inaccurate cases stem from SQL generation errors, such as failures to perform fuzzy matching for user-specified concepts (\eg, querying “Computer Science” verbatim when the database stores ``computer science'') and misidentification of the analytical entity (\eg, returning counts of researchers instead of papers). 
% the accuracy of generating incorrect Vega-Lite is low, only one case mis-encode the y axis attribute. 
% Specifically, the accuracy of correctly generating data filtering and transformation queries (SQL), together with optional analytical code (Python), is \wyf{xx}. 
% Conditional on correct data retrieval, the accuracy of generating valid visualization specifications is \wyf{xx}. 
% Figure~\ref{??} further breaks down performance by visualization type, showing consistently high success rates across chart categories.
% \wyf{Add one sentence to discuss chart type variations.}
% 
% 
% 2. vis -> analysis (two methods: follow-up question-answering, coordination)
% Note: We only need to calc the accuracy of SQL step in 2nd figure generation, no need to calc vis generation step.

Second, we assess the mapping from visualization back to analytical operations using two approaches: follow-up question-answering and inter-figure coordination. 
% 2.1 follow-up question-answering
In the follow-up question-answering task, for each figure–interaction pair, \systemname maps selected visual marks to a data query via the relation $R_t$ and generates the corresponding analytical actions. 
We examine the results of the generated SQL query $C$ and the retrieved data subset $D$. 
% 
When users select visual marks or regions on the figure, the system correctly infers the corresponding data filtering and transformation logic with \wyf{$79.8\%$} \textit{End-to-End Accuracy} (Fig.~\ref{fig:Figure6}-Follow-up Question, SQL generation). 
% failure analysis
% Among the cases with inaccurate SQL generation, 
We observe that occasional inaccuracies arise when translating GUI interactions (\eg, brushing or clicking) into SQL filtering logic.  
For instance, a continuous x-axis brush with a range of $[a, b]$ may be incorrectly mapped to a discrete ``IN'' predicate rather than a ``BETWEEN'' range condition. 
This problem highlights the need for more explicit guidance, such as structured prompts or interaction-aware constraints, to ensure that GUI-derived filtering semantics are faithfully translated into SQL predicates in future LLM system designs. 
% 2.2 coordination update
For inter-figure coordination, when users select or brush an updated region of interest, the system updates the coordinated figure by modifying the underlying SQL query to retrieve the corresponding data. 
The resulting \textit{End-to-End Accuracy} is \wyf{$91.0\%$} (Fig.~\ref{fig:Figure6}–Coordination).
% Most inaccurate cases arise from errors in updating SQL filtering logic in response to new user interactions (\ie, brushing a new region on a figure), typically due to the introduction of unnecessary filtering conditions or incorrect substitution of the original query predicates. 
% The majority of inaccurate cases are typically due to introducing unnecessary filtering conditions or incorrectly substituting the original query predicates. 

% 3. round-trip reproducibility
%\textbf{Round-trip reproducibility.}
%Because all actions, code, and parameters used to generate a figure are explicitly recorded, each LLM-native figure artifact preserves complete analytical provenance. 
%This design, by nature, enables deterministic reconstruction of the original figure by re-executing its stored codes against the underlying data. 
% as all the actions and codes of generating a figure have been recorded, our LLM-native figure artifact by nature preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
%In the majority of cases, reconstructed figures are identical to the originals at both the specification and visual levels, as the analytical workflow and visualization code are deterministically stored and replayed. 
%Deviations arise only when the original analysis involves inherently non-deterministic procedures, such as stochastic analytical operations (e.g., dimensionality reduction or random sampling without fixed seeds). 
%In these cases, discrepancies are confined to low-level visual variation or textual content, while the underlying analytical intent and semantic conclusions remain unchanged (Supplementary Note 3.3).
% including LLM-generated textual summaries and 
% High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mapping_fidelity.pdf}
    \vspace{1pt}
    \caption{
       \bodyfigurelabel{fig:Figure6}
       \textbf{Computational evaluation results.}
    }
    % \label{fig:computational-evaluation}
\end{figure}




\subsection{\newlyadded{User Study}}
\label{subsection:user-study} 

\newlyadded{To assess the potential benefits of LLM-native figures and data-driven artifacts for researchers, we conducted a within-subject user study in which SciSci researchers interacted with \systemname, our instantiation of the design. 
This study complements the computational evaluation in Sec.~\ref{subsection:computational-evaluation}, which established the fidelity of the bidirectional mapping, by examining how researchers use the system in practice to conduct exploratory analyses. 
In this study, participants performed two exploratory data analysis tasks adapted from the case studies above, using \systemname for one and a baseline representing their conventional workflows for the other. 
We \todiscuss{measured task success, completion time, perceived workload, perceived usability, and perceived value}. 
We also collected researchers' qualitative feedback on how working with \systemname affected their use of figures and their scientific discovery process. 
}


\subsubsection{\newlyadded{Participants and Study Procedure}}
\label{subsection:participants-and-study-procedure} 

\newlyadded{\textbf{Participants.} 
We recruited 12 SciSci researchers (P1--P12) through professional networks, including 5 women and 7 men, aged 24--45 years ($M = 31.3$). 
Participants spanned multiple career stages: 2 predoctoral researchers, 3 PhD students in their third year or later, 5 postdoctoral researchers, and 2 research assistant professors. 
Their experience with quantitative data analysis ranged from 3 to 10 years. 
All participants routinely analyze large-scale SciSci data and reported prior experience using LLM-based coding assistants (\eg, Claude Code~\cite{claudecode} and Codex~\cite{codex}) for code generation and for creating and editing visualizations. 
None of the participants was involved in the development of \systemname or had used it before the study. 
% Detailed demographic information is provided in \todiscuss{Supplementary Table xx}.
}

\newlyadded{\textbf{Baseline.}
The baseline system had the same computational setup as \systemname, including the server, coding environment, and database access. 
Researchers could use their preferred conventional tools (e.g., VS Code and Jupyter notebooks) and programming languages, and they had access to LLM assistance through Claude Code~\cite{claudecode}, allowing them to follow their typical data analysis workflows.
We asked participants to use Claude Sonnet 4.5 in the baseline, the same model that powers \systemname, so that differences between the two conditions could be attributed to the system design rather than to the underlying models' capabilities.
}

\newlyadded{\textbf{Study Procedure.} 
Each study session was conducted remotely via Zoom with screen sharing and lasted approximately two hours. 
Participants first completed a consent form and a demographics questionnaire. 
We then introduced the project background and provided a 15-minute \systemname tutorial using the climate change example from Sec.~\ref{subsection:conceptual-framework}.
Researchers could ask questions throughout the tutorial to clarify their understanding. 
We also helped them set up the baseline environment and gave them time to configure it to match their preferred data analysis workflows.
% 
% 
Next, we asked researchers to reproduce two exploratory data analysis tasks adapted from the case studies (Sec.~\ref{subsubsection:case2-science-policy} and Sec.~\ref{subsubsection:case3-funding-impact}). 
For each task, we provided natural-language data analysis requirements, reference chart types~\cite{ren2017chartaccent, ren2018reflecting}, and the data schema and descriptions of the underlying database. 
The tasks were decomposed into a series of analysis questions delivered one at a time, collectively covering core system features, such as figure generation, extension, and coordination analysis.
Each participant completed both tasks, using \systemname for one and the baseline system for the other. 
To fully counterbalance task-condition assignments and condition order, we used all four possible combinations (e.g., Task 1 with \systemname followed by Task 2 with the baseline, or the reverse) and assigned three participants to each.
In each task, participants worked through the steps at their own pace and were encouraged to think aloud. 
After each task, participants filled out a questionnaire to evaluate the tool's usability and a questionnaire to assess their perceived workload. 
After completing both tasks, participants answered another questionnaire on the practical value of the tool and user experience of \systemname's core features. 
We then conducted a semi-structured interview about their experiences, comparisons with their conventional workflow, and the tool's potential practical impact. 
\todiscuss{Please refer to \todiscuss{Supplementary Note xx} for the materials used in the user study.} 
This study was approved by the Institutional Review Board of Northwestern University. 
}



\subsubsection{\newlyadded{Results}}

\todiscuss{\textbf{Task performance.} 
1. completion time
2. accuracy
We review the analysis results from \systemname and the baseline. 
placeholder for now.
}

% 2. SUS & NASA-TLX 
\newlyadded{\textbf{Perceived usability}.
% 1. Overall statistical results
We assessed the tool's perceived usability using the System Usability Scale (SUS)~\cite{brooke1996sus}. 
Researchers rated \systemname as substantially more usable than the baseline ($M = 89.4$, $SD = 10.7$ for \systemname; $M = 64.8$, $SD = 20.1$ for the baseline).
% (SUS: $M = 89.4$, $SD = 10.7$ vs. $M = 64.8$, $SD = 20.1$; mean difference $24.6$, $95\% CI$ $[13.5, 35.0]$; Wilcoxon signed-rank $W = 3$, $p = 0.002$, $r = 0.92$). 
% \systemname falls in the "excellent" range, whereas the baseline falls between "OK" and "good"~\cite{bangor2008empirical}. 
Eleven of the twelve participants gave \systemname a higher usability score than the baseline. Eleven also rated \systemname above the conventional benchmark of 68~\cite{sauro2011practical}, compared with five who rated the baseline above this threshold.
}
% % 2. Different dimensions
% Item-level comparisons (Supplementary Fig. S1) show that the difference is driven by integration and consistency of functions (Q5, Q6), cumbersomeness (Q8), and ease of use and learning (Q3, Q7, Q10), whereas willingness to use the tool frequently (Q1) and confidence (Q9) were high in both conditions, consistent with participants' extensive prior experience with LLM coding agents.
% % 3. Interview results to explain the results
% xxxx
% DirectGPT: "On the System Usability Scale, and for the specifc given tasks, DirectGPT was rated 92 (typically considered “Excelent” [4]) whereas ChatGPT received a 53 (typically considered “OK”). This corresponds to a mean diference of 39 (95% CI: [27.3, 47.34], p<0.001)."


\newlyadded{\textbf{Perceived workload.}
Study results indicate that \systemname reduced participants' perceived workload.
We used the NASA Task Load Index (NASA-TLX)~\cite{hart1988development} to estimate the users' perceived cognitive load (Fig.~\ref{fig:Figure7}). 
% overall
Participants reported significantly greater workload in the baseline condition  ($M = 3.21$, $SD = 1.26$) than in the \systemname condition ($M = 1.89$, $SD = 0.81$), based on the average score of the six NASA-TLX items (Wilcoxon signed-rank, $p = .009$).
% individual breakdown
At the item level (Fig.~\ref{xx}), \systemname received significantly lower ratings than the baseline for mental demand ($p = .047$), physical demand ($p = .023$), and frustration ($p = .039$). 
Differences in temporal demand, performance, and effort were not statistically significant. 
All item-level p-values were Holm-corrected across the six subscales. 
These results suggest that \systemname substantially reduces the perceived cognitive and physical burden of conducting the analysis tasks and makes the overall process less frustrating.
}


% 3. 9 项 5 点 Likert
\newlyadded{\textbf{Perceived value of \systemname's design components.} 
We also analyzed participants' ratings of the usefulness of nine \systemname design components (Fig.~\ref{fig:Figure7}) with a 5-point scale (1 = not at all useful; 5 = extremely useful). 
% 1. Overall statistical results
All nine design components received positive ratings, with a mean above $4$ for every component. 
% 2. individual results
% 2-1. positive results
Bidirectional mapping and data-driven artifacts received the highest usefulness ratings, while the two data-management components also received high ratings. 
% Bi-directional mapping and data-driven artifacts were rated most useful which are also the core design components of our work. 
% The two data-management components, the SciSci domain database and the chat-history database, were both rated highly. 
% 2-2. negative results and discussions
Within the multi-agent engine, the workflow itself received high ratings overall ($M = 4.50$, $SD = 0.90$). However, one researcher rated it a 2, explaining that the multi-agent workflow was largely invisible to the user and the user could not directly perceive how the module operated. 
Notably, this participant nevertheless found the visible action-level reasoning useful.
Action-level reasoning received the lowest usefulness rating, although it remained positive ($M = 4.25$, $SD = 0.75$). 
Researchers generally found the streamed sequence of actions more structured and interpretable than a raw chain of thought, but preferences for the level of detail varied. 
Some wanted concise summaries of the analytical rationale behind key steps, while others preferred minimal information resembling a lightweight progress indicator rather than an explicit reasoning trace.
}

\begin{figure*}[t]
    \centering

    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/20260907/fig_tlx.pdf}
        \label{fig:feature_ratings}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/20260907/fig_feature_ratings.pdf}
        \label{fig:tlx}
    \end{subfigure}

    
    \caption{
       \bodyfigurelabel{fig:Figure7}
       \textbf{User study results.} 
    }
    % \label{fig:ratings_tlx}
\end{figure*}


% 4. Results from semi-structured interview.
\newlyadded{\textbf{Qualitative findings.}
In addition to the quantitative results on efficiency and workload, semi-structured interviews and think-aloud observations across the twelve sessions revealed three broad ways in which \systemname shaped scientific discovery. 
}

% --- Pros ----
% 1. GUI selection and interactive figures
\newlyadded{\textit{(1) Figures as interfaces for iterative discovery.}
% 1. interactive vis + LUI and GUI: make exploration more effecient and accurate
Direct manipulation of interactive figures transformed analytical operations that were awkward, inefficient, or infeasible in the baseline into lightweight visual interactions. 
All six researchers who completed the science policy task with the baseline had to approximate regions of interest using coordinate ranges, annotated screenshots, or repeated prompting.
In \systemname, researchers could instead select visual marks directly and carry those selections into subsequent analyses, reducing both interaction overhead and ambiguity in specifying analytical intent. 
Participants particularly valued the ability to derive new coordinated analyses from an existing figure and selection, replacing analytical steps that otherwise required manually modifying and rerunning code.
}

% 2. bring in new data exploration approaches beyond traditional data analysis methods
\newlyadded{More importantly, LLM-native figures changed how researchers explored data. 
Direct manipulation of these interactive figures lowered the cost of inspecting regions, subgroups, and relationships, while also prompting analyses that participants said were absent from their usual workflows. 
Researchers zoomed in on local clusters, examined subpopulations and unanticipated gender differences, and proposed extensions incorporating new variables or subgroup comparisons. 
By making emerging questions easier to pursue, interactive figures allowed new directions of inquiry to arise directly from patterns encountered during exploration.
}
% Direct manipulation enable users to inspect regions, subgroups, and relationships faster with lower cost, and also bring new exploration aspect in they reported would not normally form part of their conventional analysis workflow 
% For example, participants zoomed into localized clusters, drilled down into selected subpopulations, examined gender differences that had not been specified in advance, and proposed extending published analyses with additional variables or subgroup comparisons. 
% These observations suggest that treating figures as interactive analytical interfaces can lower the cost of pursuing emerging questions, allowing new directions of inquiry to arise directly from patterns encountered during exploration rather than requiring them to be fully articulated in advance.


% 2. Data-driven artifact and Canvas as externalized reasoning / mind map;
\newlyadded{\textit{(2) Data-driven artifacts as externalized reasoning trace.} 
Researchers repeatedly contrasted the data-driven artifact with the linear histories of computational notebooks and chats, in which branching analyses are compressed into a sequence, and the relationships among them must be maintained mentally. 
Several described the artifact as a ``mind map'' or ``mind-space'': by externalizing alternative branches, intermediate results, and their relationships, the artifact reduced the cognitive burden of tracking a project and made it easier to resume earlier directions or selectively extend particular branches. 
This externalized structure also supported communication across time and among collaborators; for example, participants saw value in using the artifact to reconstruct the reasoning behind previous decisions during advisor or team meetings, rather than rediscovering lost ideas between sessions.
% 
Participants also valued the mechanisms that preserved this reasoning trace. For example, version rollback allowed researchers to revisit earlier states without contaminating the current conversational context. 
% while anchoring intermediate states made errors easier to trace to the step at which they emerged. 
% future suggestions
They suggested future extensions to support richer reasoning structures, including parallel branches beyond subgroup drill-downs, multiple root figures within an artifact, merged branches, and text-based intermediate analyses as first-class nodes. 
They also wanted the ability to delete nodes and to record each brushing or coordination state as a revisitable version.
}

\newlyadded{More broadly, preserving a non-linear exploration history opens the possibility of carrying scientific reasoning across sessions, collaborators, and ultimately into the scholarly record itself. 
Papers typically preserve the outcomes of discovery as a coherent retrospective narrative while leaving much of the intellectual trajectory behind them undocumented: which prior work first inspired an idea, how initially separate observations became connected, why some directions were abandoned, and which unexpected findings redirected the inquiry. 
% Much of this reasoning provenance therefore disappears with the researcher who performed it. 
Data-driven artifacts could make this otherwise ephemeral layer of science persistent, inspectable, and shareable. 
% This missing layer may become particularly consequential as AI systems increasingly participate in discovery: learning to generate hypotheses or execute analyses is different from learning how scientists recognize promising leads, navigate competing possibilities, and decide what is worth pursuing. 
Externalized exploration traces could therefore provide not only a richer record of how science develops, but also a new substrate for grounding future AI systems in the process of scientific discovery rather than only in its published outcomes.
}


% 3. Verification via download / provenance used in session; T3 Replication package / SI / open science
\newlyadded{\textit{(3) Provenance as basis for reproducibility and sharing.} 
Because every figure carried its data and code, verification became part of the analysis rather than a separate recovery step. 
% P11 downloaded the underlying records twice to check the topic labels the system produced for two clusters ("Let me check … ACA, e-cigarettes … yeah, this looks correct"), P10 did the same and found a label that was too specific ("it's just cigarettes, not specifically electronic"), and P01 read the exported action file while waiting for a result. 
% This contrasts with the baseline, where provenance existed only if participants asked for it — 
% P08 had Claude Code emit a standalone HTML page with no saved code, and P03, when asked to check a result, observed that "there must be code in the back end, but I didn't ask it to output it." 
Researchers identified three broader uses for these artifacts. 
First, for replication and open science, participants saw value in preserving downloadable code to support reproducibility and requested additional features such as automatically generated replication packages and exportable runnable notebooks for inclusion in supplementary materials. 
% P06 asked whether the artifact could generate the replication package he finds "quite a hassle" to assemble, P03 wanted a one-click export to a runnable notebook "convenient to upload as SI," and P12 and P02 noted that downloadable code makes results "easier to replicate" and serves "open science." 
Second, for portability, they valued the ability to move an artifact across sessions and reopen it later without losing the computational context accumulated during a long conversation. 
They also proposed allowing users to copy an artifact into a new session while preserving the project's full exploration trajectory. 
% Second, portability: P06 wanted to move an artifact into a fresh session when a long chat's "memory messes things up," because "if I only paste an image over, it wouldn't know what it is," and P04, P10 and P11 valued reopening an artifact later ("that's super useful … unique," P04). 
Third, for science communication, participants envisioned publishing interactive artifacts alongside papers so that audiences could inspect subgroups, analytical paths, and supporting evidence, thereby making findings more accessible and increasing trust in the exploration process.
% Third, for science communication: P05 imagined a paper shipping "a traditional version plus a logic diagram of the visualization" so that "when the audience questions a sub-group, I click into it … it's defensible"; P08 argued that publishing the figure itself as an interactive artifact matters more than full replication because "people just look at the figures"; and P09 expected such artifacts to raise readers' trust "in your exploration process." 
At the same time, participants emphasized that raw code alone was insufficient to establish trust, and they differed in the types of evidence they wanted to examine. While some requested analytical step summaries, others preferred access to the underlying data or independent cross-tool verification. 
These differences suggest that provenance mechanisms will need to adapt to researchers' heterogeneous verification strategies. 
}
% they preferred concise, step-level summaries and linked views of figures, data, and actions over long execution logs.
% At the same time, participants were clear that raw code is necessary but not sufficient for trust: P03 asked for "a summary — which steps I did and what each step did," because "a person can't check line by line"; P10 wanted a per-step data panel; P08 said he would never read the action log ("it is very long") and verifies with cross-check analyses instead; and P05 considered figure–code–data linkage only a more intuitive version of what a notebook already provides.}

\newlyadded{\textbf{Design suggestions.}}
% 1. intergrate their own datasets
\newlyadded {Participants identified several opportunities to improve \systemname and extend its capabilities. The most common request was support for analyzing researchers' own or locally stored datasets with \systemname, which several participants viewed as the primary remaining advantage offered by general-purpose coding agents over \systemname. 
% P08 identified this as Claude Code's one remaining advantage, and P03 said that with local-data connection and web access the system would be "more useful than Claude."
% 2. LUI limitation - widgets rather than natural language; GUI limitation: selection limits
Participants also asked for greater interaction flexibility, including natural-language control over visual styling, style transfer from reference figures, parallel analyses and multiple root charts, annotations attached to nodes, notebook or full-package export, and lightweight interaction guidance. 
They further requested more expressive graphical selection mechanisms, such as persistent brushes across queries, multiple concurrent selections, and a natural-language fallback when built-in interactions were insufficient. 
% The second concerned flexibility: widgets rather than natural language for cosmetic edits such as colours (P09), style transfer from a reference figure (P06), parallel analyses and multiple root charts (P05, P08), notes and rationale attached to nodes (P08, P11), notebook or full-package export (P03, P04), per-chart interaction guides or an onboarding tour (P04, P08), and AI-proposed next questions when a mark is clicked (P09, P06). 
% Latency was mentioned by four participants, and we logged nine distinct interface bugs (Supplementary Note X), none of which affected task correctness except one wrong initial chart for P12.
% Researchers also mentioned limits of the current selection vocabulary: they wanted a brush to persist so that successive questions condition on exactly the same marks (P03), several selections and their results kept side by side (P01, P03, P12), statistically defined rather than hand-picked outliers (P06), and a natural-language fallback when a chart's built-in interactions do not cover a need (P08); two participants initially confused click and brush, and the selection tooltip was flaky (P02, P04, P09, P10).
% 3. other engineering issues: action reasoning - more information; system latency
Finally, several participants requested greater visibility into multi-step reasoning and faster system responses.
% P08 valued seeing "the results of multi-step reasoning at the same time," which he currently approximates by asking Claude to run every possible analysis at once and picking afterwards,
% Latency was mentioned by four participants.
}



% 0. Nexus faster / smoother / fewer prompts -- cross-validate above results
% \textit{(1) Efficiency, usefulness, and workload.}
% Participants attributed the usability and workload differences in the questionnaires to two concrete sources. 
% The first is the number of exchanges needed to get a usable result: 
% P07 found \systemname "a lot less redundant … less prone to errors, as we saw," having said of the baseline "this is why I don't use Claude, it takes too long"; P02 called the action-by-action output "more modular … clearer, more intuitive" than Claude's text; 
% P10 rated \systemname "not complex at all" with effort "very low" while calling his usual double-checking across "two or three" agent sessions "actually still pretty hard to use"; 
% and P08 concluded that, apart from the ability to run on his own data, "your system is more intuitive and easier to use." 
% % 
% The second source is where baseline time went. 
% Setting up the notebook environment cost between 13 and 30 minutes for three participants (P01, P07, P12) and caused login or permission problems for others (P03, P05), and, more importantly, verification dominated the analysis itself: P11 spent 26 minutes on the first baseline question "because I couldn't trust … did it use the right variable," P01 caught Claude Code double-counting grants that it had not de-duplicated, and P03 reported iterating "several dozen times" per figure in his daily practice because the agent "makes a bunch of mistakes." 
% The coding agent also over-produced or substituted its own choices (four plot variants for one request, P06; "it's doing much more than I ask it," P04; defaulting to top-cited rather than the first records, P09). Rough timings from the recordings, to be replaced by the coded completion times, show baseline tasks taking 17–60 minutes (median ≈ 31) against 17–31 minutes for \systemname (median ≈ 21), even though interview questions were interleaved into the \systemname tasks. Two caveats matter for interpreting these numbers. The fastest baseline runs were fast because participants did not verify: P02 pasted each instruction straight into Claude Code and finished in 17 minutes, later acknowledging "I really did not check … mine might well have problems," and P06 described his own role in the baseline as "an invisible yes-clicking machine." Conversely, \systemname was not free of cost: chart generation latency was the most common complaint (P01, P02, P09, P12; P02 rated the action-level stream "effective — 5; efficient — no"), a running analysis could not be interrupted or corrected mid-way as the Claude Code extension allows (P01, P05, P09), and interaction bugs forced restarts for P04 and P10, while P12's first chart was the only incorrect generation observed across the twelve sessions. Finally, participants noted that \systemname shifts rather than removes mental effort: P10 rated mental demand as still "fairly high, because the thinking is still very important — what science-policy question you want to investigate."

% --- Challenges ---
% 4. Verification burden as main baseline cost
% 5. Engineering suggestions: Own data / connect local data; Want human-readable step summary / intermediate data; Want less process detail (progress bar); Speed
% 6. Nexus for early exploration, not final figures

% % other limitations: trustness
% The most substantive is trust in intermediate data processing. Participants who work with many-to-many linkages (grants with several PIs and fields) worried that decisions such as de-duplication, unit of analysis, or dropping records with missing fields would be made silently: 
% % note: 我们需要把这些问题frame成：有些情况下数据处理并没有标准的答案，A和B都可以，就看researcher怎么在后期解读 -- 可能两种方法都需要尝试。
% % P01 "did not know how it handles it by default … especially drop-duplicate, this is very key," and P10, who had just noticed Claude Code's SQL excluding grants with missing age, feared that a polished chart would end verification altogether — "if it directly gives me a result, I won't double check, I'll just pass it" — and that "if you have ten processing stages and it makes a decision at each, the result may be slightly biased." 
% The remedy they asked for is not more raw output but a human-readable summary at a level between the action stream and the code ("which steps I did and what each step did … the simpler the better," P03; "a simple overview of how it did it," P01), together with per-step intermediate data (P10), editable actions (P10), and the ability to interrupt and correct a running analysis as the Claude Code extension allows (P01, P05). 
% Notably, other participants wanted less rather than more: P04 would replace the action stream with a progress bar, and P08 said he never reads such logs and verifies through cross-check analyses instead, which suggests progressive disclosure rather than a single level of detail. 
% % 总结：这也反映了不同researcher对HAI合作生成的数据结果的validation的不同要求。需要后期系统中进行个性化配置。



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below: old version (Round-Trip Reproducibility & User Study), temporally abandoned
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Round-Trip Reproducibility}
% \label{subsubsection:evaluation-reproducibility}
% \wyf{Note: test case: lack of LLM-based Python code.}
% We evaluate whether an LLM-native figure artifact preserves complete analytical provenance, such that the original figure can be deterministically reconstructed by re-executing its stored specifications against the underlying data. 
% This evaluation tests whether LLM-native figures function as reproducible computational objects rather than ephemeral presentation outputs.
% % To evaluate whether an LLM-native figure artifact provides complete provenance, enabling precise re-execution of the analytical workflow and deterministic reconstruction of the figure.

% \textbf{Test Design.} 
% We use the same set of 200 test cases described above and store all figures $F_t={V_t, D_t, C_t, M_t}$ generated succesfully during their execution. 
% For each figure, we re-execute the stored code $C_t$ against the original database to regenerate the data subset $D_g$ and the corresponding visualization $V_g$. 
% We then compare the original and reconstructed figures at two levels: (1) specification-level equivalence, assessed via structural comparison of the visualization specifications (JSON); 
% and (2) visual-level equivalence, assessed by matching visual marks, encodings, and positional attributes. 
% We report the proportion of figures that are exactly reproducible at the specification level and those that are visually identical despite potential non-semantic specification differences.

% \textbf{Results.} 
% % High reproducibility demonstrates that the artifact structure is sufficient to replay analytical steps and that figures can serve as standalone, machine-interpretable scientific artifacts.
% \wyf{
% Across the \wyf{180} generated figures, round-trip reproducibility is achieved for nearly all figures. 
% In most cases, reconstructed figures are identical at both the specification and visual levels, as the analytical and visualization code is deterministically stored and re-executed without LLM involvement. 
% This confirms that the artifact captures complete computational provenance.
% % This result must be 100\% correct, as the codes are the same and with no LLM-related component (except the science-policy case: text summary).
% % 
% Deviations occur only in cases involving inherent non-determinism, including LLM-generated textual summaries and stochastic analytical procedures (e.g., dimensionality reduction or random sampling without fixed seeds). 
% In these cases, differences are limited to textual content or low-level visual variation, while the underlying analytical semantics remain consistent.
% }.


% \subsubsection{Discussion}
% \newlyadded{
% Failure analysis (e.g., reproducibility-missing provenance, mismatched encodings, rendering differences). 
% Fill in with a short failure-mode paragraph: e.g., missing spec fields, nondeterministic defaults, or database changes. This will earn reviewer trust.
% \wyf{Erzhuo's suggestion: we also report failure cases with persentage and some examples.}
% }



% \subsection{User Study} 
% \textbf{Participants}: SciSci researchers from different "research age". 

% \textbf{Task}: three case studies, same setting of data. 

% \textbf{Benchmark}: Python/Jupyter Notebook, SciSciGPT. 

% \textbf{Evaluation dimensions}: 
% (1) Efficiency: time and accuracy. -- same analysis tasks in the case study. 
% (2) Expressiveness: number of insights generated. -- do not limit analysis tasks, only limit the high-level research question. To test: the number of insights generated; the diversity of insights generated. 

% \subsection{Expert Interview} 
% (1) Use \textit{Five-point Likert Scale} to allow users score different dimensions of the system: usability, etc. 

% (2) Qualitative evaluation: summarize their feedback in terms of hybrid user interface, LLM agent engine, and suggestions (especially for data-driven scientific discovery and LLM-native figures to be presented in their research paper -- open science related questions). 

==> sections/archive/05-method/05-method-20260127.tex <==
\section{Methods} % Nexus--A Reference Implementation for SciSci Domain}
\label{section:methods}
% Based on this conceptual framework, we further develop a proof-of-concept system, \systemname, to demonstrate how to facilitate scientific discovery using these LLM-native figures with a non-linear human exploration process. 
To demonstrate the broad applicability of this conceptual framework, we present \systemname, an instantiation of the framework that we propose, which is developed for the Science of Science (SciSci) domain---an essential field for understanding and accelerating scientific enterprise and technological innovation.
SciSci provides an ideal testbed with challenges well matched to our framework: 
rich and emerging datasets spanning grants, research papers, patents, policy documents, with complex citation linkages; 
complex analysis tasks such as tracing the evolution of knowledge and identifying emerging research frontiers; 
and high-stakes decision-making scenarios, including uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies. 
% 
We begin by providing a system overview, introduce the hybrid user interface and its multi-agent LLM engine, and end with the database design and implementation details. 


% %%%%%%%%%%%%%% Method Section Begins %%%%%%%%%%%%%%%%
% 先写motivation，再写我们为了这个motivation做了什么技术实现
\subsection{System Overview} 
% Paradigm of LUI + GUI for generative insights/visual data exploration: 可以参考了这个paper的图：Data Formulator: AI-powered Concept-driven Visualization Authoring。他也提到了一个paradigm
\systemname introduces a hybrid user interface that allow users interact with underlying AI agents and data through both natural language and direct manipulation. 
These interactions are orchestrated by a multi-agent LLM system that interprets user intent and extracts data insights efficiently in real time. 
The system consists of three modules \wyf{(Fig.~\ref{fig:system-overview})}. 
The Hybrid User Interface Module integrates the language user interface and interactive visualization-based graphical user interface into a a web frontend, allowing users to fluidly switch between language-based querying and visual exploration. 
% that are easy to be accessed by users. 
The Multi-Agent LLM Engine forms the analytical backend, comprising three coordinated agents, \planner, \executor, and \evaluator, that understand user queries, generate plans and execute analytical actions, and iteratively reflect on results to guide the analysis process. 
The Data Management Module manages three types of information: 
(1) a large scale relational database of SciSci data, 
(2) a vector database of SciSci domain literature that enables retrieval-augmented generation (RAG) for domain-aware reasoning, 
and (3) a user chat history database, specifically designed for LLM-native figure and data-driven artifact for human non-linear exploration process. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/system-overview.jpg}
    \caption{System design in \systemname.
    \textbf{a}, User input types include natural language input and graphical input. 
    \textbf{b}, The Hybrid User Interface Module serves as the frontend of the system.  
    Left: natural language interaction using a traditional chatbot and an inline chatbot. 
    Right: graphical interaction using interactive dashboards (\eg, click, brush, and hover).
    It allows users to interact in two ways, combining the accessibility of language UI with the clarity and efficiency of graphical UI, particularly in interactive visualization scenarios under data exploration. 
    \textbf{c}, The Data Management Module manages SciSci domain datasets and knowledge and chat history.
    \textbf{d}, The Multi-Agent LLM Engine servers as the backend of the system, including three agents and a set of tools. 
    }
    \label{fig:system-overview}
\end{figure}


\subsection{Hybrid User Interface}
\label{conceptual-model-hybrid-ui} 
% Allow three types of interactions: chatbox input (NL), inline input (NL), and GUI input (operations on chart -- brush/filter/click/zoom/..., and GUI Widgets -- recommendation and coordination button)
% Three types of questions: 
% 1. init a new query
% 2. drill-down analysis: extend chart
% 3. fine-grained analysis: manipulate chart (scatter => + regression; bar => stacked bar)
% 4. AI recommendation: task decomposition + next-step exploration

We design a hybrid interface that couples a Language User Interface (LUI) and a Graphical User Interface (GUI) (Fig.~\ref{fig:system-overview}b), serving as the frontend of \systemname through which users directly interact with the system (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (User Input: $I_t$)).


% 1. LUI, two parts: 
% (1) Chat history (linear)
% (2) Artifact session (inline, combined with GUI, non-linear) 
\textbf{Language User Interface (LUI)} (Fig.~\ref{fig:system-overview}b-Left). 
Language offers an expressive channel for curiosity. 
By allowing humans to ask open-ended questions in natural language, the LUI lowers the cognitive and technical barriers to data exploration. 
In addition to traditional chatbot panels, the interface also includes inline conversational widgets, which allow dialogue to unfold within the visual context itself.
Users can initiate queries via chat, request AI-generated analytical suggestions, or interact directly with visualizations to ask follow-up questions, request AI recommendations, and coordinate and filter across multiple visualizations. 
In this way, conversation becomes an analytical instrument rather than a passive query mechanism. 
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/lui-and-gui.jpg}
%     \caption{User interaction design. 
%     Left: natural language interaction using a traditional chatbot and an inline chatbot. 
%     Right: graphical interaction using interactive dashboards (\eg, click, brush, and hover).
%     It allows users to interact in two ways, combining the accessibility of language UI with the clarity and efficiency of graphical UI, particularly in interactive visualization scenarios under data exploration. 
%     }
%     \label{fig:lui-and-gui}
% \end{figure}


\textbf{Graphics User Interface (GUI)} (Fig.~\ref{fig:system-overview}b-Right).  
% clarity and efficiency of graphics UI
While language captures ideas, visualization externalizes them by transforming abstract data into a perceptible structure and provides an intuitive and efficient medium for uncovering hidden patterns through visual representation that may be difficult to articulate in statistics alone~\cite{anscombe1973graphs}. 
% interactivity
These visualizations are typically interactive, allowing users to manipulate data directly (\eg, through brushing, filtering, clicking, and zooming) to quickly and accurately access and query source data via visual elements (\eg, scatters and bars)~\cite{shneiderman1983direct, munzner2014visualization}. 
We thus use LLM-native figures (Sec.~\ref{subsection:conceptual-framework}) to enable visual data exploration ($V_t$) and trace analysis procedures and corresponding data ($C_t$ and $D_t$) at time $t$. 
% Additionally, to make these insights mutually legible to both human and AI, we present insights in multiple modalities to both human users and LLMs: static images, interactive dashboards, textual summaries, and underlying Vega-Lite specification code \wyf{(Fig.~\ref{??}}). 
% 
% (2) Domain Object: Data-driven Artifact
Building on these single figures, we further enable Data-Driven Artifact (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), a reusable, composable unit of exploration that allow users refine and extend their analytical inquiries for deeper investigation. 
Starting from an existing figure, users can send follow-up instructions to refine it (\eg, transforming a descriptive scatterplot into a correlation analysis) or explore the selected subset of the data on the figure to generate new, coordinated figures that extend the current line of exploration. 
% \wyf{[yifang: to delete repeat content below.]
% comprising one or more coordinated dashboards that encode the human's iterative analytical logic.
% Each artifact records not only the resulting visualizations but also the sequence of thought: the manipulations, drill-downs, and transitions that produced them. 
% Here, \textbf{manipulation} means edit existing visualizations to refine or reorient the analysis focus, and \textbf{drilling down} means analyzing from user-interested data points within a visualization to generate new, coordinated dashboards. 
% Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, re-examined, and shared across related tasks. }

% (3) Summary
Through this hybrid interface, which combines language UI and graphical UI, humans can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently non-linear exploration logic fundamental to human discovery processes. 


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/data-driven-artifact.jpg}
%     \caption{(A) Data-Driven Artifact and its two interaction modes. 
%     Left: \textbf{manipulating} existing visualizations to refine or reorient the analysis focus. 
%     Right: \textbf{drilling down} from user-interested data points within the visualization to generate new, coordinated dashboards that allow users to progressively deep dive into insights through interaction.
%     (B) Illustration of non-linear data exploration steps. 
%     }
%     \label{fig:data-driven-artifact}
% \end{figure}




\subsection{Multi-Agent LLM Engine} 
\label{subsection:method-llm}
Realizing above-mentioned hybrid interface requires an AI infrastructure capable of understanding heterogeneous user inputs, reasoning over complex data, and generating data insights in real time. 
Recent advances in large language models and AI agents offer transformative potential to interpret user intent and accelerate data-driven discovery with unprecedented efficiency~\cite{shao2025sciscigpt, guo2024ds}. 
Thus, we design a multi-agent LLM engine that coordinates the communication between user and the large-scale SciSci data, supporting a wide range of analytical intents and exploration pathways. 
The engine includes three core agents, \planner, \executor, and \evaluator, which operate at an \actionname{action}-level granularity (Fig.~\ref{fig:system-overview}d). 
Together, they form an automated reasoning loop that spans data analysis, visual insight generation and manipulation, dashboard coordination, and iterative exploration. 

% \subsubsection{Multi-Agent Workflow} 
% \label{subsubsection:multi-agent-workflow}
\textbf{Multi-Agent Workflow.}
To accommodate diverse analytical tasks and reasoning demands, we design a multi-agent workflow comprising three specialized AI agents, leveraging recent advances in LLM-based reasoning~\cite{yao2023react}, planning~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-improvement~\cite{madaan2023self, shinn2023reflexion}. 
% and abilities such as ReAct~\cite{yao2023react}, three-of-thoughts~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-refining and self-correction~\cite{madaan2023self}. 
% (1) Planner
The \planner Agent serves as the direct interface between the user interface and the analytical backend. 
It infers user's intentions by taking user's natural language queries and direct manipulation inputs (\eg, brushing and filtering) and formulate an initial strategy for execution. 
Specifically, if performs query triage across three distinct pathways.
For high-level complex analytical goals, it decomposes the query into structured sub-questions and returns them to users for clarification or confirmation. 
For exploratory scenarios where users seek guidance on next analytical steps, it recommends potential next steps based on exploration history and intermediate results. 
For low-level questions, it directly initiates action planning, selection, and execution procedure. 
% For low-level concrete questions, it directly returns control to the \planner Agent to invoke other tools for immediate action selection and execution.
% Including task decomposition, AI recommendation, Candidate and Optimal Action Selection, and Initial Action Sequence Generation (Initial Planning, that could be adjusted based on real-time execution results). 
% TODO: first translate user queries into typical analysis tasks (Tamara's book and the paper -- Low-Level Components of Analytic Activity in Information Visualization) 
To accomplish these tasks, the agent leverages three specialized tools: 
(1) \toolname{user_query_classifier()} tool classifies user queries into high-level (requiring decomposition) and low-level (directly executable) categories, enriched by domain knowledge retrieved via literature search; 
% high-level: which will be decomposed into sub-questions based on the user request and external domain knowledge (using \toolname{literature_search()} below) 
(2) \toolname{ai_recommender()} tool proposes follow-up exploration suggestions based on user intent, multi-modal data context, and domain knowledge; 
(3) \toolname{literature_search()} tool~\cite{shao2025sciscigpt} retrieves and summarizes relevant literature from the SciSci domain as context using retrieval-augmented generation (RAG), thereby grounding the planning process in domain context. 
% contextualizes the reasoning and planning process within the Science of Science domain, by using retrieval-augmented generation (RAG) to identify the most relevant papers in the SciSci domain and stores a summary paragraph in the context as reference to assist the plan formulation. 
% This integration ensures that data exploration is grounded in existing scientific understanding while enabling novel hypothesis generation. 
% "which is output to the user and stored in context memory to guide subsequent activities."
% LiteratureSpecialist. Understanding and contextualizing research questions within the SciSci domain is critical for determining the novelty of the research question and ensuring efficient use of existing knowledge, including previous approaches to similar scientific questions, conclusions from prior studies, and other researchers’ assessments of the implications of their findings. 
% 
(4) The core component of this agent is the \toolname{action_selector()} tool. 
It is a tree-based planning algorithm (Fig.~\ref{fig:a-star}) that synthesizes principles from tree-of-thoughts reasoning and search~\cite{yao2023tree, zhuang2023toolchain}. 
% and and A* search~\cite{zhuang2023toolchain}. 
% selects an optimal action as next-step for execution, given the user query and historical executed action sequence and results.
% The tool applies a tree-based search planning (Fig.~\ref{fig:a-star}) to capture a comprehensive decision space, built on and improve the tree of thoughts~\cite{yao2023tree} and A* search algorithm~\cite{zhuang2023toolchain}. 
The tool constructs a dynamic search tree $\mathcal{T}$, where each node represents an atomic analytical action along with its execution results, and edges encode temporal dependencies between actions. 
This design enables the exploration of multiple reasoning pathways by navigating a structured and comprehensive decision space (Supplementary Notes~\ref{subsection:si-tree-based-search}). 
% while maintaining computational tractability through intelligent pruning strategies.
% ToT: search for a comprehensive space for solutions -- better than CoT. 
% Specifically, the tool constructs a search tree $T$ with each node representing an atomic action and edge representing the ordered sequence to execute actions. 



% (2) Executor
The \executor Agent executes the selected action by invoking the corresponding tool to generate the appropriate code (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}).
% The \executor Agent executes the selected action by first generating corresponding codes by calling corresponding tool for this action (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}). 
These code snippets are then executed within three isolated sandboxes, \toolname{execute_SQL()}, \toolname{execute_Python()}, and \toolname{execute_VegaLite()}, to produce intermediate outputs in LLM-native figures, including dataframes, visualization specifications, rendered images, textual insights, etc. 
% optimization 
To optimize memory allocation and execution efficiency when operating on large-scale datasets, we adopt a staged strategy: 
each intermediate SQL-related action (\eg, filtering and transformation) is executed on a randomly sampled subset of 1000 records, while the full SQL query is deferred and executed only at the final stage of the SQL pipeline (right before data modeling or visualization).


% (3) Evaluator
The \evaluator Agent incorporates the principle of self-reflection~\cite{shinn2023reflexion} from agent design frameworks to evaluate on the outcomes of executed actions and guide subsequent planning. 
It handles two types of action outcomes, successful and failed executions, using two dedicated tools.
% 
% tool 1: success > _task_evaluator()
(1) When an action is executed successfully, the agent invokes the \toolname{task_evaluator()} tool to assess how well the result answers the user’s query. 
This assessment is accessed by LLM which produces a confidence score between 0 and 1, along with an explanation and any remaining plans. 
If the score exceeds a predefined threshold (\eg, $threshold \geq 0.8$ in our current implementation), the action selection loop terminates. 
Otherwise, the execution result, evaluation score, rationale, and remaining plans are appended to the data context (Sec.~\ref{subsection:method-implementation}) and passed back to the \planner Agent for the next round of action selection.
% 
% tool 2: falure > _action_error_handler()
(2) If an action fails, the agent triggers the \toolname{action_error_handler()} tool to process the error message and determine the next step, either (1) retrying the same action in the \executor Agent, or (2) initiating a new round of planning in the \planner Agent (\ie, finding an alternative solution path in the search tree $\mathcal{T}$). 
\wyf{Note: the actual code implementation is a slightly different. TODO: try to align with paper.}
% To support error recovery, we provide three types of linters to automatically correct common issues: a SQL linter~\cite{SQLLinter}, a Python linter~\cite{PythonLinter}, and a Vega-Lite linter~\cite{chen2021vizlinter}.
% We provide three types of linters to fix the execution error for re-running the same action: SQL linter~\cite{SQLLinter}, Python linter~\cite{PythonLinter}, and Vega-lite linter~\cite{chen2021vizlinter}. 

Together, the three agents coordinate together to generate a sequence of actions to answer user query, enhanced by advanced prompt design and context management (Sec.~\ref{subsection:method-implementation}). 



% \subsubsection{Action Space} 
% \label{subsection:method-action-space}
\textbf{Action Space.}
% what we did: 
\systemname defines a compositional action space consisting of atomic operations that serve as the fundamental execution primitives for data-driven exploration tasks. 
These actions are dynamically composed, sequenced, and executed by the multi-agent workflow to support diverse analytical tasks, including data filtering, transformation, modeling, visualization, and cross-visualization coordination, and it is designed to be refinable and extensible for adaptation across different domains~\cite{gao2025democratizing}. 
% reason: 
This action-level design offers two key advantages. 
First, it improves reasoning accuracy and execution stability by constraining the solution space to a set of well-defined operations amenable to optimization-based planning (see \planner Agent). 
Second, it promotes algorithmic transparency, allowing users to trace and validate each decision step in the analysis process clearly~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% \wyf{[Yifang] We should also mention that each action could increase LLM's performance -- avoid re-generating everything from starting.}
% This action-level granularity enhances reasoning accuracy and stability by constraining the solution space to well-defined operations with optimized action selection process, while providing algorithmic transparency that enables users to inspect and validate the decision-making process step-by-step~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% Moreover, this modular design is naturally compatible with reinforcement learning frameworks, which operate over action-level representations to optimize long-term strategies. 
% Moreover, this modular design enables future integration with reinforcement learning frameworks, which inherently rely on action-level granularity for optimizing long-term strategies. 
% lays the groundwork for future integration with reinforcement learning frameworks, which inherently require action-level granularity to enable learning from interaction histories and optimizing long-term analytical strategies. 
% Could be enhanced by reinforcement learning (which naturally require action-level design) in future work. 
% 
% implementation: 
Specifically, we design four types of actions derived from general data science tasks: \textit{data filtering}, \textit{data transformation}, \textit{data modeling}, and \textit{data visualization} (Supplementary Notes 1.1), building on techniques such as NL2SQL~\cite{liu2024survey, hong2024next}, AI4VIS~\cite{wu2021ai4vis}, and LLM for data science~\cite{guo2024ds, hong2024data}. 
The \textit{data modeling} category includes a set of actions frequently used in data science (\eg, \actionname{text_embedding} and \actionname{dimension reduction}).
% The \textit{data modeling} category reflects the methodological diversity of SciSci research~\cite{liu2023data, shao2025sciscigpt}, including statistical modeling, network analysis \wyf{([TODO: add network analysis tools])}, and machine learning. 
% For \textit{data visualization}, we incorporate two design spaces for dashboard type selection (action \actionname{add_chart_type}, \cite{shi2020calliope, wang2019datashot}) and interaction formulation (action \actionname{add_params}) (Supplementary Notes 1.1).
% and visual annotation augmentation (action \actionname{add_annotation}). 
For \textit{data visualization}, we include actions to select the visualization type (\actionname{add_chart_type}) and interaction type (\actionname{add_params}), as well as adding data (\actionname{add_data}) and visual encoding (\actionname{add_encoding}). 
% Other actions such as \actionname{add_data} and \actionname{add_encoding} are also included to generate interactive figures. 
In addition to "add" actions, we provide "update" actions to refine existing figures (\eg, \actionname{update_encoding}).
% \wyf{[yifang: to refine the writing and code: "add" could also be replaced by "refine" and "delete".} 
% 
Building on these atomic actions, the LLM engine could easily interpret the user's analytical intent using natural language instructions and graphical interactions, and use bidirectional mapping (Sec.~\ref{subsection:conceptual-framework}-bidirectional mapping) to generate, refine, and extend figures during the exploration process. 


% \subsubsection{Cross-Figure Interaction}
% \label{subsubsection:coordination}
\textbf{Coordination Across Figures.} 
% \textbf{Cross-Figure Interaction.}
% \wyf{yifang (2020109): we are able to use advanced coordination by not only filtering but also rerun python code (science-policy case), based on stored executed action sequence and code history list.}
% \wyf{要不SI里面加一个policy类似的case，但是用的是II数据。展示paper title distribution?}
\systemname supports the generation and coordination of multiple linked figures within a single data-driven artifact, enabling coherent multi-view exploration (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance).
% 1. input: GUI + LUI (only for generation)
First, input-wise, user interactions with an existing figure (e.g., brushing a region or selecting data points) are captured through the GUI and jointly interpreted with natural-language instructions by the LLM engine to infer analysis intent.
These interaction-derived constraints are injected into subsequent data-filtering actions (e.g., \actionname{filter_rows}) during execution, allowing newly generated figures to remain semantically aligned with prior exploration steps.
% First, the LLM engine will take user's GUI interactions (\eg, filtered regions or selected data points) as additional input parameters that are jointly interpreted with natural-language instructions to capture analysis intent.
% These interaction-derived constraints are injected into data-filtering actions (\eg, \actionname{filter_rows}) during execution.
% 2. DB design for generating a chart
Second, database-query-wise, when extending an artifact with additional figures, the multi-agent LLM engine is granted access to both the underlying SciSci domain database and a temporary workspace database derived from prior figures (Fig.~\ref{fig:bidirectional-mapping}c-D). 
This design allows the system to flexibly select appropriate data tables when initializing follow-up queries, supporting iterative and context-aware figure generation.
% Second, when generating a new figure from an existing one, the multi-agent LLM engine is provided with access to both the SciSci domain databases and the temporary stored workspace database derived from prior figures (Fig.~\ref{fig:bidirectional-mapping}-A3-D). 
% This design allows the system to flexibly select appropriate tables when initializing subsequent queries. 
% 3. generate chart: 
In addition, database-artifact-provenance-wise, at the end of the generation, to enable cross-figure coordination, the system generates a coordination schema for this pair of figures and store in the database, derived from the codes in executed action sequence. 
% For each coordinated figure pair, which is identified by figure IDs and a directional interaction link from the initiating figure to the derived figure, the schema stores interaction–coordination pairs that define coordination behavior. 
The coordination schema in each pair consists of one or multiple interaction types (e.g., 2D brush selection) and the corresponding LLM-generated code execution template (including SQL schema templates and, when needed, Python code). 
These templates are dynamically instantiated and re-executed as users modify interaction regions in the initiating figure.
% At the end of the generation, the system will store a coordination schema derived from the action sequence code to record pair-wise coordination rules and templates among figures.
% Specifically, for each coordinated figure pair (identified by figure IDs and directional interaction links from the initiating to the extended figure), we maintain interaction-filtering pairs that define the coordination behavior. 
% Each pair comprises an interaction type (\eg, 2D brush selection) and an LLM-generated code execution template (including SQL schema template and python code), which is dynamically instantiated as users modify filtering regions in the initiating figure in real-time. 
% This design supports efficient, flexible filtering and seamless multi-view exploration.
% 3. action sequence design for coordinating a chart
Third, coordination-wise, when users update selections in an existing figure, the LLM engine retrieves the corresponding coordination schema from the database, updates the relevant filtering parameters, and re-runs the stored code to regenerate all coordinated figures with consistent, up-to-date results. 
This design enables efficient, flexible cross-figure interaction while preserving the provenance and reproducibility of the analytical workflow (Supplementary Notes 1.4). 
% Additional implementation details are provided in the Supplementary Notes (Sec.~\ref{subsection:si-cross-figure-coordination}).
% Third, when users update the queried data region from the initial figure, the LLM engine will fetch the stored coordination schema to generate each coordinated figure in the artifact, and update the code with the updated filtering data region or point and re-run the code to get the updated results. 
% \wyf{To add content! We record the action sequence (with code) in each figure version and also artifact version (coordination schema). so that each time user choose another data region or point, LLM will fetch the historical code from chat history DB and re-run the code with the updated filtering data region or point.}
% Please refer to our supplementary information (Sec.~\ref{subsection:si-cross-figure-coordination}).





% 2. 针对不同情况，对selector和optimizor有不同的强约束。
%   - drill_down。 数据起点：ego chart 的 workspace 表（你现在的设计）。强约束：select_tables → filter_rows，filter_rows 将 brush ROI 翻译成 WHERE 条件（上一个 House Committee 案例）。→ optional join other tables to get more data。
%   - bottom_up。 数据起点：case dataset 表(含有filtering criteria的表)。强约束：select_tables → filter_rows，filter_rows 将 brush ROI 翻译成 WHERE 条件（上一个 House Committee 案例）。→ optional join other tables to get more data。其中，filter_rows 用 brush 的 time 维度（如果有）+ 从 applied_filters 里保留 time 条件，而移除 state='Florida' 这种地理限制。



% 对应figure 1: extended chart加上coordination这一步，单独实现。不要跟前面action space混在一起。删掉前面的add_coordination action. 




% % \subsubsection{Data-Driven Artifact} 
% % \label{subsection:method-data-driven-artifact}
% Our hybrid interface combining LUI and GUI introduces unique challenges for interpreting user intent. 
% % , as users can interact through both natural language and direct manipulation modalities. 
% % The communication between human users and LLM agents presents unprecedented challenges for data querying and analysis due to the hybrid user interfaces (which enable both natural language input and direct manipulations).  
% To address this, we propose two strategies for generating, manipulating, and exploring data-driven artifacts within the multi-agent workflow and action space. 

% \textbf{Hybrid User Intention Inference for Data Querying.} 
% \wyf{TODO: remove redundant from conceptual framework.}
% We first develop a dynamic prompting mechanism to accurately infer user intents from hybrid natural language and direct manipulation inputs, enabling precise data querying for filtering and transformation actions. 
% % GUI input
% For direct manipulation (\eg, brushing and clicking), we implement a semantically-aware mapping $\mathcal{M}: \mathcal{V} \leftrightarrow \mathcal{D}$ between the visualization space $\mathcal{V}$ and the underlying database space $\mathcal{D}$. 
% % For direct manipulation inputs, we employ a \wyf{semantically-aware} approach that transforms GUI interactions (\eg, brushing and clicking) into structured database queries through a bidirectional mapping function 
% % $\mathcal{M}: \mathcal{V} \leftrightarrow \mathcal{D}$ 
% % between visualization space $\mathcal{V}$ and database space $\mathcal{D}$. 
% This mapping translates GUI inputs (\ie, dashboard filtering) into structured queries by tracing visual selections back to the original database columns or entities (\eg, papers, patents, and researchers) using shared attributes from the raw data or intermediate results (Fig.~\ref{fig:action-enhancement}). % (
% % \wyf{Specifically, the filtering criteria extracted from the dashboards trace back to original database columns and data entities (\eg, paper, patent, and researcher) by using shared attributes available either directly in the database or from intermediate data structures and derived dataframes (Fig.~\ref{fig:action-enhancement}).} 

% % Overview: spatial selection + semantic context
% These GUI interactions $I_t = (i_1, ..., i_k)$ (at time $t$) are dynamically integrated with natural language inputs $NL_t$ to construct a comprehensive data query 
% $Q_{t+1} = \mathcal{T}(I_t, NL_t, \mathcal{M}_{active}, H_t)$, 
% where transformation function $\mathcal{T}$ synthesizes the current user input ($I_t$ and $NL_t$), $\mathcal{M}_{active}$ denotes the active dashboard-to-database mappings, and $H_t$ represents historical context, including current user session's intermediate data structures and derived dataframes.
% % integrates current user input with the mapping between current active visualization dashboard and database, and historical context $H_t$ (representing prior user session state and results). 
% This formulation ensures that the resulting queries preserve both the spatial constraints specified through direct manipulation from the dashboards and the semantic context expressed in natural language. 
% % The resulting queries thus preserve both spatial selection constraints from the dashboards and semantic context from natural language queries. 
% % M_context​⊂M denotes the context-specific instantiation of the base mapping that maintains provenance between currently active visual elements and their corresponding database records
% % Ht​ captures the cumulative interaction history and user session state at time t. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/action-enhancement.jpg}
%     \caption{Hybrid User Intention Inference for Data Analysis.}
%     \label{fig:action-enhancement}
% \end{figure}
% % 这个是在每个action里面，dynamic prompting to 考虑both user interaction and NL query, to generate 对应的data query or modeling
% % goals: 
%     % 1. ask follow-up quesion -> generate alter chart
%     % 2. modify current chart
%     % 3. filter data to update other charts (coordination) 
% % method: 
%     % Using filtering criteria + dynamic prompting + pre-stored dataframe in the user history database, to inject into data filtering/transformation actions. 
%     % If filtering criteria attribute is within original DB, then direct dynamic prompting
%     % If no, then trace to raw db using the pre-stored dataframe in the user history database -- a preset is, we should force these pre-stored dataframe to have at least one column in raw database.
%     % <draft>
%     % For example, to enable data querying through GUI-based visualization interactions (action: \actionname{add coordination}), we implement a multi-step filtering strategy Fig.~\ref{fig:??}). 
%     % Each data point \wyf{(before transformation and aggregation)} is bound with a unique identifier, allowing the action to trace filtered subsets of data back to the database using the GUI selection criteria and corresponding data point IDs. 
%     % % Each data point is bound with a unique identifier so that when user filter a subset of data in dashboard, we can trace back to the database by filtering based on the filtered criteria from GUI input and corresponding ID of each data point (Fig.~\ref{fig:??}). 
%     % % The \toolname{gui_inferred_data_query()} xxx. 
%     % % add mechanisms about linking user's GUI interaction to backend data (how to coordinate -- using vegalite解析 to SQL re-generation, ...) Vis coordination部分 
%     % % Coordination: 详细介绍--ID based indexing. 和User management db (temporary生成的csv for the visualization) link在一起
%     % % 先生成一个SQL语句for filtering, 再把这个SQL语句作为dynamic prompt注入到所有的tool as input parameter -- either生成融合式的SQL (filtering/transformation), or直接执行这条sql语句生成新的dataframe for analysis/visualization actions
%     % </draft>

% \textbf{Dashboard Coordination.} 
% \wyf{TODO: update with latest implementation: data-point level and aggregation-level.}
% % 这个是生成好一个artifact（multiple coordinated dashboard）以后，怎么快速支持用户刷选数据
% % Method: 生成两个关于这个artifact的coordination文件，并存储在user chat history里面：
%     % global_connection.json
%     % coordination_templates.json
% % 我们比LightVA牛逼: 他们的coordination的前提是必须share common column. 而我们可以deep dive to large-scale database to generate complex coordination
% % TODO: `replace_conditions()`这个function可能有问题--或许要替换成LLM-driven的？如果穷举不完的话
% Data-driven artifacts support cross-dashboard interactions, allowing users to filter data in one dashboard and immediately observe corresponding data changes in others. 
% To ensure real-time responsiveness, we employ an LLM-driven approach that dynamically generates and stores coordination schemas among dashboards each time a new dashboard is created within an artifact. 
% % To ensure real-time responsiveness, every time a new dashboard is generated within an artifact, we employ a LLM-driven approach to dynamically generate and stores coordination schemas among dashboards within this artifact. 
% % 
% Specifically, for each coordinated dashboard pair (identified by dashboard IDs and directional interaction links from the initiating to the extended dashboard), we maintain interaction-filtering pairs that define the coordination behavior. 
% Each pair comprises an interaction type (\eg, 2D brush selection) coupled with an LLM-generated SQL schema template that dynamically updates as users modify filtering regions in real-time. 
% % Each pair consists of an interaction type and the associated filtering SQL schema template, which is generated by LLM and can be dynamically updated based on real-time GUI input. 
% This design supports efficient, flexible filtering and seamless multi-view exploration. 
% % <interaction\_type, filtering\_schema> pair in a SQL schema templates which will be updated based on real-time GUI interaction filtering criteria. 
% % This coordination design enables efficient, dynamic filtering and seamless user exploration across dashboards.
% % To make the coordination response time in real time, we 使用一种无机的手段--保存一个data-driven artiface所有dashboard之间的coordination pair (linked by chart ID, directional, from ego chart to extended chart) and interaction-filtering pair，记录每一类interaction的filtering SQL schema template. 





% % scalable to extend and refine
% The current LLM workflow supports easy adaption to other domains by revising the action space and tool design without altering the underlying multi-agent architecture, ensuring broad applicability across computational social science and beyond. 
% % \wyf{TODO: refine integrate this sentence with the first sentence: Domain-specific customizations could be integrated into \textbf{LLM frameworks} (\eg, multi-agent systems) and \textbf{tool designs} to enhance these capabilities to specialized analytical contexts.}
% % % This modular design enables straightforward adaptation to other scientific domains beyond SciSci by allowing domain experts or AI agents to modify the action space while preserving the underlying compositional architecture, demonstrating the framework's extensibility across computational social science and broader data science applications. 
% % % The action space could be easily adjusted to other science fields beyond SciSci in computational social science and broader data science by human experts or LLM agents. 
% % % action library: could be edited to adjust to other science fields beyond SciSci/CSS — by replaces and extended by human experts or LLM agents (create new agents based on user queries)


\subsection{Data Management}
\label{subsection:method-data-module}
% Such new type of human-AI collaboration for scientific discovery requires rethinking data storage architecture itself. 
The Data Management Module rests on three interlinked databases (Fig.~\ref{fig:system-overview}c):
(1) domain databases that provide the empirical substrate for analysis--SciSci rational database; 
(2) knowledge embeddings, which are usually vectorized representations of domain knowledge that enable techniques such as retrieval-augmented reasoning (RAG) for domain-aware reasoning--vector database for SciSci literature; 
and (3) exploration histories that record non-linear human–AI interactions and data-driven artifacts, capturing the evolving logic of discovery. 
% 
% (1) SciSci
For our test domain SciSci, we incorporate two primary data sources. 
\newlyadded{The first one is a university-level dataset capturing innovation activities and researcher information~\cite{wang2023innovationinsights}, collected and preprocessed from multiple sources, including public datasets such as Microsoft Academic Graph (MAG)~\cite{wang2019review}, PatentsView~\cite{patentsview}, and Reliance on Science~\cite{marx2020reliance, marx2022reliance}, 
as well as proprietary institutional datasets from Technology Transfer Office (TTO) on invention disclosures and outcomes and HR Office on faculty roster with demographic data (e.g., name, gender, rank, and department).}
% (1) \textbf{SciSciNet}, the largest open data lake of SciSci~\cite{shao2025sciscigpt} that covers comprehensive records and entities essential for this domain, 
The second data source is SciSciCorpus~\cite{shao2025sciscigpt}, a vector database containing the key literature in this field, with paper documents chunked and indexed to support retrieval-augmented generation (RAG) for enhanced domain understanding.
% In addition, our case studies integrate proprietary SciSci datasets, including confidential data of faculty (\eg, gender and department) provided by our collaborating university's HR office.
% \wyf{In addition, our case studies integrate proprietary SciSci datasets, including \textbf{Overton}~\cite{Overton} that contains global policy documents and citation linkages between policies and papers, as well as confidential data about demographic information of faculty provided by our collaborating university’s HR office.}
% 
% (2) User Management and Data-driven Artifact Management 
% \wyf{[yifang: not only support tree but also a graph version of all dashboard linkages]}
Additionally, we design a user and chat history management database \wyf{(Supplementary Notes 1.6)} tailored to support LLM-native figures and data-driven artifacts for non-linear exploration process. 
The \code{messages} table stores individual question-answer pairs for each user \code{conversations} session, establishing the conversational foundation. 
% artifact level: 
Each message links to corresponding artifact entries in three artifact-related tables (\code{message_artifact}, \code{artifacts}, and \code{artifact_versions}), which maintains comprehensive metadata for each data-driven artifact, including a list of figure identifiers, coordination relationships and schemas that define cross-figure interactions. 
The figure identifiers in each artifact link to two tables, \code{figures} and \code{figure_versions}, which store the components of each LLM-native figure: $V$, $C$, $D$, $M$ (Sec.~\ref{subsection:conceptual-framework}), as well as action-level reasoning, codes, and results. 
The two tables, \code{artifact_versions} and \code{figure_versions}, records the exploration history as a list of temporal snapshots of artifact-level and figure-level states, such that each user input generates a new record, preserving the complete exploration history. 
% Two additional tables support detailed exploration tracking: \code{artifact_versions} table captures temporal snapshots of artifact states, while \code{artifact_operations} table logs all user interactions, including dashboard manipulations and drill-down operations. 
% dashboard level: 
% At the dashboard level, each visualization is stored in the \code{dashboard} table with multi-modal representations (\ie, Vega-Lite specifications, visualization images, and text insights). 
% The database implements immutable versioning where any dashboard modification creates a new record, preserving the complete editorial history. 
% 
This architecture enables complete reconstruction of analytical pathways, allowing users to trace their discovery processes and revert to previous analytical states transparently. 
% We also have two additional tables, \code{artifact_versions} and \code{artifact_operations}, to store the exploration history including dashboard manipulation and drilling down. 

\subsection{Implementation Details} 
\label{subsection:method-implementation} 
\textbf{Technology Stack.}
\systemname is implemented as a full-stack web application utilizing modern development frameworks and cloud infrastructure. 
The frontend employs React.js~\cite{React} for component-based user interface development, Redux.js~\cite{Redux} for state management, and Vega-Lite for declarative visualization rendering~\cite{satyanarayan2016vega}. 
The backend architecture is built on the Flask framework~\cite{Flask} with Python~\cite{Python}, providing RESTful API services and data processing capabilities. 
Specifically, the multi-agent workflow leverages LangChain~\cite{LangChain} and LangGraph~\cite{LangGraph} for complex agent coordination, with Claude 4.5 Sonnet~\cite{AnthropicAPI} serving as the primary language model. 
The system architecture supports model substitution, enabling integration with alternative LLM providers as needed. 
Data storage employs a hybrid approach: Google Big Query~\cite{BigQuery} manages relational SciSci domain datasets and user chat histories, while Pinecone~\cite{Pinecone} serves as the vector database for the retrieval-augmented generation module, storing chunked domain literature for semantic search and knowledge retrieval. 


\textbf{Action-based Streaming Output.} 
To balance analytical transparency with user experience, we implement action-level streaming output that selectively displays critical workflow information without overwhelming users with verbose LLM reasoning. 
The interface presents only essential decision points, specifically action selection and action sequence generation processes, providing users with meaningful insights into analytical behavior.
% To balance the data analysis transparency and the information overload of outputing every word of the LLM reasoning, we design an action-level streaming output in the user interface. 
% Only the action selection and action sequence generation process will be displayed. 
Upon completion of each user query, the system delivers comprehensive results including SQL queries, Python code, processed dataframes, visualization images, and structured Vega-Lite JSON outputs. 
This approach ensures users can monitor system progress through high-level action updates while accessing detailed technical artifacts for validation and reuse. 
% We also provide the final results for each user question, (SQL code, Python code, dataframe, visualization img and json etc.)
% % To balance the information transparency and the overwhelming. 
% % Output: action level reasoning (output action selection procedure, and result for each action (SQL code, Python code, ,,,)); And final result (csv, vega-lite img and json, SQL/Python codes). 
% % Future work: edit the code in each action -- allow action-level manipulation -- a tighter way for HAI collaboration.


\textbf{Prompt and Context Design.}
We employ four prompt engineering techniques to optimize our multi-agent workflow performance~\cite{white2023prompt, sahoo2024systematic}, including structured formatting, chain-of-thought reasoning, few-shot learning, and dynamic prompting. 
In addition, to make the context compact, we developed a structured data context that stores only essential information about each executed action, including action indices, objectives, execution status, results, evaluation scores and rationale, and remaining tasks (Supplementary Notes 1.5). 
% Please refer to our supplymentary information \wyf{(Sec.~\ref{subsection:si-prompt-design} and Sec.~\ref{subsection:appendix-context-design})} for more details.








% \textbf{Prompt Design.} 
% We employ four prompt engineering techniques to optimize our multi-agent workflow performance~\cite{white2023prompt, sahoo2024systematic}: 
% % 
% (1) Structured XML formatting.
% We develop a suite of XML tags to compartmentalize prompt components, such as \code{<roles>}, \code{<instructions>}, and \code{<constraints>} (Supplementary Note~\ref{section:appendix-prompt-design-structured-prompt}), to increase the clarity, accuracy, and parseability~\cite{PromptXML, sahoo2024systematic}. 
% % This structured approach improves LLM comprehension and response consistency across different agent interactions.
% % 
% (2) Chain-of-thought reasoning.
% We specifically use the \code{<internal_reasoning>} tag to guide the model work out a plan with step by step instructions, enhancing reasoning robustness and analytical coherence~\cite{wei2022chain}. 
% % 
% (3) Few-shot learning.
% We maintain an example library (Supplementary Note~\ref{subsubsection:appendix-prompt-design-fewshot-learning}) that enables dynamic retrieval and insertion of contextually relevant examples into prompt templates using the \code{<example>} tag, providing targeted guidance for diverse analytical scenarios~\cite{brown2020language}.
% This modular separation maintains prompt conciseness and facilitates system maintenance and expansion as conversational history grows, ensuring scalable performance without compromising prompt clarity. 
% % This type of separation (of an example library) keeps the original prompt short and clean and make it easier to maintain and expand when the user chat history increases. 
% % for agents and tools to retrieve and insert into the prompt template with the \code{<example>} tag~\cite{brown2020language}. 
% % This type of separation (of an example library) keeps the original prompt short and clean and make it easier to maintain and expand when the user chat history increases. 
% (4) Dynamic prompting.
% Beyond static contents, we incorporate variable contents into the prompts, such as user input (both natural language and direct manipulation), conversational context (\eg, chat history, data context, and RAG-retrieved knowledge), and few-shot learning examples, which allows more precise user intent interpretation and contextually relevant responses~\cite{sahoo2024systematic}.  
% % Future work: 
% % - 每次对这个文件retrieve 3个最相关的example
% % - Prefill Claude's response for greater output control 
% %     - TODO


% \textbf{Context Management.} 
% The iterative data exploration process and multi-modal outputs (\eg, data, code, and visualization) present challenges to deal with long context during the multi-agent workflow. 
% We design several stratifies to address this problem. 
% % (1) Within one QA round
% (1) Single-round conversation management.
% We developed a structured data context format for individual question-answer cycles that stores only essential information about action sequences, including action indices, objectives, execution status, results, evaluation scores, rationale, and remaining tasks (Supplementary Note~\ref{subsection:appendix-data-context-design}). 
% % This selective retention reduces context overhead while preserving critical workflow information. 
% % we specifically design a data context format to deal with one round of conversation (one QA round). 
% % Only the action sequence will be stored during the process, including action index, goal, action execution status (whether success or failure), action results, evaluation score, reason, and remaining tasks and plans (Supplementary Note~\ref{subsection:appendix-data-context-design}). 
% % (2) Semantic context
% (2) Cross-session semantic compression.
% For conversations spanning multiple question-answer rounds or cross-sessions, we employ automated summarization to compress chat history into concise paragraph-form representations. 
% % This approach maintains contextual coherence while preventing context window overflow, enabling sustained analytical workflows without performance degradation. 

% % For one chat session across different QA round and cross-session contexts, we summarize the chat history into a paragraph to compact the context. 

% % Note: Specifically, in addition to traditional chat history, we've 
% % 3-2 integrate vision language model (vis code and image) to infer insights and recommend next-step exploration. 
% % 3-3 只展示重要的reasoning信息，to avoid overwelming 例如action_name, result (SQL code, python code, vega-lite code, dataframe, vis image, ...) 
% % - Long context prompting tips
% %     - TODO: may need to add chat history summary
% %     - https://docs.anthropic.com/en/docs/build-with-claude/prompt-engineering/long-context-tips

==> sections/archive/05-method/05-method-20260208.tex <==
\section{Methods} % Nexus--A Reference Implementation for SciSci Domain}
\label{section:methods}

% \begin{methods}
% Based on this conceptual framework, we further develop a proof-of-concept system, \systemname, to demonstrate how to facilitate scientific discovery using these LLM-native figures with a non-linear human exploration process. 
To demonstrate the broad applicability of this conceptual framework, we present \systemname, an instantiation of the framework that we propose, which is developed for the science of science (SciSci) domain---an essential field for understanding and accelerating scientific enterprise and technological innovation.
SciSci provides an ideal testbed with challenges that are well matched to our framework: 
rich and emerging datasets spanning grants, research papers, patents, and policy documents, with complex citation linkages; 
complex analysis tasks such as tracing the evolution of knowledge and identifying emerging research frontiers; 
and high-stakes decision-making scenarios, including uncovering untapped innovation potential for university leaders or guiding strategic funding allocations by funding agencies. 
% 
We begin by providing a system overview, introduce the hybrid user interface and its multi-agent LLM engine, and end with the database design and implementation details. 


% %%%%%%%%%%%%%% Method Section Begins %%%%%%%%%%%%%%%%
% 先写motivation，再写我们为了这个motivation做了什么技术实现
\subsection{System Overview} 
% Paradigm of LUI + GUI for generative insights/visual data exploration: 可以参考了这个paper的图：Data Formulator: AI-powered Concept-driven Visualization Authoring。他也提到了一个paradigm
\systemname introduces a hybrid user interface that allow users interact with underlying AI agents and data through both natural language and direct manipulation. 
These interactions are orchestrated by a multi-agent LLM system that interprets user intent and extracts data insights efficiently in real time. 
The system consists of three modules (Fig.~\ref{fig:Figure5}). 
The Hybrid User Interface Module integrates the language user interface and interactive visualization-based graphical user interface into a web frontend, allowing users to fluidly switch between language-based querying and visual exploration. 
% that are easy to be accessed by users. 
The Multi-Agent LLM Engine forms the analytical backend, comprising three coordinated agents, \planner, \executor, and \evaluator, that understand user queries, generate plans, execute analytical actions, and iteratively reflect on results to guide the analysis process. 
The Data Management Module manages three types of information: 
(1) a large-scale relational database of SciSci data, 
(2) a vector database of SciSci domain literature that enables retrieval-augmented generation (RAG) for domain-aware reasoning, 
and (3) a user chat history database, specifically designed for LLM-native figures and data-driven artifacts for human nonlinear exploration process. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/system-overview.jpg}
    \caption{
    \bodyfigurelabel{fig:Figure5}
    System design in \systemname.
    \textbf{(a)} User input types include natural language input and graphical input. 
    \textbf{(b)} The Hybrid User Interface Module serves as the frontend of the system.  
    Left: natural language interaction using a traditional chatbot and an inline chatbot. 
    Right: graphical interaction using interactive dashboards (\eg, click, brush, and hover).
    It allows users to interact in two ways, combining the accessibility of language UI with the clarity and efficiency of graphical UI, particularly in interactive visualization scenarios under data exploration. 
   \textbf{(c)} The Data Management Module manages SciSci domain datasets and knowledge and chat history.
    \textbf{(d)} The Multi-Agent LLM Engine servers as the backend of the system, including three agents and a set of tools. 
    }
    \label{fig:system-overview}
\end{figure}


\subsection{Hybrid User Interface}
\label{conceptual-model-hybrid-ui} 
% Allow three types of interactions: chatbox input (NL), inline input (NL), and GUI input (operations on chart -- brush/filter/click/zoom/..., and GUI Widgets -- recommendation and coordination button)
% Three types of questions: 
% 1. init a new query
% 2. drill-down analysis: extend chart
% 3. fine-grained analysis: manipulate chart (scatter => + regression; bar => stacked bar)
% 4. AI recommendation: task decomposition + next-step exploration

We design a hybrid interface that couples a Language User Interface (LUI) and a Graphical User Interface (GUI) (Fig.~\ref{fig:Figure5}b), serving as the \systemname frontend through which users directly interact with the system (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (User Input: $I_t$)).


% 1. LUI, two parts: 
% (1) Chat history (linear)
% (2) Artifact session (inline, combined with GUI, non-linear) 
\textbf{Language User Interface (LUI)} (Fig.~\ref{fig:Figure5}b-Left). 
Language offers an expressive channel for curiosity. 
By allowing humans to ask open-ended questions in natural language, the LUI lowers the cognitive and technical barriers to data exploration. 
In addition to traditional chatbot panels, the interface also includes inline conversational widgets, which allow dialogue to unfold within the visual context itself.
Users can initiate queries via chat, request AI-generated analytical suggestions, or interact directly with visualizations to ask follow-up questions, request AI recommendations, and coordinate and filter across multiple visualizations. 
In this way, conversation becomes an analytical instrument rather than a passive query mechanism. 
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/lui-and-gui.jpg}
%     \caption{User interaction design. 
%     Left: natural language interaction using a traditional chatbot and an inline chatbot. 
%     Right: graphical interaction using interactive dashboards (\eg, click, brush, and hover).
%     It allows users to interact in two ways, combining the accessibility of language UI with the clarity and efficiency of graphical UI, particularly in interactive visualization scenarios under data exploration. 
%     }
%     \label{fig:lui-and-gui}
% \end{figure}


\textbf{Graphics User Interface (GUI)} (Fig.~\ref{fig:Figure5}b-Right).  
% clarity and efficiency of graphics UI
While language captures ideas, visualization externalizes them by transforming abstract data into a perceptible structure and provides an intuitive and efficient medium for uncovering hidden patterns through visual representation that may be difficult to articulate in statistics alone~\cite{anscombe1973graphs}. 
% interactivity
These visualizations are typically interactive, allowing users to manipulate data directly (\eg, through brushing, filtering, clicking, and zooming) to quickly and accurately access and query source data via visual elements (\eg, scatters and bars)~\cite{shneiderman1983direct, munzner2014visualization}. 
We thus use LLM-native figures (Sec.~\ref{subsection:conceptual-framework}) to enable visual data exploration ($V_t$) and trace analysis procedures and corresponding data ($C_t$ and $D_t$) at time $t$. 
% Additionally, to make these insights mutually legible to both human and AI, we present insights in multiple modalities to both human users and LLMs: static images, interactive dashboards, textual summaries, and underlying Vega-Lite specification code \wyf{(Fig.~\ref{??}}). 
% 
% (2) Domain Object: Data-driven Artifact
Building on these single figures, we further enable data-driven artifacts (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), reusable, composable units of exploration that allow users to refine and extend their analytical inquiries for deeper investigation. 
Starting from an existing figure, users can send follow-up instructions to refine it (\eg, transforming a descriptive scatterplot into a correlation analysis) or explore a selected subset of the data on the figure to generate new, coordinated figures that extend the current line of exploration. 
% \wyf{[yifang: to delete repeat content below.]
% comprising one or more coordinated dashboards that encode the human's iterative analytical logic.
% Each artifact records not only the resulting visualizations but also the sequence of thought: the manipulations, drill-downs, and transitions that produced them. 
% Here, \textbf{manipulation} means edit existing visualizations to refine or reorient the analysis focus, and \textbf{drilling down} means analyzing from user-interested data points within a visualization to generate new, coordinated dashboards. 
% Artifacts thus serve as both memory and medium: a living record of discovery that can be edited, extended, re-examined, and shared across related tasks. }

% (3) Summary
Through this hybrid interface, which combines language UI and graphical UI, humans can seamlessly transition between natural language queries and direct manipulation to iteratively explore hypotheses, extract insights, and inform scientific discovery and policy decisions, mirroring the inherently nonlinear exploration logic fundamental to human discovery processes. 


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/data-driven-artifact.jpg}
%     \caption{(A) Data-Driven Artifact and its two interaction modes. 
%     Left: \textbf{manipulating} existing visualizations to refine or reorient the analysis focus. 
%     Right: \textbf{drilling down} from user-interested data points within the visualization to generate new, coordinated dashboards that allow users to progressively deep dive into insights through interaction.
%     (B) Illustration of non-linear data exploration steps. 
%     }
%     \label{fig:data-driven-artifact}
% \end{figure}




\subsection{Multi-Agent LLM Engine} 
\label{subsection:method-llm}
Realizing above-mentioned hybrid interface requires an AI infrastructure capable of understanding heterogeneous user inputs, reasoning over complex data, and generating data insights in real time. 
Recent advances in large language models and AI agents offer transformative potential to interpret user intent and accelerate data-driven discovery with unprecedented efficiency~\cite{shao2025sciscigpt, guo2024ds}. 
Thus, we design a multi-agent LLM engine that coordinates the communication between user and the large-scale SciSci data, supporting a wide range of analytical intents and exploration pathways. 
The engine includes three core agents, \planner, \executor, and \evaluator, which operate at an \actionname{action}-level granularity (Fig.~\ref{fig:Figure5}d). 
Together, they form an automated reasoning loop that spans data analysis, visual insight generation and manipulation, dashboard coordination, and iterative exploration. 

% \subsubsection{Multi-Agent Workflow} 
% \label{subsubsection:multi-agent-workflow}
\textbf{Multi-Agent Workflow.}
To accommodate diverse analytical tasks and reasoning demands, we design a multi-agent workflow comprising three specialized AI agents, leveraging recent advances in LLM-based reasoning~\cite{yao2023react}, planning~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-improvement~\cite{madaan2023self, shinn2023reflexion}. 
% and abilities such as ReAct~\cite{yao2023react}, three-of-thoughts~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-refining and self-correction~\cite{madaan2023self}. 
% (1) Planner
The \planner Agent serves as the direct interface between the user interface and the analytical backend. 
It infers user's intentions by taking user's natural language queries and direct manipulation inputs (\eg, brushing and filtering) and formulate an initial strategy for execution. 
Specifically, if performs query triage across three distinct pathways.
For high-level complex analytical goals, it decomposes the query into structured sub-questions and returns them to users for clarification or confirmation. 
For exploratory scenarios where users seek guidance on next analytical steps, it recommends potential next steps based on exploration history and intermediate results. 
For low-level questions, it directly initiates action planning, selection, and execution procedure. 
% For low-level concrete questions, it directly returns control to the \planner Agent to invoke other tools for immediate action selection and execution.
% Including task decomposition, AI recommendation, Candidate and Optimal Action Selection, and Initial Action Sequence Generation (Initial Planning, that could be adjusted based on real-time execution results). 
% TODO: first translate user queries into typical analysis tasks (Tamara's book and the paper -- Low-Level Components of Analytic Activity in Information Visualization) 
To accomplish these tasks, the agent leverages three specialized tools: 
(1) \toolname{user_query_classifier()} tool classifies user queries into high-level (requiring decomposition) and low-level (directly executable) categories, enriched by domain knowledge retrieved via literature search; 
% high-level: which will be decomposed into sub-questions based on the user request and external domain knowledge (using \toolname{literature_search()} below) 
(2) \toolname{ai_recommender()} tool proposes follow-up exploration suggestions based on user intent, multi-modal data context, and domain knowledge; 
(3) \toolname{literature_search()} tool~\cite{shao2025sciscigpt} retrieves and summarizes relevant literature from the SciSci domain as context using retrieval-augmented generation (RAG), thereby grounding the planning process in domain context. 
% contextualizes the reasoning and planning process within the Science of Science domain, by using retrieval-augmented generation (RAG) to identify the most relevant papers in the SciSci domain and stores a summary paragraph in the context as reference to assist the plan formulation. 
% This integration ensures that data exploration is grounded in existing scientific understanding while enabling novel hypothesis generation. 
% "which is output to the user and stored in context memory to guide subsequent activities."
% LiteratureSpecialist. Understanding and contextualizing research questions within the SciSci domain is critical for determining the novelty of the research question and ensuring efficient use of existing knowledge, including previous approaches to similar scientific questions, conclusions from prior studies, and other researchers’ assessments of the implications of their findings. 
% 
(4) The core component of this agent is the \toolname{action_selector()} tool. 
It is a tree-based planning strategy that synthesizes principles from tree-of-thoughts reasoning and search~\cite{yao2023tree, zhuang2023toolchain}. 
% and and A* search~\cite{zhuang2023toolchain}. 
% selects an optimal action as next-step for execution, given the user query and historical executed action sequence and results.
% The tool applies a tree-based search planning (Fig.~\ref{fig:a-star}) to capture a comprehensive decision space, built on and improve the tree of thoughts~\cite{yao2023tree} and A* search algorithm~\cite{zhuang2023toolchain}. 
The tool constructs a dynamic search tree $\mathcal{T}$, where each node represents an atomic analytical action along with its execution results, and edges encode temporal dependencies between actions. 
This design enables exploration of multiple reasoning pathways by navigating a structured and comprehensive decision space (Supplementary Notes 1.2). 
% while maintaining computational tractability through intelligent pruning strategies.
% ToT: search for a comprehensive space for solutions -- better than CoT. 
% Specifically, the tool constructs a search tree $T$ with each node representing an atomic action and edge representing the ordered sequence to execute actions. 



% (2) Executor
The \executor Agent executes the selected action by invoking the corresponding tool to generate the appropriate code (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}).
% The \executor Agent executes the selected action by first generating corresponding codes by calling corresponding tool for this action (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}). 
These code snippets are then executed within three isolated sandboxes, \toolname{execute_SQL()}, \toolname{execute_Python()}, and \toolname{execute_VegaLite()}, to produce intermediate outputs in LLM-native figures, including dataframes, visualization specifications, rendered images, textual insights, etc. 
% optimization 
To optimize memory allocation and execution efficiency when operating on large-scale datasets, we adopt a staged strategy: 
each intermediate SQL-related action (\eg, filtering and transformation) is executed on a randomly sampled subset of 1000 records, while the full SQL query is deferred and executed only at the final stage of the SQL pipeline (right before data modeling or visualization).


% (3) Evaluator
The \evaluator Agent incorporates the principle of self-reflection~\cite{shinn2023reflexion} from agent design frameworks to evaluate on the outcomes of executed actions and guide subsequent planning. 
It handles two types of action outcomes, successful and failed executions, using two dedicated tools.
% 
% tool 1: success > _task_evaluator()
(1) When an action is executed successfully, the agent invokes the \toolname{task_evaluator()} tool to assess how well the result answers the user’s query. 
This assessment is accessed by LLM which produces a confidence score between 0 and 1, along with an explanation and any remaining plans. 
If the score exceeds a predefined threshold (\eg, $threshold \geq 0.8$ in our current implementation), the action selection loop terminates. 
Otherwise, the execution result, evaluation score, rationale, and remaining plans are appended to the data context (Sec.~\ref{subsection:method-implementation}) and passed back to the \planner Agent for the next round of action selection.
% 
% tool 2: falure > _action_error_handler()
(2) If an action fails, the agent triggers the \toolname{action_error_handler()} tool to process the error message and determine the next step, either (1) retrying the same action in the \executor Agent, or (2) initiating a new round of planning in the \planner Agent (\ie, finding an alternative solution path in the search tree $\mathcal{T}$). 
% \wyf{Note: the actual code implementation is a slightly different. TODO: try to align with paper.}
% To support error recovery, we provide three types of linters to automatically correct common issues: a SQL linter~\cite{SQLLinter}, a Python linter~\cite{PythonLinter}, and a Vega-Lite linter~\cite{chen2021vizlinter}.
% We provide three types of linters to fix the execution error for re-running the same action: SQL linter~\cite{SQLLinter}, Python linter~\cite{PythonLinter}, and Vega-lite linter~\cite{chen2021vizlinter}. 

Together, the three agents coordinate together to generate a sequence of actions to answer user query, enhanced by advanced prompt design and context management (Sec.~\ref{subsection:method-implementation}). 



% \subsubsection{Action Space} 
% \label{subsection:method-action-space}
\textbf{Action Space.}
% what we did: 
\systemname defines a compositional action space consisting of atomic operations that serve as the fundamental execution primitives for data-driven exploration tasks. 
These actions are dynamically composed, sequenced, and executed by the multi-agent workflow to support diverse analytical tasks, including data filtering, transformation, modeling, visualization, and cross-visualization coordination, and it is designed to be refinable and extensible for adaptation across different domains~\cite{gao2025democratizing}. 
% reason: 
This action-level design offers two key advantages. 
First, it improves reasoning accuracy and execution stability by constraining the solution space to a set of well-defined operations amenable to optimization-based planning (see \planner Agent). 
Second, it promotes algorithmic transparency, allowing users to trace and validate each decision step in the analysis process clearly~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% \wyf{[Yifang] We should also mention that each action could increase LLM's performance -- avoid re-generating everything from starting.}
% This action-level granularity enhances reasoning accuracy and stability by constraining the solution space to well-defined operations with optimized action selection process, while providing algorithmic transparency that enables users to inspect and validate the decision-making process step-by-step~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% Moreover, this modular design is naturally compatible with reinforcement learning frameworks, which operate over action-level representations to optimize long-term strategies. 
% Moreover, this modular design enables future integration with reinforcement learning frameworks, which inherently rely on action-level granularity for optimizing long-term strategies. 
% lays the groundwork for future integration with reinforcement learning frameworks, which inherently require action-level granularity to enable learning from interaction histories and optimizing long-term analytical strategies. 
% Could be enhanced by reinforcement learning (which naturally require action-level design) in future work. 
% 
% implementation: 
Specifically, we design four types of actions derived from general data science tasks: \textit{data filtering}, \textit{data transformation}, \textit{data modeling}, and \textit{data visualization} (Supplementary Notes 1.1), building on techniques such as NL2SQL~\cite{liu2024survey, hong2024next}, AI4VIS~\cite{wu2021ai4vis}, and LLM for data science~\cite{guo2024ds, hong2024data}. 
The \textit{data modeling} category includes a set of actions frequently used in data science (\eg, \actionname{text_embedding} and \actionname{dimension reduction}).
% The \textit{data modeling} category reflects the methodological diversity of SciSci research~\cite{liu2023data, shao2025sciscigpt}, including statistical modeling, network analysis \wyf{([TODO: add network analysis tools])}, and machine learning. 
% For \textit{data visualization}, we incorporate two design spaces for dashboard type selection (action \actionname{add_chart_type}, \cite{shi2020calliope, wang2019datashot}) and interaction formulation (action \actionname{add_params}) (Supplementary Notes 1.1).
% and visual annotation augmentation (action \actionname{add_annotation}). 
For \textit{data visualization}, we include actions to select the visualization type (\actionname{add_chart_type}) and interaction type (\actionname{add_params}), as well as adding data (\actionname{add_data}) and visual encoding (\actionname{add_encoding}). 
% Other actions such as \actionname{add_data} and \actionname{add_encoding} are also included to generate interactive figures. 
In addition to "add" actions, we provide "update" actions to refine existing figures (\eg, \actionname{update_encoding}).
% \wyf{[yifang: to refine the writing and code: "add" could also be replaced by "refine" and "delete".} 
% 
Building on these atomic actions, the LLM engine could easily interpret the user's analytical intent using natural language instructions and graphical interactions, and use bidirectional mapping (Sec.~\ref{subsection:conceptual-framework}-bidirectional mapping) to generate, refine, and extend figures during the exploration process. 


\textbf{Coordination Across Figures within a Data-Driven Artifact.} 
\systemname supports the generation and coordination of multiple linked figures within a single data-driven artifact, enabling coherent multi-view exploration. 
Coordination is triggered in two stages during visualization-driven analysis.
% 1. extended figure generation
First, when users generate a new figure by interacting with an existing one (e.g., brushing regions or selecting data points), the system jointly interprets GUI interactions and natural-language instructions to infer analysis intent. 
These interaction-derived constraints are injected into subsequent analytical actions, ensuring that newly generated figures remain semantically aligned with prior exploration. 
To support iterative analysis, the LLM engine can flexibly query both the underlying SciSci domain database and a temporary workspace derived from prior figures (Fig.~\ref{fig:Figure1}c–D).
% 2. coordination
Second, to enable persistent cross-figure coordination, the system records a coordination schema for each pair of linked figures at generation time, derived from the executed action sequence. 
When users later update selections in an initiating figure, the system retrieves the corresponding schema and re-executes the stored analytical workflow, which includes both data filtering and downstream analysis steps, to regenerate all coordinated figures with consistent, up-to-date results. 
This design supports flexible cross-figure interaction while preserving provenance and reproducibility of the analytical process (Supplementary Note 1.3).







% 2. 针对不同情况，对selector和optimizor有不同的强约束。
%   - drill_down。 数据起点：ego chart 的 workspace 表（你现在的设计）。强约束：select_tables → filter_rows，filter_rows 将 brush ROI 翻译成 WHERE 条件（上一个 House Committee 案例）。→ optional join other tables to get more data。
%   - bottom_up。 数据起点：case dataset 表(含有filtering criteria的表)。强约束：select_tables → filter_rows，filter_rows 将 brush ROI 翻译成 WHERE 条件（上一个 House Committee 案例）。→ optional join other tables to get more data。其中，filter_rows 用 brush 的 time 维度（如果有）+ 从 applied_filters 里保留 time 条件，而移除 state='Florida' 这种地理限制。



% 对应figure 1: extended chart加上coordination这一步，单独实现。不要跟前面action space混在一起。删掉前面的add_coordination action. 




% % \subsubsection{Data-Driven Artifact} 
% % \label{subsection:method-data-driven-artifact}
% Our hybrid interface combining LUI and GUI introduces unique challenges for interpreting user intent. 
% % , as users can interact through both natural language and direct manipulation modalities. 
% % The communication between human users and LLM agents presents unprecedented challenges for data querying and analysis due to the hybrid user interfaces (which enable both natural language input and direct manipulations).  
% To address this, we propose two strategies for generating, manipulating, and exploring data-driven artifacts within the multi-agent workflow and action space. 

% \textbf{Hybrid User Intention Inference for Data Querying.} 
% \wyf{TODO: remove redundant from conceptual framework.}
% We first develop a dynamic prompting mechanism to accurately infer user intents from hybrid natural language and direct manipulation inputs, enabling precise data querying for filtering and transformation actions. 
% % GUI input
% For direct manipulation (\eg, brushing and clicking), we implement a semantically-aware mapping $\mathcal{M}: \mathcal{V} \leftrightarrow \mathcal{D}$ between the visualization space $\mathcal{V}$ and the underlying database space $\mathcal{D}$. 
% % For direct manipulation inputs, we employ a \wyf{semantically-aware} approach that transforms GUI interactions (\eg, brushing and clicking) into structured database queries through a bidirectional mapping function 
% % $\mathcal{M}: \mathcal{V} \leftrightarrow \mathcal{D}$ 
% % between visualization space $\mathcal{V}$ and database space $\mathcal{D}$. 
% This mapping translates GUI inputs (\ie, dashboard filtering) into structured queries by tracing visual selections back to the original database columns or entities (\eg, papers, patents, and researchers) using shared attributes from the raw data or intermediate results (Fig.~\ref{fig:action-enhancement}). % (
% % \wyf{Specifically, the filtering criteria extracted from the dashboards trace back to original database columns and data entities (\eg, paper, patent, and researcher) by using shared attributes available either directly in the database or from intermediate data structures and derived dataframes (Fig.~\ref{fig:action-enhancement}).} 

% % Overview: spatial selection + semantic context
% These GUI interactions $I_t = (i_1, ..., i_k)$ (at time $t$) are dynamically integrated with natural language inputs $NL_t$ to construct a comprehensive data query 
% $Q_{t+1} = \mathcal{T}(I_t, NL_t, \mathcal{M}_{active}, H_t)$, 
% where transformation function $\mathcal{T}$ synthesizes the current user input ($I_t$ and $NL_t$), $\mathcal{M}_{active}$ denotes the active dashboard-to-database mappings, and $H_t$ represents historical context, including current user session's intermediate data structures and derived dataframes.
% % integrates current user input with the mapping between current active visualization dashboard and database, and historical context $H_t$ (representing prior user session state and results). 
% This formulation ensures that the resulting queries preserve both the spatial constraints specified through direct manipulation from the dashboards and the semantic context expressed in natural language. 
% % The resulting queries thus preserve both spatial selection constraints from the dashboards and semantic context from natural language queries. 
% % M_context​⊂M denotes the context-specific instantiation of the base mapping that maintains provenance between currently active visual elements and their corresponding database records
% % Ht​ captures the cumulative interaction history and user session state at time t. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/action-enhancement.jpg}
%     \caption{Hybrid User Intention Inference for Data Analysis.}
%     \label{fig:action-enhancement}
% \end{figure}
% % 这个是在每个action里面，dynamic prompting to 考虑both user interaction and NL query, to generate 对应的data query or modeling
% % goals: 
%     % 1. ask follow-up quesion -> generate alter chart
%     % 2. modify current chart
%     % 3. filter data to update other charts (coordination) 
% % method: 
%     % Using filtering criteria + dynamic prompting + pre-stored dataframe in the user history database, to inject into data filtering/transformation actions. 
%     % If filtering criteria attribute is within original DB, then direct dynamic prompting
%     % If no, then trace to raw db using the pre-stored dataframe in the user history database -- a preset is, we should force these pre-stored dataframe to have at least one column in raw database.
%     % <draft>
%     % For example, to enable data querying through GUI-based visualization interactions (action: \actionname{add coordination}), we implement a multi-step filtering strategy Fig.~\ref{fig:??}). 
%     % Each data point \wyf{(before transformation and aggregation)} is bound with a unique identifier, allowing the action to trace filtered subsets of data back to the database using the GUI selection criteria and corresponding data point IDs. 
%     % % Each data point is bound with a unique identifier so that when user filter a subset of data in dashboard, we can trace back to the database by filtering based on the filtered criteria from GUI input and corresponding ID of each data point (Fig.~\ref{fig:??}). 
%     % % The \toolname{gui_inferred_data_query()} xxx. 
%     % % add mechanisms about linking user's GUI interaction to backend data (how to coordinate -- using vegalite解析 to SQL re-generation, ...) Vis coordination部分 
%     % % Coordination: 详细介绍--ID based indexing. 和User management db (temporary生成的csv for the visualization) link在一起
%     % % 先生成一个SQL语句for filtering, 再把这个SQL语句作为dynamic prompt注入到所有的tool as input parameter -- either生成融合式的SQL (filtering/transformation), or直接执行这条sql语句生成新的dataframe for analysis/visualization actions
%     % </draft>

% \textbf{Dashboard Coordination.} 
% \wyf{TODO: update with latest implementation: data-point level and aggregation-level.}
% % 这个是生成好一个artifact（multiple coordinated dashboard）以后，怎么快速支持用户刷选数据
% % Method: 生成两个关于这个artifact的coordination文件，并存储在user chat history里面：
%     % global_connection.json
%     % coordination_templates.json
% % 我们比LightVA牛逼: 他们的coordination的前提是必须share common column. 而我们可以deep dive to large-scale database to generate complex coordination
% % TODO: `replace_conditions()`这个function可能有问题--或许要替换成LLM-driven的？如果穷举不完的话
% Data-driven artifacts support cross-dashboard interactions, allowing users to filter data in one dashboard and immediately observe corresponding data changes in others. 
% To ensure real-time responsiveness, we employ an LLM-driven approach that dynamically generates and stores coordination schemas among dashboards each time a new dashboard is created within an artifact. 
% % To ensure real-time responsiveness, every time a new dashboard is generated within an artifact, we employ a LLM-driven approach to dynamically generate and stores coordination schemas among dashboards within this artifact. 
% % 
% Specifically, for each coordinated dashboard pair (identified by dashboard IDs and directional interaction links from the initiating to the extended dashboard), we maintain interaction-filtering pairs that define the coordination behavior. 
% Each pair comprises an interaction type (\eg, 2D brush selection) coupled with an LLM-generated SQL schema template that dynamically updates as users modify filtering regions in real-time. 
% % Each pair consists of an interaction type and the associated filtering SQL schema template, which is generated by LLM and can be dynamically updated based on real-time GUI input. 
% This design supports efficient, flexible filtering and seamless multi-view exploration. 
% % <interaction\_type, filtering\_schema> pair in a SQL schema templates which will be updated based on real-time GUI interaction filtering criteria. 
% % This coordination design enables efficient, dynamic filtering and seamless user exploration across dashboards.
% % To make the coordination response time in real time, we 使用一种无机的手段--保存一个data-driven artiface所有dashboard之间的coordination pair (linked by chart ID, directional, from ego chart to extended chart) and interaction-filtering pair，记录每一类interaction的filtering SQL schema template. 





% % scalable to extend and refine
% The current LLM workflow supports easy adaption to other domains by revising the action space and tool design without altering the underlying multi-agent architecture, ensuring broad applicability across computational social science and beyond. 
% % \wyf{TODO: refine integrate this sentence with the first sentence: Domain-specific customizations could be integrated into \textbf{LLM frameworks} (\eg, multi-agent systems) and \textbf{tool designs} to enhance these capabilities to specialized analytical contexts.}
% % % This modular design enables straightforward adaptation to other scientific domains beyond SciSci by allowing domain experts or AI agents to modify the action space while preserving the underlying compositional architecture, demonstrating the framework's extensibility across computational social science and broader data science applications. 
% % % The action space could be easily adjusted to other science fields beyond SciSci in computational social science and broader data science by human experts or LLM agents. 
% % % action library: could be edited to adjust to other science fields beyond SciSci/CSS — by replaces and extended by human experts or LLM agents (create new agents based on user queries)


\subsection{Data Management}
\label{subsection:method-data-module}
% Such new type of human-AI collaboration for scientific discovery requires rethinking data storage architecture itself. 
The Data Management Module rests on three interlinked databases (Fig.~\ref{fig:Figure5}c):
(1) domain databases that provide the empirical substrate for analysis--SciSci rational database; 
(2) knowledge embeddings, which are usually vectorized representations of domain knowledge that enable techniques such as retrieval-augmented reasoning (RAG) for domain-aware reasoning--vector database for SciSci literature; 
and (3) exploration histories that record non-linear human–AI interactions and data-driven artifacts, capturing the evolving logic of discovery. 
% 
% (1) SciSci
For our test domain SciSci, we incorporate two primary data sources. 
The first one is a university-level dataset capturing innovation activities and researcher information~\cite{wang2023innovationinsights}, collected and preprocessed from multiple sources, including public datasets such as Microsoft Academic Graph (MAG)~\cite{wang2019review}, PatentsView~\cite{patentsview}, and Reliance on Science~\cite{marx2020reliance, marx2022reliance}, 
as well as proprietary institutional datasets from Technology Transfer Office (TTO) on invention disclosures and outcomes and HR Office on faculty roster with demographic data (e.g., name, gender, rank, and department).
% (1) \textbf{SciSciNet}, the largest open data lake of SciSci~\cite{shao2025sciscigpt} that covers comprehensive records and entities essential for this domain, 
The second data source is SciSciCorpus~\cite{shao2025sciscigpt}, a vector database containing the key literature in this field, with paper documents chunked and indexed to support retrieval-augmented generation (RAG) for enhanced domain understanding.
% In addition, our case studies integrate proprietary SciSci datasets, including confidential data of faculty (\eg, gender and department) provided by our collaborating university's HR office.
% \wyf{In addition, our case studies integrate proprietary SciSci datasets, including \textbf{Overton}~\cite{Overton} that contains global policy documents and citation linkages between policies and papers, as well as confidential data about demographic information of faculty provided by our collaborating university’s HR office.}


% (2) User Management and Data-driven Artifact Management 
% \wyf{[yifang: not only support tree but also a graph version of all dashboard linkages]}
Additionally, we design a user and chat history management database (Supplementary Notes 1.5) tailored to support LLM-native figures and data-driven artifacts for non-linear exploration process. 
The \code{messages} table stores individual question-answer pairs for each user \code{conversations} session, establishing the conversational foundation. 
% artifact level: 
Each message links to corresponding artifact entries in three artifact-related tables (\code{message_artifact}, \code{artifacts}, and \code{artifact_versions}), which maintains comprehensive metadata for each data-driven artifact, including a list of figure identifiers, coordination relationships and schemas that define cross-figure interactions. 
The figure identifiers in each artifact link to two tables, \code{figures} and \code{figure_versions}, which store the components of each LLM-native figure: $V$, $C$, $D$, $M$ (Sec.~\ref{subsection:conceptual-framework}), as well as action-level reasoning, codes, and results. 
The two tables, \code{artifact_versions} and \code{figure_versions}, records the exploration history as a list of temporal snapshots of artifact-level and figure-level states, such that each user input generates a new record, preserving the complete exploration history. 
% Two additional tables support detailed exploration tracking: \code{artifact_versions} table captures temporal snapshots of artifact states, while \code{artifact_operations} table logs all user interactions, including dashboard manipulations and drill-down operations. 
% dashboard level: 
% At the dashboard level, each visualization is stored in the \code{dashboard} table with multi-modal representations (\ie, Vega-Lite specifications, visualization images, and text insights). 
% The database implements immutable versioning where any dashboard modification creates a new record, preserving the complete editorial history. 
% 
This architecture enables complete reconstruction of analytical pathways, allowing users to trace their discovery processes and revert to previous analytical states transparently. 
% We also have two additional tables, \code{artifact_versions} and \code{artifact_operations}, to store the exploration history including dashboard manipulation and drilling down. 

\subsection{Implementation Details} 
\label{subsection:method-implementation} 
\textbf{Technology Stack.}
\systemname is implemented as a full-stack web application utilizing modern development frameworks and cloud infrastructure. 
The frontend employs React.js~\cite{React} for component-based user interface development, Redux.js~\cite{Redux} for state management, and Vega-Lite for declarative visualization rendering~\cite{satyanarayan2016vega}. 
The backend architecture is built on the Flask framework~\cite{Flask} with Python~\cite{Python}, providing RESTful API services and data processing capabilities. 
Specifically, the multi-agent workflow leverages LangChain~\cite{LangChain} and LangGraph~\cite{LangGraph} for complex agent coordination, with Claude 4.5 Sonnet~\cite{AnthropicAPI} serving as the primary language model. 
The system architecture supports model substitution, enabling integration with alternative LLM providers as needed. 
Data storage employs a hybrid approach: Google Big Query~\cite{BigQuery} manages relational SciSci domain datasets and user chat histories, while Pinecone~\cite{Pinecone} serves as the vector database for the retrieval-augmented generation module, storing chunked domain literature for semantic search and knowledge retrieval. 


\textbf{Action-based Streaming Output.} 
To balance analytical transparency with user experience, we implement action-level streaming output that selectively displays critical workflow information without overwhelming users with verbose LLM reasoning. 
The interface presents only essential decision points, specifically action selection and action sequence generation processes, providing users with meaningful insights into analytical behavior.
% To balance the data analysis transparency and the information overload of outputing every word of the LLM reasoning, we design an action-level streaming output in the user interface. 
% Only the action selection and action sequence generation process will be displayed. 
Upon completion of each user query, the system delivers comprehensive results including SQL queries, Python code, processed dataframes, visualization images, and structured Vega-Lite JSON outputs. 
This approach ensures users can monitor system progress through high-level action updates while accessing detailed technical artifacts for validation and reuse. 
% We also provide the final results for each user question, (SQL code, Python code, dataframe, visualization img and json etc.)
% % To balance the information transparency and the overwhelming. 
% % Output: action level reasoning (output action selection procedure, and result for each action (SQL code, Python code, ,,,)); And final result (csv, vega-lite img and json, SQL/Python codes). 
% % Future work: edit the code in each action -- allow action-level manipulation -- a tighter way for HAI collaboration.


\textbf{Prompt and Context Design.}
We employ four prompt engineering techniques to optimize our multi-agent workflow performance~\cite{white2023prompt, sahoo2024systematic}, including structured formatting, chain-of-thought reasoning, few-shot learning, and dynamic prompting. 
In addition, to make the context compact, we developed a structured data context that stores only essential information about each executed action, including action indices, objectives, execution status, results, evaluation scores and rationale, and remaining tasks (Supplementary Notes 1.4). 
% Please refer to our supplymentary information \wyf{(Sec.~\ref{subsection:si-prompt-design} and Sec.~\ref{subsection:appendix-context-design})} for more details.








% \textbf{Prompt Design.} 
% We employ four prompt engineering techniques to optimize our multi-agent workflow performance~\cite{white2023prompt, sahoo2024systematic}: 
% % 
% (1) Structured XML formatting.
% We develop a suite of XML tags to compartmentalize prompt components, such as \code{<roles>}, \code{<instructions>}, and \code{<constraints>} (Supplementary Note~\ref{section:appendix-prompt-design-structured-prompt}), to increase the clarity, accuracy, and parseability~\cite{PromptXML, sahoo2024systematic}. 
% % This structured approach improves LLM comprehension and response consistency across different agent interactions.
% % 
% (2) Chain-of-thought reasoning.
% We specifically use the \code{<internal_reasoning>} tag to guide the model work out a plan with step by step instructions, enhancing reasoning robustness and analytical coherence~\cite{wei2022chain}. 
% % 
% (3) Few-shot learning.
% We maintain an example library (Supplementary Note~\ref{subsubsection:appendix-prompt-design-fewshot-learning}) that enables dynamic retrieval and insertion of contextually relevant examples into prompt templates using the \code{<example>} tag, providing targeted guidance for diverse analytical scenarios~\cite{brown2020language}.
% This modular separation maintains prompt conciseness and facilitates system maintenance and expansion as conversational history grows, ensuring scalable performance without compromising prompt clarity. 
% % This type of separation (of an example library) keeps the original prompt short and clean and make it easier to maintain and expand when the user chat history increases. 
% % for agents and tools to retrieve and insert into the prompt template with the \code{<example>} tag~\cite{brown2020language}. 
% % This type of separation (of an example library) keeps the original prompt short and clean and make it easier to maintain and expand when the user chat history increases. 
% (4) Dynamic prompting.
% Beyond static contents, we incorporate variable contents into the prompts, such as user input (both natural language and direct manipulation), conversational context (\eg, chat history, data context, and RAG-retrieved knowledge), and few-shot learning examples, which allows more precise user intent interpretation and contextually relevant responses~\cite{sahoo2024systematic}.  
% % Future work: 
% % - 每次对这个文件retrieve 3个最相关的example
% % - Prefill Claude's response for greater output control 
% %     - TODO


% \textbf{Context Management.} 
% The iterative data exploration process and multi-modal outputs (\eg, data, code, and visualization) present challenges to deal with long context during the multi-agent workflow. 
% We design several stratifies to address this problem. 
% % (1) Within one QA round
% (1) Single-round conversation management.
% We developed a structured data context format for individual question-answer cycles that stores only essential information about action sequences, including action indices, objectives, execution status, results, evaluation scores, rationale, and remaining tasks (Supplementary Note~\ref{subsection:appendix-data-context-design}). 
% % This selective retention reduces context overhead while preserving critical workflow information. 
% % we specifically design a data context format to deal with one round of conversation (one QA round). 
% % Only the action sequence will be stored during the process, including action index, goal, action execution status (whether success or failure), action results, evaluation score, reason, and remaining tasks and plans (Supplementary Note~\ref{subsection:appendix-data-context-design}). 
% % (2) Semantic context
% (2) Cross-session semantic compression.
% For conversations spanning multiple question-answer rounds or cross-sessions, we employ automated summarization to compress chat history into concise paragraph-form representations. 
% % This approach maintains contextual coherence while preventing context window overflow, enabling sustained analytical workflows without performance degradation. 

% % For one chat session across different QA round and cross-session contexts, we summarize the chat history into a paragraph to compact the context. 

% % Note: Specifically, in addition to traditional chat history, we've 
% % 3-2 integrate vision language model (vis code and image) to infer insights and recommend next-step exploration. 
% % 3-3 只展示重要的reasoning信息，to avoid overwelming 例如action_name, result (SQL code, python code, vega-lite code, dataframe, vis image, ...) 
% % - Long context prompting tips
% %     - TODO: may need to add chat history summary
% %     - https://docs.anthropic.com/en/docs/build-with-claude/prompt-engineering/long-context-tips
% \end{methods}

==> sections/archive/05-method/05-method-20260315.tex <==
\section{Methods} 
\label{section:methods}
% \begin{methods}
% Based on this conceptual framework, we further develop a proof-of-concept system, \systemname, to demonstrate how to facilitate scientific discovery using these LLM-native figures with a non-linear human exploration process. 
%We describe \systemname, an instantiation of the proposed framework developed for the science of science (SciSci) domain. The system integrates heterogeneous datasets including grants, research papers, patents, and policy documents, with complex citation linkages; 
%complicated analysis tasks such as tracing the evolution of knowledge and identifying emerging research frontiers; 
%and high-stakes decision-making scenarios, including identifying untapped innovation potential for university leaders and guiding strategic funding allocations for funding agencies. 
% 

% the database design and 


% %%%%%%%%%%%%%% Method Section Begins %%%%%%%%%%%%%%%%
% \subsection{System Overview} 
\systemname consists of three modules: the hybrid user interface, the multi-agent LLM engine, and the data management module (Fig.~\ref{fig:Figure5}). 
We describe each in more detail below. 
% \systemname introduces a hybrid user interface that enables users to interact with underlying AI agents and data through both natural language and direct manipulation (Fig.~\ref{fig:Figure5}a). 
% These interactions are orchestrated by a multi-agent LLM system that interprets user intent and extracts data insights efficiently in real time. 
% The system consists of three modules. 
% The Hybrid User Interface integrates the language user interface (LUI) and interactive visualization-based graphical user interface (GUI) into a web frontend (Fig.~\ref{fig:Figure5}b). 
% % allowing users to fluidly switch between language-based querying and visual exploration (Fig.~\ref{fig:Figure5}b). 
% % that are easy to be accessed by users. 
% The Multi-Agent LLM Engine forms the analytical backend, comprising three coordinated agents: \planner, \executor, and \evaluator (Fig.~\ref{fig:Figure5}d). 
% The agents understand user queries, generate plans, execute analytical actions, and iteratively reflect on results to guide the analysis process. 
% The Data Management Module manages three types of information: 
% (1) a large-scale relational database of SciSci data, 
% (2) a vector database of SciSci domain literature that enables retrieval-augmented generation (RAG) for domain-aware reasoning, 
% and (3) a user chat history database, specifically designed for LLM-native figures and data-driven artifacts that support human nonlinear exploration processes (Fig.~\ref{fig:Figure5}c).  

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/20260217/system-overview.jpg}
    \caption{
    \bodyfigurelabel{fig:Figure5}
    \textbf{System design in \systemname.}
    \textbf{(a)} User input types include natural language input and graphical input. 
    \textbf{(b)} The Hybrid User Interface Module serves as the frontend of the system.  
    % The system allows users to interact in two ways, combining the accessibility of language UI with the clarity and efficiency of graphical UI, particularly in interactive visualization scenarios under data exploration. 
    Left: natural language interaction using a traditional chatbot and an inline chatbot. 
    Right: graphical interaction using interactive dashboards (\eg, click, brush, and hover).
   \textbf{(c)} The Data Management Module manages SciSci domain datasets and knowledge and chat history.
    \textbf{(d)} The Multi-Agent LLM Engine serves as the backend of the system, including three agents and a set of tools. 
    }
    % \label{fig:system-overview}
\end{figure}


\subsection{Hybrid User Interface}
\label{conceptual-model-hybrid-ui} 
% Allow three types of interactions: chatbox input (NL), inline input (NL), and GUI input (operations on chart -- brush/filter/click/zoom/..., and GUI Widgets -- recommendation and coordination button)
% Three types of questions: 
% 1. init a new query
% 2. drill-down analysis: extend chart
% 3. fine-grained analysis: manipulate chart (scatter => + regression; bar => stacked bar)
% 4. AI recommendation: task decomposition + next-step exploration

We design a hybrid interface that couples an LUI and a GUI (Fig.~\ref{fig:Figure5}b), serving as the \systemname frontend through which users interact directly with the system (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance).
% (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance (User Input: $I_t$))

% 1. LUI, two parts: 
% (1) Chat history (linear)
% (2) Artifact session (inline, combined with GUI, non-linear) 
\textbf{Language User Interface (LUI)} (Fig.~\ref{fig:Figure5}b-left). 
%Language offers an expressive channel for curiosity. 
By allowing humans to ask open-ended questions in natural language, the LUI lowers the cognitive and technical barriers to data exploration. 
In addition to traditional chatbot panels, the interface includes inline conversational widgets, which allow dialogue to unfold within the visual context itself.
Users can initiate queries via chat, request AI-generated analytical suggestions, or interact directly with visualizations to ask follow-up questions, request AI recommendations, and coordinate and filter across multiple visualizations. 
In this way, conversation becomes an analytical instrument rather than a passive query mechanism. 

\textbf{Graphical User Interface (GUI)} (Fig.~\ref{fig:Figure5}b-right).  
% clarity and efficiency of graphics UI
While language captures ideas, visualization externalizes them by transforming abstract data into perceptible structures, providing an intuitive and efficient medium for uncovering patterns that may be difficult to articulate through statistics alone~\cite{anscombe1973graphs}. 
% interactivity
The GUI enables users to interact directly with LLM-native figures through standard visualization operations such as brushing, filtering, clicking, and zooming. 
Through these interactions, users can quickly and accurately access underlying data through visual elements (\eg, dots in a scatterplot and bars in a bar chart)~\cite{shneiderman1983direct, munzner2014visualization}. 
LLM-native figures (Sec.~\ref{subsection:conceptual-framework}) thus enable visual data exploration while tracing the associated analytical procedures and data. 
% at time $t$. 
% Additionally, to make these insights mutually legible to both human and AI, we present insights in multiple modalities to both human users and LLMs: static images, interactive dashboards, textual summaries, and underlying Vega-Lite specification code \wyf{(Fig.~\ref{??}}). 
% 
% (2) Domain Object: Data-driven Artifact
In addition to individual figures, \systemname supports data-driven artifacts (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), which are stored as linked figures with associated coordination rules and interaction histories.
% In addition to individual figures, \systemname supports data-driven artifacts (Sec.~\ref{subsection:conceptual-framework}-Artifact and Provenance), which allow users to refine and extend their analysis.  
% Starting from an existing figure, users can enter follow-up instructions to refine it (\eg, transforming a descriptive scatterplot into a correlation analysis) or select a subset of data in the figure to generate new coordinated figures that extend the line of exploration. 


\subsection{Multi-Agent LLM Engine} 
\label{subsection:method-llm}
Creating this hybrid interface requires an AI infrastructure capable of understanding heterogeneous user inputs, reasoning over complex data, and generating data insights in real time. 
% Recent advances in large language models and AI agents offer transformative potential to interpret user intent and accelerate data-driven discovery with unprecedented efficiency~\cite{shao2025sciscigpt, guo2024ds}. 
Thus, we design a multi-agent LLM engine that coordinates the communication between the user and the large-scale underlying data, leveraging recent advances in LLM-based reasoning~\cite{yao2023react}, planning~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-improvement~\cite{madaan2023self, shinn2023reflexion} to support a wide range of analytical intents and exploration pathways. 
The engine includes three core agents, \planner, \executor, and \evaluator, which operate at an \actionname{action}-level of granularity (Fig.~\ref{fig:Figure5}d). 
Together, they form an automated reasoning loop that spans data analysis, visual insight generation and manipulation, dashboard coordination, and iterative exploration. 


\textbf{Multi-Agent Workflow.}
% To accommodate diverse analytical tasks and reasoning demands, we design a multi-agent workflow comprising the three specialized AI agents, leveraging recent advances in LLM-based reasoning~\cite{yao2023react}, planning~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-improvement~\cite{madaan2023self, shinn2023reflexion}. 
% and abilities such as ReAct~\cite{yao2023react}, three-of-thoughts~\cite{yao2023tree}, tool use~\cite{schick2023toolformer}, and self-refining and self-correction~\cite{madaan2023self}. 
% (1) Planner
The \planner Agent serves as the direct intermediary between the user interface and the analytical backend. 
It infers a user's intentions by taking the user's natural language queries and direct manipulation inputs (\eg, brushing and filtering) and formulating an initial execution strategy. 
Specifically, it performs query triage across three distinct pathways.
For high-level complex analytical goals, it decomposes the query into structured sub-questions and returns them to users for clarification or confirmation. 
For exploratory scenarios where users seek guidance on subsequent analytical steps, it recommends potential next steps based on exploration history and intermediate results. 
For low-level questions, it initiates action planning, selection, and execution procedures. 
% For low-level concrete questions, it directly returns control to the \planner Agent to invoke other tools for immediate action selection and execution.
% Including task decomposition, AI recommendation, Candidate and Optimal Action Selection, and Initial Action Sequence Generation (Initial Planning, that could be adjusted based on real-time execution results). 
% TODO: first translate user queries into typical analysis tasks (Tamara's book and the paper -- Low-Level Components of Analytic Activity in Information Visualization) 

To accomplish these tasks, the agent leverages four specialized tools: 
(1) the \toolname{user_query_classifier()} tool classifies user queries into high-level (requiring decomposition) and low-level (directly executable) categories, enriched by domain knowledge retrieved via literature search; 
% high-level: which will be decomposed into sub-questions based on the user request and external domain knowledge (using \toolname{literature_search()} below) 
(2) the \toolname{ai_recommender()} tool proposes follow-up exploration suggestions based on user intent, multi-modal data context, and domain knowledge; 
(3) the \toolname{literature_search()} tool~\cite{shao2025sciscigpt} retrieves and summarizes relevant literature from the SciSci domain using retrieval-augmented generation (RAG), thereby grounding the planning process in domain-specific context; 
% contextualizes the reasoning and planning process within the Science of Science domain, by using retrieval-augmented generation (RAG) to identify the most relevant papers in the SciSci domain and stores a summary paragraph in the context as reference to assist the plan formulation. 
% This integration ensures that data exploration is grounded in existing scientific understanding while enabling novel hypothesis generation. 
% "which is output to the user and stored in context memory to guide subsequent activities."
% LiteratureSpecialist. Understanding and contextualizing research questions within the SciSci domain is critical for determining the novelty of the research question and ensuring efficient use of existing knowledge, including previous approaches to similar scientific questions, conclusions from prior studies, and other researchers’ assessments of the implications of their findings. 
% 
(4) the \toolname{action_selector()} tool utilizes a tree-based planning strategy that synthesizes principles from tree-of-thoughts reasoning and search~\cite{yao2023tree, zhuang2023toolchain}. 
% and and A* search~\cite{zhuang2023toolchain}. 
% selects an optimal action as next-step for execution, given the user query and historical executed action sequence and results.
% The tool applies a tree-based search planning (Fig.~\ref{fig:a-star}) to capture a comprehensive decision space, built on and improve the tree of thoughts~\cite{yao2023tree} and A* search algorithm~\cite{zhuang2023toolchain}. 
The tool constructs a dynamic search tree $\mathcal{T}$, where each node represents an atomic analytical action along with its execution results, and edges encode temporal dependencies between actions. 
This design enables exploration of multiple reasoning pathways by navigating a structured and comprehensive decision space (Supplementary Note 1.2). 
% while maintaining computational tractability through intelligent pruning strategies.
% ToT: search for a comprehensive space for solutions -- better than CoT. 
% Specifically, the tool constructs a search tree $T$ with each node representing an atomic action and edge representing the ordered sequence to execute actions. 



% (2) Executor
The \executor Agent executes the selected action by invoking the corresponding tool to generate the appropriate code (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}).
% The \executor Agent executes the selected action by first generating corresponding codes by calling corresponding tool for this action (\textit{SQL} for data filtering and transformation, \textit{Python} for analysis and modeling, and \textit{Vega-Lite} for data visualization~\cite{satyanarayan2016vega}). 
These code snippets are then executed within three isolated sandboxes, \toolname{execute_SQL()}, \toolname{execute_Python()}, and \toolname{execute_VegaLite()}, to produce intermediate outputs in LLM-native figures, including dataframes, visualization specifications, rendered images, and textual insights, among others. 
% % optimization 
% To optimize memory allocation and execution efficiency when operating on large-scale datasets, we adopt a staged strategy: 
% each intermediate SQL-related action (\eg, filtering and transformation) is executed on a randomly sampled subset of 1000 records, while the full SQL query is deferred and executed only at the final stage of the SQL pipeline (right before data modeling or visualization).


% (3) Evaluator
The \evaluator Agent incorporates the principle of self-reflection~\cite{shinn2023reflexion} from agent design frameworks to evaluate the outcomes of executed actions and guide subsequent planning. 
It handles two types of action outcomes, successful and failed executions, using two dedicated tools: the \toolname{task_evaluator()} tool and the \toolname{action_error_handler()} tool.
% 
% tool 1: success > _task_evaluator()
When an action is executed successfully, the agent invokes the \toolname{task_evaluator()} tool to assess how well the result answers the user’s query. 
This assessment is accessed by the LLM which produces a confidence score between 0 and 1, along with an explanation and any remaining plans. 
If the score exceeds a predefined threshold, the action selection loop terminates. 
% ($threshold \geq 0.8$ in the current implementation)
Otherwise, the execution result, evaluation score, rationale, and remaining plans are appended to the data context (Sec.~\ref{subsection:method-implementation}) and passed back to the \planner Agent for the next round of action selection.
% 
% tool 2: falure > _action_error_handler()
If an action fails, the agent triggers the \toolname{action_error_handler()} tool to process the error message and determine the next step, either retrying the same action in the \executor Agent, or initiating a new round of planning in the \planner Agent (\ie, finding an alternative solution path in the search tree $\mathcal{T}$). 
% \wyf{Note: the actual code implementation is a slightly different. TODO: try to align with paper.}
% We provide three types of linters to fix the execution error for re-running the same action: SQL linter~\cite{SQLLinter}, Python linter~\cite{PythonLinter}, and Vega-lite linter~\cite{chen2021vizlinter}. 
% 
Together, the three agents coordinate to generate a sequence of actions that answer user queries, enhanced by advanced prompt design and context management (Sec.~\ref{subsection:method-implementation}). 



\textbf{Action Space.}
We define a compositional action space consisting of atomic operations that serve as the fundamental execution primitives for data-driven exploration tasks. 
These actions are dynamically composed, sequenced, and executed by the multi-agent workflow to support diverse analytical tasks, including data filtering, transformation, modeling, visualization, and cross-visualization coordination. The space is designed to be refinable and extensible for adaptation across different domains~\cite{gao2025democratizing}. 
% reason: 
This action-level design improves reasoning accuracy and execution stability by constraining the solution space to well-defined operations amenable to optimization-based planning in the \planner Agent, while simultaneously enhancing algorithmic transparency, enabling users to inspect and validate each analytical step~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% This action-level design offers two key advantages. 
% First, it improves reasoning accuracy and execution stability by constraining the solution space to a set of well-defined operations amenable to optimization-based planning (see \planner Agent). 
% Second, it promotes algorithmic transparency, allowing users to trace and validate each decision step in the analysis process clearly~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% \wyf{[Yifang] We should also mention that each action could increase LLM's performance -- avoid re-generating everything from starting.}
% This action-level granularity enhances reasoning accuracy and stability by constraining the solution space to well-defined operations with optimized action selection process, while providing algorithmic transparency that enables users to inspect and validate the decision-making process step-by-step~\cite{zhuang2023toolchain, hong2024data, chen2021vizlinter}.
% Moreover, this modular design is naturally compatible with reinforcement learning frameworks, which operate over action-level representations to optimize long-term strategies. 
% Moreover, this modular design enables future integration with reinforcement learning frameworks, which inherently rely on action-level granularity for optimizing long-term strategies. 
% lays the groundwork for future integration with reinforcement learning frameworks, which inherently require action-level granularity to enable learning from interaction histories and optimizing long-term analytical strategies. 
% Could be enhanced by reinforcement learning (which naturally require action-level design) in future work. 
% 
% implementation: 
Specifically, we design four types of actions derived from general data science tasks: \textit{data filtering}, \textit{data transformation}, \textit{data analysis}, and \textit{data visualization}, building on techniques such as NL2SQL~\cite{liu2024survey, hong2024next}, AI4VIS~\cite{wu2021ai4vis}, and LLM for data science~\cite{guo2024ds, hong2024data} (Supplementary Note 1.1). 
% The \textit{data modeling} category includes a set of actions frequently used in data science (\eg, \actionname{text_embedding} and \actionname{dimension reduction}).
% % The \textit{data modeling} category reflects the methodological diversity of SciSci research~\cite{liu2023data, shao2025sciscigpt}, including statistical modeling, network analysis \wyf{([TODO: add network analysis tools])}, and machine learning. 
% % For \textit{data visualization}, we incorporate two design spaces for dashboard type selection (action \actionname{add_chart_type}, \cite{shi2020calliope, wang2019datashot}) and interaction formulation (action \actionname{add_params}) (Supplementary Notes 1.1).
% % and visual annotation augmentation (action \actionname{add_annotation}). 
For \textit{data visualization}, we include actions for selecting the chart type (\actionname{add_chart_type}) and interaction type (\actionname{add_params}), as well as to attach or update data (\actionname{add_data} and \actionname{update_data}) and visual encodings (\actionname{add_encoding} and \actionname{update_encoding}). 
% Other actions such as \actionname{add_data} and \actionname{add_encoding} are also included to generate interactive figures. 
% In addition to "add" actions, we provide "update" actions to refine existing figures (\eg, \actionname{update_encoding}).
% 
Building on these atomic actions, the LLM engine can easily interpret the user's analytical intent using natural language instructions and graphical interactions, and use bidirectional mapping (Sec.~\ref{subsection:conceptual-framework}-bidirectional mapping) to generate, refine, and extend figures during the exploration process. 


\textbf{Coordination Across Figures.} 
\systemname supports the generation and coordination of multiple linked figures within a single data-driven artifact, enabling coherent multi-view exploration. 
Coordination is triggered in two stages during visualization-driven analysis.
% 1. extended figure generation
First, when users generate a new figure by interacting with an existing one, the system jointly interprets GUI interactions and natural-language instructions to infer analysis intent. 
These interaction-derived constraints are injected into subsequent analytical actions, ensuring that newly generated figures remain semantically aligned with prior exploration. 
To support iterative analysis, the LLM engine can flexibly query both the underlying SciSci domain database and a temporary workspace derived from prior figures (Fig.~\ref{fig:Figure1}c–D).
% 2. coordination
Second, to enable persistent cross-figure coordination, the system records a coordination schema for each pair of linked figures at generation time, derived from the executed action sequence. 
When users later update selections in an initiating figure, the system retrieves the corresponding schema and re-executes the stored analytical workflow, which includes both data filtering and downstream analysis steps, to regenerate all coordinated figures with consistent, up-to-date results. 
This design supports flexible cross-figure interaction while preserving provenance and reproducibility of the analytical process (Supplementary Note 1.3).


\subsection{Data Management}
\label{subsection:method-data-module}
The Data Management Module rests on three interlinked databases (Fig.~\ref{fig:Figure5}c).
(1) The SciSci relational database is a domain-specific database that provides the empirical substrate for analysis. 
It is a university-level dataset capturing innovation activities and researcher information~\cite{wang2023innovationinsights}. 
The data are collected and preprocessed from multiple sources, including public datasets such as Microsoft Academic Graph (MAG)~\cite{wang2019review}, PatentsView~\cite{patentsview}, and Reliance on Science~\cite{marx2020reliance, marx2022reliance}, as well as proprietary institutional datasets on invention disclosures and outcomes from technology transfer offices (TTOs), and faculty rosters with demographic data (e.g., name, gender, rank, and department) from university human resources offices. 
% 
(2) SciSciCorpus~\cite{shao2025sciscigpt} is a vector database for SciSci literature, in which full-text papers are chunked, indexed, and embedded to support retrieval-augmented generation (RAG). This enables more accurate and context-aware reasoning by LLM agents when addressing complex analytical queries in the SciSci domain.  
% 
% \wyf{[yifang: not only support tree but also a graph version of all dashboard linkages]}
(3) An exploration histories database is tailored to support LLM-native figures and data-driven artifacts for non-linear exploration processes, capturing the evolving logic of discovery (Supplementary Note 1.5). 
It includes a \code{conversations} table that stores all historical sessions created by the user, and a \code{messages} table that stores individual question-answer pairs for each user session, establishing the conversational foundation. 
% artifact level: 
Each message links to corresponding artifact entries in three artifact-related tables (\code{message_artifact}, \code{artifacts}, and \code{artifact_versions}), which maintain comprehensive metadata for each data-driven artifact, including a list of figure identifiers, coordination relationships, and schemas that define cross-figure interactions. 
The figure identifiers in each artifact link to two tables, \code{figures} and \code{figure_versions}, which store the components of each LLM-native figure: visualization, code, dataset, and meta information (Sec.~\ref{subsection:conceptual-framework}), as well as action-level reasoning, codes, and results. % $V$, $C$, $D$, $M$
It also includes two tables, \code{artifact_versions} and \code{figure_versions}, that
record the exploration history as a list of temporal snapshots of artifact-level and figure-level states, such that each user input generates a new record, preserving the complete exploration history. 
% The two tables, \code{artifact_versions} and \code{figure_versions}, record the exploration history as a list of temporal snapshots of artifact-level and figure-level states, such that each user input generates a new record, preserving the complete exploration history. 
% Two additional tables support detailed exploration tracking: \code{artifact_versions} table captures temporal snapshots of artifact states, while \code{artifact_operations} table logs all user interactions, including dashboard manipulations and drill-down operations. 
% dashboard level: 
% At the dashboard level, each visualization is stored in the \code{dashboard} table with multi-modal representations (\ie, Vega-Lite specifications, visualization images, and text insights). 
% The database implements immutable versioning where any dashboard modification creates a new record, preserving the complete editorial history. 
% 
This architecture enables complete reconstruction of analytical pathways, allowing users to trace their discovery processes and revert to previous analytical states transparently. 
% We also have two additional tables, \code{artifact_versions} and \code{artifact_operations}, to store the exploration history including dashboard manipulation and drilling down. 


% The Data Management Module rests on three interlinked databases (Fig.~\ref{fig:Figure5}c):
% (1) SciSci relational database, a domain database that provides the empirical substrate for analysis; 
% (2) a vector database for SciSci literature, a database of knowledge embeddings, which are vectorized representations of domain knowledge that enable techniques such as retrieval-augmented reasoning (RAG) for domain-aware reasoning; 
% and (3) an exploration histories database that records non-linear human–AI interactions and data-driven artifacts, capturing the evolving logic of discovery. 
% % 
% % (1) SciSci
% For our SciSci test domain, we incorporate two primary data sources. 
% The first is a university-level dataset capturing innovation activities and researcher information~\cite{wang2023innovationinsights}. The data are collected and preprocessed from multiple sources, including public datasets such as Microsoft Academic Graph (MAG)~\cite{wang2019review}, PatentsView~\cite{patentsview}, and Reliance on Science~\cite{marx2020reliance, marx2022reliance}, 
% as well as proprietary institutional datasets on invention disclosures and outcomes from technology transfer offices (TTOs), and faculty rosters with demographic data (e.g., name, gender, rank, and department) from university human resources offices.
% The second data source is SciSciCorpus~\cite{shao2025sciscigpt}, a vector database containing the key literature in this field, with paper documents chunked and indexed to support retrieval-augmented generation (RAG) for enhanced domain understanding.


% % (2) User Management and Data-driven Artifact Management 
% % \wyf{[yifang: not only support tree but also a graph version of all dashboard linkages]}
% Additionally, we design a user and chat history management database (Supplementary Note 1.5) tailored to support LLM-native figures and data-driven artifacts for non-linear exploration processes. 
% It includes a \code{conversations} table to store all the historical sessions created by the user, and a \code{messages} table that stores individual question-answer pairs for each user session, establishing the conversational foundation. 
% % artifact level: 
% Each message links to corresponding artifact entries in three artifact-related tables (\code{message_artifact}, \code{artifacts}, and \code{artifact_versions}), which maintain comprehensive metadata for each data-driven artifact, including a list of figure identifiers, coordination relationships and schemas that define cross-figure interactions. 
% The figure identifiers in each artifact link to two tables, \code{figures} and \code{figure_versions}, which store the components of each LLM-native figure: $V$, $C$, $D$, $M$ (Sec.~\ref{subsection:conceptual-framework}), as well as action-level reasoning, codes, and results. 
% The two tables, \code{artifact_versions} and \code{figure_versions}, record the exploration history as a list of temporal snapshots of artifact-level and figure-level states, such that each user input generates a new record, preserving the complete exploration history. 
% % Two additional tables support detailed exploration tracking: \code{artifact_versions} table captures temporal snapshots of artifact states, while \code{artifact_operations} table logs all user interactions, including dashboard manipulations and drill-down operations. 
% % dashboard level: 
% % At the dashboard level, each visualization is stored in the \code{dashboard} table with multi-modal representations (\ie, Vega-Lite specifications, visualization images, and text insights). 
% % The database implements immutable versioning where any dashboard modification creates a new record, preserving the complete editorial history. 
% % 
% This architecture enables complete reconstruction of analytical pathways, allowing users to trace their discovery processes and revert to previous analytical states transparently. 
% % We also have two additional tables, \code{artifact_versions} and \code{artifact_operations}, to store the exploration history including dashboard manipulation and drilling down. 

\subsection{Implementation Details} 
\label{subsection:method-implementation} 
\textbf{Technology Stack.}
\systemname is implemented as a full-stack web application utilizing modern development frameworks and cloud infrastructure. 
The frontend employs React.js~\cite{React} for component-based user interface development, Redux.js~\cite{Redux} for state management, and Vega-Lite for declarative visualization rendering~\cite{satyanarayan2016vega}. 
The backend architecture is built on the Flask framework~\cite{Flask} with Python~\cite{Python}, providing RESTful API services and data processing capabilities. 
Specifically, the multi-agent workflow leverages LangChain~\cite{LangChain} and LangGraph~\cite{LangGraph} for complex agent coordination, with Claude 4.5 Sonnet~\cite{AnthropicAPI} serving as the primary language model. 
The system architecture supports model substitution, enabling integration with alternative LLM providers as needed. 
Data storage employs a hybrid approach: Google Big Query~\cite{BigQuery} manages relational SciSci domain datasets and user chat histories, while Pinecone~\cite{Pinecone} serves as the vector database for the retrieval-augmented generation module, storing chunked domain literature for semantic search and knowledge retrieval. 


\textbf{Action-Based Streaming Output.} 
To balance analytical transparency with user experience, we implement action-level streaming output that selectively displays critical workflow information without overwhelming users with lengthy LLM reasoning. 
The interface presents only essential decision points, specifically action selection and action sequence generation processes, providing users with meaningful insights into analytical behavior.
% To balance the data analysis transparency and the information overload of outputing every word of the LLM reasoning, we design an action-level streaming output in the user interface. 
% Only the action selection and action sequence generation process will be displayed. 
Upon completion of each user query, the system delivers comprehensive results including SQL queries, Python code, processed dataframes, visualization images, and structured Vega-Lite JSON outputs. 
This approach ensures users can monitor system progress through high-level action updates while accessing detailed technical artifacts for validation and reuse. 
% We also provide the final results for each user question, (SQL code, Python code, dataframe, visualization img and json etc.)
% % To balance the information transparency and the overwhelming. 
% % Output: action level reasoning (output action selection procedure, and result for each action (SQL code, Python code, ,,,)); And final result (csv, vega-lite img and json, SQL/Python codes). 
% % Future work: edit the code in each action -- allow action-level manipulation -- a tighter way for HAI collaboration.


\textbf{Prompt and Context Design.}
We employ four prompt engineering techniques to optimize our multi-agent workflow performance~\cite{white2023prompt, sahoo2024systematic}, including structured formatting, chain-of-thought reasoning, few-shot learning, and dynamic prompting. 
In addition, to make the context compact, we developed a structured data context that stores only essential information about each executed action, including action indices, objectives, execution status, results, evaluation scores and rationale, and remaining tasks (Supplementary Note 1.4). 
% Please refer to our supplymentary information \wyf{(Sec.~\ref{subsection:si-prompt-design} and Sec.~\ref{subsection:appendix-context-design})} for more details.
